Minimum Viable Device Drivers for ARM TrustZone

While TrustZone can isolate IO hardware, it lacks drivers for modern IO devices. Rather than porting drivers, we propose a novel approach to deriving minimum viable drivers: developers exercise a full driver and record the driver/device interactions; the processed recordings, dubbed driverlets, are replayed in the TEE at run time to access IO devices. Driverlets address two key challenges: correctness and expressiveness, for which they build on a key construct called interaction template. The interaction template ensures faithful reproduction of recorded IO jobs (albeit on new IO data); it accepts dynamic input values; it tolerates nondeterministic device behaviors. We demonstrate driverlets on a series of sophisticated devices, making them accessible to TrustZone for the first time to our knowledge. Our experiments show that driverlets are secure, easy to build, and incur acceptable overhead (1.4x -2.7x compared to native drivers). Driverlets fill a critical gap in the TrustZone TEE, realizing its long-promised vision of secure IO.

==> bkgnd-recycle.tex <==
% !TeX root = main.tex

\section{Motivations}
\label{sec:bkgnd}

% \subsection{In-TEE IO and drivers}
% \subsection{Secure IO and the needed drivers}

\subsection{System model}
% \paragraph{Hardware model for secure IO}
\label{sec:bkgnd:model}


\Note{The flow: 
	First, we assume a gold driver impl and the  demi-deterministic device FSMs -- so that such a ``replay path'' can be extracted...
	We then define device states -- reflected by driver control flow and are agnostic to us. 
	Then describe device state transitions -- marked by state-changing events (control read/write, irqs). 
	Then we set to reproduce such a state transition path which is recorded... 
	We define replay success and correctness as follows...}

\paragraph{SoC hardware}
Our design assumes Arm TrustZone and the following support at the SoC level. 
%(1) A device instance is exclusively assigned to TEE. 
(1) A device instance is exclusively assigned to the TrustZone TEE. 
This is feasible as a modern SoC often has multiple independent instances of the same device, e.g. 4--6 MMC controllers. % each of which function independently. 
% For instance, 
% each of which can connect to separate storage peripherals. 
% At the boot time, a secure monitor at EL3 the IO devices to TEE and routes their interrupts to either accordingly. 
(2) The TEE has a dedicated address spaces. Through an address space controller (TZASC), the Arm SoC maps selected physical memory regions and device registers to the TEE, which makes them inaccessible to the normal world OS. 
% The TZASC hardware also ensures that any system bus masters respect the TrustZone. For instance, a DMA engine can only access secure memory regions when it is invoked by the TEE. 
%Because IO devices assigned to normal/secure worlds may nevertheless share common clock sources and power domains, the TEE should protect clock and power registers as done in prior work~\cite{secloak}. We will will present more details in Implementation (Section XXX). 


\paragraph{Targeted IO devices}  % (scope; device model)  
This paper focuses on IO devices that have compelling use cases in TEE. 
These devices manipulate sensitive IO data while lacking end-to-end encryption to protect data. 
Examples include flash storage, 
USB devices, 
video/audio devices, 
%USB storage and input/output devices, 
%SPI or I2C sensors, 
%cameras, 
and display controllers. 

% Our design is based on the foll
We make the following assumptions on IO devices. 

\begin{myitemize}
	
\item 
\textbf{Request/response model.}
%CPU requests a device to execute hardware jobs in a request/response fashion.  interactions support a request/response pattern (although multiple/many outstanding requests are allowed). 
Devices can execute hardware jobs in a request/response fashion (although other executions, e.g. job streaming, are possible). 
Hardware job examples include executing a USB transaction and rendering a bitmap to given screen coordinates. 
\Note{move to later                        }To execute a job, CPU configures a device's registers and/or in-memory descriptors; it requests the job execution via a register write; later, the responds with job execution outcome. % by interrupting CPU. 
\Note{Aside from user input} a request also comes from kernel contexts, e.g. DMA phys pointer...	
	

\item 
\textbf{Driver/device interactions.}
\Note{To submit jobs...}
CPU interacts with devices via registers, shared memory, and interrupts in driver code. 
CPU may use DMA to move IO data\Note{..to configure hardware jobs}. 
%We do not assume that the devices use IOMMU. 
The devices often do not use IOMMU. 
To our knowledge, these are true for today's mobile/embedded SoCs 


\item 
\textbf{Device states \& state transitions.}
\Note{In executing a job..} By hardware design, devices decide its execution behavior based on its internal FSM \textit{states}. 
The state encodes the device's current protocol step, its configuration, and pending hardware jobs;
it is, however, independent of input/output data content.
For instance, a display controller's state is independent of the pixels it renders. 

\item
\textbf{State transitions \& state-changing events.}
As the full driver interacts with the device\Note{, driving it to go through different phases of job execution...}, it induces the device's state transitions, which the driver continuously assesses through \textit{state-changing events}.
%The driver does the assessment solely based on its observation of \textit{state-changing} events, 
%i.e. interaction events that \textit{may} change the device state or indicate changes to the state. 
i.e. all interaction events that \textit{may} change the device state or indicate the state \textit{may} have changed. 
%We define state-changing events broadly, so that we err on the side of falsely assessing a successful replay as failure, rather than a failed replay as a success. The former can be overcome with re-execution while the latter will cause silent errors. Therefore, the assessment of replay success is sound. 
Our observations on state-changing events include: 
interrupts; 
control writes to device, e.g. write to a command register; 
control reads from device returning fresh values, e.g. a bit flipped in an in-memory descriptor. 
The events do not include: 
read/write of data contents; 
control reads without side effect or returning stale values, e.g. return from a performance counter. 

%\item Shared memory:  memory barrier??), which signals ... the shared memory synchronization point?
%
%\item 
%\Note{merge this}
%
%%In executing jobs, devices 
%a device's behaviors, or its state transitions, 
%For instance, a display controller's state is independent of the pixels it  renders. 
\end{myitemize}

%\paragraph{Device states}
%%\Note{To make replaying possible...the states are demi-deterministic...given an input, the interactions are deterministic in the sense of same set of register accesses..values..XXX}
%%Our rationale is based on our 
%Our guarantee is based on the following observation. 
%%We have the following observation on device states. 
%%A device's state is the device's whole knowledge for determining how it willexecute the current request. 
%A device, by hardware design, 
%%determines how it executes hardware jobs based on an internal \textit{state}. 
%decides its execution behaviors based on an internal \textit{state}. 
%The state encodes the device's current protocol step, its configuration, and pending hardware jobs. 
%%The state encodes (1) the current protocol step the device is participating in, e.g. wait for a command; (2) the device's current configuration, e.g. command types and bus width; 
%%(3) any hardware jobs the device has admitted and yet to complete. 
%%(3) any intermediate results the device may have (??). 
%The state, however, is independent of input/output data content per our model in \sect{bkgnd:model}.
%%As the full driver interacts with the device and submits a series of hardware jobs, the device's state follows a path of transitions. 
%As the full driver interacts with the device, it induces the device's state transitions. 
%the device's state changes accordingly.  
%We define a device state as a tuple <P,C>, where P is the device's protocol step, e.g. WAIT\_FOR\_COMMAND or COMPLETED; C is the the device's current configuration, e.g. data rate and bus width. 
% including in-memory descriptors visible to the device. 

%\paragraph{Causes of state divergence}
%Even to repeat the same interaction sequence, the device state in replay may diverge from recording. 
% Why the device state in replay may diverge from recording, 
%even with the same interaction sequence?
%Why would device state divergence occur, 
%even if CPU repeats the same sequence of hardware jobs? 
%Why might a device's state diverge, 
%even if it repeats the same sequence of hardware jobs? 
%even if CPU replays the same  interaction sequence?
%The major sources are two. 
%Even to execute the same hardware jobs, a device may show different state transitions across runs. 
%What if the device state transitions at the replay time diverge from those at the record time? 
%How to handle divergences in device state transitions?
%Even to execute the same hardware jobs, a device may follow different paths of state transitions across runs. 
%If left unconstrained, a device may take different paths of state transitions to 
%Even to execute the same hardware jobs, 
%a device's path of state transitions in replay may diverge from what was recorded. 

%Since a successful run always follow the same device state transitions. 
%We therefore associate replay correctness to device state transitions: 
%The above analysis shows that a successful replay is implied by device state transitions: 
%The above analysis shows that a successful replay always reproduces the recorded device state transitions: 
%With the above analysis, we consider a successful replay as:

%\paragraph{Observation of device state}
%\paragraph{Assessing device state transitions}
%
%Built on the above definition, 
%the replayer assesses replay success by comparing device state transitions in the replay run with those in the recording run. 
%%\Note{recording run itself is non-deterministic...define such a ``gold'' path which is exemplified by recordings...}
%%How does the full driver detect device state divergence? 
%%How does the replayer detect device state divergence? 
%%How does the replayer keep track of device state transitions? 
%However, a device's state is often internal and is not directly visible to software. 
%
%Our solution is for the replayer to reproduce the full driver's events of changing the device state. 
%%The rationale is as follows.
%We have the following observations. 
%%By its design, 
%%the full driver interacts with the device continuously and As the driver interacts with the device in many rounds, assesses if the device state have deviated from known correct transitions. 
%In the recording run, 
%%the full driver has been assessing if the device state have deviated from known correct transitions. 
%the full driver's confidence in execution correctness is based on its continuous assessment of device states.
%%have deviated from known correct transitions. 
%The driver does the assessment solely based on its observation of \textit{state-changing} events, 
%%i.e. interaction events that \textit{may} change the device state or indicate changes to the state. 
%i.e. all interaction events that \textit{may} change the device state or indicate the state \textit{may} have changed. 
%%We define state-changing events broadly, so that we err on the side of falsely assessing a successful replay as failure, rather than a failed replay as a success. The former can be overcome with re-execution while the latter will cause silent errors. Therefore, the assessment of replay success is sound. 
%State-changing events include: 
%interrupts; 
%control writes to device, e.g. write to a command register; 
%control reads from device returning fresh values, e.g. a bit flipped in an in-memory descriptor. 
%The events do not include: 
%read/write of data contents; 
%control reads without side effect or returning stale values, e.g. return from a performance counter. 
%\Note{maybe tie this to control flow decisions -- driver relies on control reads to make control flow decisions, etc. 
%	Example is reading performance counters, power states etc. are unconditional -- no control flow dependent on them. 
%	However, reading IRQ status reg is control-flow dependent, i.e. state-changing, where the driver assesses the bit masks and make decisions. 
%}

%To implement the comparison, the recorder extracts from its interaction trace a subsequence of state-changing events and compare the subsequence to that from the recorded trace. 

\input{fig-code}

\textit{Example:}
Figure~\ref{fig:code} shows an example, where the state-changing events in the recording run are highlighted. 
Replay run 1 is successful, because its state-changing events match those in the recording run, despite the discrepancy in other events. 
Replay run 2 fails, because its state-changing events diverge from those in the recording run. 

%\textbf{Define: equivalence of interaction sequences}
%A recursive definition? Why needed? Used to prune execution paths. 

\begin{comment}
\begin{myitemize}
\item 
an interrupt, including its semantics and source (?); 
\item 
write of a register of device configuration or metadata;
\item 
read of a register (configuration or metadata) returning different value from previous read
\item
read of an in-memory descriptor field returning a different value 
\end{myitemize}

Non-example: ...
\begin{myitemize}
\item 
read of register returns the same value. And the read has no side effect. 
\item 
read of statistics registers (performance counters)
\end{myitemize}
\end{comment}


%A device often does not expose its internal FSM (e.g. there is no register showing it). 
%During driver/device interactions, a driver continuously assesses the device state. 
%The driver does so by learning from interaction events that suggest potential device state changes, or \textit{state-changing events}. 

%We define state-changing events: interaction events that may affect device behavior in request execution. (waypoints of the device state transitions)

%For instance, an MMC controller... determined by the ...
%rendering to a specific screen region, reading one block from eMMC, 

%As a driver interacts with the device, the driver continuously assesses (learns) device states from the interaction events that indicate possible updates to the device state. 

% assess if the device state diverges from the correct transitions. 

% If we make the following assumption: 
%If we assume the full driver is correct: 
%\begin{assumption}[A golden driver]
%	The full driver performs interactions sufficient to detect any device state divergence. 
%\end{assumption}

\paragraph{The golden full driver.}
Finally, we assume the full driver performs interactions sufficient to detect any device state divergence... 


%The above assumptions lead to a simple, practical design. 
We will discuss its limitations in Section XXX. 

%IOMMU -- what if devices depend on it? Can we discover the use of IOMMU? 

\Note{merge or move to record section?}

\paragraph{Discovering driver/device interfaces} % which must be recorded. 
At the record time, 
\sys{} needs to take a series of snapshots of the interfaces. 
(1) CPU and devices share a wide interface: registers, DMA buffers, and in-memory descriptors. 
To accommodate complex driver/device interactions, 
in-memory descriptors may further embed pointers to each other, e.g. to form a scatter-gather list. \Note{cite}
%The data structures must be captured as part of the device/driver interactions. For instance, DMA is controlled by an 8-word in-memory data structure... The VCHIQ ...  firmware ... FSM ... containing pointers to each other to form a list...
(2) 
\sys{} should identify \textit{parameterizable} interface fields, i.e. to be overridden with new values at the replay time. 
Examples include registers pointing to the base of in-memory descriptors and 
fields in in-memory descriptors pointing to input/output buffers. 
Their values depend on physical memory layout which can vary across runs. 
%The replayer must override these fields at run time, because their values depend on physical memory layout which can varies across runs. 
(3) 
The interface may span additional hardware components such as a standalone DMA engine in a separate address range and power controllers (??).




MVP drivers work with devices whose behavior is purely dictated by user and kernel inputs. 
This can be elaborated as:
\begin{myitemize}
	\item 
	Given an input, the \st{code path} FSM transitions are deterministic.
%	\Note{this implicitly specifies data is out of device FSM transitions}.	
	That is, the data is out of the FSM transition path.
	
	\item 
	Have parameterizable fields for reuse.
	FSM state transitions are driven by different inputs\Note{maybe separate user input vs kernel inputs};
\end{myitemize}

\paragraph{Threat model}
We follow the threat model in TrustZone research. 
On the target machine: we trust the SoC hardware including any firmware it runs; 
we trust software inside the TEE; we do not trust the OS in the normal world. 
The developer's machine runs stock OS and drivers, which we assume are uncompromised. 
The rationale is that the developer's environment is part of a software supplychain and has much stronger security than target machines. 
Compromising the developer machines often requires high capability and long infiltration campaigns \Note{cite}. 
%It is therefore more difficult to attack than target machines. 
We do not preclude them from containing semantic bugs. 
\Note{may move to sec analysis}

%We do not consider hardware attack, e.g. bus snooping..take out \& destroy the MMC card....



%\paragraph{Key trustlets for motivations}
\subsection{Example trustlets of secure IO}
% We are motivated by the following trustlets that benefit from secure IO significantly. 
%\Note{refer back to prior study on trustlets. a more thorough study}
We are motivated by the following use cases. 
In all cases, secure IO prevents the OS from observing sensitive data and tampering with the data. 

\begin{myitemize}
\item Secure storage. 
%Trustlets store sensitive data on flash storage, e.g. SD card and eMMC. 
Trustlets store and retrieve sensitive data, such as credentials, biometric data such as fingerprints, and user contents such as emails. 
A storage controller and its flash medium, such as eMMC, are assigned to the TEE. 
%Secure IO hence shields the data from the OS. 
% shielding the data from the OS. 
% Despite recent flash hardware (e.g. RPMB) supports end-to-end data encryption,  with secure IO the TEE can truly shields the data path from the OS, e.g.  eliminating OS attacks via side channels \Note{cite}. 

\item Trusted perception. 
Trustlets read in sensitive data from sensors assigned to TEE. 
% without exposing the data to the normal world OS or 
% Examples include data of biometric, fingerprint, iris, and GPS. 
A particular interesting example is video, which often contains privacy sensitive contents and requires non-trivial camera drivers. 
% Secure IO prevents the OS from observing the data or tampering with the data. 


\item Trusted UI. 
Trustlets render security-sensitive contents such as verification codes for online services and bank account information; 
they also read in user inputs such as key presses and touch. 
% Doing so ensures UI confidentiality and integrity. 
%They prevent the OS from observing the UI contents and tampering with the contents. 
\Note{cite}

\end{myitemize}

% \paragraph{What trustlets need and do not need}
\paragraph{IO functions needed by trustlets}
The above use cases all build on trustworthy device drivers. 
%The drivers should meet the stringent programming constraints of TEE and not introduce new vulnerabilities. 
The drivers should suit the lean TEE and not introduce vulnerabilities. 
Compared to normal apps, 
trustlets show relaxed requirements, which provide opportunities to the driver realization. 

\begin{myitemize}
\item 
Lower sensitivity to IO performance.
For instance, 
secure storage does not to demand high throughput in accessing user credentials or email contents; trusted vision for surveillance can be satisfied with low frame rate and median to low resolution (e.g. 720P at 1FPS \Note{cite}). 

\item 
%A small set of 
IO requests with simple semantics. 
For their simple functions, trustlets can be served with write/read of individual blocks, acquisition of individual video frames, or rendering given bitmaps. 
We rarely see trustlets needing complex device features, e.g. USB hotplug. 
\Note{better example?}

\item 
% They are unlikely to execute with high concurrency. 
Tolerant of coarse-grained IO sharing. 
Concurrent trustlets are far fewer than normal-world apps. 
Even when multiple trustlets share the same device, their requests can be serialized without notable user experience degradation. 
Examples include only allowing one query executed over secure storage at a time. 
%Examples include executing a batch rendering of commands from one trustlet at a time and to execute one database query at a time. 

% sequential access to an IO device. 

%because both the amount of private data and the number of concurrent trustlets are smaller.
\end{myitemize}


% the drivers should be simple (meet the stringent programming constraints of TEE), secure (not introducing new vulnerabilities to TEE), and robust (for handling critical/sensitive data). 
% On the other hand, the trustlets demand fewer IO functions and performance than normal world apps. 


% We make compromise on on device dynamism, high concurrency, and optimal performance. 

%\subsection{Design implications and goals}
%\subsection{A case for XXX}
\subsection{Prior art}
\label{sec:design:prior}

% \paragraph{Why full drivers do not fit}
%\paragraph{Why are commodity drivers complex}
\paragraph{Mature device drivers}
%Device drivers in commodity OSes are designed to be comprehensive. 
%Their complexity is often overkill to trustlets. 
The drivers in commodity OSes are often overkills to trustlets because of the following design goals.
(1) \textit{Optimal performance}. 
%Full drivers tune devices meticulously. 
For instance, an MMC driver tunes bus parameters periodically (every XXX seconds). 
% They handle (detect) various runtime errors and recover with minimum performance loss (despite many errors are rare). 
It implements a complex state machine for handling corner cases, so that the driver can recover from exceptions with minimum loss of work. 
% by resuming and minimum performance loss. 
%For example, in the FSM for MMC, each work state has connections to a variety of error states and driver/device protocols for recovery from those error states. As a result, XXX states in a MMC driver and hundreds of transitions among these states. 
% 
(2) \textit{Fine-grained sharing}. 
%Commodity  drivers bake in support for multiple concurrent clients. 
A driver maintains separate contexts for concurrent apps. 
The driver multiplexes requests at short time intervals. 
Some drivers, e.g. \Note{XXX} USB (??), implement sophisticated request scheduling for app fairness. 
%
(3) \textit{Device dynamism}. 
The drivers support full dynamism as permitted by the device specifications. 
Notable examples include runtime power management and device hotplug. \Note{cite}
%For instance, XX\% of the MMC driver states are for handling dynamic power management; XX\% of 
%XXX SLoC and XXX states in MMC drivers are for handling  and hotplug (e.g. ``what if the device sleeps in state X, Y, and Z'').
  


\begin{comment}
\paragraph{Architectures of commodity drivers}
% The above observation motivates \textit{defeaturing} a full driver to suit TEE. 
% Device drivers in commodity OS are constructed in a way that makes reusing difficult. 
% The codebase of full drivers poses multiple obstacles. 
Reusing commodity driver code for TEE is difficult because the ways they are constructed: 

\begin{myitemize}
\item % \textit{Abstraction/generality}
% \textit{Multiple levels of abstraction.}
\textit{Extensive abstraction.}
A commodity OS often structures drivers of the same class as frameworks. 
For instance, Linux implements the MMC protocol as an MMC ``core'' and instantiates various hardware-specific drivers atop it. 
There further exists frameworks for synchronization, power, and XXX...
% E.g. `struct mmc-host' is a feature for accommodating different models of host controllers under one unified data structure.

\item 
\textit{Generality}
A driver often supports multiple devices. 
Even in a single source file, the code for a (large) family of devices. 
Conditional compilation. 
Function pointers are not uncommon. 
Code branches are taken based on runtime device discovery, e.g. through device trees.
It becomes obscure which code needs to be ported for TEE. 
\Note{conditional compilation, runtime dispatch, various configurations...}



\item
\textit{Deep kernel dependency}. 
Full drivers are programmed against a kernel environment. 
They invoke kernel services such as page allocator, clock, timer, synchronization. 
They configure own behaviors based on device trees provided by the kernel. 
Some drivers further require kernel threads for deferred execution. 
Porting drivers to TEE requires to port (or emulate) these services in the TEE as well. 
It often ends up (re-)building a smaller kernel environment in the TEE. 	
\end{myitemize}

\end{comment}

\paragraph{Why existing approaches are inadequate}
%Existing techniques have their shortcomings. 

(1) 
\textit{``Lift and shift''} 
One may bundle a full driver with all its kernel dependencies and port to the TEE. \Note{cite Linux kernel library, rumpkernel}. 
While easing porting, 
this approach often adds substantial code (XXXX) and driver vulnerabilities to the TEE. 
% and incurs vulnerabilities. 
%The driver code often supports multiple devices. even in a single source file, the code for a (large) family of devices. 
TrustZone developer communities suggested this approach as unfavorable \cite{XXX}

(2) \textit{``Trim down''}
Developers may manually carve out only the needed driver functions, e.g. block read/write from an MMC driver. 
Accordingly, they simplify driver/device protocols, driver FSMs, and resource management. 
This is how simple drivers such as UART are built for TEE.
% the required effort for complex drivers (e.g. USB, eMMC, cameras as we target)
When it comes to non-trivial drivers, however, trimming is daunting. 
Doing so requires deep knowledge on driver code (``what code invokes this callback, given extensive function pointers, macro expansions, and kernel configurations?'') and the device (e.g. ``will disabling USB SoF~\cite{XXX} break  mass storage access?''). 
Trimming also requires intense trial and error. 
%Second, drivers are full of conditional paths taken based on runtime conditions, e.g. through device trees.
%It becomes obscure which code needs to be ported for TEE. 
\sect{case} presents our own experiences for three drivers. 

%For the reasons above, even taking a driver out of the original kernel and recompiling within TEE is difficult \Note{cite}, let alone reasoning and carving out its specific functions. 

(3) \textit{``Synthesis''} 
It is possible to automatically synthesize some drivers -- if the device FSM is fully known. \Note{cite}
%which could either come from a formal specification or reverse engineering. 
Targeting drivers with full features, % without any reference implementation, 
this approach requires non-trivial efforts. 
Developers have to write specification, driver templates, and glue code. 
The resultant code is complex and less interpretable. 
Such efforts are less warranted in TEE, 
where trustlets only need basic IO functions and the source code of mature drivers is often available. 
%Driver synthesis misses opportunities in TEE: 
%trustlets only need basic IO functions and the source code of mature drivers is often available. 
%A much simpler solution should suffice. 


% This approach is likely an overkill to trustlets which only require a subset of driver functions. 


%\input{tab-dev-knowledge}

%\subsection{Design considerations}
%\label{sec:design:theory}

%\paragraph{Our idea \& challenges}
%We derive drivers for TEE in a different way: instead of reusing an existing driver's \textit{code}, we reuse its \textit{behaviors} of interacting with the device.  
% running the driver and recording the driver/device interactions at the software/hardware boundary;  

%To do so, we run the full driver and record the driver/device interactions; 
%we process the interactions to be segments of interaction events; 
%we replay the interactions from the TEE. 

%We record segments of driver/device interactions and replay them at run time.  

\subsection{Replay correctness}
%\subsection{Device state and replay correctness}
\label{sec:design:theory}
%The replayer provides the same level of correctness guarantee as a full driver does. 
%does in \textit{assessing} the correctness of a request execution. 
%if a request is completed successfully. 
%This means that when the replayer deems a request is completed successfully, the assessment is as sound as one made by the full driver. 
%This means that when the replayer assesses that the GPU has completed a request successfully, the assessment is as sound as one made by the full driver. 
%Our approach -- replaying driver/device interactions -- raises the following questions. 
Our approach -- replaying driver/device interactions -- raises a first-class question: 
how do we assure that a replay run is correct?
We want the replayer to provide the same level of correctness guarantee as the full driver does: 
when the replayer asserts that it completes hardware jobs with success, the assertion is as sound as one made by the full driver. 
 
%when the replayer asserts a replay run completes with success, the assertion is as sound as one made by the full driver. 
%This means that an assessment of successful request completion made by the replayer is as sound as one made by the full driver. 

%Our rationale is based on the following observations. 
% on devices and mature drivers: 
%We have the following observations on driver designs: 
%Our rationales are as follows. 
%on equivalence of device state transitions. 

%\textit{cc and replay correctness}: 
Built on our model of device states and transitions in Section~\ref{sec:bkgnd:model}....
We define replay success by the device state transitions: 

Built on the above definition, 
the replayer assesses replay success by comparing device state transitions in the replay run with those in the recording run. 
%\begin{theorem}
\begin{definition}[Replay success]
If in a replay run, the path of device state transitions exactly matches that in a successful recording run, then both runs complete the same sequence of jobs and the replay succeeds. 
%\end{theorem}
\end{definition}
\Note{path is vague -- same sequence of state-changing events? }
Our rationale is as follows. 
%To repeat the same hardware jobs, a device's paths of state transitions only diverge for two reasons. 
%(1) Some divergences reflect alternative paths to finish the same hardware jobs. 
%First, there exist alternative paths to finish the same hardware jobs correctly. 
First, we constrain a device's state space so there is only one path to finish given hardware jobs correctly.
A notable source of alternative transition paths is a device's hardware concurrency. \xzlNote{more?}
%When multiple jobs are queued with the device, the number of completion interrupts and their order can be nondeterministic. 
For instance, if CPU submits multiple USB transfers at a time, a USB controller may  opportunistically coalesce the completion interrupts of these transfers. 
In response, we eliminate all but one alternative path of transitions. 
For example, we serialize hardware job submissions both in the recording run and in the replay run. 
Second, 
all other device state transitions deviated from the successful path imply failure in job executions. 
%other than the successful path, all other device state transitions imply failure in job executions. 
%Resource availability at the SoC level, 
The common causes are: \xzlNote{be systematic}
(1) fluctuation in chip-level hardware resources, 
including power supply, clock rates, and memory bandwidth. 
For example, an under-current condition of an SD card occurring at the replay time can trigger an interrupt that was not recorded. 
(2) unexpected hardware failures. 
For example, an MMC controller losing the flash media because of SD card removal. 
%it may finds incorrect message CRC because of bus error; 
%a bus transaction may time out because the flash peripheral has a power failure. 
%heavy contention on the main memory will cause commands to media accelerator to timeout.
These divergences cannot be fully prevented. 
The replayer detects them and re-attempt the execution. 

\Note{lwg:}

The key idea is to extract a ``stable/beaten'' path. 
To this end, we assume a \textit{demi}-deterministic device model for drivers we target... 
That is, for a given set of fixed/controlled inputs, the device will only go through one fixed FSM transition path -- the path we set to extract;
yet they may exhibit different hw/sw interactions (e.g. reg access values) by appearance. \Note{these will be reflected in recording...}

These inputs are 
1) user inputs, i.e. block IDs requested by users; 
2) kernel contexts\Note{a little vague -- kernel states used to bookkeep device states??}, 
3) spontaneous events: e.g. device hotplug.\Note{is this a user input?}

During recording we exploit the \st{demi-deterministic} nature.
We control/fix the inputs by eliminating sharing and hardware concurrency.
At one time, the path takes only one job submitted us; 
there's no background activities such as runtime suspend/resume, merging of user jobs.

We establish replay \textit{correctness} based on interaction events:  

%As the above definition associate replay correctness to device states, 
%it raises two questions. 
%The above definition raises two design questions. 
 
%A device's state changes as interactions and execution continue. 

%\begin{theorem}[Replay correctness by observational equivalence]
\begin{theorem}[Replay correctness]
If the replayer observes the same state-changing events (including types, order, and parameters) as the full driver observes at the record time, 
%If the replayer observes the same sequence of state-changing events as recorded, 
then as far as the driver is concerned, the device state transitions are the same as recorded. % and the device completes the same request. 
% (despite of difference in IO data contents).
%The replay therefore succeeds. 
The replay is therefore correct. 
\end{theorem}

Suppose the replayer fails to detect a state divergence, e.g. a MMC controller corrupts data silently despite of all matched state-changing events. 
Thus the divergence could have been missed by the mature driver as well, a situation should not occurring in a golden implementation. 


%If we assume that the full driver is a golden implementation: 
%it performs interactions sufficient to detect any device state divergence, then the above theorem establishes replay \textit{correctness} based on comparison of interaction traces.  








\begin{comment}
\paragraph{Request execution equivalence}
From the driver's POV, 
its \textit{full} knowledge about device state transitions is 
the sequence of state-changing events (including their semantics, parameters, and values read/written). 
If in separate runs the driver sees \textit{equivalent} sequences of state-changing events, 
then as far as the driver (the golden implementation) is concerned, the device goes through the same state transitions and has finished the same request (albeit on different input/output). 
Example: a USB controller accesses 500 registers...

The same rationale applies to a replayer, whose goal is to reproduce a request as recorded.
If the replayer sees the same series of state-changing events as recorded, 
%then as far as the driver is concerned (to the best knowledge of the driver), 
then the device in the replay has finished the same request as recorded. 

For this reason, the replayer is as capable as the full driver on assessing device states (i.e. detecting correctness violation). 
If there is a state divergence undetected to the replayer (e.g. silent data corruption despite equivalent state-changing histories), it could have been missed by the full driver as well. 
This means there is a bug in the driver. 

Its assessment of request correctness is sound. 

%This means that when the replayer deems a request is completed successfully, the assessment is sound. 

\end{comment}







\begin{comment}
\begin{myitemize}
\item 
%As it executes, a full driver continuously determines the device state based on its observations of the device (register reads, interrupts, memory state update). 
%The interactions are the only way for the driver to observe the device state. 

%As it executes, a full driver continuously interacts with the device. 
%Its observations from the interactions (register reads, interrupts, memory state update) are all the driver's knowledge to determine the device state. 
%Solely based on the observation, 

As it executes, a full driver continuously interacts with the device. 
At interaction events, the driver makes a series of observations of the device state. (register reads, interrupts, memory state update)
By design, this is the \textit{only} information used by the driver to determine the device state. 

\item 
%If in a test run, the driver's observations matches those of a previous run (at all interaction events), 
%then to the best knowledge of the driver, in the two runs the device goes through the same state transitions.
%% ; its executions at replay time is  equivalent to the record time. 
%We will define observation equivalence later.
If in two separate runs, the driver's observations match at all interaction events,  
then as far as the driver is concerned, the device goes through the same state transitions in the runs. 

\item 
A replayer interacts with the device as the full driver did. 
If the replayer's observations match (at all interaction events) those of the recording run, 
then to the best knowledge of the driver, the device in the replay run goes through the same state transitions. 

\item 
For this reason, the replayer is as capable as the full driver on detecting device state divergence. 
If there is a state divergence undetected to the replayer (e.g. all observation history matches but there is silent data corruption), it could have been missed by the full driver as well. 
\end{myitemize}
\end{comment}



\begin{comment}
\Note{Not needed?}
Our rationales are that (1) the basic driver functions needed by trustlets can be captured as short segments of interactions. 
Favoring simplicity (engineering ease) over driver completeness or FSM coverage, 
% Exercising only driver beaten paths omits many corner cases (runtime conditions) and complex logic for handling them. 
we deliberately do not seek to capture all possible interaction segments which entails symbolic execution that itself may require higher efforts than porting. \Note{cite}
% (2) By constraining the behaviors of the full driver,  the resultant interaction segments can be recorded and replayed with determinism. 
(3) Capturing and replaying the interactions would require much less knowledge and efforts than constructing/refactoring a driver. 
Table XXX compares our approach to prior ones. 
Section XXX will present concrete example devices. 
\end{comment}

% To record the interaction sequences (segments), we exercise a full driver with a small set of request primitives sufficient to serve the trustlets; as the full driver executes its \textit{beaten paths}, we record the driver/device interactions to be replayed. 

% We instead rely on simple runtime mechanisms to detect and recover from faults. 



==> eval-recycle.tex <==
% !TeX root = main.tex

\section{Analysis}
\label{sec:security}



%\paragraph{Correctness}
\subsection{Correctness}
%\sys{}'s replay correctness depends on a ``golden'' driver implementation, as stated in Section XXX. 
\sys{}'s replay correctness can be affected by semantics bugs existing in the recording environment: the OS and full driver. 
Such bugs can result in malformed recordings, which in turn lead to incorrect replay outcome. 
For example, triggered by a specific input value, the full driver may emit  device commands with glitches. 
\sys{} neither mitigate nor exacerbates such semantic bugs. 

\sys{}'s recorder and replayer may bring in semantic bugs. 
However, we expect such bugs are rare because of software simplicity: the recorder the replayer are only XXX SLoC. 
Our experimental validation in XXX enhances the confidence. 

\subsection{Security}
\paragraph{Threat model}
We follow a common threat model in TrustZone research. \xzlNote{cite}
On the target machine: we trust the SoC hardware including any firmware it runs; 
we trust software inside the TEE; we do not trust the OS in the normal world. 

The developer's machine runs a stock OS and drivers for recording. 
We assume that they are uncompromised. 
The rationale is that developers machines are often part of a software supplychain with strong security measures. 
%and often has strong security. 
Compromising the developer machines often requires high capability and long infiltration campaigns \Note{cite}. 

\paragraph{Attacks thwarted}
% \sys{} relieves the TEE from running full device drivers
\sys{} keeps full device drivers out of TEE. 
It is therefore immune to vulnerabilities within the driver code. 
Such vulnerabilities are known extensive and could have been exploited by adversarial devices (packets from USB peripherals, messages from media accelerators, etc.) or malformed requests sent to the TEE/trustlets. \xzlNote{check}. 
Examples include dirtyCoW~\cite{dirtycow} and BadUSB~\cite{badusb}. \xzlNote{more examples}

\paragraph{Attacks against \sys{}}
(1) Attacks against the recording environment or distribution. 
These are the only ways to tamper with recordings, since the recordings are signed by developers and verified by the TEE. 
As described above, this is difficult as the attackers must subvert the defense of software supplychain. 
Nevertheless, successful attackers can fabricate recordings\Note{how?}. 
The fabricated recordings may result in replay failures but cannot subvert the security checks enforced by the replayer (Section XXX).
\Note{can the attack corrupt the data?} 
(2) Attacks against the replayer. 
If the replayer code has vulnerabilities, an adversarial OS may attempt to exploit by sending malformed requests to TEE; an adversarial device may inject malformed hardware packets. 
Successful attackers may compromise the replayer or even the whole TEE. 
Nevertheless, the replayer's low codebase (only XXX SLoC) and simple logic (simple memory management, well-defined semantics for replay actions) makes such vulnerabilities unlikely. 

\begin{comment}

\xzlNote{------ old writing, pick \& merge ------}

\subsection{Validating recording security}

\textbf{Our claim:} MVP drivers are more \textit{secure-able} than native drivers.
The reasons are threefold:

%\Note{the following may not be needed}
%Though highly unlikely it may trigger a vulnerability during recording, it does not damage the host machine since the test input is controlled by \sys{} and does not contain malicious payload, and simply re-records. %is kernel's responsibility to fix the vulnerability.

%There are two reasons:
%1) \sys{} only records hw/sw interactions.
%They donot contain kernel memory allocation, thread scheduling, etc. which are sites of vulnerabilities.
%2) vulnerabilities are hibernating on site until triggered by malicious payload at runtime.
%Recordings are taken from the beaten path and controlled inputs -- which is less likely to tread on vulnerabilities.
%Even if we accidentally do, due to lack of malicious payload the kernel often simply hangs and we just restarts the recording.

Second, recording and treating non-determinism systematically (\S~\ref{sec:design:summarize}) ensures observational equivalence (\S~\ref{sec:design:theory}) -- at replay time, \sys{} drives devices to undergo the same, exact state transitions \textit{as if} they're driven by native drivers.
%Second, recording and systematic treatment of divergence ensures the correctness by equivalence (\S~\ref{sec:design:theory} Theorem 1) -- at replay time, \sys{} drives the devices to undergo the same, exact state transitions \textit{as if} they're driven by native ones for the same request.
%As orthogonal efforts, the recordings can be vetted for further assurance, because to the core they are baremetal commands to devices, which are finite \& non-ambiguous. 
%By looking up \& understanding the command semantics the developer shall be as confident as running a \textit{golden} kernel driver. 
%Down to their core they are only commands to device, which are finite \& non-ambiguous. 
%By looking up \& understanding the command semantics the developer shall be as confident as running a \textit{golden} kernel driver.

%(as orthogonal efforts) 
Last, vetting the recordings is more promising than the whole native drivers.
They are much smaller (tens to hundres of entries);
they do not share states with host environment except for memory allocation; 
they are simply baremetal commands to devices, which are finite and non-ambiguous. 
%as a best effort the replayer enforces extensive security checks (\S~\ref{sec:design:replay} when using the recordings to mitigate any damage caused by corrupted recordings. 



\textit{What makes recording secure/secure-able?}
\begin{myitemize}
	\item 
	Recording does not inherit kernel vulnerabilities.
	There are two reasons:
	1) \sys{} only records hw/sw interactions.
	They donot contain kernel memory allocation, thread scheduling, etc. which are sites of vulnerabilities.
	2) vulnerabilities are hibernating on site until triggered by malicious payload at runtime.
	Recordings are taken from the beaten path and controlled inputs -- which is less likely to tread on vulnerabilities.
	Even if we accidentally do, due to lack of malicious payload the kernel often simply hangs and we just restarts the recording.
	
	
	\item 
	\Note{the liability is on kernel -- we trust it for semantic correctness}

	
	\item 
	In case recordings are corrupted, \sys{} presents the following checks to further harden its security: 
	
	
\end{myitemize}



%\sys{} trusts code integrity of the developer machine being recorded from but not their bug-freeness (\S\ref{sec:bkgnd}), as they're from upstream kernel.
%%Yet, \sys{} does not assume they \& the resultant recordings are bug-free, as they're from upstream kernel.
%As a result, several scenarios/bugs(?) may happen to recordings: 
%\begin{myitemize}	
%	\item 
%	Static values of the recordings are corrupted when storing to disk, e.g. bits get flipped. 
%%	can detect by statically verify \& applying checksum. 
%	
%	
%	\item 
%	Driver semantics bugs are recorded.
%	\sys{} does not record driver memory bug (e.g. mem allocation), but may inherit semantic bugs at hardware/software interaction.
%	E.g. reads mis-records as writes, or have side effects additional to the request (e.g. overwriting other sectors).
%	
%	\item 
%	Value resolution error. 
%	May be caused by incorrect impl. of replayer. 
%	E.g. register offsets are resolved wrongly,
%	parameterize-able byte offsets are solved wrongly (apply to VCHIQ only).
%	
%	\item
%	More? 
%\end{myitemize}
%
%To this end, \sys{} further hardens runtime security by enforcing following invariant:
%\sys{}'s recordings include segments of register access address offsets with their values, and memory dumps (for DMA desc. \& VCHIQ slots).
%At run time, the replayer applies the offsets to base virtual address mapped by TEE and parameterizes the annotated fields as requested by trustlet.
%Meanwhile it ensures the following security invariant:
%\paragraph{Verifying recording semantics.}
%We first verify the achieves same function as intended (thorough tests are presented later in \S\ref{sec:eval:correctness}).
%Then we examine the MMC, USB SCSI, and VCHIQ MMAL commands to ensure there are no hidden side effects, e.g. overwriting unrequested data blocks.

\subsection{Validating replayer security}
%Compared with pull whole drivers inside TEE, what are the benefits?
%What are the possible attacks to our system? 
%In TEE, MVP drivers directly interacts with devices via the replayer without being noticed by the OS -- 
%register access \& their values are fully confidential;
%the backing memory used for DMA \&  message passing (VCHIQ) is protected by TEE.

%\textit{Attack against TEE-OS interfaces.}
%They are the largest class of attacks against a TEE.
%\sys{} thwarts those involving supported drivers, e.g. Iago attack\cite{trustshadow} of block devices \& image data\Note{cite}, and file access side channel attack~\cite{xxx}.
%%Examples include active ones, e.g. Iago attack\cite{trustshadow}, and TEE kernel buffer overflow (CVE-2019-1010298\Note{cite}), which feed malicious payload to TEE, and passive ones, e.g. access side channel attack~\cite{xxx}, which infers trustlet secrets via non-encrypted file calls forwarded by TEE to an OS.
%This is because drivers are driven solely by the (trusted) trustlet and operate independently of an OS, not accepting \textit{any} of its inputs.

%While MVP drivers enjoy fully isolated execution in TEE, 
We validate the security of replayer by considering following attacks under the threat model described in Section~\ref{sec:bkgnd}:
%

%\textit{Attack against .}
\textit{Attack against replayer.}
%\Note{Is this for the full driver or the MVP driver?}
%Attackers exploit vulnerabilities in driver code implementations to launch buffer overflow~\cite{cve}, dirty CoW ~\cite{dirtycow}, BadUSB~\cite{badusb} attacks.
%\sys{} thwarts the class of attack by not including the implementations at all as described earlier.
The replayer only takes input from trustlet and the recordings.
It verifies the integrity of recordings via checksum (\S~\ref{sec:design:replay});
it does stringent boundary checks (e.g. block/memory address) on both to mitigate attacks exploiting memory bugs.
It limits concurrency to avoid dangerous race conditions. 
%aggressively limits parameterizable/dynamic values to only data address (i.e. block address, DMA page address) and size and does stringent security checks on them. 
%
%Malicious peripherals (hijacked by an attacker) may exploit driver code vulnerabilities~\cite{XX} to inject code to kernel for execution (e.g. BadUSB attack\Note{cite}). 
%\sys{} thwarts the attack by defeaturing the original (vulnerability-hibernating) driver code into a lean/tight replayer loop, backed by only three dynamic values at runtime -- register access offsets, DMA descriptor address, and parameterized fields.
%We do not claim the replayer code is bug-free in an absolute sense;
%instead we argue it is much \textit{vettable} than a native device driver.
%We will describe checks at runtime to further mitigate such attacks in next section.

\textit{Attack against TEE via other TEE-OS interface.}
\teedrivers{} shut down pre-existing interfaces forwarding MMC, USB, and VCHIQ requests to normal world OS but not others.
Attacks may still exploit those interfaces to corrupt the replayer or even TEE, e.g. buffer overflow~\cite{optee-crypt-memorybug} in TEE crypto interface, cache side channel attack~\cite{armageddon}.
Mitigating them are orthogonal efforts of TEE, e.g. by deploying TEE kernel stack canaries or eliminates sharing.
%\Note{Should this be ``attack against the TEE via other TEE-OS interface?''}

\end{comment}

%\textit{Attack against shared devices.}
%A malicious OS may turn off devices shared by the whole platform (e.g. power/clock) to mount Denial-of-Service attack against MVP drivers in TEE. 
%\sys{} thwarts this by mediating access to mailbox WRITE register, as described in \S\ref{sec:case:mediate}.
%\Note{We addresses this in S5.5, right?}

%\Note{May remove the following}
%\textit{Attack against device hardware -- out of scope.}
%They are largely out of scope. 
%We list them for a complete discussion.
%\begin{myitemize}
%	\item Device removal:
%	An attacker may simply remove the physical device, e.g. SD card, USB storage, and the camera.
%	\sys{} can detect such attacks retrospectively (i.e. replayer times out waiting for command completion) but cannot prevent them. 
%	
%	\item Bus snooping:
%	Despite TEE isolation, an attacker may snoop the memory bus for data packets traversing between DRAM and devices, thus uncovering the MVP driver activities. 
%	Admittedly, \sys{} is vulnerable to this attack, as any other TEE kernel/apps. 
%\end{myitemize}

\section{Evaluation}
\label{sec:eval}

%In Section~\ref{sec:case} we have analyzed the engineering efforts needed to build a MVP driver using \sys{}. 
In this section we answer the following research questions:
\begin{myenumerate}
	\item 
	What is the overhead of MVP drivers? (\S\ref{sec:eval:overhead})
	
	\item 
	Why are MVP drivers correct and secure? (\S\ref{sec:eval:analysis})
	
	\item
	What efforts are needed if developers build the drivers manually?  (\S\ref{sec:eval:efforts})
	
\end{myenumerate}

%the following questions:
\subsection{Methodology}
%\paragraph{Experimental setup}
%Table~\ref{tab:plat} summarizes our test platform.
%We choose Rpi3 XXX for its popularity and good support for~\tz{}. 
%\Note{redundant maybe}

\paragraph{Benchmarks.}
1) \textbf{SQLite-MMC}: we choose SQLite, a commonly used lightweight database to test MMC.
We pick three test scripts to diversify read/write ratios: select3 (9:1), selectG (6:4), insert3 (5:5) from the testing suites and measure their execution time.
To avoid porting the whole POSIX app to TEE, we record their disk accesses and replay them in TEE.
2) \textbf{SQLite-USB}: we test USB bulk device with the same tests from SQLite mentioned above.
3) \textbf{Camera:} in TEE we request VCHIQ to capture 1, 10, and 100 images frames at 720P, 1080P, and 1440P (the highest resolution) from the camera's still port and measure the latency of each request.
We throttle the replay speed by imposing a 50ms delay between replay actions for VCHIQ to catch up with new messages... 
%4) \textbf{Display:} to test display.
%We ask VCHIQ to render one frame at 720P, 1080P, and 1440P (i.e. the highest resolution) and measure the latencies.\Note{XXX}

%\xzlNote{what template interfaces are invoked?}
Each benchmark invokes 3-10 different templates under the record campaign of the device.
Templates are dynamically selected by the replayer once the given inputs satisfy the constraints;
their details are shown earlier in Table~\ref{tab:mmc:replay_action},~\ref{tab:usb:replay_action}, and~\ref{tab:vchiq:replay_action} for MMC, USB, VCHIQ respectively.
%represented by the record campaign, which consists of 3-10 different templates;
%the replayer dynamically choose a template whose constraints are satisfied by the new inputs. 
%We build the benchmarks using the replayer interface (\S~\ref{sec:design:replay}).
During benchmarks, MVP drivers coexist with normal OS without triggering any kernel fault.

\paragraph{Comparisons.}
We compare MVP drivers (\textbf{ours}) with full-fledged drivers (\textbf{native}) on Linux 4.14 in normal world.
%We turn on and off O\_SYNC flags (i.e. \textbf{native-sync}, \textbf{native-async}) for fair comparisons\Note{discuss}.
We drive same benchmarks as follows:
for \textbf{SQLite}, we replay the block accesses on the MMC \& USB block device with default flags (i.e. O\_SYNC is off) respectively;
for \textbf{Camera}, we run \code{v4l2-ctl} (which we records traces from) to request the same number of frames at corresponding resolutions.
%3) for \textbf{Dispaly}, we render the same image using XXX.
%\xzlNote{native-sync, native-async -- explain}
%\begin{myitemize}
%	\item 
%	V1: Linux. 
%	Benchmarks all run in normal world OS. 
%	This serves as a baseline for performance, which simplified TEE driver desires to achieve.
%	
%	\item 
%	V2: Outsourcing.
%	Device runs Linux and TEE. 
%	Benchmarks run inside TEE but outsource the functions (e.g. disk ops, frame capturing) to Linux drivers. 
%	Disk blocks and image data are copied through shared memory from normal OS to TEE.
%\end{myitemize}
%
%\Note{Ours:} a TEE storage backend which serves disk ops from normal world?



%\subsection{Engineering efforts}
%
%We argue \sys{} requires much less human efforts to develop a functional device driver that suits basic TEE needs than porting.
%
%From the codebase perspective, the device drivers of MMC, USB, and VCHIQ  alone (w/o considering dependent kernel subsystems) consist of XXX SLoC, which translates to XXX man-manth on a COCOMO model.
%In comparison, \sys{}'s replayer only consists of XXX SLoC (XXX man-month), an order of magnitude smaller than the driver codebase.
%Additionally, to develop such a large codebase, the developers must understand XXX different data structures which implement messages, commands.
%In comparison on \sys{}, the \textit{only} data structure the developer needs to understand is DMA descriptor format (XXX, XXX, XXX bytes for MMC, USB, and VCHIQ). 
%
%From the development time's perspective, we trace back to their commit logs on GitHub. 
%For MMC, the first release of core framework takes XXX days to build, involving YYY developers and the host driver takes XXX days, involving YYY developers;
%for USB, it takes XXX days (YYY developers) to build the first release of core framework and XXX days (YYY developers) to build the host driver;
%for VCHIQ, it takes XXX days(YYY developers).
%In comparison, our experience in building them with \sys{} has been smooth\Note{make the work look trivial?}: 
%only XXX days for building the recorder and YYY days for the replayer; 
%in total it takes XXX days for TEE to utilize \sys{} and build trustlets.


% below may be useful
\begin{comment} 
\begin{myitemize}
	\item 
	Scale of codebase in SLoC, compared with existing kernel drivers.  
	This is a direct measurement of engineering efforts.  
	\sys{} should only has a very small fraction (<1\%?) but covers 80\%(?) needed functions.
	This is also about TCB, which is smaller the better.
	
	\item 
	Man-month from COCOMO model. \Note{see also the SLoC utility's calculation of man-month}.
	This shows how fast the developer can develop the driver (at a low cost).
	\Note{analyze the actual development process} -- (from Github and kernel mailing list): 
	how many rounds of code reviews have happened;
	how many developers are involved;
	how long it takes for the first stable release; 
	
	% keywords: software complexity measure; linux kernel complexity
	\item 
	Measures of software complexity \Note{related: Program Comprehension and Code Complexity Metrics: An fMRI Study (ICSE'21); Rethinking complexity for software code structures: A pioneering study on Linux kernel code repository} and \sys{}'s reduction on it:
	\begin{itemize}
		\item binary analysis using entropy \Note{related: An entropy-based measure of software complexity (TSE'91)}. The higher the more complex (more chaotic).
		Our should have a few orders of magnitude smaller entropy.
		
		\item static code analysis: how many kernel subsystems we get rid of; 
		how many host OS (TEE) subsystem rely on (compared with porting);
		
		\item the bytes of data structures the developer should understand.
		\sys{} only requires developer to understand \textbf{a few bytes}, which are only DMA descriptor formats where as for MMC the developer must understand command encoding, etc. for USB developer must understand XXX; for VCHIQ the developer must understand message format which is XXX.
		the number of \Note{device registers} the developers should know to program should also be reduced.
		
		\item 
		The number of pages of the specification. \Note{a little bit weak}
		To implement the same (basic) functions as \sys{}, they need to understand XXX out of thousands of pages of specification (if there's any).  
	\end{itemize}
\end{myitemize}
\end{comment}

\begin{comment}
To systematically study the possible fault scenarios during runtime, we inject random faults at benchmark times.
For storage devices (USB \& MMC) whose software/hardware interactions are mainly through registers, we inject random writes to their command registers (e.g. SDCMD for MMC, HISTS for USB);
for camera (VCHIQ) whose interactions are through messages, we modify the intended request with random values on fields that specify tx position, data size, etc.

We have found the following errors:
\begin{myitemize}
\item 
Reply timeout. 
It is the most common error on three devices -- no response has been received for max timeout (XXX, XXX, and XXX ms for MMC, USB, and VCHIQ) after sending out the latest request.
This is due to incorrect values are written to XXX fields of XXX registers, and XXX fields of the message, which confuses the device FSM and fails to process the request (as intended).
\sys{} detects such an error, aborts the transaction, and does a soft reset on the device, which takes XXX ms to complete. 

\item 
Data CRC. 
Specific to MMC \& USB during block read/write and the syndrome is reported in XXX register, where the transmitted data has been corrupt and needs re-transmission. 
It takes \sys{} XXX ms to redo the transmission.

\item 
Bus error.
It happened to all devices when being supplied non-DMAable addresses (?) or when their power domains are turned off. 
The syndrome is reported in XXX, XXX, and XXX registers respectively for MMC, USB, and VCHIQ. 
It takes \sys{} XXX, XXX, and XXX ms to recover.

\item 
More??

\end{myitemize}
Figure~\ref{fig:fault} shows the time to complete a request in the occurrence of a fault.
Can we recover? What is the cost of recovery - delays, loss of data, etc. 
\end{comment}


\subsection{Overhead}
\label{sec:eval:overhead}
\input{fig-exp-sqlite}
\input{fig-exp-mmc}
\input{fig-exp-usb}
%\input{fig-exp-e2e}
\input{fig-exp-lat}

\subsubsection{Macrobenchmarks}
In this section we report the overhead of aforementioned benchmarks.
\Note{current eval seems simple. Add time breakdown of the benchmarks?}
\paragraph{SQLite-MMC.}
Figure~\ref{fig:eval:mmc-sqlite} shows the results. %for SQLite-MMC and SQLite-USB, respectively.
The MVP driver achieves a decent performance -- an average 422 IOPS, enough to facilitate over 100 SQLite queries per second.
%MVP achieves a decent performance on both MMC and USB: when running 256-sector requests, read throughput of MMC is 2 MB/s, and write throughput is 1.3 MB/s; for USB they are 4.6 MB/s, and 3.1 MB/s, respectively.
%\Note{using QPS? IOPS?}
The performance is a few orders of magnitude better than existing RPMB solution\Note{cite}.

Compared with native, MVP drivers incur moderate overhead, given its simplicity -- it extends execution time by 73\% on average (select3 XX\%, selectG YY\%, insert3 XX\%).
%(MMC: 77\%, USB: 70\%);
Read-most workloads (select3) incurs the slightest overhead by only 43\% and write-most (insert3) contributes the most (99\%).
%The cause for the overhead is MVP drivers (intentionally) eliminates a-synchrony: writes must poll for completion before continuing.
The cause for the overhead is MVP drivers (intentionally) mandate synchronous execution: each request must wait for the previous one to finish before continuing.
%even writes must poll for completion before continuing.
We confirm this by turning on O\_SYNC flag (\textbf{native-sync}) and observe a similar performance difference ($\sim$9\%) with MVP driver.
%\Note{consider discuss microbench in a separate section}
%this work does not address the debate whether TEE should implement/introduce async.


%Figure~\ref{fig:eval:mmc-sqlite} shows the results. %for SQLite-MMC and SQLite-USB, respectively.
%MVP drivers achieves a decent performance on both MMC and USB running the benchmark: MMC has an average 422 IOPS and USB has 361 IOPS, enough to facilitate over 200 queries per second. 
%%MVP achieves a decent performance on both MMC and USB: when running 256-sector requests, read throughput of MMC is 2 MB/s, and write throughput is 1.3 MB/s; for USB they are 4.6 MB/s, and 3.1 MB/s, respectively.
%%\Note{using QPS? IOPS?}
%The performance is a few orders of magnitude better than existing RPMB solution\Note{cite}.
%
%Compared with native, MVP drivers incur moderate overhead, given its simplicity -- it extends execution time by 73\% on average (MMC: 77\%, USB: 70\%);
%read-most workloads (select3) incurs the slightest overhead by only 43\% and write-most (insert3) contributes the most (99\%).
%%The cause for the overhead is MVP drivers (intentionally) eliminates a-synchrony: writes must poll for completion before continuing.
%The cause for the overhead is MVP drivers (intentionally) mandate sequential execution: even writes must poll for completion before continuing.
%We confirm this by running native with O\_SYNC flag on (native-sync) and observe a similar performance difference ($\sim$9\%) with \sys{}.

%Compared with existing RPMB solution, it is a few orders of magnitude better (XXX$\times$ and YYY$\times$ better). Write throughput to RPMB is 2KB/s\Note{cite}).
%This is because accesses to RPMB are splitted into short 512-Byte (i.e. sector) RPMB reads/writes data frames\Note{what about security compared with RPMB?} while \sys{} supports large (e.g. 256 sectors) reads/writes with DMA. 
\paragraph{SQLite-USB.}
Figure~\ref{fig:eval:usb-sqlite} shows the results.
Our USB MVP driver has 361 IOPS, enough to facilitate over 90 queries per second. 
For the same benchmarks, it incur even less overhead than MMC by extending execution time by 70\% on average (select3 XX\%, selectG YY\%, insert3 XX\%). 
The reason is native USB driver is more complex (\S\ref{sec:case:usb}) and slower than MMC (XX\%), which favors the simple MVP driver constituting merely a few hundred replay actions.
Similar to SQLite-MMC, read-most workloads (select3) incurs the slightest overhead by only 43\% while write-most (insert3) contributes the most (99\%).
This is also verified with \textbf{native-sync} -- making writes synchronous brings the performance gap to X\%.

\paragraph{Camera.}
Figure~\ref{fig:eval:cam-lat} shows the results.
At the highest resolution (i.e. 1440P), the latency of \teedriver{} to request one image is 2.9s and that of requesting one hundred frames is 83.6s, which translates to 1.2 FPS, a practical throughput seen on many webcams~\Note{cite}.
The latency of \teedriver{} increases gracefully with the number of requested frames, e.g. 2.1s (one frame) to 61.5s (one hundred frames) at 720P.
This is because per one request, it only pays once a fixed cost (41 interactions) to set up and enable the camera at beginning;
afterwards, it only takes 5 interactions to capture each image.
 
Compared with native, our latency is only 11\% higher for request to capture one frame and is on average 2.7$\times$ higher when capturing one hundred frames.
%Compared with native, \sys{}'s FPS drops by average 42\% (38\%, 44\% and 65\% drop at 720P, 1080P, 1440P respectively).  
%This is because on each interaction, native only queues a single message, which takes less than 1ms while \sys{} has to load up the corresponding memory dump, each taking $\sim$10ms.
The is because we throttle the speed of replaying by imposing a fixed 50ms delay between interaction. %\xzlNote{should state in methodology}
As requests contain more interactions (e.g. 63 vs 567 interactions to capture 1 and 100 frames, respectively), the delays are more pronounced, comprising more than 90\% the overhead.
%\sys{} achieves a close latency (only 11\% larger) with native in capturing a single image when it has least interactions thus the least extra delays.

%the driver means to request frames one-by-one in a sequential and synchronous manner, which aligns with the simple, sequential logic of \sys{} replayer.
% obsolete
%In addition, while recording only software/hardware interactions, \sys{} bypasses the complex kernel stack for managing video buffers, etc. in V4L2 layer, which consists of XXX SLoC and XXX\% of execution time. 
%
%Compared with V2, \sys{} continues to have a leading throughput by XXX\% (XXX FPS) while V2 only has XXX FPS.
%The reason is: in addition to bypassing kernel V4L2 layer, \sys{} further eliminates data move (again), which is subject to resolution and can account for XXX MB at highest (1440P?) resolution and takes XXX\% of the time.
%This trend is shown in Figure~\ref{fig:macro-cam} as well -- as resolution gets higher, \sys{}'s throughput improves by XXX\%. 

\begin{comment}
\paragraph{Frame capturing latency.}

Figure~\ref{fig:lat} shows the results.
Compared with the stock Linux driver, \sys{} is even XX\%-YY\% (average XX\%) better in capturing a frame. 
The reduced latency benefits from bypassing complex kernel abstractions. 
Unlike block layer which optimizes for performance, the bypassed kernel layer manages video buffer and camera configuration, etc., which relies on complicated data structure (e.g. rb tree).
Besides, the workload does not involve large data move -- the highest resolution (1440P) image frame is only XX MB (<2MB), taking less than XX ms for DMA to access.

Compared with outsourcing, \sys{} has a larger margin in reducing latency (XXX\%). 
This is because besides the complex kernel abstraction outsourcing must go through, it must also move to image data into TEE. 

The major overhead for \sys{} is loading the XXX segments (as a whole) to interaction, but is negligible costing only XXX ms, XX\% of total time.
\end{comment}
 
\subsubsection{Microbenchmarks}
We next report the overhead of single read/write request latencies of MMC and USB and the memory consumption of MVP drivers.  
\Note{vchiq microbench?}
\paragraph{Storage read/write latency}
We measure the completion time of completing a single read/write request for MMC and USB, shown in Figure~\ref{fig:eval:mmc-read} and \ref{fig:eval:usb-write} respectively.

In both reads/writes, \teedrivers{}' latency is near-native or even slightly better (12\% for MMC and 13\% for USB).
When there are more blocks (e.g. 256) to write in USB, \teedriver{} is even much 40\% better;
this is due to it does not run complex USB transfer scheduling kernel code to send 4KB data pages to device one-by-one.
%Compared with native asynchronous writes, our latency is 13$\times$-41$\times$ longer, which is expected.
%It's noteworthy that reading one block incurs higher latency than reading eight, because the former goes through the PIO path while the latter goes through DMA path (\S\ref{sec:case}).
%We have noticed the obvious difference between synchronous vs asynchronous writes;
%it is left for future work to address. \xzlNote{what does this mean}

%\xzlNote{the purpose of study native-async writes? And how is the latency measured?}
 
\paragraph{Memory overhead.}
Interaction templates are linked as part of the TEE kernel and loaded into TEE memory.
After compression, their memory overhead is only XXX KB for MMC, XXX KB for USB.
By comparison, native drivers consume XXXKB, which are on average XXX\% larger than \sys{}.
Templates for VCHIQ are larger as they contain mostly memory dumps.
\sys{} uses delta encoding~\Note{cite} to incrementally store dumps;
as a result, 597 dumps that capture 100 frames consumes XXX KB(<100?) of memory.

TEE reserves 4MB as DMA memory for \sys{}, which is enough to host data buffers (up to 128KB for MMC \& USB, 2MB for camera JPEG) and also DMA descriptors (tens of bytes each).

\subsection{Analysis}
\label{sec:eval:analysis}
We discuss correctness and security breaches separately. 
Correctness violation is caused by semantics bugs in the software stack; 
security breaches are caused by active attackers who compromise the software stack. 
%We present an analysis in three aspects: correctness, security, and developer efforts in building MVP drivers.

\subsubsection{Correctness}

We thoroughly test the correctness of MVP drivers as follows.

First, we have empirically verified the replay correctness of all benchmarks.
We manually examine their data content: for MMC \& USB, we verify our reads match those by native drivers, and our writes can be read back by native drivers;
for VCHIQ, we dump captured images in normal world and verify their intact JPEG header and content.
%Additionally, we plant extensive tracing points to reflect comprehensive execution states and compare them with existing recordings. 
We also collect their device interactions and compare them with existing recordings. 
%we dump over 50 \& 500 register values (e.g. SDCMD \& GNPTXSTS as status registers) of MMC \& USB during execution;
%we dump over 400 bytes of fields containing VCHIQ messages for VCHIQ;
we examine their values \& verify they fall into the envolope interactions listed in Table~\ref{tab:replay_actions}. %and is not state-changing hence negligible. 

Second, we have stress tested our MVP drivers:
for MMC \& USB, we have run read/write requests over each sector within bound (over 30 million sectors for MMC, 15 million for USB) and examine their data content as before; 
for VCHIQ, we have run the frame capturing requests continuously for 10K times whereas every run produces consistent \& deterministic interactions, and reliably capture the frames.
During the stress test, it takes 30us, 100us, 90ms for MMC, USB, VCHIQ to reset, respectively.

\xzlNote{make connection to prior RnR validation. This is also what they did}


\subsection{End-to-end use case}
\input{fig-use-case}

We build a trustlet for secure surveillance using MVP Drivers, which requests one image frame from the camera and persists it on MMC card.
Figure~\ref{fig:eval:use-case} shows the code snippet. 
The drivers are easy to use -- the trustlet only has to include one header file which specifies the callable interfaces of camera and MMC;
it then supplies concrete inputs to the interfaces. 
During replay, the replayer dispatches the corresponding template which satisfies the constraint on inputs. 
In case any state transition divergence (e.g. card is removed), it prompts error for user to handle, who may simply reset the device and re-execute. 


\begin{comment}
\paragraph{Iozone throughput.}
\input{fig-exp-tput}
Figure~\ref{fig:tput} shows the results.
Compared with stock Linux driver which has an optimal (desirable?) performance, the in-TEE storage device shows a slight throughput drop (MMC XXX\%, USB XXX\%, on average XXX\%), 
The reason is due to simplicity of \sys{}:
1) by mapping the block read/write (block address \& read/write size) directly into recorded driver interaction, \sys{} bypasses the block layer which is responsible for re-ordering and merging block requests to improve throughput. 
We confirm this by profiling the block layer;
we have found it re-arranged XXX block ops and merged XXX block ops. 
Turned off, the throughput is down by XXX and is close to \sys{};
2) sporadic block access such as strided read/write do not fully utilize block commands (e.g. CMD XXX) because they're out of the beaten path and \sys{} do not record them;
3) occasional soft reset of the device halts the replay pipeline from time to time. 
The soft reset is triggered due to a mismatched value in XXX register, indicating the current command has not finished;
while stock driver will parse the value and wait for timeout, \sys{} chose to directly abort the transaction and reset, which hinders the throughput.

Compared with the outsourcing, \sys{} is slightly better (YYY\%).
This is due to despite the full block layer the outsourcing approach has, it wastes significant time in data move from normal OS to TEE (XXX\% of th time), while \sys{} directly read data into TEE memory.
\end{comment}

\begin{comment}
\paragraph{An example trustlet: Trusted Camera}
\input{fig-exp-e2e}
\Note{unclear}
We build a trustlet atop the in-TEE device drivers enabled by \sys{}.
The trustlet is a trusted camera, which periodically captures a frame of various resolutions and stores the frame in the underlaying MMC storage;
we consider the end-to-end latency \& throughput as the performance metrics and compare them with stock Linux.

Figure~\ref{fig:e2e} shows the results.
The performances are practical for trustlets -- XX ms and XXX FPS at high-resolution (1080P).
Compared with Linux driver, \sys{} does not suffer from noticeable performance loss across different resolutions, only XX\% and XX\%. 
In lower resolutions, \sys{} has even better performance, i.e. smaller latency -- only XXX ms and larger throughput -- XXX FPS.
As resolution gets higher, \sys{}'s latency slightly increases by XX\% and throughput drops by XX\% due to larger image size but they are still on a par with stock kernel comparisons.

%\paragraph{Implications on trustlets}
%Consider typical trustlets: is the above performance practical? How is it translated to trustlet performance? 
\end{comment}



==> fig-devices.tex <==
% !TeX root = main.tex
\begin{figure}
\centering
	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/devices}
	%\vspace{-5mm}
	\caption{Device stack. XXX: add mailbox?? TODO-- switch USB vs MMC}
	\label{fig:dev}
	%\vspace*{-3em}		% use as needed
\end{figure}


==> fig-discovery-example.tex <==
% !TEX root = main.tex
\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth{}]{./figs/fig_discovery_example}
	\caption{\sys{} finds in-memory descriptors recursively via differential analysis.}
	\label{fig:discovery_example}
%	\vspace*{-1em}
\end{figure}


==> fig-exp-e2e.tex <==
% !TeX root = main.tex
\begin{figure}
\centering
	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/fig_vchiq_fps}
	%\vspace{-5mm}
	\caption{FPS of Trusted Camera}
	\label{fig:eval:cam}
	%\vspace*{-3em}		% use as needed
\end{figure}


==> fig-exp-tput.tex <==
% !TeX root = main.tex
\begin{figure}
\centering
	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/plot/tput/plot}
	%\vspace{-5mm}
	\caption{throughput of storage device}
	\label{fig:tput}
	%\vspace*{-3em}		% use as needed
\end{figure}


==> fig-exp-usb.tex <==
% !TeX root = main.tex
\begin{figure}[h]
	\begin{minipage}[t]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figs/plot/micro/usb/fig_usb_read_micro}
		%\vspace{-5mm}
		\subcaption{Read latency}
		\label{fig:eval:usb-read}
	\end{minipage}
	\begin{minipage}[t]{0.23\textwidth}
		\centering
		\includegraphics[width=\textwidth]{./figs/plot/micro/usb/fig_usb_write_micro}
		%\vspace{-5mm}
		\subcaption{Write latency}
		\label{fig:eval:usb-write}
	\end{minipage}
	\caption{Mircrobenchmarks for USB}
	\label{fig:eval:usb-micro}
	%\vspace*{-3em}		% use as needed
\end{figure}


==> fig-impl.tex <==
% !TEX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/impl}
%	\vspace{-2em}
	\caption{Recorder implementation.}
	\label{fig:impl}
%	\vspace*{-2em}
\end{figure}


==> fig-polling-example.tex <==
% !TEX root = main.tex
\begin{figure}[h]
	\centering
	\includegraphics[width=0.35\textwidth{}]{./figs/fig_polling_example}
	\caption{\sys{} summarizes register polling into replay action with confirmation from the developer.}
	\label{fig:polling_example}
%	\vspace*{-1em}
\end{figure}


==> fig-proto.tex <==
% !TeX root = main.tex
\begin{figure}
\centering
	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/proto}
	%\vspace{-5mm}
	\caption{Devices used in prototype:XXX:map the block diagram to the photo??}
	\label{fig:proto}
	%\vspace*{-3em}		% use as needed
\end{figure}


==> fig-rec-path.tex <==
% !TEX root = main.tex
\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth{}]{./figs/rec-path}
	\caption{The idea of \sys{}. LWG: add divergence handling XXX add replay?}
	\label{fig:rec-path}
%	\vspace*{-1em}
\end{figure}


==> fig-replay.tex <==
% !TEX root = main.tex
\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth{}]{./figs/replay}
	\caption{Replay workflow}
	\label{fig:btt}
%	\vspace*{-1em}
\end{figure}


==> impl-old.tex <==
% !TeX root = main.tex

%\section{Implementations and Experiences}
\section{Implementation \& experiences}
\label{sec:case}


%\Note{TODO: show a table of discovered values \& registers, similar to table 1 in Discoverer paper}

%\Note{Section title -- } Implementation \& experiences? 

\input{fig-exp-setup}

\input{fig-devices}

%\input{fig-proto}

\input{tab-case-study}

\input{tab-trace}

Figure~\ref{fig:dev} shows devices recorded by \sys{} and their software stack.

We applied \sys{} to a variety of devices
Our criteria for selecting devices: 
\begin{myitemize}
\item 
the device has important use cases of secure IO 
\item 
the device driver is complex and known difficult for TEE 
\end{myitemize}

Our test platform is Rpi3. 
We choose it because of its popularity and good support for open-source TEE software.
As we will show, despite an active community and high attention for Rpi4, (far more than most other SoC hardware), building TEE drivers is nevertheless difficult. 
\Note{It is also a device} with proper amount of open-source vs proprietary components -- while difficulty in implementing a TEE driver is in hindsight (i.e. largely through reverse engineering), we can still reason about it from its open-source implementation.

The recording environment is Raspbian Linux. The kernel version is XXX. 
All recording harnesses are user programs. 
The TEE for replay is OPTEE-4.2 on the same machine. 

\Note{turn off for submission}
\subsection{Thoughts}

\begin{myitemize}
\item we seek to understand -- what is the least dynamism required for a device to perform its basic functions (e.g. rw data, capture datapoint)?

\item defeaturing is not only getting rid of (unnecessary) kernel contexts but also a large part of code that deals with "dynamism", which leads to many conditional branches (i.e. FSM transitions) -- \Note{this also our key mechanism to get rid of vulnerabilities}


\item experimentally, the only dynamism required (or divergence allowed) is about data but not control, e.g. data dst/src, size. 
This is true in storage and vchiq cam.

\item consequently, the \textit{only} knowledge developer needs to understand is data structure that describes the data (i.e. DMA desc.). 
E.g. which offsets specify data src during replay, proper DMA descriptor.

\item 
the impl. of test harness directly affects the recording. 
Can provide "enough" options (e.g. img res, format) of test harness and thus supplying "diverse enough" recordings to replay.
\Note{how to select the "right" test harness if there's a performance difference?}

\item robustness of replay on non-recoverable divergence. 
Simple dev like SDhost might be settled by resetting. 
VideoCore is much more complex -- firmware is an OS. 
What if the states are messed up (e.g. firmware is overflowed and re-written) lead to non-recoverable divergence? 

\item heuristics and assumptions: 1) device has no iommu; 2) DMA address must imply data move between kernel \& device and needs attention. 

\item Partial-porting is infeasible -- one cannot easily and cleanly decouple a single path out of the whole complex FSMs.

\item how to decide if one field is parameterizeable? Size is not. What about starting address? \Note{have a table}

\item What about the constraints on parameterized field? Alignment, size, etc. 

\item what if the parameterized user input is not straightforward? E.g. being encoded inside a few bits in a cmd.

\item set relations: dynamic values = parameterizable fields V ignorable values

\end{myitemize}

\subsection{MMC}

MMC is a common interface to off-chip flash, e.g. SD cards and eMMC. 
% To access flash storage, 
%To implement secure storage, the TEE should run its own MMC driver bypassing the untrusted OS. 
Lacking MMC drivers, a current TEE saves data by invoking the untrusted OS and applies end-to-end data encryption \Note{cite} 
%This method suffers from a few drawbacks: as data flows through the OS, it is vulnerable to availability attacks and side channel attacks. 
It is vulnerable to availability attacks and side channel attacks mounted by the OS. 
it requires special flash partition (e.g. RPMB) which is limited in size and speed. \Note{cite}


%\paragraph{Long-wanted secure storage.}
\paragraph{Device overview}
Figure XXX shows an MMC stack. 
Applications \Note{filesystem?? block layer??} submits block read or write to the device driver, which in turn operates on an MMC controller. 
The MMC controller implements the bus protocol communicating with the flash. 
%A MMC host's finite state machine (FSM) is standardized. \Note{cite}
A MMC host's finite state machine (FSM) consists of 13 states with hundreds of possible transitions among them. 
As stated in Section XXX, the complexity roots in 
(1) performance optimization: not only transferring individual blocks but streaming blocks; dynamic tuning of bus clock; 
(2) dynamism: multiple cards; connected/disconnected at any time (even in the middle of transfer); open-ended transfer without pre-defined sizes;  
(3) corner cases: assuming MMC bus/medium is volatile; attempt to recover from bus/medium error in place. 

MMC controllers have diverse instantiations. % and do not conform to standard. 
%A controller's interfaces (registers and DMA descriptors) are vendor-specific.
Their interfaces are often either undisclosed (e.g. Rpi3 ...) or poorly documented. 
%even if they are public, the documentation of host hardware is often long (e.g. XXX pages). 
Undocumented silicon bugs are not uncommon \Note{cite}. 

%Linux implements the MMC FSM and drivers for a myriad of MMC hosts. 
Linux incorporates a large MMC framework. 
It abstracts the common driver logic as a ``MMC core'' (15K SLoC in 40 files), atop which it implements device-specific code for a myriad of MMC controllers (around 4K SLoC each \Note{check the numbers}). 
The MMC core and a controller driver communicate via a wide interface -- 44 callbacks and 4 structs (XXX fields) 
%which spans 60K SLoC in 107 files. 
%mmc_host_ops: 19, mmc_pwrseq: 4, mmc_bus_ops: 12, mmc_cqe_ops: 9, 
\Note{present any existing vulnerabilities in driver?}

% Such a method suffers from capacity limitation, 

%\textbf{Functions}:
%\paragraph{Selected requests}
\paragraph{Workflow}
We choose to implement only XXX requests: 
% read \& write of a single data block; read \& write of multiple data blocks, where the block count can only be 8, 64, 128, or 256.
read \& write of data blocks, where the block count can only be 1, 8, 64, 128, or 256.
A request accepts two arguments: the starting block number and the physical address of data buffer. 
(1) By setting a fixed block count for each request, we ensure each handler sees deterministic device state transitions. 
As we will show below, the transitions of device states can vary significantly  when different numbers of blocks are read/written. 
(2) The above block counts (and their combinations) are sufficient to trustlets we target. 
%  the driver will take different execution paths 
%  and \textit{size}.

%Separate single block read/write from multi-block rw is to fit into kernel behavior when smallest DMA-able unit is a page (4KB).

%\Note{merge}
%For instance, the transactions for MMC driver include read/write of a block, tune the MMC bus, and rescan the medium for changes.
%
%Storage device: (rw, block \#, size), use `dd' or `iozone'

\paragraph{Discovered interfaces}
%\sys{} traces the full MMC driver for its initialization, reset, and the requests selected by us. 
%\sys{} records MMC initialization at driver probing stage. 
%During the stage, kernel reads in MMC's device tree blob (DTB) entries;
%they specify the clean-state (i.e. initial) MMC states (e.g. power, clock) and therefore instruct MMC initialization sequence. 
\sys{} traces request execution by running the user utility `dd' with the sync \& direct flag. 
From the test, \sys{} discovers 15 (??) registers, including their physical addresses and the source locations of access. 
\sys{} flags a register (DMA\_ADDR) as a physical pointer to an in-memory DMA descriptor spanning 8 words; 
\Note{refer to table}
it further flags the descriptor's word 2nd, 3rd, and 6th as another three  physical pointers. 
By examining XXXX source lines that populate these pointers, we confirm \sys{}'s findings: word 2 and 3 point to a scatter-gather buffer (i.e. data buffer) for DMA transfer and word 6 chains multiple DMA descriptors as a scatter-gather list. 
Based on discovered interface, \sys{} records the access of 15 registers, takes snapshots of the DMA descriptor list, and parameterizes the addresses of each scatter-gather buffer addresses.  \Note{how to deal with the last one}
\Note{take DMA snapshot does not need to understand XXX..}

% developer examines the MMC descriptor.It is a 8-word data structure, where the first five words specify data length and address (also a DMA address) and the 6th word specify the next chained descriptor, if any.

\paragraph{Segments of interactions}
Table~\ref{tab:trace} lists XXX segments of interactions emitted by \sys{}, which constitute the TEE driver ready for deployment. 
It is worth noting that these raw traces vary greatly in length. 
The request of read a single block, for example, may result in 30 --- 130 register accesses. 
\sys{} attributes the non determinism to two loops of register polling, which we confirm with ease. 

\paragraph{Post analysis}
Although not required by generating the TEE driver, we analyze the recordings and correlate them with the full driver code to shed light on 1) what are discovered and recorded and 2) how much effort would be needed to produce the same driver behaviors. 
\Note{also contribute to verifying correctness}

The registers discovered by \sys{} fall into three groups: for configuring the controllers (e.g. SDCDIV to set clock; SDVDD to set voltage; SDHCFG to configure interrupt, bus width), for sending/receiving commands/responses to the MMC peripherals (SDCMD, SDARG), and for controlling the DMA transactions (DMA\_CS, DMA\_ADDR). 

The segment for device initialization has captured rich interactions. 
Notably, the driver configures the MMC clock by communicating with the firmware. 
It does so by sending a SET\_SDHOST\_CLOCK to firmware containing a 3-word payload; 
\sys{} records the payload as magic values, which lack public documentation\Note{cite}.
The driver resets the rest of MMC state machine by writing other magic values (all 0s or 1s) to 10 different  registers. 
The driver further probes various device registers in order to calibrate command timeout. 

% 	The process contain 18 accesses to 10 different host registers, where there are 17 writes and 1 read to SDEDM register.
%It first resets most registers by writing 0's or 1's to clear the status, then based on the clock \& clean-slate state read from DTB, the driver calibrates command timeout and sets up corresponding registers.
%\sys{} also records delays of waiting for device state transitions (e.g. power state, FSM).  
	

% https://github.com/raspberrypi/firmware/wiki/Mailbox-property-interface
% missing tag documentation: https://github.com/raspberrypi/firmware/issues/719
%Configuring the clock. 
%It is done by firmware. 
%The driver prepares a message containing a 3-word tuple as payload (0x0, 0xffffffff, 0xffffffff) and a header specifying SET\_SDHOST\_CLOCK tag.
%It then sends the message to firmware through mailbox interface to enable the clock.
%It is noteworthy that these message formats lack comprehensive documentation\Note{https://github.com/raspberrypi/firmware/issues/719}, which is overcome by \sys{}'s recording approach.
	

Interactions in requests exhibit two patterns which correspond to two distinct driver paths. 
(1) to read/write fewer than 8 blocks, the full driver shifts individual words from/to the controller's register (SDDATA). 
(2) to read/write greater than or equal to 8 blocks), the driver uses DMA transactions to move the data. 
Notably, even when using the DMA transaction, the driver moves the last 3 words via register access. 
%By examining the driver source, we find 
% discovers a comment stating 
This seems to work around an undocumented bug in the SoC's DMA engine, which cannot move the last few words of a transfer. 
\Note{experiences: sector alignment... must be multiple of 8}

% only the the 9 host registers are used (PIO paths); 
% Initial runs of \sys{} locates in total 11 registers in use during tests, among which 9 (i.e. SDDATA, SDHSTS, SDHCFG, SDRSP0, SDCMD, SDEDM, SDARG, SDHBCT, SDHBLC) belong to the host controller and the other 2 (DMA\_CS, DMA\_ADDR) are of the global DMA engine for initiating DMA transactions. \Note{registers used in initialization are not counted here, e.g. to set clock, SDVDD to set VDD}

% The first (PIO) path (read/write size <4KB) contains 160 $\sim$ 1300 register accesses while the DMA path (read/write size > 4KB) only contains $\sim$ 64 register accesses.  

% 2) otherwise, two DMA registers are additionally used, with 3 words of tailing SDDATA register access.  Interestingly, we check out the source code and find the tailing SDDATA register accesses overlaps with the first PIO path;
% it is due to a silicon bug of RPi3 -- its DMA engine cannot access last few words of the DMA page, which can only accessed through PIO.

%\paragraph{What-if analysis}
\paragraph{Analysis of developer efforts}
Table XXX lists the efforts required by \sys{}: inspecting XXX lines of code (XXX locations in XXX files) to confirm annotations of XXX registers. 

%\textit{The efforts for building a small driver from scratch}
\textit{If developers build a small driver from scratch...}
(1) The developers must identify device state transitions for each request, for which they reason about the MMC standard (a document of 231 pages). 
Even for a simple request, e.g. multi-block write, the developers picks one of possible transition paths: open-ended write, writes with pre-defined block count, and  reliable writes with predefined block count. 
(2) Each transition path require different selections of MMC commands, each encoding different fields and flags. 
Odd enough, not all MMC controllers support all MMC commands, e.g. some controller lacks CMD 23 (set block count). 
(3) The developers map the selected commands to the concrete MMC controller registers and 
produce 1300 reads/writes of 15 distinct registers. 
They will encounter the silicon bugs, e.g. the DMA quirk as stated above, which requires tedious guess work and trial-and-error debugging. 
%which seems difficult, if not impossible to fix without internal documentation. 


\begin{comment} ---- useful --- 
The developer must understand:
1) A trimmed state transition path of the selected function (e.g. read/write multiple blocks).
To this end, the developer must navigate through the MMC standards, which is a 231-page documentation\Note{cite}. 
It is a hard process -- the developer not only flips pages to put individual commands into a full path, but also he must choose wisely such a path.
E.g. for the single event of writing multiple blocks, the specification provides at least three paths: 
1. open-ended write which must end with a CMD 12 (stop transmission); 
2. writes with pre-defined block count (i.e. the recorded one) which starts with a CMD 23 (set block count).
3. reliable writes with predefined block count and a reliable write parameter, which even has two versions. 
2) The semantics of commands on the chosen path.
In our case, there are at least the six ones used in our workload (i.e. CMD13 send status, 17 read single, 18 read multiple, 23 set block count, 24 write single, 25 write multiple).
This is tedious and non-trivial as commands have multiple fields for encoding different flags \& control (e.g. whether the command is new, whether it's expecting valid CRC). 
More importantly, developer must clearly understand when and what flags to use, which is dependent on the hardware capability (e.g. some controller may not support CMD 23).
3) The developer must map the above two parts of knowledge to the actaul MMC hardware.
To do so, they refer to the hardware manual (if any), identify register/in-memory descriptors needed for the device/driver interactions. 
Even for a request as simple as reading one block, the interactions are non trivial (e.g. 1300 reads/writes of 15 distinct registers)
They will encounter the silicon bugs, e.g. the DMA quirk as stated above, which seems very difficult, if not impossible to fix without internal documentation. 

%To always issue CMD 23 before CMD 18 and 25 but not before CMD 17 and 24. 
% http://yourcmc.ru/wiki/images/5/55/EMMC_JESD84-A441.pdf

%The developers: choose the request semantics to implement and trim down the FSM accordingly: 
%examine the MMC standard, identify needed states and implement the related transitions. \Note{TBD: more specific}
%They map the required state transitions to the actual MMC host hardware. 
%To do so, they refer to the hardware manual (if any), identify register/in-memory descriptors needed for the device/driver interactions. 
%Even for a request as simple as reading one block, the interactions are non trivial  (e.g. XXX reads/writes of XXX distinct registers; access of XXX in memory descriptors)
%They will encounter the silicon bugs, e.g. the DMA quirk as stated above, which seems very difficult, if not impossible to fix without internal documentation. 
%
%Hardware (SoC) specific; hardware quirks, details.
%Tuning. probing, configuration, clock, power, bus width, bus speed. e.g. periodic tuning ... register formats, hardware quirks, different voltages supported by cards (dual voltages), etc.
\end{comment}
\Note{compress}
\textit{If developers port the Linux MMC driver...}

Compile -- thousands of errors. broken dependency. What is worth fixing? What is not needed? 

(1) Reason about the MMC driver codebase (XXX SLoC in XXX files). 
Identify the frameworks (platform\_drv, clock, power, block) the MMC drivers register to; identify the interface (callback functions, struct to fill). 
Identify source files that need recompilation. 

(2) Code tailoring with MMC domain knowledge. 
Developers constantly face a dilemma: 
removing unused code requires deep MMC knowledge and high efforts (including debugging); requires trial and error. 
moving code as-is bloats the TEE and requires to port more dependencies (a vicious cycle, dependency snowball)
No guarantee tailoring attempts will succeed. Trial and error. Earlier decisions may turn out to be wrong (e.g. a removed feature breaks the needed functions in a subtle way). 

Two examples. 
A substantial amount of driver code (XXX) is for dynamic discovery of MMC cards.  
To simplify the functionality, developers need to understand related MMC concepts -- IOS, bus width, voltage, data rate (device class: HS200, HS400), powerclass; CSD register parsing; capabilities. 
Decide which features are needed by the selected requests (simple block read/write). 
Some concepts only apply to specific flash types (eMMC versions). 
Which of them apply to the device of interest? 
If developers forgo the effort and instead keep all the discovery code for ease, they have to port the kernel dependency -- kernel device tree (for reading static device capabilities) and power frameworks (for voltage, regulators, etc)

Another example, to simplify/remove periodic bus retuning (or slot rescan), developers need to understand its role in MMC protocol (the performance significance of periodic tuning) and carefully peel off all the related code (XXX SLoC in XXX functions). 
This process is error prone, though: 
developers must not eliminate \textit{initial} bus tuning, as doing so would leave MMC bus parameters unset and barely usable performance. 
If they decide to keep the retuning feature just for porting ease, they will have to port/emulate all the mechanisms underneath retuning, e.g. kernel thread. 
% To minimize the TCB, they need to reason about the codebase. 
% e.g. if concurrent request submission is not needed, developers may remove such a feature; 
% otherwise, they will have to implement work deferral. 
% is e.g. replacing tens of runtime power management (???) callbacks with dummy functions. 
% This further requires to examine the code and remove \Note{XXX} features such as host device abstraction, runtime power management, slot rescan and retune daemon threads, request queue, debugfs, etc.; 
% resolve compilation issues. 


(4) Reasoning about kernel dependencies. 
Even after aggressive trim down, the resultant MMC driver code need essential kernel dependencies: scheduler, workqueue, allocator, deferred work. Have to port or emulate. 
An example is DMA API. It is a generic kernel framework. Complex with less documentation. 
Developers need to understand the API semantics (which is x86 oriented for historic reason; far from the developer goal of MMC). The APIs further dynamically dispatch to CPU/architecture-specific implementations which the developers have to identify and port. Examples: software IO TLB. Pure software abstraction. 

\textbf{Lines of code}

These services will have to be ported or emulated (with the same interfaces, there are XXX function callbacks) inside the TEE. 
Deal with compilation and debugging issues. 

%This process of code reasoning and refactoring is tedious and error-prone. 
%For example, if developers deem periodic bus retuning (or slot rescan) as  unneeded, they shall identify and carefully peel off all the related code. 
%However, improper removal of the initial tuning breaks MMC functions and crash the device. 
%If they decide to keep the retuning feature just for porting ease, they will have to port/emulate all the mechanisms underneath retuning, e.g. the kernel thread, which further requires to port more c ode. 


%\Note{the following still needed?}
%The reason for such a stark difference in number of register accesses is discovered at sequence alignment time: 
%on the first path, \sys{} discovers value divergence of access to SDDATA registers;
%\sys{} traces back these values are from tests and are transmitted to device word-by-word through the SDDATA register\Note{do we have this level of automation??}.
%On the second path, \sys{} discovers physical addresses being written to DMA\_ADDR register, hence suggesting the developer de-reference a DMA descriptor;
%the developer then locates and annotates the DMA descriptor, which instructs the device to transmit a large chunk of data in one shot, accessing $\sim$ 40 registers to set up set up DMA address, kick off, and complete the data transfer.
%Additionally, the only non-deterministic interactions discovered by \sys{} is the number of reads to SDCMD register on the PIO read path, differing by 1 $\sim$ 9 times;
%\sys{} hence suggests a polling exists and prompts the developer to fix/annotate it.

%It does not find divergence in terms of values \& types registers being written to and read from.
%It however discovers across two recordings, the number of read from SDARG (\Note{confirm}) are different, which is due to polling. 
%The tool then prompts the developer to summarize the polling behavior, which will be reflected at replay time.

%\Note{useful}
%\textbf{Finding the software/hardware interaction:}
%Upon each test/function invocation:
%\begin{myenumerate}
%	\item 
%	The tool first instruments call stacks of the read/write function using existing kernel function tracing facility.
%	As its discovery, there are two different paths involved in the function:
%	
%	\item 
%	After locating the involving devices, the tool instruments all 1) ioremap, 2) register access, 3) DMA memory allocation, and 4) data barrier \& delays.  	
%
%	\item 
%	The tool then runs the test function again and learns from the instrumentation:
%	\begin{myenumerate}
%		\item from 1) the tool records the physical address of the SDhost and DMA engine, which will be mapped at replay time
%		
%		\item from 2) the tool records what values are being written and read to/from which register in order.
%		These values include command encodings, data addresses, sizes, \& their sequence (e.g. CMDa -> CMDb -> CMDc for read function), device status, etc. and are core to driving the read/write function;
%		
%		\item from 3) the tool discovers in-memory DMA descriptor.
%		This is done by correlating the value allocated physical pointer \& the value written to device registers (i.e. SDARG register in host). 
%		It is a 8-word data structure, where the bytes specify whether to turn on DMA IRQ, DMA address, its size and pointer to the next DMA descriptor. 
%		
%		\item from 4) the tool summarizes command timeout during replay.
%		The value was calibrated by the kernel driver after XXX rounds of sampling and was done by YYY SLoC.
%	\end{myenumerate}
%	
%	\item 
%	The tool run the test function again to find divergence (align sequence).
%	It does not find divergence in terms of values \& types registers being written to and read from.
%	It however discovers across two recordings, the number of read from SDARG (\Note{confirm}) are different, which is due to polling. 
%	The tool then prompts the developer to summarize the polling behavior, which will be reflected at replay time.
%	
%\end{myenumerate}


%\paragraph{Replay:}
%
%\textbf{Interface:} block interface as in `/dev/blk'.
%POSIX-like interfaces for `read' and `write' (rw/, off, size).
%
%\textbf{Simplistic replayer in TEE}
%
%The kernel daemon processes for MMC includes a request queue, a cmd timeout timer, a periodic retune/rescan timer...
%
%Due to simplicity goal we reduce them in TEE...
%
%1) request queue -- original designed for sharing, async exec in normal world;
%in TEE there's no notion of concurrent trustlets thus no sharing.
%The request queue is reduced to a simple handler which continuously serves the reg access from replayer...
%Reads are synchronous; writes can be async...
%
%2) no timeout timer daemon.
%The timeout logic is embedded into replayer (?)
%
%3) no continuous rescan daemon.
%Our assumption is the card/emmc stays put...

%
%\Note{merge this}
%\textbf{Symbolize data entries only.}
%The insight is it only takes 4 entries to describe any data op, i.e. data source, destination, starting address, and length of the op.
%\sys{} asks developers to annotate only these entries in source code (w/ customized decorations recognized by compiler) before recording.
%Recorder only symbolizes these entries while treating all other values fixed/static, as part of the deterministic replay context.
%\Note{this includes commands passed in register AND in memory (e.g. DMA command)}

%\Note{merged}
%\paragraph{Example: embedded flash drivers} (interleave)
%
%{Overview...architecture}
%
%https://wiki.st.com/stm32mpu/wiki/MMC\_overview
%
%Flash driver is complex:
%
%We did a code analysis of XXX flash drivers.
%Why complex? rich protocol, support for diverse medium, error prone.
%
%The specification mandates a core set of semantics.
%Other details of behaviors, implementation, etc... are SoC specific.
%
%\paragraph{Observation}
%code complexity (and hence engineering difficulty) come from configuration, power/clock management; tuning;
%
%\paragraph{Simplified...}
%
%No abort. No partial transfer. No stream transfer. No open-ended transfer (all transactions have pre-defined size)
%
%No multiple card (connected, disconnected)
%
%No stream transfer. Only block-oriented transfer.
%
%No clock control. used by host to slow down the card.
%Misc: write protection; no password (defeaturing)
%
%How about Trim, secure Trim, Erase?
%
%\paragraph{Failures}
%
%Embedded flash is error prone. Corner cases of errors (card removal, timeout, card failure, etc.)
%
%See JEDEC standard 7.8
%
%CRC error; timeout (no response); invalid command; loss of medium; ...
%
%illegal parameters from the host side (out of range, write protect violation, etc)

\begin{comment}
\subsection{DMA transactions}
\textbf{SoC specific:}
Capture in-memory descriptors? Like DMA

\paragraph{RPI3}
DMA engine separate from MMC host.
3 directly writable registers for controlling DMA engine, CONDBLK\_ADDR, CS, DEBUG.
CONDBLK\_ ADDR stores the phys addr of head of the linked control block data structure;
a control block is an 8-word data structure that guides data tx/rx behavior of DMA, each word containing: transfer information, data src addr, dst addr, dma len, stride, next cb addr;
rest two words are reserved.
 
Other fields are self-explanatory (next cb addr = 0x0 at tail control block).

SDhost initiates the data transfer process by reading/writing some sdhost regs to setup starting block addr, block size, etc.
Then the control is transferred to DMA engine side to set up the control blocks, including allocating DMA mem and filling each word entry.
It kicks off the DMA by writing 1 to CS reg of DMA.

Once the DMA completes, an IRQ is sent to trigger DMA IRQ handler.
In the DMA handler, kernel acknowledges the IRQ, then calls into SDHost callbacks to acknowledge some statuses on the SD hosts.
An interesting thing is host seems to keep a counter for DMA control block in SDEDM.
Read to SDDATA register will decrement it until it reaches 0.

\Note{Thoughts: handling} the cross-dependency between sd host and DMA drivers?

Our design eliminates the callback mechanism which is only a "feature" which is simply a good software practices.
The system implements IRQ handler as a large, monolithic reg access replayer (i.e. DMA reg and SDHost reg co-locates in the same namespace, unlike kernel).
This is due to simplicity and goal of defeaturing.

\paragraph{Limitation on TEE}
DMA might be limited on TEE, depending on the configuration of TZASC.
It requires DMA engine can access the partitioned secure memory inside TEE (i.e. a bus address).
Also the memory has to physically contiguous.
\end{comment}


%\subsection{USB Mass Storage}
\subsection{USB}

%USB is a pervasive interface for peripheral devices, e.g. mass storage, cameras, microphone. 
% Lacking USB drivers, the current TEE misses the opportunities of accessing these devices. 
% A USB driver within TEE opens door to many more opportunities of other devices. 

\paragraph{Device overview}
USB serves as a common transport between CPU and diverse peripherals, e.g. cameras, keyboards, and flash drives. 
Figure~\ref{fig:dev} illustrates a USB stack. 
A device driver programs the USB controller to initiate \textit{transfers}, 
each comprising a series of \textit{transactions}. 
A typical USB controller exposes more than 100 registers. % and uses DMA for data move. 
The USB controller translates each transaction into multiple packets on the bus. 
% registers and moves data to/from the controller; % by register accesses or DMA transactions. 
%the USB bus carries four types of \textit{transfer}, e.g. bulk transfer for mass storage. % and interrupt transfer for keyboards. 
%Each transfer is a series of transactions between the USB controller and a peripheral; each transaction further comprises multiple on-wire packets. 
The USB standards mandates the transaction details as well as 
the controller FSMs during each transaction. 

%A USB controller bridges CPU with USB peripherals, 
%the USB controller translates the access to on-wire protocol interfacing with the peripherals. 

% In the stack, the driver implements much of the USB standard which consists of complex state machines. 

%USB serves as a common transport for diverse peripherals. 
%By definition, each USB peripheral (e.g. a camera) consists of multiple configurations, each of which consists of multiple endpoints. 
%To support diverse devices, 
%Atop the transfers as building blocks, drivers further implement data exchange protocols specific to peripherals.  

\paragraph{Current status}
Linux kernel fully implements the driver FSMs as mandated by the USB standard. 
The driver code comprises 21K SLoC in 82 files. 
These FSMs are big in order to accommodate rich features (e.g. dynamic discovery of bus topology, hot plug) and various runtime conditions (e.g. device speed mismatch, bus checksum errors, over current). 

% See impl of enum usb_otg_state {}
%In total, a full USB driver implements 14 states, YYY transitions\Note{how to know \# of transitions?}, XXX message types, and numerous branches for corner conditions. 

We focus on USB mass storage for its significance to TEE's secure storage. 
The driver accepts block requests, translates the requests to various SCSI commands, and further maps the commands to USB bulk transfers. 

\paragraph{Recording experience}

We configure the USB driver as follows. 
We do not record interactions for the USB device discovery process and hotplug;
we disable SoF for meaningful recordings. 
USB has autonomous/periodic IRQs, called Start-of-Frame (SoF) interrupt including IRQ, ISO, Control transfer type.
After user issues requests, the device driver schedules the resultant USB requests at SOF ticks and handle the response on these ticks;
Fired per 1ms, SOF acts like a timer tick for CPU scheduler.
This does not fit our model because it is not CPU-driven and does not belong to a request-reply model. 

\paragraph{Selected requests}
We record the following requests: read/write of 1, 8, 32, 128, 256 blocks at a block number specified by the test. \Note{what does this mean}
We also record interactions for initializing the bulk transfer device for soft reset.

\paragraph{Discovered interfaces} 
From initial runs, \sys{} identifies 14 USB controller registers out of XXX KB of register range. 
\sys{} flags one register as a trigger register. 
%From the source code reported by \sys{}, 
From the reported source code, we confirm that a write to this register (channel characteristics) enables a channel and triggers interrupt. 
\sys{} flags one register as a pointer to an in-memory descriptor, which we configure as the base of a DMA descriptor (HCDMA). 
\sys{} discovers DMA descriptors of three lengths: 31, 512, and 4096 bytes.  
It reports the source lines (50 SLoC in the SCSI library; 60 SLoC in the USB driver) that assign these fields. 
From the source code, we confirm that the former two wrap SCSI commands and the last one points to a user data buffer.
%despite that the driver only declares opaque types (unsigned int) for the descriptor's fields. 
We annotate the SCSI command's LBA field (its data address) and the user data buffer as parameterizable. 

% After being prompted by \sys{}, developer looks up the DMA descriptor in corresponding header file \Note{this handwaving?} and discovered it is a 2-quadlet (i.e. 2 4-byte words) structure, where first quadlest specifies size in 16 bits and control flags in the rest 16 bits and the other quadlet contains a DMA address, which points to either the SCSI command or user data buffer.

\paragraph{Segment of interactions}
\sys{} emits XXX segments of interactions. 
In test, we observed little nondeterminism in driver/device interactions. 
For instance, 
to write 8 blocks, the driver always issues exactly 500 register accesses. 
By doing so, the driver initiates 18 \st{packets} transfers (512 bytes each): 
5 for SCSI commands, 5 for querying command status, and 8 for data move. 
%The transfers contain among which 5 contain SCSI commands (i.e. 2 x test unit ready, 2 x allow medium removal, 1 write 10), 5 query the command status (i.e. get CSW), and 8 are data packets.
%\sys{} emits XXX sites of register polling (for XXXX). 
\sys{} reports one register that may read different values across runs. 
From the source lines, we identify the register as HFNUM, a performance counter showing the number of transmitted frames. %  since the device reset. 
Because the register is for statistics purpose, we annotate \sys{} to tolerate the value difference. (XXXX... 


\Note{Initialization ...}


\Note{Reset ...}

%\sys{} discovers XXX non-deterministic number of reads of device status register across XXX runs, hence suggesting a polling loop in place and reporting the source line number to the developer.
%We check out the source code and confirm the cases.


%\Note{below obsolete}
%\paragraph{Challenge: extracting access traces from a noisy background}
%practical and might be useful.
%SOF -- obsolete, we don't deal with, not because it is noise but because it does not fit our driver model.
%
%Ensuring exclusivity during recording is important (as it must the context of replay);
%clean separation must be done at IRQ level.
%The challenge is how to extract the register access exclusively belong to the device \& application activity when the device itself has non-activity-related register accesses.
%
%E.g. The state-of-frames (SOF) of USB devices, which triggers irq at high frequency (every ms)..
%Adding much noise to the collected trace.
%
%The obstacle is these noise cannot be simply shut down.
%Although one might turn if off (in a new impl. e.g. Circle), it is generally hard because modifying device driver behavior (e.g. turn off SoF) requires intimate device knowledge.
%It might also bring bugs to devices.

\paragraph{Post analysis}
\sys{} has automatically discovered a variety of registers, which: 
manage the USB peripheral state (5), including examining device power state, device configuration, and reflecting transmission FIFO size; 
manage the controller itself (3), including interrupts and frame number; 
manage the transmission channels (6), including setting channel speed, data transmission size, and DMA. 

\sys{} has also captured the non-trivial mapping between requested blocks to SCSI's logic block address (LBA). 
The driver rounds up the give blocks (512 byte each) to the LBA boundary (4KB). 
In case the accessed blocks are smaller than one LBA, the driver reads back the entire LBA, updates in memory, and writes back. 
The driver also selects the best SCSI commands: 
there exist five multiple variants of SCSI commands, which have different lengths and can encode different ranges of LBA; 
the driver picks the 2nd shortest ones just long enough to encode the requested LBA addresses. 

\Note{Check above: anything missing?}

\Note{TODO: transactions, transfers, states, etc}

\begin{comment}
1) Core interface. 
Five registers are used to control USB's device states -- two for interrupt control, one for examining power state, one for device configuration, and one to reflect transmission FIFO size.
2) Host interface.
Three registers are used to manage the controller in host mode -- 
two to configure interrupt and one for reflecting frame number. 
3) Host channel.
Remaining six registers are one bank of host channel-specific registers (among 15 other channels) to kick off DMA transmission.
Two are used for interrupt, one to specify data transmission size, two to configure the channel (e.g. full/half speed, channel), and one DMA register.




\begin{myitemize}
	\item 
	Block layer is responsible for translating the sector into logical block  of the SCSI read/write commands. 
	For USB, the LBA is wrapped around at a 4KB boundary (i.e. the smallest DMA size). 
	E.g. write to sector 0-7 will translate to a LBA=0 in SCSCI command, whereas to sector 8-15 will be LBA=1.
	
	\item 
	Block layer treats accesses based on LBA boundary in two following ways:
	\begin{myitemize}
		\item 
		Reads/writes across different LBAs will be broken down into multiple accesses.
		
		\item 
		Writes that are smaller than 4KB will also be broken down into multiple accesses -- block layer first issues SCSI read to the whole 4KB region, then modifies the corresponding data, then issues 4KB writeback.    		
	\end{myitemize}

	\item 
	For each read/write command, there are five variants which have 6, 10, 12, 16, 32 bytes. 
	The more bytes the command has, the more data blocks it can address and larger data size it can transfer. 
	Out of the 5 variant, our testing shows SCSI layer picks the 10-byte one, which contains a 4-byte LBA field (each field is a 4KB) and is enough to cover over 16TB address space.
\end{myitemize}
\end{comment}

\paragraph{Analysis of developer efforts}
Table XXX lists the efforts required by \sys{}: inspecting XXX lines of code (XXX locations in XXX files) to confirm annotations of XXX registers. 

\paragraph{Efforts with alternative approaches}
\textit{If one wants to build a tiny driver from scratch...}
1) They have to reason about the USB standard, a document of 650 pages. 
They identify and implement the FSMs related to the bulk transfer (eight of them) \Note{why so many?}
They must be aware of device classes (low/full/high-speed), because the protocols for different classes may differ, e.g. a high-speed device has additional handshake packets.
2) Developers must understand the SCSI protocol. They must implement the command mapping and selection for selected requests as \sys{} discovers. 
3) They map the FSM transitions and selected SCSI commands to USB transactions. 
They program the actual USB controller accordingly with register access and DMA transfers. 

% --- the longer version --- 
\begin{comment}
\textit{If one wants to build a tiny driver from scratch...}
% https://www.usb.org/sites/default/files/usbmassbulk_10.pdf
%https://doc.lagout.org/science/0_Computer%20Science/9_Others/9_Misc/USB%20Complete%20The%20Developer%27s%20Guide%204th%20Ed.pdf
1) They have to understand the USB standard, i.e. a document of 650 pages plus 96 pages of supplement of On-The-Go (OTG) device specification, which is even longer and more complex than MMC standard.
% page 213-220 of USB specs 
From the myriad of pages, they have to identify the transfer types to support (i.e. bulk in our case), and implement the corresponding FSMs.
This is non-trivial -- as we roughly calculate there are in total 45 state machines; 
for the one bulk transfer alone, there are at least 8 directly related FSMs (i.e. not device-wise FSMs) with over 10 conditional transitions each.
Even at the lowest layer, they must be aware the transfer protocol differences for low/full/high-speed devices, where high-speed device has additional handshake packets.
2) For bulk transfer, they must additionally understand the SCSI protocol \& command encodings that instruct the data move.
As described earlier, even for the same block read/write request SCSI has multiple encodings. 
This places an extra burden to developers.
3) At last, they need to map learned FSM transitions and USB packet encodings (with wrapped SCSI command) to actual hardware. 
To this end they learn the manual of the USB host in order to program the registers and DMA transfers, which constitutes XXX pages of extra specification.
E.g. to calculate bus time, they must combine the host controller-specific timing to a formula provided by the standard...
%As shown above, the mapping is non trivial. 
%The developers must also understand the SCSI protocol and map it to the USB transfers.
%As shown above, the mapping is non trivial. 
% The whole process is error prone and debugging is difficult.
\end{comment}

\textit{If one wants to refactor the Linux driver...}

(1) Reason about USB driver codebase: for USB mass storage, understand USB core (drivers/usb/core) and storage frameworks (drivers/usb/storage), the host driver. 
Their interfaces, callbacks, structs. 

(2) Code tailoring with USB domain knowledge.
To keep the code only needed by USB mass storage (bulk transfers), we first need to understand tens of USB concepts used in the codebase, e.g. IN/OUT endpoints, microframes, XXX. 
An example: the USB controller optionally generates periodic (1000Hz) interrupts (called Start-of-Frame, SoF). 
The driver invests XXX SLoC in handling SoF in order to schedule transfers. 
%It tracks missed SoF packets; it implements a queue to schedule packets on SoF tick.
We find it difficult to decide if SoF is necessary to bulk transfers. 
And even if we are sure, removing the SoF code scattered in XXX files is tedious. 


% --- the longer version --- 
\begin{comment}
Assuming they can do similar things, e.g. using ftrace to aforementioned codebases, they still need a comprehensive understanding of the USB standard and the codebase and have to endure the tedious build-test-debug cycles. 

E.g. the discovery process is unneeded in our scenario because it is left for the OS to do. 
How to cleanly separate the path from the codebase? What functions to remove? What device states are left after initialization done by discovery and how to cater to it at first request? 
E.g. Start-of-Frame is also unneeded for the bulk transfer type and can be removed.
Yet the driver spends XXX SLoC handling its comprehensive cases, e.g. it will track missed SoF packets; it implements a queue structure to schedule packets on SoF tick.
The codebase is deeply entangled with its IRQ handler and cannot be simply removed. 
\end{comment}
(3) Reasoning about and porting kernel dependencies.
Similar to MMC, USB drivers depend on memory allocator, scheduler, and DMA. 
A new dependency is the SCSI library, for which we need to examine the structure of XXX SLoC and recompile for TEE. 
%The driver relies on block layer to translate the block address into LBA (XXX LoC);
%it relies on SCSI library to encode the LBA into the right commands (XXX LoC). 

%Porting these layers are also hard: block layer consists of XXX SLoC, spanning XXX files;
%SCSI layer consists of XXX SLoC and XXX files, which specify XXX types of different commands and is implemented from a specification over 500 pages. 




%\subsection{VCHIQ (multimedia accelerator)}
\subsection{Multimedia accelerator}
On modern SoC, CPU typically offloads video/audio processing to accelerators. 
%Examples include DSPs for signal processing, NPU for machine learning, and VPU for capturing images/videos in JPEG or H.264. 
%They communicate with the CPU through proprietary protocols. 
% These accelerators run their own firmware processing pipelines and 
A unique challenge, compared to other devices, is that these accelerators  communicate with CPU primarily via messages backed by shared memory. % with minimum use of registers). 
The message passing protocols are often proprietary and sophisticated. 

\paragraph{Device overview}
We studied VC4, the multimedia accelerator on the Rpi3 SoC. 
According to the limited information, VC4 implements key multimedia services, including camera input, display, audio output. 
It communicates with the CPU via a complex, proprietary message queue called VCHIQ.
Using VCHIQ as a transport, each media service further defines its message format and protocol, e.g. MMAL (MultiMedia Abstraction Layer) for cameras. 
The details of VCHIQ, as well as internals of VC4, remain largely undocumented. 

The above protocols are implemented by the Linux VCHIQ driver. 
The codebase of VCHIQ driver spans 10K SLoC in 60 files. 
The driver consists of three layers: message parsing, event handling, and queue management. 
As described in Section XXX, much of the complexity is for performance optimization and concurrency. 
For instance, the driver defines 14 message types, each with different payloads of XXX to YYY fields (need better examples); 
% sema_init(...)
21 fine-grained semaphores and condition variables; 
it incorporates 3 threads in order to support concurrent user threads to request different service types from VC4. 

We focus on two media services essential to secure IO: image capture from a CSI camera (a pervasive image sensor interface); display that supports modern formats such as HDMI, DVI, and DSI.  
% framebuffer-based simple display). 


\paragraph{Workflow}

\paragraph{Selected requests}

Besides device initialization and reset, we record the following requests. 

For image capture: 
We choose one single request: to acquire a single image frame in JPEG with a set of configurable resolutions (e.g. 1440p, 1080p, 720p). 
We exercise the driver with a simple user program in 10 SLoC of Python code calling the Linux video ioctl API. 

For display: 
We choose the following requests. 
\begin{myitemize}
\item Load a bitmap (fixed size) to the display surface
\item Create paths out of fonts (in XXX format)
\item Load a vector path (fixed size) to the display surface
\item Display glyphs at give surface coordinates
\end{myitemize}
Our test program is a simple graphics program from command line. 
It renders to the whole screen and does not invoke X window. 
Hence, we only support full screen rendering; no windowing mode is supported. 


%and one mailbox register to communicate between firmware. 
% With one additional run, \sys{} discovers that the VCHIQ\_INIT message 

\paragraph{Discovered interfaces}
\sys{} identifies the small bank of three registers.  
\sys{} flags two of them as trigger registers. 
We inspect the source code and confirm that they are a pair of ``doorbells'' for raising inter-processor interrupts between CPU and the accelerator (for message send and receive, respectively). 
The third register is a ``mailbox'', which, during device initialization, is used to set the base address of a shared memory region. 
The memory region spans 66 pages and 264 KBs in total.

\sys{} scans the shared memory region and has found only one physical pointer at XXXth segment. 
%of which 40 bytes are dynamic values, 4 bytes belong to a physical pointer, and the rest bytes are all static encodings. 
%\sys{} leaves the treatment of dynamic bytes at alignment time later;
At the pointed memory region, \sys{} further identifies an in-memory descriptor. % which contains an array of physical pointers. 
Prompted by \sys{}, we locate the relevant kernel source (about 60 SLoC in file XXXX which has XXX SLoC in total) that populates populates a descriptor. 
From the source code, we confirm that these fields are part of a DMA descriptor, whose 1st-3rd words describe the data size \& offset and 4th word forward is a scatter-gather list that describe the data buffers.
Additionally, we have found the 12 Least Significant Bits (LSBs) of each pointer encode the number of following contiguous pages, as an optimization of the firmware;
for simplicity we omit the optimization and populate individual pages without merging the contiguous ones.

At the end, \sys{} discovered (and we confirmed) the semantics of 2 fields (i.e. one DMA descriptor and one VCHIQ\_INIT message, consisting of only XXX words), which is only XXX\% a tiny fraction of whole memory dumps and remains oblivious to the semantics (and formats) of the remaining. 
It parameterizes fields XXX and XXX. 

\paragraph{Segments of interactions}
Table XXX summarizes the interaction segments emitted by \sys{}: 
\begin{myitemize}
	\item  
	For device initialization.
	Two register accesses (to BELL2 and to mailbox register\Note{haven't introduced yet}) and two memory dumps (one for VCHIQ one for firmware message); 
	\item 
	For each request: 100 memory dumps with XX-YY register accesses in between. 
	Each memory dump is a snapshot of the shared memory region of 264 KBs that backs the message queue, whose base address is parameterized and notified during initialization;
	the possible divergences are annotated in the corresponding offset in the memory dump, such that during replay they can be either ignored or parameterized as mentioned before.
\end{myitemize}


%VCHIQ driver also shows a highly-deterministic and request-reply pattern across the recorded XXX segments.
Across repeated runs, \sys{} discovers no register polling. 
\sys{} discovers 40 bytes of discrepancies in memory dumps. 
% which belong to different MMAL or VCHIQ messages.
% For each diverging byte, \sys{} looks backward for the ascii code of "MMAL" and "VCHIQ", which are the header of MMAL and VCHIQ messages, respectively.
% After locating the message header, \sys{} maps the diverging bytes to a field in the message and reports as follows:
\sys{} maps back these bytes to the message definitions in the driver source.
We inspect the definitions: 
\begin{myenumerate}
	\item The 4th word of MMAL request header, pointing to the message's kernel context.
	\item The 1st word of COMPONENT\_CREATE request, pointing to the message's kernel context.
%	\item 16th word of VCHIQ slot zero, indicating tx pos of the next message. 
	\item 10-11th double word of PORT\_PARAMETER\_GET reply, rflecting VC startup timestamp.
	\item 22th word of BUFFER\_TO\_HOST, pointing to buffer kernel address.
	\item 18-19th double word of BUFFER\_FROM\_HOST, pts -- presentation timestamp.
	\item 4th word of BULK\_RX message, (to received) data size -- \textbf{to parameterize}
	\item 5th word of BULK\_RX message, (to received) data DMA descriptor address -- \textbf{to parameterize}
\end{myenumerate}

Based on the semantics, we instruct \sys{} to omit 1-5th divergence but parameterize 6-7th since they describe the data buffer in the DMA descriptor.
Subsequent XXX runs all fall into this interaction envelope. 
It is worth noting that we only examined a small fraction of message fields (XXX out of XXX). 


\paragraph{Post analysis}
%The example of "setup everything in memory" scenario is the CSI camera on RPI3 via VCHIQ interface.
The driver and VC4 communicates via a circular message queue.
Catering to concurrent media services, the message queue has the following sophisticated structure. 
% backed by the shared memory region discovered by \sys{}. 

The memory region is divided into many 4KB slots, each is assigned either CPU or VC4 for holding messages they write. 
Messages have varying lengths. 
Each slot can hold multiple messages. 
CPU and VC4 independently enqueue messages to their respective slots. 
Slot 0 is special, as it contains metadata that describes the whole message queue, e.g. number of slots, slot allocations, read/write locations in the message queue. 
%The data structure has two major responsibilities: 1) it configures the memory region, e.g. setting up the slot size and total number of slots; 
%2) it maintains the transmission states, which contain pointers to next message to-be-sent or to-be-received in the memory region.
% Diff ports: VCHIQ relies on port \# to communicate, similar to sockets.
CPU writes to the doorbell registers to notify VC4: 
one register to signal new messages for VC4 to read; 
one register to signal CPU is ready to receive more messages from VC4. 

%At last, the driver triggers the event by writing a one to the doorbell register to notify VideoCore about the incoming message.
%Receiving a message is a mirror process, where another doorbell is rung on the VC side and received by the CPU.

A single user request (e.g. capture a frame, render graphics) entails over 100 VCHIQ messages exchanged between the driver and the device. 
Ranging from 28 bytes to 306 bytes, these messages belong to tens of types. 
They are either for configuring the device, e.g. opening a service ``port'' of VC4, setting frame resolution; or for moving data. 
The physical pointer discovered by \sys{} is within a message of bulk transmission/reception. 

\begin{comment} % --- useful ---
To control the device (CSI camera, HDMI display), the driver sends VCHIQ messages to VC firmware at lowest level, as shown in Figure~\ref{fig:dev}. 
For a single event (e.g. capture a frame, render a graphics), there are two types of VCHIQ message: 1) data, 2) bulk transmit(TX)/receive(RX); 
the former contains MMAL commands and the latter launches DMA transmission to or from the device. %of the data buffer, which transmits or receives the data from the device (e.g. a frame).

The payload of VCHIQ data messages are 8 MMAL commands (each has a request and a reply format) being used: GET\_VERSION queries VC version -- this checks if the firmware supports the device, PORT\_ACTION to open communication port on VC, PORT\_INFO\_SET/GET to configure the port, PORT\_PARAMETER\_SET to configure the device parameter connected to the port (e.g. frame resolution), COMPONENT\_CREATE/ENABLE/DISABLE to turn on/off the device. 
The commands size from 28 bytes (i.e. request of COMPONENT\_ENABLE/DISABLE) to 306 bytes (i.e. request of PORT\_INFO\_SET).
The payload of VCHIQ bulk tx/rx message is the scatter-gather list structure as mentioned earlier. 
\end{comment}

%\textit{Initialization.}
%%VCHIQ initialization is simple. 
%To initialize VCHIQ, the driver first allocates a region of DMA memory as the message circular buffer, and initializes the first 4KB page, which specify the initial states (e.g. next message position, message counter).
%It then notifies the firmware by passing a VCHIQ\_INIT message containing the address of the VCHIQ message buffer through the mailbox interface mentioned before.

%Power \& clock is taken care of by firmware prior to kernel bootup.





\paragraph{What-if analysis}
\textit{If one wants to build a tiny driver from scratch.}
The developers face complex, poorly documented VC4 interfaces and protocols.
Even for the simple requests we target, developers have to populate the circular message queue, in particular the metadata at slot 0. 
The knowledge seems only available from the hardware vendor. 
They also have to craft the sequence of hundreds of messages that execute image capture and display. 
Debugging is tedious: any incorrect fields could render the media services unusable and VC4 provides no mechanism to report what fields may cause the problem. 

\begin{comment}
Beyond the driver code released under GPL, the key challenge is public documentation of VC is lacking.
As a proprietary software, it packs complex software stack (e.g. OpenVG) inside;
it relies solely message passing to receive commands from CPU, yet both the request and reply message formats that are accessible to public are the fruit of reverse-engineering\Note{cite}.
Secondly, the developer efforts are high. 
As we calculate roughly, there are in total XXX different data structures that are crucial to control (e.g. slot zero for initialization), which consist of XXX fields/bytes that require non-trivial developer understanding.
Thirdly, it is hard to implement it correctly.
Due to the shared-mem message passing nature, data barriers are not uncommon.
In total XXX callsites are placed with read/write barriers; 
if one shall miss, it may lead to incorrect execution, e.g. the updated transmission pointer is not seen properly by the VC, which makes it read the wrong message.
Moreover, debugging the raw memory region is tedious. 
This can be reflect by the numerous of debugging trace planted in the source code, where XXX functions are instrumented and XXX fields are dumped. 
\end{comment}

\textit{If one wants to refactor the Linux driver.}
VCHIQ driver poses three unique challenges to efforts refactoring kernel drivers into TEE: 
1) its kernel driver model misfits TEE.
To effectively communicate with VC4, the kernel driver implements a handler daemon thread to poll any incoming messages in the memory region, guarded by XXX semaphores to control concurrency.
This mismatches TEE design, which has no notion of a daemon thread and assumes limited concurrency.
2) TEE lacks comprehensive (advanced?) DMA services.\Note{clarify we only need much simpler DMA allocator?}
The driver relies heavily on kernel DMA allocator, scatter-gather list and its family functions to efficiently manipulate data pages.
Refactoring them will likely end up pulling the whole DMA facility inside TEE, which accounts for XXX SLoC.
3) configuring the device properly is not easy. \Note{this may go to the above paragraph}
Besides simply understanding the message data structure, a developer must also thoroughly understand its payload, which is used to configure the device. 
E.g. which encoding sets the resolution to 1440P and which switches the format from BMP to JPEG?
 



\paragraph{Quirks}

\begin{myitemize}
	
%	The recorded ones are usually local 2 remote 88 -- sometimes it will change to remote 87 ?? -- this will make replay fail each time.
%	\Note{this is due to firmware is compromised}.
	
	\item DMA desc.: called pagelist. 
	Simple structure -- size, offset, and then starting the list of DMA address containing (size/page\_size) pages. 
	The 12 LSBs of the address contain the \# of contiguous pages.
	
	\item 
	At development time, \sys{} discovers abnormally excessive divergences in the recorded memory dumps.
	Even in the same, the simplest VCHIQ message (e.g. GET\_VERSION), there are tens of bytes difference, which is over 80\% of the message size.
	We manually discovered that it is because the driver allocates message data from stack without initializing it with 0. 
	As a result, the unused fields are full of garbage values, which diverge each time.
	
	
\end{myitemize}


%So far the above discussions only considered interaction with device through register.
%It assumes in-memory descriptor as bus addresses are passed to registers.
%This is not the case for VCHIQ driver used for picam, which only has two `signaling' registers, which does not contain the bus address of the message but only serves as an IPI to notify GPU the message is coming.
%
%The real data is stored inside the messages themselves (for camera its mmal message), following a (header, data) format, where the header specifies message type and size.



%\paragraph{Solution: memory snapshot}
%Despite it is message-passing and in-memory.
%The overall principle still stands -- record/snapshot the hardware/software interaction.
%
%Therefore the tool records the interaction by dumping the whole slot queue memory contents prior to each trigger, driven by the event.
%\Note{On the RX path}, it also snapshots the memory content, which is used to detect divergence..
%
%Note that it still symbolizes the data address in the memory snapshot and instantiates them during replay time.

\subsection{Mediating accesses to shared devices}
\label{sec:case:mediate}

While TEE owns MMC, USB, and VCHIQ exclusively, and fully confine their registers accesses, they rely on power and clock domains to operate, which is inevitably shared by the entire SoC.
Once initialized, \sys{} prevents any unauthorized writes to dependent and shared domains, in order to protect TEE-owned devices from availability attacks (e.g. shutting down power and clock).

On Rpi3 (i.e. the test platform), the control of power and clock domains is delegated to GPU firmware by CPU, which only sends a command.
In total, there are 21 commands for the task (e.g. GET/SET\_CLOCKS, GET/SET\_DOMAIN\_STATE, GET/SET\_CLOCK\_RATE, GET/SET\_VOLTAGE). 
% useful: rpi3 mailbox 
% https://www.programmersought.com/article/7170472059/
% https://github.com/raspberrypi/firmware/wiki/Accessing-mailboxes
They are sent to GPU through the mailbox interface, which is controlled by 10 registers (e.g. READ, WRITE, PEEK, SENDER). 
\sys{} mediates each write to the WRITE register, which contains the DMA address pointing to the command.
It does so by configuring TZASC and to mandate secure-only access to the register;
this is similar to SeCloak~\cite{secloak}.
Each non-secure access will be trapped by TZASC and captured by \sys{};
\sys{} examines the command payload and ensures that they are not one of the 21 commands nor can they change any domain states.


==> impl-recycle.tex <==
% !TeX root = main.tex

%\section{Implementations and Experiences}
\section{Implementation \& experiences}
\label{sec:case}


%\Note{TODO: show a table of discovered values \& registers, similar to table 1 in Discoverer paper}

%\Note{Section title -- } Implementation \& experiences? 

\input{fig-exp-setup}

\input{fig-devices}

%\input{fig-proto}

\input{tab-trace}

\input{tab-case-study}

We applied \sys{} to a variety of devices, namely MMC, USB, and VCHIQ.
We select them because they have important use cases of secure IO and their drivers are complex and known difficult for TEE.
%\begin{myitemize}
%\item 
%the device has important use cases of secure IO 
%\item 
%the device driver is complex and known difficult for TEE 
%\end{myitemize}
Figure~\ref{fig:dev} shows their software stack.

Our test platform is Rpi3;
Table~\ref{tab:plat} shows the detail.
We choose it because of its popularity and good support for open-source TEE software.
As we will show, despite an active community and high attention for Rpi3, (far more than most other SoC hardware), building TEE drivers is nevertheless difficult. 
%\Note{It is also a device} with proper amount of open-source vs proprietary components -- while difficulty in implementing a TEE driver is in hindsight (i.e. largely through reverse engineering), we can still reason about it from its open-source implementation.
Table~\ref{tab:trace} lists selected requests and test harnesses which are user programs.

%The recording environment is Raspbian Linux. The kernel version is XXX. 
%All recording harnesses are user programs. 
%The TEE for replay is OPTEE-4.2 on the same machine. 

For each driver, we first gives an overview, then describe recording findings. 
At last we present a post analysis of recordings which correlates them with native driver to shed light on 1) what are discovered and recorded (i.e. do recordings what they were asked to?), 2) how much effort would be needed to produce the same driver behaviors.
%Although not required by generating the TEE driver, we analyze the recordings and correlate them with the full driver code to shed light on 1) what are discovered and recorded and 2) how much effort would be needed to produce the same driver behaviors. 
%\Note{turn off for submission}
%\input{thoughts}
We quantify these efforts as described in Section~\ref{sec:design:summarize}:
\begin{myitemize}
	\item 
	SLoC checked, when summarizing a \code{read-until} action.
	
	\item 
	Fields checked, when summarizing \code{read-range}, \code{write-syn} replay actions.	
\end{myitemize}
Note \code{read/write} and \code{read/write-para} are automatically summarized;
developer efforts are optional to confirm the latter.


\subsection{MMC}

MMC is a common interface to off-chip flash, e.g. SD cards and eMMC. 
% To access flash storage, 
%To implement secure storage, the TEE should run its own MMC driver bypassing the untrusted OS. 
Lacking MMC drivers, the current TEE saves data on flash by invoking the untrusted OS and encrypts the data \Note{cite} 
%This method suffers from a few drawbacks: as data flows through the OS, it is vulnerable to availability attacks and side channel attacks. 
This method is vulnerable to availability attacks and side channel attacks mounted by the OS. 
It also requires special flash partition (e.g. RPMB) that is capable of cryptographic operations. % is limited in size and speed. \Note{cite}

\subsubsection{Device overview}
%\paragraph{Long-wanted secure storage.}
%\paragraph{Device overview}
Leftmost part of Figure~\ref{fig:dev} shows an MMC stack: 
%apps via a filesystem \& block layer submit block read/write to the device driver, which in turn operates on an MMC controller. 
apps invoke a filesystem, which submits block read/write to the Linux MMC framework. 
The framework supports more than 20 MMC controller models, which 
have different interfaces and are often poorly documented. 
The framework abstracts the common driver logic as a ``core'' with 15K SLoC in 40 files; 
a driver for a concrete MMC controller plugs in the MMC core via a wide interface, including 44 callbacks and four structs (XXX fields).
The driver itself often has a few K SLoC. 
All combined, the MMC framework implements a FSM with thirteen states and hundreds of transitions among them.
The FSM supports rich features, including streaming access of blocks and medium hotplug. 


%The driver operates on an MMC controller, which communicates with the flash peripheral. 
%A MMC host's finite state machine (FSM) is standardized. \Note{cite}
%As stated in Section~\ref{sec:design:prior}, 
%It tries to implement features stated in Section~\ref{sec:design:prior}.
%E.g. streaming blocks in addition to transferring individuals ones for performance optimization; 
%hotplug of card (even in the middle of transfer) for dynamism;
%bus/medium error recovery in place considering the corner cases.


%As stated in Section~\ref{sec:design:prior}, the complexity originates in 
%(1) performance optimization: not only transferring individual blocks but streaming blocks; dynamic tuning of bus clock; 
%(2) dynamism: multiple cards; connected/disconnected at any time (even in the middle of transfer); open-ended transfer without pre-defined sizes;  
%(3) corner cases: assuming MMC bus/medium is volatile; attempt to recover from bus/medium error in place. 


%A controller's interfaces (registers and DMA descriptors) are vendor-specific.
%Their interfaces are often either undisclosed (e.g. Rpi3 ...) or poorly documented. 
%%even if they are public, the documentation of host hardware is often long (e.g. XXX pages). 
%Undocumented silicon bugs are not uncommon \Note{cite}. 

%Linux implements the MMC FSM and drivers for a myriad of MMC hosts. 

%around 4K SLoC each \Note{check the numbers} 

%implements device-specific code for a myriad of MMC controllers (around 4K SLoC each \Note{check the numbers}). 
%The MMC core and a controller driver communicate via a wide interface -- 44 callbacks and 4 structs (XXX fields) 
%which spans 60K SLoC in 107 files. 
%mmc_host_ops: 19, mmc_pwrseq: 4, mmc_bus_ops: 12, mmc_cqe_ops: 9, 
%\Note{present any existing vulnerabilities in driver?}

% Such a method suffers from capacity limitation, 
%\textbf{Functions}:
%\paragraph{Selected requests}
\subsubsection{Recording experience}
% lwg: paper template have alignment issue if no text between \subsection{} and \paragraph{}

%\paragraph{Selected requests}
We choose to implement ten block read/write requests as listed in Table~\ref{tab:trace}.
% read \& write of a single data block; read \& write of multiple data blocks, where the block count can only be 8, 64, 128, or 256.
%read/write of five fixed block counts (1, 8, 32, 128, and 256). 
Each request accepts two arguments: the starting block ID and the physical address of data buffer. 
We avoid making the block counts parameterizable, 
because as we will show below, requests will show very different device state transitions if their block counters differ. 
%the device state transitions in a request will vary significantly as the block count changes. %are read/written.
%ensure each recording run sees deterministic device state transitions
%(1) By setting a fixed block count for each request, we ensure each handler sees deterministic device state transitions. 
%As we will show below, the transitions of device states can vary significantly  when different numbers of blocks are read/written. 
%(2) The above block counts (and their combinations) are sufficient to trustlets we target. 
%  the driver will take different execution paths 
%  and \textit{size}.
%Their test harnesses are listed in Table~\ref{tab:trace}. %where the block count can only be 1, 8, 64, 128, or 256.
%Separate single block read/write from multi-block rw is to fit into kernel behavior when smallest DMA-able unit is a page (4KB).
%\sys{} records initialization \& reset at driver probing stage.

%\Note{merge}
%For instance, the transactions for MMC driver include read/write of a block, tune the MMC bus, and rescan the medium for changes.
%
%Storage device: (rw, block \#, size), use `dd' or `iozone'

\paragraph{Discovered interfaces}
%\sys{} traces the full MMC driver for its initialization, reset, and the requests selected by us. 
%\sys{} records MMC initialization at driver probing stage. 
%During the stage, kernel reads in MMC's device tree blob (DTB) entries;
%they specify the clean-state (i.e. initial) MMC states (e.g. power, clock) and therefore instruct MMC initialization sequence. 
%\sys{} traces request execution by running the user utility `dd' with the sync \& direct flag. 
\sys{} discovers 15 different registers plus one in-memory descriptor in use as summarized in Table~\ref{tab:tab_case_study}.
It is noteworthy that as \sys{} snapshots DMA descriptors, it captures different number of them for different block counts but only one is written to DMA register DMA\_ADDR; \Note{reword this above sentence}
\sys{} finds out that each descriptor contains two physical pointers, one pointing to another descriptor and one pointing to a data buffer.
Later we confirm such a chained structure indeed exists for descriptors.

%\sys{} flags a register (DMA\_ADDR) as a physical pointer to an in-memory DMA descriptor spanning 8 words; 
%\Note{refer to table}
%it further flags the descriptor's word 2nd, 3rd, and 6th as another three  physical pointers. 
%By examining XXXX source lines that populate these pointers, we confirm \sys{}'s findings: word 2 and 3 point to a scatter-gather buffer (i.e. data buffer) for DMA transfer and word 6 chains multiple DMA descriptors as a scatter-gather list. 
%Based on discovered interface, \sys{} records the access of 15 registers, takes snapshots of the DMA descriptor list, and parameterizes the addresses of each scatter-gather buffer addresses.  \Note{how to deal with the last one}
%\Note{take DMA snapshot does not need to understand XXX..}

% developer examines the MMC descriptor.It is a 8-word data structure, where the first five words specify data length and address (also a DMA address) and the 6th word specify the next chained descriptor, if any.

\paragraph{Recorded interactions}
\sys{} emits 30-150 interactions, which constitute the TEE driver ready for deployment;
Table~\ref{tab:trace} breaks down specific replay actions.
It is worth noting that these raw traces vary greatly in length. 
The request of read a single block, for example, may result in 130 -- 150 register accesses. 
\sys{} attributes the non determinism to two loops of register polling (i.e. SDCMD and SDEDM), which we confirm with ease. 

\subsubsection{Post analysis}
%\paragraph{Post analysis}
%Although not required by generating the TEE driver, we analyze the recordings and correlate them with the full driver code to shed light on 1) what are discovered and recorded and 2) how much effort would be needed to produce the same driver behaviors. 
%\Note{also contribute to verifying correctness}
The 15 registers discovered by \sys{} fall into three groups: for configuring the controllers (e.g. SDCDIV to set clock; SDVDD to set voltage; SDHCFG to configure interrupt, bus width), for sending/receiving commands/responses to the MMC peripherals (SDCMD, SDARG), and for controlling the DMA transactions (DMA\_CS, DMA\_ADDR). 

\sys{} captures non-trivial interactions on these register accesses.
E.g. 
%four different SD commands (CMD13-read single, CMD14-write single, CMD18-read multiple, CMD25-write multiple) are sent to SDCMD register, and arguments (block ID) are sent to SDARG register, which must be a multiple of 8;
five different SD commands (CMD17, 18, 23, 24, 25) are sent to SDCMD register, and arguments (block ID) are sent to SDARG register, which must be a multiple of 8;
CMD23 (set block count) is used on the read path but not write path;
during initialization, SDCDIV is used in conjunction with a SET\_SDHOST\_CLOCK message to firmware whose payload is a 3-word magic value, lacking published documentation\Note{cite}.

%The segment for device initialization has captured rich interactions. 
%Notably, the driver configures the MMC clock by communicating with the firmware. 
%It does so by sending a SET\_SDHOST\_CLOCK to firmware containing a 3-word payload; 
%\sys{} records the payload as magic values, which lack public documentation\Note{cite}.
%The driver resets the rest of MMC state machine by writing other magic values (all 0s or 1s) to 10 different  registers. 
%The driver further probes various device registers in order to calibrate command timeout. 
% 	The process contain 18 accesses to 10 different host registers, where there are 17 writes and 1 read to SDEDM register.
%It first resets most registers by writing 0's or 1's to clear the status, then based on the clock \& clean-slate state read from DTB, the driver calibrates command timeout and sets up corresponding registers.
%\sys{} also records delays of waiting for device state transitions (e.g. power state, FSM).  
	

% https://github.com/raspberrypi/firmware/wiki/Mailbox-property-interface
% missing tag documentation: https://github.com/raspberrypi/firmware/issues/719
%Configuring the clock. 
%It is done by firmware. 
%The driver prepares a message containing a 3-word tuple as payload (0x0, 0xffffffff, 0xffffffff) and a header specifying SET\_SDHOST\_CLOCK tag.
%It then sends the message to firmware through mailbox interface to enable the clock.
%It is noteworthy that these message formats lack comprehensive documentation\Note{https://github.com/raspberrypi/firmware/issues/719}, which is overcome by \sys{}'s recording approach.
	
We have also observed two distinct driver paths w.r.t different block counts. 
(1) to read/write fewer than 8 blocks, the full driver shifts individual words from/to SDDATA. 
(2) to read/write greater than or equal to 8 blocks), the driver uses DMA transactions to move the data. 
Notably, even when using the DMA transaction, the driver moves the last 3 words via SDDATA on read path. 
%By examining the driver source, we find 
% discovers a comment stating 
This seems to work around an undocumented bug in the SoC's DMA engine, which cannot move the last few words of a transfer. 
%\Note{experiences: sector alignment... must be multiple of 8}

% only the the 9 host registers are used (PIO paths); 
% Initial runs of \sys{} locates in total 11 registers in use during tests, among which 9 (i.e. SDDATA, SDHSTS, SDHCFG, SDRSP0, SDCMD, SDEDM, SDARG, SDHBCT, SDHBLC) belong to the host controller and the other 2 (DMA\_CS, DMA\_ADDR) are of the global DMA engine for initiating DMA transactions. \Note{registers used in initialization are not counted here, e.g. to set clock, SDVDD to set VDD}

% The first (PIO) path (read/write size <4KB) contains 160 $\sim$ 1300 register accesses while the DMA path (read/write size > 4KB) only contains $\sim$ 64 register accesses.  

% 2) otherwise, two DMA registers are additionally used, with 3 words of tailing SDDATA register access.  Interestingly, we check out the source code and find the tailing SDDATA register accesses overlaps with the first PIO path;
% it is due to a silicon bug of RPi3 -- its DMA engine cannot access last few words of the DMA page, which can only accessed through PIO.

%\paragraph{What-if analysis}
\paragraph{Analysis of developer efforts}
Table~\ref{tab:tab_replay_actions} lists the efforts required by \sys{}: inspecting 40 lines of code (two locations in one file) to checking 2 interface fields in a DMA descriptor. 

%\textit{The efforts for building a small driver from scratch}
\textit{If developers build a small driver from scratch...}
They must (1) reason about the MMC standard (231 pages) to identify device state transitions for selected requests. 
Even for a write request, the developers has to decide one from possible paths: open-ended write, writes with pre-defined block count, and reliable writes with predefined block count.
(2) select correct MMC commands and encodings.
E.g. a bit in CMD23 enables reliable write while odd enough, not all MMC controllers support the command. 
%all MMC commands, e.g. CMD23 used in our recordings is unsupported in some controller. 
(3) map the selected commands to the concrete MMC controller registers and produce up to 130 reads/writes of 15 distinct registers. 
They will encounter the silicon bugs, e.g. the DMA quirk as stated above, which requires tedious guess work and trial-and-error debugging. 
%which seems difficult, if not impossible to fix without internal documentation. 

\begin{comment} ---- useful --- 
The developer must understand:
1) A trimmed state transition path of the selected function (e.g. read/write multiple blocks).
To this end, the developer must navigate through the MMC standards, which is a 231-page documentation\Note{cite}. 
It is a hard process -- the developer not only flips pages to put individual commands into a full path, but also he must choose wisely such a path.
E.g. for the single event of writing multiple blocks, the specification provides at least three paths: 
1. open-ended write which must end with a CMD 12 (stop transmission); 
2. writes with pre-defined block count (i.e. the recorded one) which starts with a CMD 23 (set block count).
3. reliable writes with predefined block count and a reliable write parameter, which even has two versions. 
2) The semantics of commands on the chosen path.
In our case, there are at least the six ones used in our workload (i.e. CMD13 send status, 17 read single, 18 read multiple, 23 set block count, 24 write single, 25 write multiple).
This is tedious and non-trivial as commands have multiple fields for encoding different flags \& control (e.g. whether the command is new, whether it's expecting valid CRC). 
More importantly, developer must clearly understand when and what flags to use, which is dependent on the hardware capability (e.g. some controller may not support CMD 23).
3) The developer must map the above two parts of knowledge to the actaul MMC hardware.
To do so, they refer to the hardware manual (if any), identify register/in-memory descriptors needed for the device/driver interactions. 
Even for a request as simple as reading one block, the interactions are non trivial (e.g. 1300 reads/writes of 15 distinct registers)
They will encounter the silicon bugs, e.g. the DMA quirk as stated above, which seems very difficult, if not impossible to fix without internal documentation. 

%To always issue CMD 23 before CMD 18 and 25 but not before CMD 17 and 24. 
% http://yourcmc.ru/wiki/images/5/55/EMMC_JESD84-A441.pdf

%The developers: choose the request semantics to implement and trim down the FSM accordingly: 
%examine the MMC standard, identify needed states and implement the related transitions. \Note{TBD: more specific}
%They map the required state transitions to the actual MMC host hardware. 
%To do so, they refer to the hardware manual (if any), identify register/in-memory descriptors needed for the device/driver interactions. 
%Even for a request as simple as reading one block, the interactions are non trivial  (e.g. XXX reads/writes of XXX distinct registers; access of XXX in memory descriptors)
%They will encounter the silicon bugs, e.g. the DMA quirk as stated above, which seems very difficult, if not impossible to fix without internal documentation. 
%
%Hardware (SoC) specific; hardware quirks, details.
%Tuning. probing, configuration, clock, power, bus width, bus speed. e.g. periodic tuning ... register formats, hardware quirks, different voltages supported by cards (dual voltages), etc.
\end{comment}
%\Note{compress}
%Compile -- thousands of errors. broken dependency. What is worth fixing? What is not needed? 
\textit{If developers trim the Linux MMC driver...}
%They may selectively port only the code path belong to the same requests.
They must have comprehensive MMC domain knowledge to decouple select code path from the driver code.
E.g. cards dynamic discovery is off the path and thus not needed.  
Its code is hidden after IRQ handler parses CSD register to configure IOS \& card class (HS200, HS400); 
ironically, they must understand these MMC-related concepts to know they're not useful to eventually remove them. 
They must resolve the kernel dependencies around the path.
E.g. on the path, the controller invokes four functions of DMA subsystem, six of MMC framework, four of SG list;
they must ensure the ABI compatibility if they were to emulate the kernel services.

%(1) Reason about the MMC driver codebase -- MMC core framework \& controller implementation are as described earlier. 
%Identify the frameworks (platform\_drv, clock, power, block) the MMC drivers register to; 
%identify the interface (callback functions, struct to fill). 
%Identify source files that need recompilation. 
%
%(2) Code tailoring with MMC domain knowledge. 
%\Note{move below para to motivation}
%Developers constantly face a dilemma: 
%removing unused code requires deep MMC knowledge and high efforts (including debugging); requires trial and error. 
%moving code as-is bloats the TEE and requires to port more dependencies (a vicious cycle, dependency snowball)
%No guarantee tailoring attempts will succeed. Trial and error. Earlier decisions may turn out to be wrong (e.g. a removed feature breaks the needed functions in a subtle way). 
%Lots functions are not required by TEE, e.g. dynamic discovery of MMC cards (XXX LoC).  
%To simplify the functionality, developers need to understand related MMC concepts -- IOS, bus width, voltage, data rate (device class: HS200, HS400), powerclass; CSD register parsing; capabilities. 
%Decide which features are needed by the selected requests (simple block read/write). 
%Some concepts only apply to specific flash types (eMMC versions). 
%Which of them apply to the device of interest? 
%If developers forgo the effort and instead keep all the discovery code for ease, they have to port the kernel dependency -- kernel device tree (for reading static device capabilities) and power frameworks (for voltage, regulators, etc)

% Useful
%Another example, to simplify/remove periodic bus retuning (or slot rescan), developers need to understand its role in MMC protocol (the performance significance of periodic tuning) and carefully peel off all the related code (XXX SLoC in XXX functions). 
%This process is error prone, though: 
%developers must not eliminate \textit{initial} bus tuning, as doing so would leave MMC bus parameters unset and barely usable performance. 
%If they decide to keep the retuning feature just for porting ease, they will have to port/emulate all the mechanisms underneath retuning, e.g. kernel thread. 
% To minimize the TCB, they need to reason about the codebase. 
% e.g. if concurrent request submission is not needed, developers may remove such a feature; 
% otherwise, they will have to implement work deferral. 
% is e.g. replacing tens of runtime power management (???) callbacks with dummy functions. 
% This further requires to examine the code and remove \Note{XXX} features such as host device abstraction, runtime power management, slot rescan and retune daemon threads, request queue, debugfs, etc.; 
% resolve compilation issues. 


%(3) Reasoning about kernel dependencies. 
%Even after aggressive trim down, the resultant MMC driver code need essential kernel dependencies: scheduler, workqueue, allocator, deferred work. Have to port or emulate. 
%An example is DMA API. It is a generic kernel framework. Complex with less documentation. 
%Developers need to understand the API semantics (which is x86 oriented for historic reason; far from the developer goal of MMC). The APIs further dynamically dispatch to CPU/architecture-specific implementations which the developers have to identify and port. Examples: software IO TLB. Pure software abstraction. 
%
%\textbf{Lines of code}
%
%These services will have to be ported or emulated (with the same interfaces, there are XXX function callbacks) inside the TEE. 
%Deal with compilation and debugging issues. 

%This process of code reasoning and refactoring is tedious and error-prone. 
%For example, if developers deem periodic bus retuning (or slot rescan) as  unneeded, they shall identify and carefully peel off all the related code. 
%However, improper removal of the initial tuning breaks MMC functions and crash the device. 
%If they decide to keep the retuning feature just for porting ease, they will have to port/emulate all the mechanisms underneath retuning, e.g. the kernel thread, which further requires to port more c ode. 


%\Note{the following still needed?}
%The reason for such a stark difference in number of register accesses is discovered at sequence alignment time: 
%on the first path, \sys{} discovers value divergence of access to SDDATA registers;
%\sys{} traces back these values are from tests and are transmitted to device word-by-word through the SDDATA register\Note{do we have this level of automation??}.
%On the second path, \sys{} discovers physical addresses being written to DMA\_ADDR register, hence suggesting the developer de-reference a DMA descriptor;
%the developer then locates and annotates the DMA descriptor, which instructs the device to transmit a large chunk of data in one shot, accessing $\sim$ 40 registers to set up set up DMA address, kick off, and complete the data transfer.
%Additionally, the only non-deterministic interactions discovered by \sys{} is the number of reads to SDCMD register on the PIO read path, differing by 1 $\sim$ 9 times;
%\sys{} hence suggests a polling exists and prompts the developer to fix/annotate it.

%It does not find divergence in terms of values \& types registers being written to and read from.
%It however discovers across two recordings, the number of read from SDARG (\Note{confirm}) are different, which is due to polling. 
%The tool then prompts the developer to summarize the polling behavior, which will be reflected at replay time.

%\Note{useful}
%\textbf{Finding the software/hardware interaction:}
%Upon each test/function invocation:
%\begin{myenumerate}
%	\item 
%	The tool first instruments call stacks of the read/write function using existing kernel function tracing facility.
%	As its discovery, there are two different paths involved in the function:
%	
%	\item 
%	After locating the involving devices, the tool instruments all 1) ioremap, 2) register access, 3) DMA memory allocation, and 4) data barrier \& delays.  	
%
%	\item 
%	The tool then runs the test function again and learns from the instrumentation:
%	\begin{myenumerate}
%		\item from 1) the tool records the physical address of the SDhost and DMA engine, which will be mapped at replay time
%		
%		\item from 2) the tool records what values are being written and read to/from which register in order.
%		These values include command encodings, data addresses, sizes, \& their sequence (e.g. CMDa -> CMDb -> CMDc for read function), device status, etc. and are core to driving the read/write function;
%		
%		\item from 3) the tool discovers in-memory DMA descriptor.
%		This is done by correlating the value allocated physical pointer \& the value written to device registers (i.e. SDARG register in host). 
%		It is a 8-word data structure, where the bytes specify whether to turn on DMA IRQ, DMA address, its size and pointer to the next DMA descriptor. 
%		
%		\item from 4) the tool summarizes command timeout during replay.
%		The value was calibrated by the kernel driver after XXX rounds of sampling and was done by YYY SLoC.
%	\end{myenumerate}
%	
%	\item 
%	The tool run the test function again to find divergence (align sequence).
%	It does not find divergence in terms of values \& types registers being written to and read from.
%	It however discovers across two recordings, the number of read from SDARG (\Note{confirm}) are different, which is due to polling. 
%	The tool then prompts the developer to summarize the polling behavior, which will be reflected at replay time.
%	
%\end{myenumerate}


%\paragraph{Replay:}
%
%\textbf{Interface:} block interface as in `/dev/blk'.
%POSIX-like interfaces for `read' and `write' (rw/, off, size).
%
%\textbf{Simplistic replayer in TEE}
%
%The kernel daemon processes for MMC includes a request queue, a cmd timeout timer, a periodic retune/rescan timer...
%
%Due to simplicity goal we reduce them in TEE...
%
%1) request queue -- original designed for sharing, async exec in normal world;
%in TEE there's no notion of concurrent trustlets thus no sharing.
%The request queue is reduced to a simple handler which continuously serves the reg access from replayer...
%Reads are synchronous; writes can be async...
%
%2) no timeout timer daemon.
%The timeout logic is embedded into replayer (?)
%
%3) no continuous rescan daemon.
%Our assumption is the card/emmc stays put...

%
%\Note{merge this}
%\textbf{Symbolize data entries only.}
%The insight is it only takes 4 entries to describe any data op, i.e. data source, destination, starting address, and length of the op.
%\sys{} asks developers to annotate only these entries in source code (w/ customized decorations recognized by compiler) before recording.
%Recorder only symbolizes these entries while treating all other values fixed/static, as part of the deterministic replay context.
%\Note{this includes commands passed in register AND in memory (e.g. DMA command)}

%\Note{merged}
%\paragraph{Example: embedded flash drivers} (interleave)
%
%{Overview...architecture}
%
%https://wiki.st.com/stm32mpu/wiki/MMC\_overview
%
%Flash driver is complex:
%
%We did a code analysis of XXX flash drivers.
%Why complex? rich protocol, support for diverse medium, error prone.
%
%The specification mandates a core set of semantics.
%Other details of behaviors, implementation, etc... are SoC specific.
%
%\paragraph{Observation}
%code complexity (and hence engineering difficulty) come from configuration, power/clock management; tuning;
%
%\paragraph{Simplified...}
%
%No abort. No partial transfer. No stream transfer. No open-ended transfer (all transactions have pre-defined size)
%
%No multiple card (connected, disconnected)
%
%No stream transfer. Only block-oriented transfer.
%
%No clock control. used by host to slow down the card.
%Misc: write protection; no password (defeaturing)
%
%How about Trim, secure Trim, Erase?
%
%\paragraph{Failures}
%
%Embedded flash is error prone. Corner cases of errors (card removal, timeout, card failure, etc.)
%
%See JEDEC standard 7.8
%
%CRC error; timeout (no response); invalid command; loss of medium; ...
%
%illegal parameters from the host side (out of range, write protect violation, etc)

\begin{comment}
\subsection{DMA transactions}
\textbf{SoC specific:}
Capture in-memory descriptors? Like DMA

\paragraph{RPI3}
DMA engine separate from MMC host.
3 directly writable registers for controlling DMA engine, CONDBLK\_ADDR, CS, DEBUG.
CONDBLK\_ ADDR stores the phys addr of head of the linked control block data structure;
a control block is an 8-word data structure that guides data tx/rx behavior of DMA, each word containing: transfer information, data src addr, dst addr, dma len, stride, next cb addr;
rest two words are reserved.
 
Other fields are self-explanatory (next cb addr = 0x0 at tail control block).

SDhost initiates the data transfer process by reading/writing some sdhost regs to setup starting block addr, block size, etc.
Then the control is transferred to DMA engine side to set up the control blocks, including allocating DMA mem and filling each word entry.
It kicks off the DMA by writing 1 to CS reg of DMA.

Once the DMA completes, an IRQ is sent to trigger DMA IRQ handler.
In the DMA handler, kernel acknowledges the IRQ, then calls into SDHost callbacks to acknowledge some statuses on the SD hosts.
An interesting thing is host seems to keep a counter for DMA control block in SDEDM.
Read to SDDATA register will decrement it until it reaches 0.

\Note{Thoughts: handling} the cross-dependency between sd host and DMA drivers?

Our design eliminates the callback mechanism which is only a "feature" which is simply a good software practices.
The system implements IRQ handler as a large, monolithic reg access replayer (i.e. DMA reg and SDHost reg co-locates in the same namespace, unlike kernel).
This is due to simplicity and goal of defeaturing.

\paragraph{Limitation on TEE}
DMA might be limited on TEE, depending on the configuration of TZASC.
It requires DMA engine can access the partitioned secure memory inside TEE (i.e. a bus address).
Also the memory has to physically contiguous.
\end{comment}


%\subsection{USB Mass Storage}
\subsection{USB}

%USB is a pervasive interface for peripheral devices, e.g. mass storage, cameras, microphone. 
% Lacking USB drivers, the current TEE misses the opportunities of accessing these devices. 
% A USB driver within TEE opens door to many more opportunities of other devices. 
USB serves as a common transport between CPU and diverse peripherals, e.g. cameras, keyboards, and flash drives. 
\subsubsection{Device overview}
Middle part of Figure~\ref{fig:dev} illustrates a USB stack. 
A device driver programs the USB controller to initiate \textit{transfers}, 
each comprising a series of \textit{transactions}. 
A typical USB controller exposes more than 100 registers. % and uses DMA for data move. 
The USB controller translates each transaction into multiple packets on the bus. 
% registers and moves data to/from the controller; % by register accesses or DMA transactions. 
%the USB bus carries four types of \textit{transfer}, e.g. bulk transfer for mass storage. % and interrupt transfer for keyboards. 
%Each transfer is a series of transactions between the USB controller and a peripheral; each transaction further comprises multiple on-wire packets. 
The USB standards mandates the transaction details as well as 
the controller FSMs during each transaction. 

%A USB controller bridges CPU with USB peripherals, 
%the USB controller translates the access to on-wire protocol interfacing with the peripherals. 

% In the stack, the driver implements much of the USB standard which consists of complex state machines. 

%USB serves as a common transport for diverse peripherals. 
%By definition, each USB peripheral (e.g. a camera) consists of multiple configurations, each of which consists of multiple endpoints. 
%To support diverse devices, 
%Atop the transfers as building blocks, drivers further implement data exchange protocols specific to peripherals.  

%\paragraph{Current status}
Linux kernel fully implements the driver FSMs as mandated by the USB standard. 
The driver code comprises 21K SLoC in 82 files. 
These FSMs are big in order to accommodate rich features (e.g. dynamic discovery of bus topology, hot plug) and various runtime conditions (e.g. device speed mismatch, bus checksum errors, over current). 

% See impl of enum usb_otg_state {}
%In total, a full USB driver implements 14 states, YYY transitions\Note{how to know \# of transitions?}, XXX message types, and numerous branches for corner conditions. 

We focus on USB mass storage for its significance to TEE's secure storage. 
The driver accepts block requests, translates the requests to various SCSI commands, and further maps the commands to USB bulk transfers. 

\subsubsection{Recording experience}

We configure the USB driver as follows. 
We do not record interactions for the USB device discovery process and hotplug;
we disable Start-of-Frame (SoF) for meaningful recordings. 
SoF is autonomous/periodic IRQs of USB;
like a scheduler timer tick, it fires per 1ms and upon each SoF tick the driver schedules requests from all USB devices.
%USB has autonomous/periodic IRQs, called Start-of-Frame (SoF) interrupt including IRQ, ISO, Control transfer type.
%
%After user issues requests, the device driver schedules the resultant USB requests at SOF ticks and handle the response on these ticks;
%Fired per 1ms, SOF acts like a timer tick for CPU scheduler.
%This does not fit our model because it is not CPU-driven and does not belong to a request-reply model. 
%\paragraph{Selected requests}
We record same requests as MMC since both are storage devices, listed in Table~\ref{tab:trace}. %: read/write of 1, 8, 32, 128, 256 blocks. 
%Each request also accepts two arguments: block ID and physical address of data buffer.
We also record interactions for initializing the bulk transfer device and for soft reset.

\paragraph{Discovered interfaces} 
\sys{} identifies 14 USB controller registers out of XXX KB of register range. %including one trigger register (HCCHAR), one DMA register (HCDMA).
%Among them, \sys{} flags HCCHAR as trigger register, HCDMA as it contains in-memory descriptor address, as seen in Table~\ref{tab:tab_case_study}.
%\sys{} flags one register as a trigger register. 
%%From the source code reported by \sys{}, 
%From the reported source code, we confirm that a write to this register (channel characteristics) enables a channel and triggers interrupt. 
%\sys{} flags one register as a pointer to an in-memory descriptor, which we configure as the base of a DMA descriptor (HCDMA). 
\sys{} snapshots in-memory descriptors of three fixed lengths: 31, 512, and 4096 bytes.  
%It reports the source lines (50 SLoC in the SCSI library; 60 SLoC in the USB driver) that assign these fields. 
From their snapshot, we confirm that the former two wrap SCSI commands and the last one points to a user data buffer.
%despite that the driver only declares opaque types (unsigned int) for the descriptor's fields. 
\sys{} annotates the SCSI command's LBA field (i.e. block ID) and the user data buffer as parameterizable. 
% After being prompted by \sys{}, developer looks up the DMA descriptor in corresponding header file \Note{this handwaving?} and discovered it is a 2-quadlet (i.e. 2 4-byte words) structure, where first quadlest specifies size in 16 bits and control flags in the rest 16 bits and the other quadlet contains a DMA address, which points to either the SCSI command or user data buffer.

\paragraph{Recorded interactions}
%\sys{} emits 300 segments of interactions. 
In test, we observed little nondeterminism in driver/device interactions. 
For instance, to write 8 blocks, the driver always issues exactly 259 register accesses, initiating 18 transfers (512 bytes each) -- 5 for SCSI commands, 5 for querying command status, and 8 for data move.
%The transfers contain among which 5 contain SCSI commands (i.e. 2 x test unit ready, 2 x allow medium removal, 1 write 10), 5 query the command status (i.e. get CSW), and 8 are data packets.
%\sys{} emits XXX sites of register polling (for XXXX). 
\sys{} reports one register that reads dynamic values across runs. 
From the source lines, we identify the register as HFNUM, a performance counter showing the number of transmitted frames. %  since the device reset. 
Because the register is not used in bulk transfer, we annotate \sys{} to ignore the value difference. %(XXXX... 
\sys{} records 40 \& 10 interactions for initialization and reset respectively. 
In both, it summarizes two sites of register polling to the same reset status register.
Details are in Table~\ref{tab:tab_case_study}.

%\sys{} discovers XXX non-deterministic number of reads of device status register across XXX runs, hence suggesting a polling loop in place and reporting the source line number to the developer.
%We check out the source code and confirm the cases.


%\Note{below obsolete}
%\paragraph{Challenge: extracting access traces from a noisy background}
%practical and might be useful.
%SOF -- obsolete, we don't deal with, not because it is noise but because it does not fit our driver model.
%
%Ensuring exclusivity during recording is important (as it must the context of replay);
%clean separation must be done at IRQ level.
%The challenge is how to extract the register access exclusively belong to the device \& application activity when the device itself has non-activity-related register accesses.
%
%E.g. The state-of-frames (SOF) of USB devices, which triggers irq at high frequency (every ms)..
%Adding much noise to the collected trace.
%
%The obstacle is these noise cannot be simply shut down.
%Although one might turn if off (in a new impl. e.g. Circle), it is generally hard because modifying device driver behavior (e.g. turn off SoF) requires intimate device knowledge.
%It might also bring bugs to devices.

\subsubsection{Post analysis}

Among the 14 registers discovered by \sys{}:
5 manage the USB peripheral state (e.g. examining device power state, transmission status); 
3 manage the controller itself (e.g. interrupts); 
6 manage the transmission channels (e.g. setting channel speed, data transmission size, DMA). 

Notably, \sys{} has captured the non-trivial mapping between requested block IDs to SCSI's logic block address (LBA). 
The driver rounds up the given blocks (512 byte each) to the LBA boundary (4KB). 
In case the accessed blocks are smaller than one LBA, the driver reads back the entire LBA, updates in memory, and writes back. 
The driver also selects the best SCSI commands: 
there exist five multiple variants of SCSI commands, which have different lengths and can encode different ranges of LBA; 
the driver picks the 2nd shortest ones just long enough to encode the requested LBA addresses. 

%\Note{Check above: anything missing?}
%
%\Note{TODO: transactions, transfers, states, etc}

\begin{comment}
1) Core interface. 
Five registers are used to control USB's device states -- two for interrupt control, one for examining power state, one for device configuration, and one to reflect transmission FIFO size.
2) Host interface.
Three registers are used to manage the controller in host mode -- 
two to configure interrupt and one for reflecting frame number. 
3) Host channel.
Remaining six registers are one bank of host channel-specific registers (among 15 other channels) to kick off DMA transmission.
Two are used for interrupt, one to specify data transmission size, two to configure the channel (e.g. full/half speed, channel), and one DMA register.




\begin{myitemize}
	\item 
	Block layer is responsible for translating the sector into logical block  of the SCSI read/write commands. 
	For USB, the LBA is wrapped around at a 4KB boundary (i.e. the smallest DMA size). 
	E.g. write to sector 0-7 will translate to a LBA=0 in SCSCI command, whereas to sector 8-15 will be LBA=1.
	
	\item 
	Block layer treats accesses based on LBA boundary in two following ways:
	\begin{myitemize}
		\item 
		Reads/writes across different LBAs will be broken down into multiple accesses.
		
		\item 
		Writes that are smaller than 4KB will also be broken down into multiple accesses -- block layer first issues SCSI read to the whole 4KB region, then modifies the corresponding data, then issues 4KB writeback.    		
	\end{myitemize}

	\item 
	For each read/write command, there are five variants which have 6, 10, 12, 16, 32 bytes. 
	The more bytes the command has, the more data blocks it can address and larger data size it can transfer. 
	Out of the 5 variant, our testing shows SCSI layer picks the 10-byte one, which contains a 4-byte LBA field (each field is a 4KB) and is enough to cover over 16TB address space.
\end{myitemize}
\end{comment}

\paragraph{Analysis of developer efforts}
Table~\ref{tab:tab_case_study} lists the efforts required by \sys{}: inspecting XXX lines of code (XXX locations in XXX files) to confirm annotations of XXX fields. 

\textit{If developers build a small driver from scratch...}
They must (1) reason about the USB standard (650 pages) to identify and implement approximately eight FSMs related to the bulk transfer.
They must understand device classes (low/full/high-speed), which may have different protocols, e.g. a high-speed device has additional handshake packets.
(2) understand the SCSI protocol (XXX pages) to select and implement the command mapping. % and selection for selected requests as \sys{} discovers. 
(3) map the FSM transitions and selected SCSI commands to USB transactions.
This may be overwhelmingly difficult if not impossible, due to unpublished documentation, which is the case for Rpi3 USB device`. 
%They program the actual USB controller accordingly with register access and DMA transfers. 

% --- the longer version --- 
\begin{comment}
\textit{If one wants to build a tiny driver from scratch...}
% https://www.usb.org/sites/default/files/usbmassbulk_10.pdf
%https://doc.lagout.org/science/0_Computer%20Science/9_Others/9_Misc/USB%20Complete%20The%20Developer%27s%20Guide%204th%20Ed.pdf
1) They have to understand the USB standard, i.e. a document of 650 pages plus 96 pages of supplement of On-The-Go (OTG) device specification, which is even longer and more complex than MMC standard.
% page 213-220 of USB specs 
From the myriad of pages, they have to identify the transfer types to support (i.e. bulk in our case), and implement the corresponding FSMs.
This is non-trivial -- as we roughly calculate there are in total 45 state machines; 
for the one bulk transfer alone, there are at least 8 directly related FSMs (i.e. not device-wise FSMs) with over 10 conditional transitions each.
Even at the lowest layer, they must be aware the transfer protocol differences for low/full/high-speed devices, where high-speed device has additional handshake packets.
2) For bulk transfer, they must additionally understand the SCSI protocol \& command encodings that instruct the data move.
As described earlier, even for the same block read/write request SCSI has multiple encodings. 
This places an extra burden to developers.
3) At last, they need to map learned FSM transitions and USB packet encodings (with wrapped SCSI command) to actual hardware. 
To this end they learn the manual of the USB host in order to program the registers and DMA transfers, which constitutes XXX pages of extra specification.
E.g. to calculate bus time, they must combine the host controller-specific timing to a formula provided by the standard...
%As shown above, the mapping is non trivial. 
%The developers must also understand the SCSI protocol and map it to the USB transfers.
%As shown above, the mapping is non trivial. 
% The whole process is error prone and debugging is difficult.
\end{comment}

\textit{If developers trim down the Linux USB driver...}
They must (1) separate bulk transfer FSMs from others.
%They need to understand tens of USB concepts used in the codebase, e.g. IN/OUT endpoints, microframes.
We find separating SoF particularly challenging.
The driver invests XXX SLoC in it and scatter them in XXX files for optimization. %in order to schedule transfers. 
%It tracks missed SoF packets; it implements a queue to schedule packets on SoF tick.
They must understand USB standard to surely decide SoF is unnecessary to bulk transfer; 
removing their code is tedious. 
%We find it difficult to decide if SoF is necessary to bulk transfers. 
%And even if we are sure, removing the SoF code scattered in XXX files is tedious. 
(2) resolve the new SCSI library dependency, in addition to DMA, memory allocation, workqueue already used by MMC. 
They need to examine the structure of XXX SLoC and recompile for TEE. 

%(1) Reason about USB driver codebase: for USB mass storage, understand USB core (drivers/usb/core) and storage frameworks (drivers/usb/storage), the host driver. 
%Their interfaces, callbacks, structs. 
%(2) Code tailoring with USB domain knowledge.
%To keep the code only needed by USB mass storage (bulk transfers), we first need to understand tens of USB concepts used in the codebase, e.g. IN/OUT endpoints, microframes, XXX. 
%An example: the USB controller optionally generates periodic (1000Hz) interrupts (called Start-of-Frame, SoF). 
%The driver invests XXX SLoC in handling SoF in order to schedule transfers. 
%%It tracks missed SoF packets; it implements a queue to schedule packets on SoF tick.
%We find it difficult to decide if SoF is necessary to bulk transfers. 
%And even if we are sure, removing the SoF code scattered in XXX files is tedious. 
% --- the longer version --- 
\begin{comment}
Assuming they can do similar things, e.g. using ftrace to aforementioned codebases, they still need a comprehensive understanding of the USB standard and the codebase and have to endure the tedious build-test-debug cycles. 

E.g. the discovery process is unneeded in our scenario because it is left for the OS to do. 
How to cleanly separate the path from the codebase? What functions to remove? What device states are left after initialization done by discovery and how to cater to it at first request? 
E.g. Start-of-Frame is also unneeded for the bulk transfer type and can be removed.
Yet the driver spends XXX SLoC handling its comprehensive cases, e.g. it will track missed SoF packets; it implements a queue structure to schedule packets on SoF tick.
The codebase is deeply entangled with its IRQ handler and cannot be simply removed. 
\end{comment}
%(3) Reasoning about and porting kernel dependencies.
%Similar to MMC, USB drivers depend on memory allocator, scheduler, and DMA. 
%A new dependency is the SCSI library, for which we need to examine the structure of XXX SLoC and recompile for TEE. 
%The driver relies on block layer to translate the block address into LBA (XXX LoC);
%it relies on SCSI library to encode the LBA into the right commands (XXX LoC). 

%Porting these layers are also hard: block layer consists of XXX SLoC, spanning XXX files;
%SCSI layer consists of XXX SLoC and XXX files, which specify XXX types of different commands and is implemented from a specification over 500 pages. 


%\subsection{VCHIQ (multimedia accelerator)}
\subsection{Multimedia accelerator}
On modern SoC, CPU typically offloads video/audio processing to accelerators. 
%Examples include DSPs for signal processing, NPU for machine learning, and VPU for capturing images/videos in JPEG or H.264. 
%They communicate with the CPU through proprietary protocols. 
% These accelerators run their own firmware processing pipelines and 
A unique challenge, compared to other devices, is that these accelerators  communicate with CPU primarily via messages backed by shared memory. % with minimum use of registers). 
The message passing protocols are often proprietary and sophisticated. 

\subsubsection{Device overview}
We studied VC4, the multimedia accelerator on the Rpi3 SoC. 
According to limited information, VC4 implements key multimedia services, including camera input, display, audio output. 
It communicates with the CPU via a complex, proprietary message queue called VCHIQ.
Using VCHIQ as a transport, each media service further defines its message format and protocol, e.g. MMAL (MultiMedia Abstraction Layer) for cameras. 
The details of VCHIQ, as well as internals of VC4, remain largely undocumented. 

The above protocols are implemented by the Linux VCHIQ driver. 
The codebase of VCHIQ driver spans 10K SLoC in 60 files. 
The driver consists of three layers: message parsing, event handling, and queue management. 
%As described in Section~\ref{sec:design:prior}, much of the complexity is for performance optimization and concurrency -- 
For performance optimization and concurrency, it deploys 3 threads to support concurrent user threads to request different services from VC4, backed by tens of fine-grained semaphores;
it implements comprehensive error handling logic detect and recover from incoherent states shared by VC4.
%For instance, the driver defines 15 message types, each with different payloads of XXX to YYY fields (need better examples); 
% sema_init(...)
%21 fine-grained semaphores and condition variables; 

We focus on one media service essential to secure IO: image capture from a CSI camera (a pervasive image sensor interface used in modern mobile devices).
%display that supports modern formats such as HDMI, DVI, and DSI.  
% framebuffer-based simple display). 


\subsubsection{Recording experience}

%\paragraph{Selected requests}
Besides device initialization and reset, we choose 9 image capturing requests, as listed in Table~\ref{tab:trace}.
% to acquire 1, 10, 100 image frames in JPEG at three resolutions, i.e. 1440p (the highest resolution), 1080p, 720p. 
%We exercise the driver with v4l2-ctl invoking the Linux video ioctl API. 

%For display: 
%We choose the following requests. 
%\begin{myitemize}
%\item Load a bitmap (fixed size) to the display surface
%\item Create paths out of fonts (in XXX format)
%\item Load a vector path (fixed size) to the display surface
%\item Display glyphs at give surface coordinates
%\end{myitemize}
%Our test program is a simple graphics program from command line. 
%It renders to the whole screen and does not invoke X window. 
%Hence, we only support full screen rendering; no windowing mode is supported. 


%and one mailbox register to communicate between firmware. 
% With one additional run, \sys{} discovers that the VCHIQ\_INIT message 

\paragraph{Discovered interfaces}
\sys{} identifies a small set of three registers.  
\sys{} flags two of them as trigger registers;
%We inspect the source code and confirm that they are a pair of ``doorbells'' for raising inter-processor interrupts between CPU and the accelerator (for message send and receive, respectively). 
from the reported source we confirm that they are a pair of ``doorbells'' for raising inter-processor interrupts between CPU and VC4 (for message send and receive, respectively). 
The third register is a mailbox WRITE register used to send a firmware message during device initialization;
from its memory dump, \sys{} finds (and we confirm) it contains the base address of a shared memory region spanning 66 pages and 264 KBs in total, which we paramaterize.
% is used to set the base address of a shared memory region, spanning 66 pages and 264 KBs in total.

\sys{} scans the shared memory region and has found only one physical pointer;
it follows the pointer and finds tens of data buffer address.
\sys{} reports code source that populates them.
%of which 40 bytes are dynamic values, 4 bytes belong to a physical pointer, and the rest bytes are all static encodings. 
%\sys{} leaves the treatment of dynamic bytes at alignment time later;
%At the pointed memory region, \sys{} further identifies an in-memory descriptor. % which contains an array of physical pointers. 
%Prompted by \sys{}, we locate the relevant kernel source (about 60 SLoC in file XXXX which has XXX SLoC in total) that populates the descriptor. 
From the code, we confirm it points to a in-memory descriptor which specifies the list of data buffer addresses;
we annotate to parameterize the pointer and the data buffers.
%whose 1st-3rd words describe the data size, offset and direction (to/from device).
%Starting from the 4th word is a scatter-gather list filled with the data buffer addresses, which we annotate to parameterize.
%Additionally, we have found the 12 Least Significant Bits (LSBs) of each pointer encode the number of following contiguous pages, as an optimization of the firmware;
%for simplicity we omit the optimization and populate individual pages without merging the contiguous ones.

%At the end, \sys{} discovered (and we confirmed) the semantics of 2 fields (i.e. one DMA descriptor and one VCHIQ\_INIT message, consisting of only 8 words), which is only XXX\% a tiny fraction of whole memory dumps and remains oblivious to the semantics (and formats) of the remaining. 

\paragraph{Recorded interaction}
For each request, there are 63-560 register accesses, accompanying same number of memory dumps. 
Each memory dump snapshots the 264-KB shared memory region that backs the message queue; %whose base address is parameterized and notified during initialization;
XX fields (in total 40 bytes) are annotated to be parameterized or tolerated, shown in Table~\ref{tab:tab_case_study}.
%during replay they are either ignored or parameterized as mentioned before.	
For device initialization, there are two register accesses (to BELL2 and to mailbox WRITE) and two memory dumps (one of the shared memory region, one 8-word message to firmware). 
%Table XXX summarizes the interaction emitted by \sys{}.

%VCHIQ driver also shows a highly-deterministic and request-reply pattern across the recorded XXX segments.
\begin{comment}
Across repeated runs, \sys{} discovers no register polling. 
\sys{} discovers 40 bytes of discrepancies in memory dumps. 
% which belong to different MMAL or VCHIQ messages.
% For each diverging byte, \sys{} looks backward for the ascii code of "MMAL" and "VCHIQ", which are the header of MMAL and VCHIQ messages, respectively.
% After locating the message header, \sys{} maps the diverging bytes to a field in the message and reports as follows:
\sys{} maps back these bytes to the message definitions in the driver source.
We inspect the definitions: 
\begin{myenumerate}
	\item The 4th word of MMAL request header, pointing to the message's kernel context.
	\item The 1st word of COMPONENT\_CREATE request, pointing to the message's kernel context.
%	\item 16th word of VCHIQ slot zero, indicating tx pos of the next message. 
	\item 10-11th double word of PORT\_PARAMETER\_GET reply, rflecting VC startup timestamp.
	\item 22th word of BUFFER\_TO\_HOST, pointing to buffer kernel address.
	\item 18-19th double word of BUFFER\_FROM\_HOST, pts -- presentation timestamp.
	\item 4th word of BULK\_RX message, (to received) data size -- \textbf{to parameterize}
	\item 5th word of BULK\_RX message, (to received) data DMA descriptor address -- \textbf{to parameterize}
\end{myenumerate}

Based on the semantics, we instruct \sys{} to omit 1-5th divergence but parameterize 6-7th since they describe the data buffer in the DMA descriptor.
Subsequent XXX runs all fall into this interaction envelope. 
It is worth noting that we only examined a small fraction of message fields (XXX out of XXX). 
\end{comment}

\subsubsection{Post analysis}
%The example of "setup everything in memory" scenario is the CSI camera on RPI3 via VCHIQ interface.
%The driver and VC4 communicates via a circular message queue.
Catering to concurrent media services, the memory region backing the message queue has the following sophisticated structure. 
% backed by the shared memory region discovered by \sys{}. 
It is divided into many 4KB slots, each is assigned either to CPU or VC4 for holding messages they write. 
Each slot holds multiple messages, of varying lengths. 
CPU and VC4 independently enqueue messages to their respective slots. 
Slot 0 is special, as it contains metadata that describes the whole message queue and will be updated by both CPU and VC4, e.g. number of slots, slot allocations, read/write locations in the message queue. 
%The data structure has two major responsibilities: 1) it configures the memory region, e.g. setting up the slot size and total number of slots; 
%2) it maintains the transmission states, which contain pointers to next message to-be-sent or to-be-received in the memory region.
% Diff ports: VCHIQ relies on port \# to communicate, similar to sockets.
The doorbell registers -- 
BELL0, BELL2 signals CPU and VC4 to parse new message, respectively. %is ready to receive more messages from VC4;
%BELL2 signals new messages for VC4 to read.
Upon a new doorbell, a slot handler thread actively polls and parses the message; a sync thread synchronizes CPU-VC4 shared states in slot0; a recycle thread actively frees and recycles used slots.

%At last, the driver triggers the event by writing a one to the doorbell register to notify VideoCore about the incoming message.
%Receiving a message is a mirror process, where another doorbell is rung on the VC side and received by the CPU.
A single user request (e.g. capture a frame) entails over 60 VCHIQ message exchanges.%between the driver and the device. 
Ranging from 28 bytes to 306 bytes, these messages belong to tens of types. 
They are either for configuring the device, e.g. opening a service ``port'' of VC4, setting frame resolution; or for moving data. 
The physical pointer discovered by \sys{} is within a message of bulk transmission/reception. 

\begin{comment} % --- useful ---
To control the device (CSI camera, HDMI display), the driver sends VCHIQ messages to VC firmware at lowest level, as shown in Figure~\ref{fig:dev}. 
For a single event (e.g. capture a frame, render a graphics), there are two types of VCHIQ message: 1) data, 2) bulk transmit(TX)/receive(RX); 
the former contains MMAL commands and the latter launches DMA transmission to or from the device. %of the data buffer, which transmits or receives the data from the device (e.g. a frame).

The payload of VCHIQ data messages are 8 MMAL commands (each has a request and a reply format) being used: GET\_VERSION queries VC version -- this checks if the firmware supports the device, PORT\_ACTION to open communication port on VC, PORT\_INFO\_SET/GET to configure the port, PORT\_PARAMETER\_SET to configure the device parameter connected to the port (e.g. frame resolution), COMPONENT\_CREATE/ENABLE/DISABLE to turn on/off the device. 
The commands size from 28 bytes (i.e. request of COMPONENT\_ENABLE/DISABLE) to 306 bytes (i.e. request of PORT\_INFO\_SET).
The payload of VCHIQ bulk tx/rx message is the scatter-gather list structure as mentioned earlier. 
\end{comment}

%\textit{Initialization.}
%%VCHIQ initialization is simple. 
%To initialize VCHIQ, the driver first allocates a region of DMA memory as the message circular buffer, and initializes the first 4KB page, which specify the initial states (e.g. next message position, message counter).
%It then notifies the firmware by passing a VCHIQ\_INIT message containing the address of the VCHIQ message buffer through the mailbox interface mentioned before.

%Power \& clock is taken care of by firmware prior to kernel bootup.





\paragraph{Analysis of developer efforts}
\textit{If developers build a tiny driver from scratch...}
They face complex, poorly documented VC4 interfaces and protocols.
Even for the simple requests we target, developers have to populate the circular message queue, in particular the metadata at slot 0. 
The knowledge seems only available from the hardware vendor. 
They also have to craft the sequence of hundreds of messages that execute image capture and display. 
Debugging is tedious: any incorrect fields could render the media services unusable and VC4 provides no mechanism to report what fields may cause the problem. 

\begin{comment}
Beyond the driver code released under GPL, the key challenge is public documentation of VC is lacking.
As a proprietary software, it packs complex software stack (e.g. OpenVG) inside;
it relies solely message passing to receive commands from CPU, yet both the request and reply message formats that are accessible to public are the fruit of reverse-engineering\Note{cite}.
Secondly, the developer efforts are high. 
As we calculate roughly, there are in total XXX different data structures that are crucial to control (e.g. slot zero for initialization), which consist of XXX fields/bytes that require non-trivial developer understanding.
Thirdly, it is hard to implement it correctly.
Due to the shared-mem message passing nature, data barriers are not uncommon.
In total XXX callsites are placed with read/write barriers; 
if one shall miss, it may lead to incorrect execution, e.g. the updated transmission pointer is not seen properly by the VC, which makes it read the wrong message.
Moreover, debugging the raw memory region is tedious. 
This can be reflect by the numerous of debugging trace planted in the source code, where XXX functions are instrumented and XXX fields are dumped. 
\end{comment}

\textit{If developers trim down the Linux VCHIQ driver...}
The unique challenges is dealing with its optimization for concurrency unneeded by TEE.
For lower latency, the kernel driver implements three daemon threads to poll for any incoming messages, synchronizing states, and actively recycling slots.
The threads modify slots concurrently and are guarded by XXX semaphores shared by VC4.
If developers modify or simply remove them, it may leave states out of sync with VC4 and break the service;
if developers keep them and their threads, it misfits TEE, in which there is no daemon thread. 

%This mismatches TEE design, which has no notion of a daemon thread and assumes limited concurrency.
%2) TEE lacks comprehensive (advanced?) DMA services.\Note{clarify we only need much simpler DMA allocator?}
%The driver relies heavily on kernel DMA allocator, scatter-gather list and its family functions to efficiently manipulate data pages.
%Refactoring them will likely end up pulling the whole DMA facility inside TEE, which accounts for XXX SLoC.
%3) configuring the device properly is not easy. \Note{this may go to the above paragraph}
%Besides simply understanding the message data structure, a developer must also thoroughly understand its payload, which is used to configure the device. 
%E.g. which encoding sets the resolution to 1440P and which switches the format from BMP to JPEG?
%\paragraph{Quirks}
%
%\begin{myitemize}
%	
%%	The recorded ones are usually local 2 remote 88 -- sometimes it will change to remote 87 ?? -- this will make replay fail each time.
%%	\Note{this is due to firmware is compromised}.
%	
%	\item DMA desc.: called pagelist. 
%	Simple structure -- size, offset, and then starting the list of DMA address containing (size/page\_size) pages. 
%	The 12 LSBs of the address contain the \# of contiguous pages.
%	
%	\item 
%	At development time, \sys{} discovers abnormally excessive divergences in the recorded memory dumps.
%	Even in the same, the simplest VCHIQ message (e.g. GET\_VERSION), there are tens of bytes difference, which is over 80\% of the message size.
%	We manually discovered that it is because the driver allocates message data from stack without initializing it with 0. 
%	As a result, the unused fields are full of garbage values, which diverge each time.
%\end{myitemize}


%So far the above discussions only considered interaction with device through register.
%It assumes in-memory descriptor as bus addresses are passed to registers.
%This is not the case for VCHIQ driver used for picam, which only has two `signaling' registers, which does not contain the bus address of the message but only serves as an IPI to notify GPU the message is coming.
%
%The real data is stored inside the messages themselves (for camera its mmal message), following a (header, data) format, where the header specifies message type and size.



%\paragraph{Solution: memory snapshot}
%Despite it is message-passing and in-memory.
%The overall principle still stands -- record/snapshot the hardware/software interaction.
%
%Therefore the tool records the interaction by dumping the whole slot queue memory contents prior to each trigger, driven by the event.
%\Note{On the RX path}, it also snapshots the memory content, which is used to detect divergence..
%
%Note that it still symbolizes the data address in the memory snapshot and instantiates them during replay time.

\subsection{Mediating accesses to shared devices}
\label{sec:case:mediate}

While TEE owns the device instance and fully confines their registers accesses, they rely on power and clock domains to operate, which are inevitably shared by the entire SoC.
Once initialized, \teedrivers prevent any unauthorized writes to dependent and shared domains, in order to protect TEE-owned devices from availability attacks (e.g. shutting down power and clock).

On Rpi3, the control of power and clock domains is delegated to GPU firmware by sending commands.
In total, there are 21 commands for manipulating power/clocks. 
%(e.g. GET/SET\_CLOCKS, GET/SET\_DOMAIN\_STATE, GET/SET\_CLOCK\_RATE, GET/SET\_VOLTAGE). 
% useful: rpi3 mailbox 
% https://www.programmersought.com/article/7170472059/
% https://github.com/raspberrypi/firmware/wiki/Accessing-mailboxes
They are sent to GPU through the mailbox interface by triggering its WRITE register. %controlled by 10 registers (e.g. READ, WRITE, PEEK). 
To mediate such write to it, which contains the in-memory descriptor address pointing to the command.
It does so by configuring TZASC and to mandate secure-only access to the register;
this is similar to SeCloak~\cite{secloak}.
Each non-secure access will be trapped by TZASC and captured by \sys{};
it examines the command payload and ensures they do not belong to the 21 commands. %nor can they change any domain states.


==> intro-old.tex <==
\xzlNote{------ old writing ------}

\sys{} does not replay raw traces of interaction events; 
instead, it summarizes the trace as an \template{}, a key construct to \xzlNote{generalize ... and tolerate ... how about the template inputs?}
The \sys{} recorder derives an template from the raw trace of a single run. 
to exercise the ... golden FSM ... reproduce the hardware jobs in the recording run ...
It ... generalizes the raw trace in two important ways ....
accepts ... 
tolerates ...
\Template{} strikes a balance between recording simplicity and usefulness. 
An \template{} comprises a list of interaction meta-events \xzlNote{what's meta event}, each with parameterized arguments. 
To produce an \template{}, developers only invoke the full driver once with one concrete input, which exercises the device's ``golden'' FSM path that completes the hardware jobs for the given input. 
\sys{} lifts the resultant raw interaction trace to an \template{}: 
the \template{} accepts as a wide range input values as possible and allows as many alternative interaction sequences as possible -- as long as the device state does not deviate the recorded FSM path. 
To identify such ranges, the recorders uses symbolic execution on the concrete path to explore the input's effect on replay correctness. 
%and generates on the input constraints. 



First, complex driver/device interfaces, 
% automatic discovery of the driver/device interfaces, 
which comprise not only registers but also in-memory descriptors. 
These descriptors embed pointers to form complex data structures. 
 e.g. XXX descriptors for DMA transactions.
%These interfaces are poorly documented. 
The recording process should discover all the interface and in particular the fields that must overridden with new values at the replay time. 
%To identify these interfaces by hand, in particular the fields that must be parameterized (to be overridden by replayer) , e.g. addresses of data buffers, would require tedious, error-prone code analysis. 

Second, non-deterministic interactions. 
Even to execute the same request, the device will show different responses, e.g. different register values and interrupts. 
%the replayer cannot expect exactly the same device responses as recorded, e.g. different register values and different interrupts. 
For this reason, the replayer cannot replay raw interaction traces as recorded. 
% For instance, even in executing a simple request (e.g. ``read a flash block'') an MMC driver may read different register values and receive different interrupts (see Section XXX for details). 
% If the system replays recorded interactions \textit{verbatim}, 

Third, device state divergence. 
During replay, a device may enter unexpected states that have not occurred at the record time, e.g. transient bus errors or power overcurrent. 
How to prevent divergence as much as possible; and detect any remaining divergence and recover from it so that replay correctness is guaranteed. 


We present \sys{}, a system for generating and executing MVP drivers using record and replay, as shown in Figure~\ref{fig:overview}. 
\sys{} builds on the following insight. 
Its goal of replay is to ensure an IO device to finish the same sequence of hardware jobs as recorded. 
%This goal is achieved as long as the IO device goes through the same state transitions as recorded. 
%This goal is achieved as long as the state transitions of IO device at the replay time exactly match those at the record time. 
This goal is achieved as long as the IO device follows the same \textit{path of state transitions} as recorded. 
For this reason, \sys{} analyzes and differentiates interaction events in record and replay.
It \textit{tolerates} non-deterministic interactions that do not affect the device state; 
it \textit{prevents} many device state divergence by eliminating their sources; it \textit{detects} non-preventable divergence and recovers from them. 
Our approach to nondeterminism sets \sys{} apart from prior record-and-replay systems. \Note{cite}
Targeting debugging (often CPU programs), they seek to reproduce the original execution with high fidelity such as instruction-level precision. They therefore log all non-deterministic events and preserve them in replay. 

\sys{} contributes the following designs.
(1) It mandates a simple model for MVP drivers, which constrains the driver's behaviors to a collection of request handlers that are executed as transactions. 
%\st{This leaves little room for device state divergence.}
The model reduces the device's state space and chances of state divergence.
(2) 
\sys{} discovers the device/driver interfaces automatically. 
It exercises a full driver in multiple runs and 
varies the driver memory layouts incrementally. 
It performs differential analysis over the resultant traces and uses taint tracking to identify parameterizable fields. 
% \sys{} automatically discovers the driver/device interfaces and the fields for rewrites, e.g. hardware pointers for input/output buffers.
The recorder summarizes raw interaction traces as replay actions, which are the \textit{envelope} of driver/device interactions at the replay time. 
(3) 
\sys{} makes replay robust. 
The replayer detects device state divergence with strong guarantee -- at the same level as the full driver. 
The replay is also interpretable. 
It maps any replay action back to the source lines and execution context in the full driver, which facilitate developer debugging and analysis. 
\Note{debugging support?}

it \textit{p revents} many device state divergence by eliminating their sources; it \textit{detects} non-preventable divergence and recovers from them. 

\Note{merge this}
Prior use of RnR is mainly for bug finding, as one type of differential analysis (i.e. same inputs, observe divergence).
The intuition behind the use case is -- it assumes a symbolic execution tree/FSM for the code being tested (e.g. userspace program, driver); 
by replaying, it deterministically controls the inputs to drive FSM transitions/instantiating symbols of the execution tree, so as to expose bugs due to non-determinism (i.e. state divergence). 

\xzlNote{------ old writing end ------}

==> motiv.tex <==
% !TEX root = main.tex
\section{A case for in-TEE MMC driver}

\note{what is fundamental benefit of isolating driver code vs user code in TEE?}

\note{answer the research question -- what is minimal code to run a driver w/ comparable perf?}

\paragraph{State-of-the-art approaches are inadequate.}
Currently there's only one way to enable storage for \trustlet{}, that is, outsourcing/offloading to storage managed by normal OS.

Under this, there are two approaches: 
\begin{myenumerate}
	\item Store filedata as encrypted blobs atop a normal fs (in a disk partition).
	
	\item Directly operate on a (RPMB) partition using KV store, TEE-fs. 
\end{myenumerate}

The inadequacies come from:
\begin{myenumerate}
	\item Hard to reason about data persistence. 
	This is because malicious normal OS might silently drop the request to store. 
	
	\item Leak storage activities. E.g. write to file offset, sizes. 
	This is a known side channel that leaks user input. 
	
\end{myenumerate}

In comparison, isolating MMC driver inside \tz{} offers unique benefits:
\begin{myenumerate}
	\item 
	Easier for TEE to reason about data persistence.
	Driver code is free from tampering. 
	Assurance of persistence. 
	
	\item 
	Can function autonomously from normal OS... 
	
	\item 
	Confidentiality of storage activities. 
	
	
\end{myenumerate}


\paragraph{Goals}

\begin{myenumerate}
	\item Data confidentiality, integrity. 
	
	\item Lean impl.
	
	\item Comparable perf. 
	
\end{myenumerate}

==> overview-recycle.tex <==
% !TeX root = main.tex

\section{\sys{}}


\input{thoughts}

%\input{fig-workflow}

\begin{comment}

Manual efforts/knowledge needed: dependencies of devices (IRQ MMC DMA); command format (as register values AND as in-memory data structure).

Observation: 
A subset of behaviors (common denominator) that can be captured. We only make the following assumptions:  

Register taxonomy; 
Operations: init, read, write; 
periodic maintenance activities (mmc scan?? retuning??)
\end{comment}


%\subsection{A simplified/minimalist driver model}
%\subsection{A simple driver model}
\subsection{The MVP driver model}

The model specifies how a MVP driver works.
It is a small subset of a full driver's behaviors that are extracted by recording. 
The key is to constrain the device state space and therefore eliminate many sources of nondeterminism. 

%Rationale: the longer the driver executes, the more likely some unrecorded events will occur; the device state diverges from what was recorded. 

% \sys{} makes a tradeoff between driver simplicity and functionality. 
%\sys{} mandates a simple driver model. 
%The model constrains a driver's state space. 

\textit{Requests.}
An MVP driver exposes a small set of requests for trustlets to invoke. 
Examples include reading one block from an MMC storage and capturing an image at some resolution. 
%For instance, a request of MMC storage driver reads 1 block. 
%While commodity drivers expose complex request interfaces, e.g. XXXX, 
%Because of the simple semantics, the device state transitions in executing each request are simple. 
All requests have simple semantics. 
Accordingly, the device state transitions in executing each request are simple. 
%The trustlets compose multiple requests to meet their needs. 
This is analogous to the RISC vs. CISC tradeoffs. 
%For instance, the requests for MMC storage are read/write of a range of blocks, where the block counts are a set of fixed values (1,4, 16, 128).  

%According to the model, \sys{} only exercises the full driver with the requests and replays these requests. 

%\paragraph{Request-driven executions}
%\paragraph{Request-response executions}
% \textit{Atomic handlers}
\textit{Transactional handlers}
An MVP driver comprises a collection of request handlers. 
A handler is a sequence of \textit{replay actions}, including register accesses; loads of memory snapshots; delays; 
depositing/extracting output or input at specified memory locations. 
%Each register access site: source line information; callstack trace. 
% All requests are initiated from the CPU side, either by trustlets or a periodic timer. 
% The device cannot initiate requests to the driver. 

%A handler is atomic.
%To execute it, the TEE driver always starts from the clean-slate state and returns to the state. 
%A TEE driver only handles one request from trustlets at a time. % and hence does not execute handlers concurrently. 
An MVP driver limits concurrency and eliminates the entailed nondeterminism. 
The driver only executes one handler at a time; 
a handler submits one hardware job to the device at a time. 
% at one given moment, the driver submits at most one outstanding request to the device. 
A handler is idempotent by design. 
In case of execution failures, e.g. device state divergence, a handler will be re-executed. 
Failed execution attempts have no side effect on the eventual execution success. 

%\Note{atomic? transactional? (allows re-execution? idempotent)}

\textit{Reset to the clean slate.}
Upon boot up, the driver executes an initialization handler and reaches a device state where the device is idle and ready for the next request. 
At any moment during execution, the driver may take the device to exactly the same state by executing a soft-reset handler. 

% The execution of any subsequent request takes the device out of the quiescent state and returns to the state. 

\textit{Beaten paths only.}  
% The TEE driver only performs the most common executions in the full driver. On the beaten paths, no device faults or exceptions occur. 
%The replay actions in a handler take the device state through pre-determined  transitions. 
%These state transitions correspond to a beaten path in the full driver, on which no hardware errors occur and all resource demands are satisfied. 
%The handler contains no logic for handling device states going off the beaten path, e.g. XXX. 
Of a handler, 
the device state transitions are the same as in a successful run of the request, where no hardware or software errors occur. %  occur and all needed resources are available. 
The handler contains no actions to recover from any device state divergence. 
Once it detects a divergence, the handler soft-resets the device back to the clean slate and re-executes the handler. 
Only including beaten paths greatly simplifies recording. 
As we will show in Section XXX, re-execution is adequate to work around most of the state divergences which are transient. 

% the replayer simply soft-resets the device to the clean-slate state and re-executes the handler. 
% While the driver/device may still interact in a non-deterministic fashion, our system learns the \textit{envelop} of the interactions and emits simple logic (code) to accommodate the non determinism. 
% The replayer the driver simply soft-resets the device, bring it back to the clean-slate state, and re-executes the handler. 


% Ex: MMC: loss of medium/card (removal), device bus errors (so that message CRC is wrong); bus timeout (takes too long to response? device power errors? )
% Section XXX also studies fatal divergences (albeit rare) that cannot be handled in this way. 

% \paragraph{Debugging information}
% \paragraph{Mapping execution to the full driver}
%\paragraph{Holding the full driver accountable}
%\textit{Interpretable replay}
%\textit{Mapping interaction events to the full driver}
\textit{Accountable interactions}
%The TEE driver ensures accountability for its replay. 
%The recorder emits debugging information to accompany driver/device interactions. 
The recorder maps each replay action to a context in the full driver execution where the action was recorded. 
The information includes 
the source code location and a callstack trace. 
%  the source line and the callstack trace in the full driver. 
%The replayer hence associates every interaction it replays with a source location and a callstack trace in the full driver. 
This associates a sequence of interaction events to an execution path of the full driver. 
To debug any replay bugs, developers just reason about the corresponding full driver execution. 

%For instance, 
%in case any action triggers device state divergence, the developers can always  pinpoint a location and a context in the full driver, allowing them to reason about any replay issues just reason about the full driver execution. 

%Limit driver dynamism. Use or configure driver for deterministic interactions.

\paragraph{Limitations}
For simplicity, \sys{} gives up on devices where state transitions depend on IO data \textit{content}, a behavior commonly seen on network interface cards (NICs).
% Notable examples include network interface cards. 
%Notable examples include network interface cards. 
An example is BCM4329, a WiFi NIC that implements 802.11 MAC in its firmware. 
Its Linux driver sends different commands to the NIC based on the header content of received WiFi packets. 
%Related to above, \sys{} cannot replay interrupt handlers with control flows dependent This is because our recording method cannot capture all possible branches (thus interrupt events) in the interrupt handler. For each handler, the type of expected interrupt event is pre-determined. 
%  --- NOTE: the above is fine, we can detect it; the only problem is there can be lots of divergences at replay time. 
Fortunately, protecting NICs with secure IO is not as crucial as other devices, because security-sensitive network traffic through NIC is often protected with end-to-end encryption. 

%Fortunately, we deem NICs are \textit{not} our priority, as the TEE can protect network packets with end-to-end encryption. 
%Record and replay must be on same model of hardware platform. same device?? same SoC??? The hardware configuration should agree. 

\Note{fix the following}
Recording start after kernel power/clock init.. which is assumed to be integral..
We donot record their init (as reg access) due to the complexity beyond MMC....

%Cannot dynamically switch between configurations (?). \Note{maybe we can?}


\begin{comment}
1) need to verify recorded trace; 2) annotate deep device dependencies (e.g. how does developer know MMC involves DMA); 3) handling complex device initialization (e.g. firmware loading).

TZASC granularity -- addresses of instances need to be at least 4KB(?) apart. 
\end{comment}







==> record-impl-old.tex <==
% !TeX root = main.tex
\subsection{Recorder}
\label{sec:record:impl}

We implement the recorder in 2K SLoC C code based on S2E~\cite{s2e}, a popular symbolic execution engine. %based on QEMU~\cite{qemu}.
We choose it because it provides in-house support for analyzing Linux kernel drivers and is based on QEMU~\cite{qemu}, which uses dynamic binary translation and is easy to interpose on instruction-level execution states.
\paragraph{Concolic execution.}
%We choose it because it provides in-house support for analyzing Linux kernel drivers and is based on QEMU~\cite{qemu}, which uses dynamic binary translation to provide instruction-level tracing.
%However, QEMU emulates device IOs via guest file operations;
%it does not emulate device FSMs, which emits actual register values to a driver.
%We overcome this by tapping into QEMU and forwarding device IOs to an actual device, similar to Charm~\cite{charm}.
%This is shown in Figure XXX. 
%For most tasks, we use existing S2E plugins, which work out of box. 
%Only some need minor modifications.
The overall idea is to exercise the driver in S2E, use S2E trace printer to log the driver execution, and distill an \template{} from the logs. 
Parsing the logs is trivial, which is done by a Python script of 1K SLoC.
The key question is how to log the symbolic execution results as S2E executes. 
Fortunately, for most logs we retrofit rich S2E plugins and only add minor modifications to dump more information (e.g. concrete values, callsites): 
e.g. \code{ExecutionTracer} to log path conditions, \code{MemoryTracer} to log taint propagation, \code{LoopDetector} to extract loops.
%a list of them and our modifications are summarized in Table~\ref{tab:s2e}.
%\input{tab-s2e}
%we modifies \code{ExecutionTracer}
%\code{PathLimiter} to prune paths that have divergent device state transitions;
%\code{LoopDetector} for locating polling loops. 
%work out of box and some need minor modifications. 
To overcome the key challenge of reaching deeply (i.e. to mitigate path explosion), we run S2E on a workstation and set up a separate target SoC, which runs the same record campaign;
the architecture is shown in Figure~\ref{fig:impl}.
We record concrete input values from the SoC during driver execution and use them to seed symbolic execution of S2E. 
Specifically, they are values from actual device registers/descriptors and invocation of kernel APIs. 
We describe our experience as follows.
%We describe our experience of overcoming several implementation challenges as follows.
%Complete following modules...
%\Note{talk about template implementation and format?}
\input{fig-impl}

\paragraph{Seeding with actual inputs from device}
%\paragraph{Seeding actual device inputs to reach deeply}
%The known problem of symbolically executing a large program is to reach deep path and avoid path explosion. 
Input values from a device need to be symbolized for comparing state transitions on forked paths. 
A device may have hundreds of symbolized input values which easily lead to path explosion. 
To make it worse, QEMU cannot supply concrete values by itself, as it only emulates device IOs via guest OS file operations without reproducing a device FSM. 
We overcome this by recording the concrete device input values from a real device and seed S2E with them, shown in Figure~\ref{fig:impl}.
We do this iteratively: as soon as the execution is curbed by path explosion on a device input, we seed it with a concrete value recorded from a real device.
%This is shown in Figure XXX. 
Alternatively, actual device inputs may come from online driver execution~\cite{charm}, which we forgo due to complexity.

\paragraph{Emulating kernel functions}
Input events at \textit{Env$\leftrightarrow$Driver} interface are kernel API invocations. 
We only care about its arguments (e.g. DMA allocation size) and return results (e.g. DMA address);
their internal invocations may cause path explosion and pollute the log.
We prevent the symbolic execution path from digressing by emulating their APIs.
We leverage the \code{FunctionModels} plugin for the purpose: without implementing any internal logic, it directly returns a symbol with a seed from the actual device, e.g. a legal DMA address.
%Table~\ref{tab:emu} lists all emulated kernel functions. 
%\xzlNote{fix missing ref}

\input{tab_instrumentation}
%
%\paragraph{Distilling templates}
%Use FunctionTrace and MemoryTrace


%\paragraph{Static code instrumentation}
%%We uses userspace test harness to exercise the full driver of interest in a Linux kernel. 
%%We control the test inputs, such as physical address of the input/out data buffers, and their lengths.
%%We instrument the kernel code for the following purposes. 
%The recorder interposes the following kernel source locations on the three interfaces. % automatically. 
%Table~\ref{tab:instrumentation} provides detailed functions.
%
%\begin{myenumerate}
%	\item 
%	$Program\leftrightarrow driver$: the set of syscalls back the record entry, which may span multiple syscalls (e.g. multiple ioctl for retrieving images from camera). 
%	The recorder taints their arguments. % syscall number (?).
%	E.g. for pread, the recorder taints its file descriptor pointing to the device file, the output buffer, the offset (i.e. block id), and read size (i.e. block count).
%	
%	\item 
%	$Driver\leftrightarrow environment$: they are a set of standard kernel services provided to drivers. 
%	The recorder logs their inputs and outputs.
%	Notably for DMA APIs (e.g \code{dma\_alloc\_coherent}), the recorder customizes the DMA pool and mandates each allocation for descriptor lands in a separate page.
%	The recorder logs allocation sizes and addresses;
%	it symbolizes and taints the addresses for reconstructing the pointer structure of them.
%	
%	\item 
%	$Driver\leftrightarrow device$: the recorder manipulates page permission bits to capture and log register accesses, descriptors writes, and to dump descriptor memory.
%	%	To do so, it disables RW bits for register address pages and W bits for descriptor pages.
%	%	In the page fault handler which traps accesses to these pages, the recorder enables the permission bits temporarily to log access type (i.e. read/write), addresses and values.
%	%	If the value being written is a descriptor address, the recorder dumps its content; 
%	%	additionally, the recorder places stubs in interrupt handlers to dump all descriptors immediately after an IRQ.
%	To do so, it flips RW bits for register pages and W bits for descriptor pages.
%	Upon trapped accesses, the recorder logs the access type (RW), physical address, and values.
%	%	In the page fault handler which traps accesses to these pages, the recorder enables the permission bits temporarily to log access type (i.e. read/write), addresses and values.
%	If the write value points to a descriptor page, the recorder dumps the page and keeps updating a most recent one.
%	%	in case the recorder keeps updating the dump for the same descriptor (i.e. identified by its page), 
%	%	additionally, the recorder places stubs in interrupt handlers to dump all descriptors immediately after an IRQ.
%	%	The recorder places stub in two places to dump the descriptor content:
%	%	the recorder logs kernel's standard register accessors to dump their types (readl/writel), register addresses and values. 
%	%	Last, it injects code to dump their content (e.g. via hex\_dump) in two places: 
%	%	1) whenever their address are used being written an output event and 2) immediately after an interrupt.
%	%	This is to ensure the dumped content is consistent with the one used by device;
%	This ensures recording completeness and consistency of descriptor seen by device: 
%	the rational is by the time a descriptor address is sent to the device, it is ready to be used (and to be dumped);
%	%		the rational is by the time its address is sent to the device or from the device, it is ready to be used;
%	even if the driver modifies the descriptor after the dump, the recorder traps and logs the modifications, which will be replayed.
%	%the recorder bookkeeps all allocated descriptors and tracks their addresses and sizes. 
%	%	To ensure the dumped content is consistent with the one used by device, the recorder bookkeeps all allocated descriptors and tracks their addresses and sizes. 
%	%	The rationale is by the time its address is notified to the device, it is ready to be used.
%	%	In case their content change even after they are dumped, the recorder sets read-only permission of their pages to trap any writes and re-dump them.
%	%	However, in practice we have not found any such writes. 	
%\end{myenumerate}
%
%The recorder runs static code analysis to extract polling loop.
%It logs entry/exits of the polling loop as well as the loop conditions.
%Note that loop body, which is the polling of a register is captured via instrumentation in $driver\leftrightarrow device$ interface. 
%%Note that loop body, which is the polling of a register is captured via instrumentation in driver/device interface. 
%In practice we have found simple code analysis tool (e.g. XXX) suffices to recover almost all loops.
%
%Most of the instrumentation is automatic. The only manual effort is to identify and annotate a handful of kernel APIs. 
%Because these APIs are independent of specific drivers, the annotation is done once for each kernel version. 
%
%\begin{comment}
%\Note{old writing-- }
%
%(1) Driver input from the kernel.
%The propose is to interposes a set of standard kernel APIs and trace the input values: % and inject new values as needed. 
%allocating DMA memory (e.g. dma\_alloc\_coherent), timekeeping (), and \xzlNote{add}.  % random number generator 
%The recorder bookkeeps allocated memory regions in order to dump them. 
%%Notably, the recorder overrides the kernel's DMA memory allocator with a custom allocator, allowing customization of the driver's memory layouts. \xzlNote{needed?}
%%The custom allocator serves pages from a pool reserved at boot time at control of \sys{} (Linux CMA). 
%%Note that memory efficiency is not a concern, because the replayer does not inherit memory layout at recording time. 
%
%(2) Driver/device interactions. 
%The purpose is to log the raw interaction events. 
%%and functions that map register banks declared in device trees (e.g. ioremap);
%%We also trap access to iomem by toggling the read/write bit of their PTEs to ensure no register is left out.
%The recorder instruments register accessors (readl/writel). 
%It injects code to dump device memory regions prior to submission of a hardware job and right after a job's completion \xzlNote{how is this done}. 
%%The recorder identifies device memory regions via interposing the kernel's DMA allocations. 
%% right before trigger register writes, i.e. a register write that kicks off an upcoming hardware job and immediately precede an interrupt notifying the job status. 
%%The snapshots contain in-memory descriptors as part of the driver/device interfaces. 
%%We identify trigger registers in a dry run prior to recording. 
%
%(3) 
%Polling loops. The purpose is to tolerate the nondeterministic number of iterations as discussed above. 
%%The number of iterations is nondeterministic depending on timing. 
%%Examples include wait for register to be ready, wait hardware FIFO to become available. 
%%Symbolic execution of loop creates a large number of execution paths. 
%As done in prior systems~\cite{symdrive}, the recorder runs static code analysis to recognize polling loops and parse them. 
%For each polling loop, the instrumented code emits one replay action, 
%which preserves the loop structure: the terminating conditions and the interaction events within the loop body. 
%%As a result, recording does not generate alternative execution paths. 
%%Optionally, the loop's body repeats a segment of interactions. 
%
%%(4) Bulk data copy. 
%(4) DMA data copy. 
%The purpose is to track tainted input data as the data is moved with an DMA engine, e.g. across user/kernel buffers. \Note{discuss}
%The recorder instruments the DMA APIs. 
%\end{comment}
%
%%Note that the above instrumentation is done only to a number of generic kernel APIs that are independent of specific drivers. 
%%It is a one-time effort for a given kernel release. 
%
%%\paragraph{Dumping shared memory}
%%\xzlNote{Liwei fill in}
%%``when to dump DMA memory?''
%%``what if the driver changes the memory after the DMA addr is assigned to a reg?''
%%
%%%After static code instrumentation, prior to the very initial recording, the first question \sys{} faces is -- when to dump shared memory during recording?
%%While \sys{} instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
%%It does not know \textit{when} drivers fill them with commands, messages, etc.
%%Taking their snapshots at arbitrary times results in inconsistent values.
%%%E.g. they may be modified by driver at different layers and times.
%%
%%Our solution is to take snapshots of all of them before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
%%Our rationale is simple: the write to trigger register is a handoff point; 
%%at the point, the driver must provide the device final information about the hardware job. 
%%Finding the trigger register is straightforward: \sys{} runs a test once and identifies register writes that immediately precede interrupts, which are often used to notify job status.
%%This heuristics narrows down from tens of registers to 1--2 registers per device.
%\begin{comment}
%\paragraph{Logging DMA interactions}
%Besides register accesses, shared DMA memory serves as the alternative driver/device interaction. 
%To capture such interactions, the overarching guideline is to log DMA allocations and dump their content as well. 
%The recorder addresses following three specific problems:
%
%\textbf{When to dump in-memory descriptors?}
%While the recorder instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
%It does not know \textit{when} drivers fill them with commands, messages, etc.
%Dumping their contents at arbitrary times results in inconsistent values.
%To address this, the recorder dumps their memory as long as their addresses are consumed, i.e. when being written into a register or another descriptor, and keeps the most recent one.
%This is because by the time the device is notified about descriptor addresses, it expects them to be ready. 
%\xzlNote{what if data contents changed afterwards}
%
%\textbf{How to reconstruct linked descriptor structure?}
%A device may use multiple descriptors for one userdata transfer with a large length, e.g. each descriptor contains only one 4KB page. 
%Instead of being used individually, the descriptors may embed pointers to each other, forming a linkedlist.
%The recorder must capture the data structure for a faithful replay.
%To this end, it taints the allocated addresses of the descriptors, propagates them to registers and other descriptors, and enforces a constraint on them, e.g. the field must be filled by address of some dumped descriptor. 
%%later when the descriptor is loaded during replay, the replayer address 
%By doing this, the recorder preserves the same pointer structure. 
%Section~\ref{sec:case:mmc} will show a detailed example.
%%For example 
%\end{comment}
%
%\begin{comment}
%% obsolete
%1. propagates the driver input to DMA allocation size
%2. logs every DMA allocation (addr, size) as part of the raw trace;
%3. taints the allocated addr and propagates to registers/descs (for reconstruct descriptor pointers);
%
%Differentiate allocations for data vs. for metadata. 
%\end{comment}
%
%\paragraph{Exercising the full driver}
%\Note{check impl details} \xzlNote{can compress given we have 4.2}
%The recorder executes the driver on S2E with dynamic taint analysis:
%%\Note{repeat}
%it kicks off the driver with concrete inputs supplied by a harness program; 
%along the concrete execution path, it explores the effect of inputs by collecting path conditions, propagating taint operations, and comparing state-changing events.  
%%The recorder executes the driver with concrete inputs supplied by developers. 
%%On the same code path, it also performs symbolic execution with the input replaced as symbols.  
%The purposes are (1) to discover the input constraints $C$ needed to detect and avoid device state divergence; 
%(2) to discover data dependencies between input and output events to parameterize replay actions. 
%\Note{check the conflicts of path conditions. In theory these shall not happen.}
%\Note{check constraints -- can it refer to symbol? how to resolve? or simply define constraints are set of relations between input value and concrete values}
%%\Note{overlap with taint tracking? The goals seems to only identify predicates}
%% (2) to discover the input constraints $C$ needed to stay on the current path of device transitions. 
%
%%Developers provide concrete inputs, which are used to select execution paths (prune execution paths). 
%%It propagates the transformation applied to input symbols. 
%
%Example: 
%in a record run, one of the driver's input variable $BlkCount$ is assigned with a concrete value 6. 
%Later, the driver's executing path reaches a conditional predicate $BlkCount>8$.
%The recorder's symbolic executor forks the execution into two copies: one with constraint $BlkCount<=8$ and one with $BlkCount>8$. 
%The recorder runs both copies and compare their subsequent device state transitions (by matching their state-changing events as described in Section XXXX). 
%If the state transitions diverge later, 
%e.g. because the driver invokes only one DMA transfer when $BlkCount<=8$ and invokes more when $BlkCount > 8$, 
%the recorder only continues the executing path exercised by the concrete input ($BlkCount=6$) and prunes the other; 
%it adds $BlkCount<=8$ to the input constraint.
%%A possible cause, for example, is that the driver configures the device to use DMA data transfer only when $C>=16$. 
%If the two copies show no divergence in device transitions, 
%no input constraint will be added. 
%This is because the path conditions only affect the driver's control flow without alternating the device states, 
%e.g. the driver uses different memory allocation strategies per the $BlkCount$ value.
%%e.g. the driver does different bookkeeping depending on the $BlkCount$ value.
%
%%not visible to the device. 
%
%% ---- useful example --- 
%\begin{comment}
%The same applies to the inputs from kernel environment $S_{ker}$.
%Kernel environments: reproduce with high fidelity
%Example: block count, the driver checks for its value. 
%If it is less than a page size (i.e. eight 512-byte blocks), driver combines them as one page access through DMA.
%The analysis captures such an "if" check, conditioned on block count and hence deem the input non-parameterizable. 
%
%Otherwise, the execution constrains the input X to select the same path as the concrete input x; 
%it prunes alternative paths. 
%The rationale is only to record the beaten path exercised by the concrete input (our hypothesis). 
%This avoids state (path) explosion and makes recording inexpensive. 
%\end{comment}
%
%% The recorder also uses symbolic execution to explore the effect of 
%%The recorder also explores the effect of device response. 
%%The recorder applies the same techniques to explore the of device response, 
%The recorder applies the same techniques to treat input values from \textit{driver $\leftrightarrow$ device} interface, 
%%i.e. values flowing from the device to the driver in interaction events. 
%i.e. values read from device registers or in-memory descriptors. 
%%For a response $r$, e.g. a register read, 
%%(1) The recorder replaces a device-response value $r$ with a symbol $R$ and propagates $R$ in the subsequent driver execution. 
%(1) The recorder uses a concrete input value $V$ from device in the subsequent driver execution. 
%% to program-visible outputs or subsequent interaction events. 
%For example, the driver reads a register showing the buffer size needed by the device for storing incoming data; %the next image frame; 
%%the recorder then propagates the symbol to the size argument of a subsequent call to DMA buffer allocation. 
%the recorder symbolizes the value then propagates it to the size argument of a subsequent call to DMA buffer allocation. 
%%the device specifies its demanded buffer size via a register value; the recorder propagates the size to a future kernel buffer allocation. 
%(2) The recorder derives a constraint on the input event which $V$ belongs to. 
%If $V$ is already known as a state-changing event, e.g. read from a command status register returning a new value $v$, 
%the recorder mandates that the concrete value $v$ must be exactly matched in replay. 
%Otherwise, the recorder executes with the symbol to discover the constraint on $V$ that will prevent the subsequent device state transitions from deviating the transitions induced by the concrete input $V=v$.
%\Note{USB device ID, USB data toggle} 
%%Otherwise, the recorder uses symbolic execution to discover the constraint on $R$ that will prevent the subsequent device state transitions from deviating the transitions induced by the concrete input $R=r$. 
%%The recorder then mandates the value of the must satisfy the constraint. 
%% will raises an error if it observes the value of $r$ violates the constraint. 
%%The replayer will raises an error if it observes the value of $r$ violates the constraint. 
%% The resultant trace template raises an replay-time errors when $r$'s 
%
%%The device inputs are concrete and also assigned with symbols. 
%%The symbols are propagated in subsequent execution. 
%%If divergence in state transitions are found dependent on any device input symbols, \sys{} stops with errors -- it does not support that. 
%
%
%%\paragraph{Emitting \template{}s}
%\paragraph{Trace processor}
%%\Note{needs work}
%%Based on the trace of interaction events, the discovered dependencies, and the value constraints, 
%%Based on traced driver inputs and interaction events, 
%%Based on the sequence of traced interaction events, 
%%the recorder emits the sequence of replay actions. % all register accesses,  device memory dumps, and interrupts. 
%%In the replay actions, 
%emits replay actions from the raw logs of instrumented code and concolic driver execution in a single record run, producing an interface template.
%The implementation is straightforward: 
%\begin{myitemize}
%	\item
%	For \code{read},
%	it emits input events by replacing concrete program/environment/device input values of a raw log entry with parameters and adds their constraints, which are an expected value or a range.
%	
%	\item 
%	For \code{write},
%	it replaces the concrete values being written to device in the raw log with accumulative taint operations from its taint source, if any;
%	
%	\item 
%	For \code{poll}, 
%	it fills the loop condition with the conditions logged by static code analysis results;
%	
%	
%	\item 
%	For other replay actions: 
%	it emits a \code{load\_mem} whenever a descriptor is snapshotted;
%	it emits a \code{wait\_for\_irq} whenever an IRQ occurred in a record run;
%	it emits a \code{delay} as logged from kernel delay functions.
%\end{myitemize}
%%The recorder derives a sequence of replay actions from raw interaction events.
%%to emit input events, it replaces concrete program/environment/device input values of a raw log entry with parameters and adds their constraints, which are an expected value or a range;
%%%for replay actions that output values to the device, e.g. a register write,
%%to emit output events, it replaces the concrete values being written to device in the raw log with accumulative taint operations from its taint source, if any;
%%to emit 
%%%For replay actions that consume values from the device, e.g. a register read,
%%%the recorder annotate with the viable ranges of expected values. 
%%%if value dependency is present, e.g. a checksum of output data, or concrete values if the dependency is absent, e.g. control commands. 
%%%(from the device or the driver) as well as any transformation applied. 
%%%Examples: the data buffer address shifts right then left 3 bits in an field of the descriptor; checksum. 
%%%\sys{} records concrete values of interaction events if no value dependency is discovered, e.g. the registers encoding control commands and device status. 
%%%Other interface fields are recorded as concrete value only; they do not encode input symbols, e.g. they may encode request or protocol semantics. 
%%The recorder also emits time intervals between interaction events. 
%
%\begin{comment}
%\textbf{Resolving input-dependent fields.}
%The following is an example list of them:
%\begin{myitemize}
%\item 
%\textit{Block ID} specifies starting sector to access in a storage device. 
%
%\item 
%\textit{Block count} specifies how many sectors to access. 
%
%\item 
%\textit{Input/output buffer address} specifies data page source or destination.
%
%\item 
%\textit{Input/output Buffer length} specifies size of the input/out buffer.
%
%\item
%\textit{Descriptor address} specifies locations of in-memory descriptors. 
%
%\item 
%\textit{Descriptor size} specifies size of the descriptors. 
%Note the information about descriptor address \& size is not tracked from user inputs but from kernel DMA APIs. 
%\end{myitemize}
%\end{comment}

==> record-impl-recycle.tex <==
% !TeX root = main.tex
\subsection{Recorder implementation}
\label{sec:record:impl}

The recorder instantiates as a harness program, % to exercise the driver, 
a suite of kernel instrumentation, % to trace interactions, 
and a symbolic execution engine retrofitted from S2E~\cite{s2e}, which is based on QEMU~\cite{qemu}.
%and a trace processor. 
Harness programs are device-specific and will be described device-specific in Section~\ref{sec:case}.
We focus on last two components in this section.

We implement the recorder based on S2E v2.0~\cite{s2e}, a popular symbolic execution engine. %based on QEMU~\cite{qemu}.
We choose it because it provides in-house support for analyzing Linux kernel drivers and is based on QEMU~\cite{qemu}, which uses dynamic binary translation and provides instruction-level tracing.
However, QEMU emulates device IOs via guest file operations;
it does not emulate device FSMs, which emits actual register values to a driver.
We overcome this by tapping into QEMU and forwarding device IOs to an actual device, similar to Charm~\cite{charm}.
The architecture is shown in Figure~\ref{fig:impl_arch}

We leverage the 



%This is shown in Figure XXX. 
\xzlNote{need figure?}

\begin{comment}
\Note{moved from S2}
\paragraph{Discovering driver/device interfaces} % which must be recorded. 
At the record time, 
\sys{} needs to take a series of snapshots of the interfaces. 
(1) CPU and devices share a wide interface: registers, DMA buffers, and in-memory descriptors. 
To accommodate complex driver/device interactions, 
in-memory descriptors may further embed pointers to each other, e.g. to form a scatter-gather list. \Note{cite}
%The data structures must be captured as part of the device/driver interactions. For instance, DMA is controlled by an 8-word in-memory data structure... The VCHIQ ...  firmware ... FSM ... containing pointers to each other to form a list...
(2) 
\sys{} should identify \textit{parameterizable} interface fields, i.e. to be overridden with new values at the replay time. 
Examples include registers pointing to the base of in-memory descriptors and 
fields in in-memory descriptors pointing to input/output buffers. 
Their values depend on physical memory layout which can vary across runs. 
%The replayer must override these fields at run time, because their values depend on physical memory layout which can varies across runs. 
(3) 
The interface may span additional hardware components such as a standalone DMA engine in a separate address range and power controllers (??).
\end{comment}


\paragraph{Static code instrumentation}
%We uses userspace test harness to exercise the full driver of interest in a Linux kernel. 
%We control the test inputs, such as physical address of the input/out data buffers, and their lengths.
%We instrument the kernel code for the following purposes. 
The recorder interposes the following kernel source locations on the three interfaces. % automatically. 
Table~\ref{tab:instrumentation} provides detailed functions.
\input{tab_instrumentation}

\begin{myenumerate}
	\item 
	$Program\leftrightarrow driver$: the set of syscalls back the record entry, which may span multiple syscalls (e.g. multiple ioctl for retrieving images from camera). 
	The recorder taints their arguments. % syscall number (?).
	E.g. for pread, the recorder taints its file descriptor pointing to the device file, the output buffer, the offset (i.e. block id), and read size (i.e. block count).
	
	\item 
	$Driver\leftrightarrow environment$: they are a set of standard kernel services provided to drivers. 
	The recorder logs their inputs and outputs.
	Notably for DMA APIs (e.g \code{dma\_alloc\_coherent}), the recorder customizes the DMA pool and mandates each allocation for descriptor lands in a separate page.
	The recorder logs allocation sizes and addresses;
	it symbolizes and taints the addresses for reconstructing the pointer structure of them.
	
	\item 
	$Driver\leftrightarrow device$: the recorder manipulates page permission bits to capture and log register accesses, descriptors writes, and to dump descriptor memory.
	%	To do so, it disables RW bits for register address pages and W bits for descriptor pages.
	%	In the page fault handler which traps accesses to these pages, the recorder enables the permission bits temporarily to log access type (i.e. read/write), addresses and values.
	%	If the value being written is a descriptor address, the recorder dumps its content; 
	%	additionally, the recorder places stubs in interrupt handlers to dump all descriptors immediately after an IRQ.
	To do so, it flips RW bits for register pages and W bits for descriptor pages.
	Upon trapped accesses, the recorder logs the access type (RW), physical address, and values.
	%	In the page fault handler which traps accesses to these pages, the recorder enables the permission bits temporarily to log access type (i.e. read/write), addresses and values.
	If the write value points to a descriptor page, the recorder dumps the page and keeps updating a most recent one.
	%	in case the recorder keeps updating the dump for the same descriptor (i.e. identified by its page), 
	%	additionally, the recorder places stubs in interrupt handlers to dump all descriptors immediately after an IRQ.
	%	The recorder places stub in two places to dump the descriptor content:
	%	the recorder logs kernel's standard register accessors to dump their types (readl/writel), register addresses and values. 
	%	Last, it injects code to dump their content (e.g. via hex\_dump) in two places: 
	%	1) whenever their address are used being written an output event and 2) immediately after an interrupt.
	%	This is to ensure the dumped content is consistent with the one used by device;
	This ensures recording completeness and consistency of descriptor seen by device: 
	the rational is by the time a descriptor address is sent to the device, it is ready to be used (and to be dumped);
	%		the rational is by the time its address is sent to the device or from the device, it is ready to be used;
	even if the driver modifies the descriptor after the dump, the recorder traps and logs the modifications, which will be replayed.
	%the recorder bookkeeps all allocated descriptors and tracks their addresses and sizes. 
	%	To ensure the dumped content is consistent with the one used by device, the recorder bookkeeps all allocated descriptors and tracks their addresses and sizes. 
	%	The rationale is by the time its address is notified to the device, it is ready to be used.
	%	In case their content change even after they are dumped, the recorder sets read-only permission of their pages to trap any writes and re-dump them.
	%	However, in practice we have not found any such writes. 	
\end{myenumerate}

The recorder runs static code analysis to extract polling loop.
It logs entry/exits of the polling loop as well as the loop conditions.
Note that loop body, which is the polling of a register is captured via instrumentation in $driver\leftrightarrow device$ interface. 
%Note that loop body, which is the polling of a register is captured via instrumentation in driver/device interface. 
In practice we have found simple code analysis tool (e.g. XXX) suffices to recover almost all loops.

Most of the instrumentation is automatic. The only manual effort is to identify and annotate a handful of kernel APIs. 
Because these APIs are independent of specific drivers, the annotation is done once for each kernel version. 

\begin{comment}
\Note{old writing-- }

(1) Driver input from the kernel.
The propose is to interposes a set of standard kernel APIs and trace the input values: % and inject new values as needed. 
allocating DMA memory (e.g. dma\_alloc\_coherent), timekeeping (), and \xzlNote{add}.  % random number generator 
The recorder bookkeeps allocated memory regions in order to dump them. 
%Notably, the recorder overrides the kernel's DMA memory allocator with a custom allocator, allowing customization of the driver's memory layouts. \xzlNote{needed?}
%The custom allocator serves pages from a pool reserved at boot time at control of \sys{} (Linux CMA). 
%Note that memory efficiency is not a concern, because the replayer does not inherit memory layout at recording time. 

(2) Driver/device interactions. 
The purpose is to log the raw interaction events. 
%and functions that map register banks declared in device trees (e.g. ioremap);
%We also trap access to iomem by toggling the read/write bit of their PTEs to ensure no register is left out.
The recorder instruments register accessors (readl/writel). 
It injects code to dump device memory regions prior to submission of a hardware job and right after a job's completion \xzlNote{how is this done}. 
%The recorder identifies device memory regions via interposing the kernel's DMA allocations. 
% right before trigger register writes, i.e. a register write that kicks off an upcoming hardware job and immediately precede an interrupt notifying the job status. 
%The snapshots contain in-memory descriptors as part of the driver/device interfaces. 
%We identify trigger registers in a dry run prior to recording. 

(3) 
Polling loops. The purpose is to tolerate the nondeterministic number of iterations as discussed above. 
%The number of iterations is nondeterministic depending on timing. 
%Examples include wait for register to be ready, wait hardware FIFO to become available. 
%Symbolic execution of loop creates a large number of execution paths. 
As done in prior systems~\cite{symdrive}, the recorder runs static code analysis to recognize polling loops and parse them. 
For each polling loop, the instrumented code emits one replay action, 
which preserves the loop structure: the terminating conditions and the interaction events within the loop body. 
%As a result, recording does not generate alternative execution paths. 
%Optionally, the loop's body repeats a segment of interactions. 

%(4) Bulk data copy. 
(4) DMA data copy. 
The purpose is to track tainted input data as the data is moved with an DMA engine, e.g. across user/kernel buffers. \Note{discuss}
The recorder instruments the DMA APIs. 
\end{comment}

%Note that the above instrumentation is done only to a number of generic kernel APIs that are independent of specific drivers. 
%It is a one-time effort for a given kernel release. 

%\paragraph{Dumping shared memory}
%\xzlNote{Liwei fill in}
%``when to dump DMA memory?''
%``what if the driver changes the memory after the DMA addr is assigned to a reg?''
%
%%After static code instrumentation, prior to the very initial recording, the first question \sys{} faces is -- when to dump shared memory during recording?
%While \sys{} instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
%It does not know \textit{when} drivers fill them with commands, messages, etc.
%Taking their snapshots at arbitrary times results in inconsistent values.
%%E.g. they may be modified by driver at different layers and times.
%
%Our solution is to take snapshots of all of them before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
%Our rationale is simple: the write to trigger register is a handoff point; 
%at the point, the driver must provide the device final information about the hardware job. 
%Finding the trigger register is straightforward: \sys{} runs a test once and identifies register writes that immediately precede interrupts, which are often used to notify job status.
%This heuristics narrows down from tens of registers to 1--2 registers per device.
\begin{comment}
\paragraph{Logging DMA interactions}
Besides register accesses, shared DMA memory serves as the alternative driver/device interaction. 
To capture such interactions, the overarching guideline is to log DMA allocations and dump their content as well. 
The recorder addresses following three specific problems:

\textbf{When to dump in-memory descriptors?}
While the recorder instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
It does not know \textit{when} drivers fill them with commands, messages, etc.
Dumping their contents at arbitrary times results in inconsistent values.
To address this, the recorder dumps their memory as long as their addresses are consumed, i.e. when being written into a register or another descriptor, and keeps the most recent one.
This is because by the time the device is notified about descriptor addresses, it expects them to be ready. 
\xzlNote{what if data contents changed afterwards}

\textbf{How to reconstruct linked descriptor structure?}
A device may use multiple descriptors for one userdata transfer with a large length, e.g. each descriptor contains only one 4KB page. 
Instead of being used individually, the descriptors may embed pointers to each other, forming a linkedlist.
The recorder must capture the data structure for a faithful replay.
To this end, it taints the allocated addresses of the descriptors, propagates them to registers and other descriptors, and enforces a constraint on them, e.g. the field must be filled by address of some dumped descriptor. 
%later when the descriptor is loaded during replay, the replayer address 
By doing this, the recorder preserves the same pointer structure. 
Section~\ref{sec:case:mmc} will show a detailed example.
%For example 
\end{comment}

\begin{comment}
% obsolete
1. propagates the driver input to DMA allocation size
2. logs every DMA allocation (addr, size) as part of the raw trace;
3. taints the allocated addr and propagates to registers/descs (for reconstruct descriptor pointers);

Differentiate allocations for data vs. for metadata. 
\end{comment}

\paragraph{Exercising the full driver}
\Note{check impl details} \xzlNote{can compress given we have 4.2}
The recorder executes the driver on S2E with dynamic taint analysis:
%\Note{repeat}
it kicks off the driver with concrete inputs supplied by a harness program; 
along the concrete execution path, it explores the effect of inputs by collecting path conditions, propagating taint operations, and comparing state-changing events.  
%The recorder executes the driver with concrete inputs supplied by developers. 
%On the same code path, it also performs symbolic execution with the input replaced as symbols.  
The purposes are (1) to discover the input constraints $C$ needed to detect and avoid device state divergence; 
(2) to discover data dependencies between input and output events to parameterize replay actions. 
\Note{check the conflicts of path conditions. In theory these shall not happen.}
\Note{check constraints -- can it refer to symbol? how to resolve? or simply define constraints are set of relations between input value and concrete values}
%\Note{overlap with taint tracking? The goals seems to only identify predicates}
% (2) to discover the input constraints $C$ needed to stay on the current path of device transitions. 

%Developers provide concrete inputs, which are used to select execution paths (prune execution paths). 
%It propagates the transformation applied to input symbols. 

Example: 
in a record run, one of the driver's input variable $BlkCount$ is assigned with a concrete value 6. 
Later, the driver's executing path reaches a conditional predicate $BlkCount>8$.
The recorder's symbolic executor forks the execution into two copies: one with constraint $BlkCount<=8$ and one with $BlkCount>8$. 
The recorder runs both copies and compare their subsequent device state transitions (by matching their state-changing events as described in Section XXXX). 
If the state transitions diverge later, 
e.g. because the driver invokes only one DMA transfer when $BlkCount<=8$ and invokes more when $BlkCount > 8$, 
the recorder only continues the executing path exercised by the concrete input ($BlkCount=6$) and prunes the other; 
it adds $BlkCount<=8$ to the input constraint.
%A possible cause, for example, is that the driver configures the device to use DMA data transfer only when $C>=16$. 
If the two copies show no divergence in device transitions, 
no input constraint will be added. 
This is because the path conditions only affect the driver's control flow without alternating the device states, 
e.g. the driver uses different memory allocation strategies per the $BlkCount$ value.
%e.g. the driver does different bookkeeping depending on the $BlkCount$ value.

%not visible to the device. 

% ---- useful example --- 
\begin{comment}
The same applies to the inputs from kernel environment $S_{ker}$.
Kernel environments: reproduce with high fidelity
Example: block count, the driver checks for its value. 
If it is less than a page size (i.e. eight 512-byte blocks), driver combines them as one page access through DMA.
The analysis captures such an "if" check, conditioned on block count and hence deem the input non-parameterizable. 

Otherwise, the execution constrains the input X to select the same path as the concrete input x; 
it prunes alternative paths. 
The rationale is only to record the beaten path exercised by the concrete input (our hypothesis). 
This avoids state (path) explosion and makes recording inexpensive. 
\end{comment}

% The recorder also uses symbolic execution to explore the effect of 
%The recorder also explores the effect of device response. 
%The recorder applies the same techniques to explore the of device response, 
The recorder applies the same techniques to treat input values from \textit{driver $\leftrightarrow$ device} interface, 
%i.e. values flowing from the device to the driver in interaction events. 
i.e. values read from device registers or in-memory descriptors. 
%For a response $r$, e.g. a register read, 
%(1) The recorder replaces a device-response value $r$ with a symbol $R$ and propagates $R$ in the subsequent driver execution. 
(1) The recorder uses a concrete input value $V$ from device in the subsequent driver execution. 
% to program-visible outputs or subsequent interaction events. 
For example, the driver reads a register showing the buffer size needed by the device for storing incoming data; %the next image frame; 
%the recorder then propagates the symbol to the size argument of a subsequent call to DMA buffer allocation. 
the recorder symbolizes the value then propagates it to the size argument of a subsequent call to DMA buffer allocation. 
%the device specifies its demanded buffer size via a register value; the recorder propagates the size to a future kernel buffer allocation. 
(2) The recorder derives a constraint on the input event which $V$ belongs to. 
If $V$ is already known as a state-changing event, e.g. read from a command status register returning a new value $v$, 
the recorder mandates that the concrete value $v$ must be exactly matched in replay. 
Otherwise, the recorder executes with the symbol to discover the constraint on $V$ that will prevent the subsequent device state transitions from deviating the transitions induced by the concrete input $V=v$.
\Note{USB device ID, USB data toggle} 
%Otherwise, the recorder uses symbolic execution to discover the constraint on $R$ that will prevent the subsequent device state transitions from deviating the transitions induced by the concrete input $R=r$. 
%The recorder then mandates the value of the must satisfy the constraint. 
% will raises an error if it observes the value of $r$ violates the constraint. 
%The replayer will raises an error if it observes the value of $r$ violates the constraint. 
% The resultant trace template raises an replay-time errors when $r$'s 

%The device inputs are concrete and also assigned with symbols. 
%The symbols are propagated in subsequent execution. 
%If divergence in state transitions are found dependent on any device input symbols, \sys{} stops with errors -- it does not support that. 


%\paragraph{Emitting \template{}s}
\paragraph{Trace processor}
%\Note{needs work}
%Based on the trace of interaction events, the discovered dependencies, and the value constraints, 
%Based on traced driver inputs and interaction events, 
%Based on the sequence of traced interaction events, 
%the recorder emits the sequence of replay actions. % all register accesses,  device memory dumps, and interrupts. 
%In the replay actions, 
emits replay actions from the raw logs of instrumented code and concolic driver execution in a single record run, producing an interface template.
The implementation is straightforward: 
\begin{myitemize}
	\item
	For \code{read},
	it emits input events by replacing concrete program/environment/device input values of a raw log entry with parameters and adds their constraints, which are an expected value or a range.
	
	\item 
	For \code{write},
	it replaces the concrete values being written to device in the raw log with accumulative taint operations from its taint source, if any;
	
	\item 
	For \code{poll}, 
	it fills the loop condition with the conditions logged by static code analysis results;
	
	
	\item 
	For other replay actions: 
	it emits a \code{load\_mem} whenever a descriptor is snapshotted;
	it emits a \code{wait\_for\_irq} whenever an IRQ occurred in a record run;
	it emits a \code{delay} as logged from kernel delay functions.
\end{myitemize}
%The recorder derives a sequence of replay actions from raw interaction events.
%to emit input events, it replaces concrete program/environment/device input values of a raw log entry with parameters and adds their constraints, which are an expected value or a range;
%%for replay actions that output values to the device, e.g. a register write,
%to emit output events, it replaces the concrete values being written to device in the raw log with accumulative taint operations from its taint source, if any;
%to emit 
%%For replay actions that consume values from the device, e.g. a register read,
%%the recorder annotate with the viable ranges of expected values. 
%%if value dependency is present, e.g. a checksum of output data, or concrete values if the dependency is absent, e.g. control commands. 
%%(from the device or the driver) as well as any transformation applied. 
%%Examples: the data buffer address shifts right then left 3 bits in an field of the descriptor; checksum. 
%%\sys{} records concrete values of interaction events if no value dependency is discovered, e.g. the registers encoding control commands and device status. 
%%Other interface fields are recorded as concrete value only; they do not encode input symbols, e.g. they may encode request or protocol semantics. 
%The recorder also emits time intervals between interaction events. 

\begin{comment}
\textbf{Resolving input-dependent fields.}
The following is an example list of them:
\begin{myitemize}
\item 
\textit{Block ID} specifies starting sector to access in a storage device. 

\item 
\textit{Block count} specifies how many sectors to access. 

\item 
\textit{Input/output buffer address} specifies data page source or destination.

\item 
\textit{Input/output Buffer length} specifies size of the input/out buffer.

\item
\textit{Descriptor address} specifies locations of in-memory descriptors. 

\item 
\textit{Descriptor size} specifies size of the descriptors. 
Note the information about descriptor address \& size is not tracked from user inputs but from kernel DMA APIs. 
\end{myitemize}
\end{comment}

==> record-recycle.tex <==
% !TeX root = main.tex

\section{Record}
\Note{register taxonomy:} configuration reg, trigger reg, status reg, data reg..
\Note{multiple runs of same request:}
* run 1: same argument, the goal is to summarize polling behavior 

* run 2: vary parameterizeable field -- correlate them with driver interaction

As shown in Figure XXX, recording is done in two phases. 

\begin{myitemize}
\item Interface discovery: 
%\sys{} exercises the driver and traces the driver/device interactions. 
\sys{} exercises the full driver in many iterations and varies the recording environments. 
It analyzes the driver/device interactions and incrementally discovers the interfaces. 

\item Recording emission: After the interface is discovered, \sys{} runs the selected requests. 
It summarizes the collected traces as segments of replay actions, each for one request. 
%which are the envelope of nondeterministic interactions. 
\end{myitemize}

\sys{} automates most of this process. It needs developer efforts on confirming the discovered interfaces and annotating a small number of interface fields. 

\subsection{Setting a controlled recording environment}
We run the full driver of interest in a Linux kernel. 
We instrument the kernel, which is the driver's environment. 
To capture full interaction, the instrumentation must contain (1) complete register accesses as well as shared memory allocations, (2) distinguishable physical pointers to facilitate differential analysis later, in case kernel allocates same DMA memory address across different runs.

To this end, we instrument the kernel as follows:
%The instrumentation serves two purposes: 
%(1) it traces register access, which bootstraps the discovery of the remaining interfaces; 
%(2) it randomizes the driver's memory layouts across runs. 
%Later, the recorder does differential analysis over the resultant traces and discovers physical pointers and parameterizable fields. 
%

% We turn off the driver's configurable features, if any, that mismatch our simple driver model. (Section XXX will provide more details).The device hardware configuration must be the same as the replay time. For instance, a single-level USB device topology. 

%\sys{} relies on ``hints'' from kernel and instrument them to infer key information about the driver during recording . They are the following: 
\begin{myitemize}
	\item 
	Tracing register access. 
	The identified registers will bootstrap the discovery of the remaining interfaces.
	We instrument register accessors (readl, writel) and the functions that parse the register declaration in device trees and map them (device tree XXX, ioremap);
	we also trap each access to them by toggling the page read/write bit of their mapped pages.
	The redundancy gives us higher confidence that no register is left out. 
%	We protect the region in order to intercept any access. 
%	The addresses of registers are easy to find: a device's registers are in a contiguous address range; they are clearly defined in source headers; there are extensive kernel tracing facilities to find out register accesses. 
	
		
	\item 
%	Register access \& DMA are the only two ways to control the driver. 
%	Physical pointer to DMA memory always refers to control block/descriptor understandable by the device.
	Locating memory regions shared between CPU and the device. 
	These memory regions are part of the driver/device interface and will be dumped for recording. 
	We instrument the DMA APIs (dma\_zalloc\_coherent, dmam\_zalloc\_coherent), which are the kernel's standard methods to allocate memory that is not always CPU-coherent. 
	
	\item 
	Substitute the stock page allocator with a custom one. 
	This allows \sys{} to change the driver's memory layouts across runs and does differential analysis over the resultant traces. 
	% and discovers physical pointers and parameterizable fields. 	
	The custom allocator serves pages from a dedicated pool reserved at boot time (via Linux CMA). 		
	The allocator is as simple as XXX SLoC. 
	Note that memory efficiency is not a concern, because the replayer 
	will not inherit memory layout from the recording time but allocate memory at its own discretion and 
	
	% ; it allows \sys{} to allocate the same physical memory chunks 
	% \sys{} substitutes the kernel's page allocator. 
	% The new memory allocator creates a large pool of contiguous memory pool at boot time (via Linux CMA) and serves the target driver from the pool in lieu of the stock allocator. 
		
\end{myitemize}
Note that the above instrumentation is done only to a number of generic kernel APIs that are independent of specific drivers. 
It is a one-time effort for a given kernel release. 

\subsection{Discovering software/hardware interfaces}
%\Note{assumption:} read has no side effects; only write change states.
\begin{comment}
\paragraph{Choosing test requests}
Given a driver, \sys{} runs a test suite that issues requests as needed by target trustlets. 
While commodity drivers expose complex request interfaces, e.g. XXXX, 
we pick requests with simple semantics so that each request finishes an atomic task.  
By doing so, we keep each request handler (and the device state transitions within) simple. 
This is analogous to the RISC vs. CISC debate. 
For instance, the requests for MMC storage are read/write of a range of blocks, where the block counts are a set of fixed values (1,4, 16, 128).  
In addition to requests, \sys{} records interaction segments during device initialization and device reset, respectively. 
\end{comment}

The basic idea is to exercise the driver in many runs, take snapshots of the interface, and analyze the snapshots incrementally. 


\paragraph{Snapshotting at trigger registers}
After setting up the environment, prior to the very initial recording, the first question \sys{} faces is -- when to snapshot shared memory regions during recording?
While \sys{} instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
It does not know \textit{when} drivers fill them with commands, messages, etc.
Taking their snapshots at arbitrary times results in inconsistent values.
%E.g. they may be modified by driver at different layers and times.

Our solution is to take snapshots of all of them before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
Our rationale is simple: the write to trigger register is a handoff point; 
at the point, the driver must provide the device final information about the hardware job. 
Finding the trigger register is straightforward: \sys{} runs a test once and identifies register writes that immediately precede interrupts, which are often used to notify job status.
This heuristics narrows down from tens of registers to 1--2 registers per device.
Repeated runs can eliminate false positives if any, e.g. register writes by a background thread unrelated that happen to precede an interrupt. 
Finally, \sys{} prompts the developers to confirm the finding the trigger registers. 
More details are described later in Section~\ref{sec:case}. 
 
%\paragraph{Time snapshots by triggering registers}
%The first question is to \textit{time} the snapshots. 
%Taking a snapshot at arbitrary times results in inconsistent values. 
%For instance, an interface field may contain invalid physical pointers to memory regions yet to be allocated. 
%
%Our solution is to take snapshots before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
%Because our driver model limits hardware concurrency, 
%the driver and device interact in a request/response pattern: 
%the driver \st{configures the devices, } prepares a hardware job (e.g. to initiate a USB transaction) and starts the job with a register write (e.g. the USB controller's HCCHAR register); 
%later, the device responds with an interrupt. 
%Note that to execute a request the driver often submits many hardware jobs. 
%Prior to trigger register writes, the interface is guaranteed to be consistent, because the device is not updating the interface (it finishes the prior job) and the driver has done preparing for the next job. 
%%Writes of trigger registers are the moments when driver/device synchronize on in-memory descriptors and the descriptors are guaranteed to be consistent 
%
%To find the trigger registers, \sys{} parses the interaction trace and identifies register writes that immediately precede interrupts. 
%This heuristics narrows down from tens of registers to 1--2 registers per device.
%Repeated runs can eliminate false positives if any, e.g. register writes by a background thread unrelated that happen to precede an interrupt. 
%Finally, \sys{} prompts the developers to confirm the finding the trigger registers. 
%
%(see case study). 
%
%\Note{what about triggering that does not raise an interrupt?}
%\Note{what about asynchronous workqueues?}
\paragraph{Discover software/hardware interfaces}
After setting up the snapshotting point at trigger registers, \sys{} runs test again to discover interfaces, i.e. registers and in-memory descriptors.%for differential analysis. 

Straightforwardly, from the recording \sys{} discovers all registers used by the driver as hardware/software interfaces.
%Additionally, the interfaces also rely extensively on in-memory descriptors to pack complex information (e.g. SCSI command, DMA control block). 
\sys{} discovers in-memory descriptors by looking for any register writes with physical pointers allocated by our custom allocator. 
Since they themselves may embed pointers pointing another descriptor, \sys{} follows the physical pointers inside first discovered in-memory descriptor until now new one is found.
\sys{} provides richer information for in-memory descriptors: it associates their physical pointers with DMA instrumentation and reports the sites of their allocation, with which the developer can easily tell their type and fields for annotation.
%\sys{} does backward slicing starting from the site of trigger register writes until it reaches the most recent source line that writes to a field. 
%\sys{} provides evidence for developers to confirm: 
%the source lines that assign the pointer field; 
%the source lines that map the DMA region. 
\paragraph{Differential analysis on discovered interfaces}
Then \sys{} runs differential analysis on each discovered interfaces of the recordings. 
To do so, it runs tests repeatedly;
for each run, it resets the driver to the clean slate state, randomizes its DMA pool (using our custom allocator), and runs the test with same argument.
%As a result, each test run produces a recording, which is a sequence of register access (physical address and their read/write values), with a bunch of memory snapshots (with data contents, allocated address, size, etc.) taken at trigger registers as supplements.
For all interface \textit{fields} collected in the recordings, \sys{} looks for the three possible differences:
\begin{myenumerate}
	\item 
	Static values (i.e. no difference), e.g. protocol communications, command encoding, device configuration, etc. 
	The values are identical across runs. 
%	They  will be replayed as-is during replay. 
%	No efforts/inputs are needed from developers. 
%	These constitute most of the interface fields. 
		
	\item  
	Data-dependent, e.g. data lengths, addresses for input/output buffers, checksum\Note{not seen yet}.
%	They are concrete values that change with test parameters, e.g. (addr, size) and data content (if it's MMC PIO). 
%	These values shall be overridden and parameterized at the replay time. 
%	\sys{} annotate the semantics of the fields (input, output, lengths) and asks confirmation from developers. 
%	Typically there are several such fields per device. 

	\item 
	Dynamic values, e.g. command serial numbers, timestamps, progress, device power states) 
%	\sys{} flags the fields and related source code, asking developers/replayer to provide logic for handling (or synthesizing) values. 
%	Such fields are rare. 

\end{myenumerate} 

For the first type of difference, they  will be replayed as-is during replay -- register read/write with same value, fields of in-memory descriptors remain the same. 
No efforts/inputs are needed from developers. 
These constitute most of the interface fields. 

The second type are concrete values that change with test parameters, e.g. (addr, size) and data content (if it's MMC PIO).
Typically there are several such fields per device. 
\sys{} automatically finds, annotate the semantics of the fields (input, output, lengths), and asks confirmation from developers. 
%\paragraph{Find in-memory descriptors}
%The objective is to identify registers that point to these descriptors and the possible pointers that these descriptors embed to point each other. 
%
%Our idea is to run differential analysis over snapshots across runs. 
%Our observations are: 
%all interface \textit{fields}, including registers or in-memory descriptors, 
%fall into three categories: 
%
%\begin{itemize}
%\item 
%Static values, e.g. protocol communications, command encoding, device configuration, etc. 
%The values are identical across runs. 
%They  will be replayed as-is during replay. 
%No efforts/inputs are needed from developers. 
%These constitute most of the interface fields. 
%
%\item  
%Data-dependent: data lengths, addresses for input/output buffers, checksum
%concrete values that change with test parameters, e.g. (addr, size) and data content (if it's MMC PIO). 
%These values shall be overridden at the replay time. 
%\sys{} annotate the semantics of the fields (input, output, lengths) and asks confirmation from developers. 
%Typically there are several such fields per device. 
%
%\item Dynamic values: (command serial numbers, timestamps, progress, device power states) 
%\sys{} flags the fields and related source code, asking developers/replayer to  provide logic for handling (or synthesizing) values. 
%Such fields are rare. 
%\end{itemize}
%
%\sys{} discovers the interface incrementally. 
%%The recorder starts from the known interface (initially, the set of registers). 
%The recorder maintains a known interface S, which, at the beginning of the discovery phase, includes only the register set. 
%It repeats the following process. 
%
%\begin{itemize}
%\item 
%Reset the driver to the clean slate state. 
% 
%\item 
%% \sys{} mutates physical memory layout. 
%\sys{} introduces random changes to the driver's physical memory allocation. 
%Of all the memory allocations in the test, it changes the location of one region. 
% 
%\item 
%Prior to each write to a trigger register, 
%\sys{} takes a snapshot of S (all the interface fields it knows so far). 
%It compares the snapshot to those snapshots taken at the same trigger register write in previous runs. 
%
%\item 
%\sys{} flags the fields with values that change with the memory layout. 
%It further vets each candidate field with heuristics: 
%does the field value fall in the address range of any allocated memory region? 
%does the absolute change in the field value equal to the change in the buffer addresses?
%does the field value change if the memory layout remains \textit{unchanged}?
%
%\item 
%\sys{} follows a found physical pointer to discover the in-memory descriptor pointed to (S').
%To do so,  
%\sys{} does backward slicing starting from the site of trigger register writes until it reaches the most recent source line that writes to a field. 
%\sys{} provides evidence for developers to confirm: 
%the source lines that assign the pointer field; 
%the source lines that map the DMA region. 
%\sys{} determines the length of S' by checking the size of the struct or the length of the mapped region. 
%
%\item 
%Add the newly discovered in-memory descriptor S' to S: S=S+S'. 
%Repeat the test run which compares the snapshots of the updated S. 
%This is to discover any physical pointers embedded in S'. 
%\end{itemize}
%
%Repeat the runs until no new descriptors are found. 
%\paragraph{Find parameterizable fields}
%On the software/hardware interface, the parameterizable fields are data-dependent. 
%That is, addresses and lengths of input/output buffers. 
%Devices will get/put output or input data from these buffers. 

%These fields contain data dependent values. 
%The procedure is similar to the above. 
%Similar to above, the discovery procedure centers on 
%Similar to descriptor discovery, \sys{} discovers the fields for buffer addresses with differential analysis. 
%Similarly, \sys{} discovers the fields for buffer addresses also with differential analysis. 
To automatically discover the fields for buffer addresses, \sys{} controls the test harness and varies the buffer locations supplied from the test programs to the driver. 
Through differential analysis, 
\sys{} identifies as candidates the interface fields that only change with buffer locations. 
To validate the findings, \sys{} \textit{taints} the buffers and 
looks for the taint values at the memory regions pointed by the candidate fields. 
%By doing so, \sys{} can finally determine the fields that point to input/output buffers. 

The values of buffer length fields may come from three sources. 
(1) Specified by device protocols. 
For instance, the command buffers of USB driver are always 31 bytes if we only record 4 commands. 
Since the values are fixed, \sys{} will record them obliviously without any discovery. 
(2) Supplied as a request parameter from trustlets. 
\sys{} discovers such fields by running requests with different data sizes, e.g. 8 vs 32 sectors. 
(3) Requested by the device. 
For instance, a media accelerator (camera?) requests the driver to allocate a buffer as large as an incoming video frame (see Section~\ref{sec:case} for details). 
To discover it, \sys{} scans the interface snapshots (register and shared memory) that precede to the buffer allocation and looks for values that match the allocation size. 
% Assumption: physical buffer addresses are stored in registers and/or in-memory descriptors. 
% The lengths are stored in similar fashion. However, the values stored may be in different units (e.g. not necessarily bytes but pages, etc)

For the last type, \sys{} flags the fields and related source code, asking developers to summarize their actions, which we will discuss shortly in \S~\ref{sec:design:summarize}.
Such fields are rare. 


\begin{comment} % --- useful???----		
\paragraph{Hints on interaction pattern}
There are limited patterns we rely on as hints to align recording sequences. 
\begin{myitemize}
	\item 
	Data sizes must be aligned/identical in the (annotated) data fields (e.g. in register as well as in DMA descriptors) during interactions. 
	There are only three types of data sizes: fixed, user specified, device requested.
	Fixed size: e.g. < 1 sector access to storage will be fixed to 1 sector access.
	User specified: e.g. > 1 sector access to storage. The data size will be as specified by user (w/ round ups).
	Device requested: e.g. sensor data transfer from device to host, which is variable in sizes.
	
	\item 
	Device-specific initialization is done upon kernel driver probing, which is the entry point upon loading the driver module.

	\Note{below seems not needed}
	
	\item 
	Any states are quiescent until triggered.
	I.e. To align values written to register, \sys{} only cares about the most recent write before trigger register.

	\item 
	Read same register consecutively for multiple times suggest a polling.
	Usually are status register.
	May have busy/idle wait in between the reads.
	Final value of the reads is the stationary (converging?) point. 
	\Note{what about write to same register for consecutive multiple times?} The scenario only happens in MMC PIO path		
\end{myitemize}
\end{comment}


\begin{comment}
\Note{--- below obsoleted ---}

\paragraph{Identify dependent devices}. Example: DMA engines. MMC can use both PIO and DMA; w/o knowing the knowledge, developer misses DMA's register accesses;

\paragraph{Timing -- delays}
\textbf{Step 3: annotate in-memory descriptors at bus address.}
The rationale of picking bus addresses for treatment is because that's what devices only recognize;
each bus address is deemed to refer to an in-memory descriptor that needs annotation.
The system then prompts the developers of the descriptor, supplying the developer with the location where it happens. 
The developer then annotates the fields that contain dst, src, addr, and size, which will be symbolized. 
For other fields, the tool simply records as-is (and treat them as static command/configuration).
If a buf address occurs in the fields again, the tool follows the address and iteratively records the descriptor pointed by the address until no buf address left.

An empirical solution to find such data structures is to examine the types of their entries -- if a data structure consist of entries of only \textbf{primitive} types (e.g. uint32), it refers to an in-memory descriptor which will be sent to device.
This is similar to on-disk data structures, which must consist of the primitive types.

Currently we directly assume a "chained" descriptor design. 
It might make sense because if it is not "chained", what is the point of having the bus address? 
It could just statically populate the entries instead of introducing a pointer. 
\end{comment}

\subsection{Summarize driver/device interactions}
\label{sec:design:summarize}
%
%\Note{this is to extract higher order information -- loop, wait, etc.}
%
%\Note{merge the following}
We summarize them as an interaction action: one or more adjacent interaction events that may show nondeterminism (meaning types and numbers may vary across runs) but do not change device state. 

The objective is to discover non-deterministic interactions that may nevertheless occur on the beaten path. 
\sys{} summarizes the interactions by generating an envelope for them. 
The replayer acts based the envelope interactions and tolerates any discrepancies that may emerge.

To do so, \sys{} repeats a request on the driver with the \textit{same} environment (memory layout). 
On the traces across multiple runs, it performs \textit{sequence alignment} (\Note{at the XXX boundary, using XXX algorithm}) and matches the following patterns:  

\begin{myenumerate}
	\item 
	\textbf{Register polling. } 
	Commonly seen in most drivers, 
	the driver repeatedly a sequence of register accesses until a register read returns a different value. and The repeated times vary across runs. 
	This is caused by busy wait in a while() loop. 
	\sys{} emits a (read-until) replay action.
		
	\item 
	%\textbf{Driver reads a different value from device.} 
	\textbf{Read different values from the same field.} 
%	Examples include read of a register or a descriptor returns different values across runs. 
	The fields may be dynamic in nature, as described earlier. 
	Prompt the developers to examine the field semantics; developers may annotate to tolerate the value difference at the replay time. 
							
	\item 
	\textbf{Writes of different values.} 
	In addition to parameterized fields discovered, the driver writes to the same register with a different value across runs. 
	Examples include a register that expects a cookie (a random integer) \Note{cite} or a timestamp provided by CPU. 
%	Happens to some command/configuration register. E.g. CMD\_NEW flag might be added when writing to CMD register.
	\sys{} uses backward slice to identify the source code that produces the value, and prompts developers to synthesize the value at replay time. 
		
	\item 
	\textbf{Read/write of different registers.}
	This indicates the driver's control flow diverges across test runs. 
	Based on some of its runtime environments, the driver decides to operate the device in a different way. 
	\sys{} identifies the source location where control flow diverges and prompts the developers to inspect and address the difference in runtime environments. 
	To our experience, this rarely happens. 
\end{myenumerate}

% obsolete 
%observation: 
%1) the pattern \& source of divergence -- driver reads status (feedback) register to decide what to do next;
%the value gives enough information for the most of time.
%\Note{some still need assistance from kernel data structure to pinpoint}
%2) do something pattern: the driver really does something is after the read divergence it writes to register (signaling??).
%
%
%This is the source of divergence. 
%From the code level, different values being \textbf{read} leads to different execution paths (than what's recorded);
%from the 
% 

%\subsection{Replay}






==> record-recycle2.tex <==
% !TeX root = main.tex

\section{Recorder}

\xzlNote{--- Obsolete ---}

As shown in Figure XXX, recording is done in two phases. 
\Note{to revise}

\begin{myitemize}
\item Interface discovery: 
%\sys{} exercises the driver and traces the driver/device interactions. 
\sys{} exercises the full driver in many iterations and varies the recording environments. 
It analyzes the driver/device interactions and incrementally discovers the interfaces. 

\item Recording emission: After the interface is discovered, \sys{} runs the selected requests. 
It summarizes the collected traces as sequences of \textit{replay actions}, each for one request. 
%which are the envelope of nondeterministic interactions. 
\end{myitemize}

\sys{} automates most of this process. It needs developer efforts on confirming the discovered interfaces and annotating a small number of interface fields. 

\subsubsection{Setting up a controlled recording environment}
%\Note{to compress}
%We uses userspace test harness to exercise the full driver of interest in a Linux kernel. 
%We control the test inputs, such as physical address of the input/out data buffers, and their lengths.
We instrument the kernel, the driver's environment to capture full software/hardware interactions:
%To capture full software/hardware interaction, the instrumentation must contain (1) complete register accesses of the device, (2) shared memory allocations in case interactions happen via in-memory descriptors. %distinguishable physical pointers to facilitate differential analysis later, in case kernel allocates same DMA memory address across different runs.
%To this end, we instrument the kernel as follows:
%\Note{compress}
%The instrumentation serves two purposes: 
%(1) it traces register access, which bootstraps the discovery of the remaining interfaces; 
%(2) it randomizes the driver's memory layouts across runs. 
%Later, the recorder does differential analysis over the resultant traces and discovers physical pointers and parameterizable fields. 
%

% We turn off the driver's configurable features, if any, that mismatch our simple driver model. (Section XXX will provide more details).The device hardware configuration must be the same as the replay time. For instance, a single-level USB device topology. 

%\sys{} relies on ``hints'' from kernel and instrument them to infer key information about the driver during recording . They are the following: 
\begin{myitemize}
	\item 
	Tracing register access. 
%	The identified registers will bootstrap the discovery of the remaining interfaces.
	We instrument kernel register accessors (readl/writel). %and functions that map register banks declared in device trees (e.g. ioremap);
	We also trap access to iomem by toggling the read/write bit of their PTEs to ensure no register is left out.
%	The redundancy gives us higher confidence that no register is left out. 
%	We protect the region in order to intercept any access. 
%	The addresses of registers are easy to find: a device's registers are in a contiguous address range; they are clearly defined in source headers; there are extensive kernel tracing facilities to find out register accesses. 
	
		
	\item 
%	Register access \& DMA are the only two ways to control the driver. 
%	Physical pointer to DMA memory always refers to control block/descriptor understandable by the device.
	Locating shared memory regions of CPU and devices, which host in-memory descriptors as a driver/device interface. 
	We instrument DMA APIs (e.g. dma\_alloc\_coherent), kernel's standard methods to allocate device cache-coherent memory. 
	We snapshot the regions right before trigger register writes, i.e. a register write that kicks off an upcoming hardware job and immediately precede an interrupt notifying the job status. 
%	We snapshot them as part of the recording right before writes to trigger registers, i.e. a register write that kicks off the upcoming hardware job. 
	We identify trigger registers in a dry run prior to recording. %as those being written immediately precede interrupts, which are used often as notification of job status.
	
	\item 
	Customize the page allocator for the device. 
	This allows \sys{} to change the driver's memory layouts and DMA allocations across runs. %which is crucial for differential analysis over recordings later. 
	% and discovers physical pointers and parameterizable fields. 	
	The custom allocator serves pages from a pool reserved at boot time at control of \sys{};
	it is as simple as 500 SLoC. 
%	Note that memory efficiency is not a concern, because the replayer does not inherit memory layout at recording time. 
%	will not inherit memory layout from the recording time but allocate memory at its own discretion and 
	
	% ; it allows \sys{} to allocate the same physical memory chunks 
	% \sys{} substitutes the kernel's page allocator. 
	% The new memory allocator creates a large pool of contiguous memory pool at boot time (via Linux CMA) and serves the target driver from the pool in lieu of the stock allocator. 
		
\end{myitemize}

Note that the above instrumentation is done only to a number of generic kernel APIs that are independent of specific drivers. 
It is a one-time effort for a given kernel release. 

%\paragraph{Snapshotting at trigger registers}
%\Note{warm up run}
%After setting up the environment, prior to the very initial recording, the first question \sys{} faces is -- when to snapshot shared memory regions during recording?
%While \sys{} instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
%It does not know \textit{when} drivers fill them with commands, messages, etc.
%Taking their snapshots at arbitrary times results in inconsistent values.
%%E.g. they may be modified by driver at different layers and times.
%
%Our solution is to take snapshots of all of them before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
%Our rationale is simple: the write to trigger register is a handoff point; 
%at the point, the driver must provide the device final information about the hardware job. 
%Finding the trigger register is straightforward: \sys{} runs a test once and identifies register writes that immediately precede interrupts, which are often used to notify job status.
%This heuristics narrows down from tens of registers to 1--2 registers per device.
%Repeated runs can eliminate false positives if any, e.g. register writes by a background thread unrelated that happen to precede an interrupt. 
%Finally, \sys{} prompts the developers to confirm the finding the trigger registers. 
%More details are described later in Section~\ref{sec:case}. 


%\subsection{Record}
\subsubsection{Automatic software/hardware interface discovery}
%\Note{assumption:} read has no side effects; only write change states.
\begin{comment}
\paragraph{Choosing test requests}
Given a driver, \sys{} runs a test suite that issues requests as needed by target trustlets. 
While commodity drivers expose complex request interfaces, e.g. XXXX, 
we pick requests with simple semantics so that each request finishes an atomic task.  
By doing so, we keep each request handler (and the device state transitions within) simple. 
This is analogous to the RISC vs. CISC debate. 
For instance, the requests for MMC storage are read/write of a range of blocks, where the block counts are a set of fixed values (1,4, 16, 128).  
In addition to requests, \sys{} records interaction segments during device initialization and device reset, respectively. 
\end{comment}

%\Note{key idea is to use differential analysis to facilitate automation}
%\Note{objectives of differential analysis on two things:} 1) find in-memory descriptors as encoding may be disguise as a physical pointer, 2) parameterizable fields.
%
%
%The basic idea is to exercise the driver in many runs, take snapshots of the interface, and analyze the snapshots incrementally. 
%\paragraph{Time snapshots by triggering registers}
%The first question is to \textit{time} the snapshots. 
%Taking a snapshot at arbitrary times results in inconsistent values. 
%For instance, an interface field may contain invalid physical pointers to memory regions yet to be allocated. 
%
%Our solution is to take snapshots before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
%Because our driver model limits hardware concurrency, 
%the driver and device interact in a request/response pattern: 
%the driver \st{configures the devices, } prepares a hardware job (e.g. to initiate a USB transaction) and starts the job with a register write (e.g. the USB controller's HCCHAR register); 
%later, the device responds with an interrupt. 
%Note that to execute a request the driver often submits many hardware jobs. 
%Prior to trigger register writes, the interface is guaranteed to be consistent, because the device is not updating the interface (it finishes the prior job) and the driver has done preparing for the next job. 
%%Writes of trigger registers are the moments when driver/device synchronize on in-memory descriptors and the descriptors are guaranteed to be consistent 
%
%To find the trigger registers, \sys{} parses the interaction trace and identifies register writes that immediately precede interrupts. 
%This heuristics narrows down from tens of registers to 1--2 registers per device.
%Repeated runs can eliminate false positives if any, e.g. register writes by a background thread unrelated that happen to precede an interrupt. 
%Finally, \sys{} prompts the developers to confirm the finding the trigger registers. 
%
%(see case study). 
%
%\Note{what about triggering that does not raise an interrupt?}
%\Note{what about asynchronous workqueues?}
%\subsubsection{Differential analaysis.}

We uses userspace test harness of selected requests to exercise the full driver; % of interest in a Linux kernel. 
we control the test inputs, such as physical address of the input/out data buffers, and their lengths.
With the instrumentation set up, each test produces a raw recording, consisting of hundreds of register accesses and KBs of memory dumps.
They are filled with magic values, command encodings, and physical pointers, which hide in-memory descriptors.
%their fields need to be further distilled (e.g. parameterization and annotation).
%How to automatically analyze them to reduce developers efforts as much as possible? 
%\Note{to distill a MVP driver..}
To relieve developers from tedious manual analysis, sys{}'s key insight is through differential analysis: by systematically introducing random changes to memory and test inputs, \sys{} stresses the dynamism in a driver to manifest all dynamic values, only to which developers need attention.\Note{rephrase}

%Specifically, \sys{} looks for the following three possible differences for all interface \textit{fields}, including registers and in-memory descriptors across recordings: 
Our observation is: under controlled test runs, all interface \textit{fields}, including registers and in-memory descriptors manifest in following three categories:
\begin{myenumerate}
	\item 
	Static values (i.e. no difference), e.g. protocol communications, command encoding, device configuration, etc. 
	The values are identical across runs. 
%	They  will be replayed as-is during replay. 
%	No efforts/inputs are needed from developers. 
%	These constitute most of the interface fields. 
	
	\item 
	Dynamic values, e.g. command serial numbers, timestamps, statistic counter, job status, device power states.
	They change across runs but independent of \sys{}.
%	\sys{} flags the fields and related source code, asking developers/replayer to provide logic for handling (or synthesizing) values. 
%	Such fields are rare. 
	
	\item  
	Data-dependent, e.g. data lengths, addresses for input/output buffers, checksum.
	They are concrete values that change with test parameters and data content (i.e. PIO). %(if it's MMC PIO). 
%	These values shall be overridden and parameterized at the replay time. 
%	\sys{} annotate the semantics of the fields (input, output, lengths) and asks confirmation from developers. 
%	Typically there are several such fields per device. 
\end{myenumerate}

Bearing the three categories, \sys{} runs the automated differential analysis as follows.

\paragraph{Find in-memory descriptors}
\input{fig-discovery-example}
\sys{} kicks off differential analysis by finding all in-memory descriptors, the interfaces beyond registers. %for completeness. 
To do so, it runs tests with same arguments repeatedly;
it randomizes device's DMA pool for each run.
%since they are data-dependent (e.g. contain data buffers), \sys{} randomizes device's DMA pool for each run.

\sys{} first looks for any register writes containing physical pointer \textit{value} within the range of our pool.
\sys{} asserts it points to an in-memory descriptor only if the same register writes change values in different runs and the values always belong to our pool, as shown in Figure~\ref{fig:discovery_example}.
This is important to rule out false positives, e.g. magic values/encodings accidentally falls into the range of our pool.
In case the descriptors embeds pointer to another, \sys{} extends the analysis recursively to its memory snapshot -- asserting any physical pointers and following them until no new one is found.
\sys{} has found such a structure for the DMA descriptors of MMC, and will be shown in Section~\ref{sec:case}.

%For the first type of difference, their values are identical across runs, independent of the changes \sys{} introduces. 
%They will be replayed as-is -- register read/write with same value, fields of in-memory descriptors remain the same.  
%These constitute most of the interface fields. 
%For the second type, their values vary across runs, independent of the changes \sys{} introduces.
%\sys{} flags the fields and related source code, asking developers to provide logic for handling (or synthesizing) values.
%Such fields are rare and will be shown in Section~\ref{sec:case}. 
%
%The last type are concrete values that change with \sys{} test input.
%Typically there are several such fields per device. 
%They are important as they contain addresses for in-memory descriptor, input/out buffers and must be overridden/parameterized at replay time.
%\sys{} automatically finds, annotate the semantics of the fields (input, output, lengths), and asks confirmation from developers. 

%\paragraph{Discover software/hardware interfaces}
%After setting up the snapshotting point at trigger registers, \sys{} runs test again to discover interfaces, i.e. registers and in-memory descriptors.%for differential analysis. 
%
%Straightforwardly, from the recording \sys{} discovers all registers used by the driver as hardware/software interfaces.
%%Additionally, the interfaces also rely extensively on in-memory descriptors to pack complex information (e.g. SCSI command, DMA control block). 
%\sys{} discovers in-memory descriptors by looking for any register writes with physical pointers allocated by our custom allocator. 
%Since they themselves may embed pointers pointing another descriptor, \sys{} follows the physical pointers inside first discovered in-memory descriptor until now new one is found.
%\sys{} provides richer information for in-memory descriptors: it associates their physical pointers with DMA instrumentation and reports the sites of their allocation, with which the developer can easily tell their type and fields for annotation.
%\sys{} does backward slicing starting from the site of trigger register writes until it reaches the most recent source line that writes to a field. 
%\sys{} provides evidence for developers to confirm: 
%the source lines that assign the pointer field; 
%the source lines that map the DMA region. 
%\paragraph{Differential analysis on discovered interfaces}
%Then \sys{} runs differential analysis on each discovered interfaces of the recordings. 
%To do so, it runs tests repeatedly;
%for each run, it resets the driver to the clean slate state, randomizes its DMA pool (using our custom allocator), and runs the test with same argument.
%%As a result, each test run produces a recording, which is a sequence of register access (physical address and their read/write values), with a bunch of memory snapshots (with data contents, allocated address, size, etc.) taken at trigger registers as supplements.
%For all interface \textit{fields} collected in the recordings, \sys{} looks for the three possible differences:
%\begin{myenumerate}
%	\item 
%	Static values (i.e. no difference), e.g. protocol communications, command encoding, device configuration, etc. 
%	The values are identical across runs. 
%%	They  will be replayed as-is during replay. 
%%	No efforts/inputs are needed from developers. 
%%	These constitute most of the interface fields. 
%		
%	\item  
%	Data-dependent, e.g. data lengths, addresses for input/output buffers, checksum\Note{not seen yet}.
%%	They are concrete values that change with test parameters, e.g. (addr, size) and data content (if it's MMC PIO). 
%%	These values shall be overridden and parameterized at the replay time. 
%%	\sys{} annotate the semantics of the fields (input, output, lengths) and asks confirmation from developers. 
%%	Typically there are several such fields per device. 
%
%	\item 
%	Dynamic values, e.g. command serial numbers, timestamps, progress, device power states) 
%%	\sys{} flags the fields and related source code, asking developers/replayer to provide logic for handling (or synthesizing) values. 
%%	Such fields are rare. 
%
%\end{myenumerate} 


%\paragraph{Find in-memory descriptors}
%The objective is to identify registers that point to these descriptors and the possible pointers that these descriptors embed to point each other. 
%
%Our idea is to run differential analysis over snapshots across runs. 
%Our observations are: 
%all interface \textit{fields}, including registers or in-memory descriptors, 
%fall into three categories: 
%
%\begin{itemize}
%\item 
%Static values, e.g. protocol communications, command encoding, device configuration, etc. 
%The values are identical across runs. 
%They  will be replayed as-is during replay. 
%No efforts/inputs are needed from developers. 
%These constitute most of the interface fields. 
%
%\item  
%Data-dependent: data lengths, addresses for input/output buffers, checksum
%concrete values that change with test parameters, e.g. (addr, size) and data content (if it's MMC PIO). 
%These values shall be overridden at the replay time. 
%\sys{} annotate the semantics of the fields (input, output, lengths) and asks confirmation from developers. 
%Typically there are several such fields per device. 
%
%\item Dynamic values: (command serial numbers, timestamps, progress, device power states) 
%\sys{} flags the fields and related source code, asking developers/replayer to  provide logic for handling (or synthesizing) values. 
%Such fields are rare. 
%\end{itemize}
%
%\sys{} discovers the interface incrementally. 
%%The recorder starts from the known interface (initially, the set of registers). 
%The recorder maintains a known interface S, which, at the beginning of the discovery phase, includes only the register set. 
%It repeats the following process. 
%
%\begin{itemize}
%\item 
%Reset the driver to the clean slate state. 
% 
%\item 
%% \sys{} mutates physical memory layout. 
%\sys{} introduces random changes to the driver's physical memory allocation. 
%Of all the memory allocations in the test, it changes the location of one region. 
% 
%\item 
%Prior to each write to a trigger register, 
%\sys{} takes a snapshot of S (all the interface fields it knows so far). 
%It compares the snapshot to those snapshots taken at the same trigger register write in previous runs. 
%
%\item 
%\sys{} flags the fields with values that change with the memory layout. 
%It further vets each candidate field with heuristics: 
%does the field value fall in the address range of any allocated memory region? 
%does the absolute change in the field value equal to the change in the buffer addresses?
%does the field value change if the memory layout remains \textit{unchanged}?
%
%\item 
%\sys{} follows a found physical pointer to discover the in-memory descriptor pointed to (S').
%To do so,  
%\sys{} does backward slicing starting from the site of trigger register writes until it reaches the most recent source line that writes to a field. 
%\sys{} provides evidence for developers to confirm: 
%the source lines that assign the pointer field; 
%the source lines that map the DMA region. 
%\sys{} determines the length of S' by checking the size of the struct or the length of the mapped region. 
%
%\item 
%Add the newly discovered in-memory descriptor S' to S: S=S+S'. 
%Repeat the test run which compares the snapshots of the updated S. 
%This is to discover any physical pointers embedded in S'. 
%\end{itemize}
%
%Repeat the runs until no new descriptors are found. 
\paragraph{Find parameterizable fields}
%On the software/hardware interface, the parameterizable fields are data-dependent. 
%That is, addresses and lengths of input/output buffers. 
%Devices will get/put output or input data from these buffers. 
%These fields contain data dependent values. 
%The procedure is similar to the above. 
%Similar to above, the discovery procedure centers on 
%Similar to descriptor discovery, \sys{} discovers the fields for buffer addresses with differential analysis. 
%Similarly, \sys{} discovers the fields for buffer addresses also with differential analysis. 
After locating all interfaces (i.e. registers plus in-memory descriptors), \sys{} conducts another round of differential analysis on all their \textit{fields} to find parameterizable ones, e.g. addresses and lengths of input/output buffers will be parameterized by trustlets' at replay time.
%They are data-dependent and are tested similarly with before.
%\Note{alignment?..}

To discover buffer address fields, \sys{} varies the buffer addresses supplied from the test harness to the driver.
Similar to finding in-memory descriptors, it only asserts those that change with buffer addresses supplied by \sys{}.
%Through differential analysis, \sys{} identifies as candidates interface fields that only change with buffer addresses. 
To validate the findings, \sys{} \textit{taints} the buffers and looks for the taint values at the memory regions pointed by the candidate fields. 
%By doing so, \sys{} can finally determine the fields that point to input/output buffers. 
\sys{} has found the buffers addresses in both register writes and also in in-memory descriptors.

To discover buffer length fields, \sys{} specifies different data lengths in test harness, e.g. 512 vs 4096 bytes, similar to the discovery of buffer address.
In case the length may not be specified by \sys{} but by the device (e.g. a camera notifies the driver of the incoming image size), 
%Under the differential analysis, they will be prompted as `dynamic values' since they change continuously and independently to \sys{}.
\sys{} scans the interface fields (register and shared memory) that precede to the buffer allocation and looks for values that match the allocation size. 
%\sys{} treats the special case and scans the interface fields (register and shared memory) that precede to the buffer allocation and looks for values that match the allocation size. 

%The values of buffer length fields may come from three sources. 
%(1) Specified by device protocols. 
%For instance, the command buffers of USB driver are always 31 bytes if we only record 4 commands. 
%Since the values are fixed, \sys{} will record them obliviously without any discovery. 
%(2) Supplied as a request parameter from trustlets. 
%\sys{} discovers such fields by running requests with different data sizes, e.g. 8 vs 32 sectors. 
%(3) Requested by the device. 
%For instance, a media accelerator (camera?) requests the driver to allocate a buffer as large as an incoming video frame (see Section~\ref{sec:case} for details). 
%To discover it, \sys{} scans the interface snapshots (register and shared memory) that precede to the buffer allocation and looks for values that match the allocation size. 
% Assumption: physical buffer addresses are stored in registers and/or in-memory descriptors. 
% The lengths are stored in similar fashion. However, the values stored may be in different units (e.g. not necessarily bytes but pages, etc)

%While \sys{} discover parameterizeable fields automatically, optionally it prompts the developer for confirmation. 
Along with the above two rounds of analysis, \sys{} hitchhikes the discovery of \textit{static values}, which remain the same in both two rounds and constitute most fields (99\%), and \textit{dynamic values} which change in both two rounds but are rare.
%For static values, \sys{} emits read/write with same values as replay actions.
%It only prompts the developer to annotate dynamic values, which we discuss next.
%Most of them do not change device states (e.g. command serials, timestamps) and can be confirmed to ignore with ease.
%\sys{} treats others which reflect runtime device states (e.g. job status, power states) and may impact device state transitions in the next section.

\begin{comment} % --- useful???----		
\paragraph{Hints on interaction pattern}
There are limited patterns we rely on as hints to align recording sequences. 
\begin{myitemize}
	\item 
	Data sizes must be aligned/identical in the (annotated) data fields (e.g. in register as well as in DMA descriptors) during interactions. 
	There are only three types of data sizes: fixed, user specified, device requested.
	Fixed size: e.g. < 1 sector access to storage will be fixed to 1 sector access.
	User specified: e.g. > 1 sector access to storage. The data size will be as specified by user (w/ round ups).
	Device requested: e.g. sensor data transfer from device to host, which is variable in sizes.
	
	\item 
	Device-specific initialization is done upon kernel driver probing, which is the entry point upon loading the driver module.

	\Note{below seems not needed}
	
	\item 
	Any states are quiescent until triggered.
	I.e. To align values written to register, \sys{} only cares about the most recent write before trigger register.

	\item 
	Read same register consecutively for multiple times suggest a polling.
	Usually are status register.
	May have busy/idle wait in between the reads.
	Final value of the reads is the stationary (converging?) point. 
	\Note{what about write to same register for consecutive multiple times?} The scenario only happens in MMC PIO path		
\end{myitemize}
\end{comment}


\begin{comment}
\Note{--- below obsoleted ---}

\paragraph{Identify dependent devices}. Example: DMA engines. MMC can use both PIO and DMA; w/o knowing the knowledge, developer misses DMA's register accesses;

\paragraph{Timing -- delays}
\textbf{Step 3: annotate in-memory descriptors at bus address.}
The rationale of picking bus addresses for treatment is because that's what devices only recognize;
each bus address is deemed to refer to an in-memory descriptor that needs annotation.
The system then prompts the developers of the descriptor, supplying the developer with the location where it happens. 
The developer then annotates the fields that contain dst, src, addr, and size, which will be symbolized. 
For other fields, the tool simply records as-is (and treat them as static command/configuration).
If a buf address occurs in the fields again, the tool follows the address and iteratively records the descriptor pointed by the address until no buf address left.

An empirical solution to find such data structures is to examine the types of their entries -- if a data structure consist of entries of only \textbf{primitive} types (e.g. uint32), it refers to an in-memory descriptor which will be sent to device.
This is similar to on-disk data structures, which must consist of the primitive types.

Currently we directly assume a "chained" descriptor design. 
It might make sense because if it is not "chained", what is the point of having the bus address? 
It could just statically populate the entries instead of introducing a pointer. 
\end{comment}

\subsubsection{Summarize driver/device interactions}
\label{sec:design:summarize}
\input{fig-polling-example}
\input{tab-replay-actions}
%
%\Note{this is to extract higher order information -- loop, wait, etc.}
%
%\Note{merge the following}
%After former two rounds of differential analysis, \sys{} preserves static values, annotates, and parameterize static, dynamic, and data-dependent respectively. 
%Unfortunately, this is not enough because static recordings may not reflect all non-deterministic interactions due to timing.
To produce a final recording, \sys{} summarizes the driver/device interactions into \textit{replay actions}, as listed in Table~\ref{tab:tab_replay_actions}.

Former two rounds have discovered static and parameterizale fields.
%Summarizing them is intuitive -- 
To summarize static values, \sys{} emits \code{read/write} replay action to replay them as-is.
it emits \code{read/write\_para} to parameterize data-dependent fields and optionally prompts the developer for confirmation. 

%\code{read/write} replays interactions as-is for static values; \code{read/write-para} parameterizes data-dependent fields at runtime.
Dynamic values, and different number of accesses to fields, cannot be captured by above simple replay actions. %show nondeterminism but do not change device state.
E.g. in different runs, reads to SDCMD register show dynamic values but for the same reason of waiting for command completion. 

%We summarize them as an interaction action: one or more adjacent interaction events that may show nondeterminism (meaning types and numbers may vary across runs) but do not change device state. 
%The objective is to discover non-deterministic interactions that may nevertheless occur on the beaten path. 
\sys{} addresses this by summarizing them into an envelope of interactions; 
the replayer acts based the envelope interactions and tolerates any discrepancies that may emerge.
To do so, \sys{} repeats a request on the driver with the \textit{same} memory layout. 
On the traces across multiple runs, it performs \textit{sequence alignment}, using Needleman-Wunsch algorithm~\cite{xx} and matches the following patterns:
\begin{myenumerate}
	\item 
	\textbf{Register polling. } 
	Repeated reads to a sequence of registers until a certain value is read. %and The repeated times vary across runs. 
%	This is caused by busy wait in a while() loop. 
	\sys{} prompts the developer to check source for busy wait in a while() loop. 
	\sys{} emits a \code{read-until} replay action to mimic the polling behavior.
		
	\item 
	%\textbf{Driver reads a different value from device.} 
	\textbf{Same field, different read.} 
%	Examples include read of a register or a descriptor returns different values across runs. 
	The fields may be dynamic in nature (e.g. timestamp), as described earlier. 
	\sys{} prompts the developer to examine the field semantics;
	\sys{} emits a \code{read-tolerate} replay action to tolerate a range of differences (or ignore them) at replay time.
%	developers may annotate to tolerate the value difference at the replay time. 
							
	\item 
	\textbf{Same field, different write.} 
	Besides parameterized fields, the driver writes to the same field with a different value across runs. 
	E.g. a field expects a command serial number provided by CPU. 
%	Happens to some command/configuration register. E.g. CMD\_NEW flag might be added when writing to CMD register.
	\sys{} uses backward slice to identify the source code that produces the value, and prompts developers to synthesize the value at replay time.
	\sys{} emits a \code{write-syn} replay action plus a callback to synthesis function.
		
	
	\item 
	\textbf{Read/write of different fields.}
	This indicates the driver's control flow diverges across test runs. 
%	Based on some of its runtime environments, the driver decides to operate the device in a different way. 
	\sys{} identifies the source location where control flow diverges and prompts the developers to inspect and address the difference in runtime environments. 
	To our experience, this rarely happens. 
\end{myenumerate}

Table~\ref{tab:tab_replay_actions} summarizes all replay actions.
Finally, \sys{} groups these replay actions by request and reply (i.e. interactions in IRQ handler) in order as the final recording. 


% obsolete 
%observation: 
%1) the pattern \& source of divergence -- driver reads status (feedback) register to decide what to do next;
%the value gives enough information for the most of time.
%\Note{some still need assistance from kernel data structure to pinpoint}
%2) do something pattern: the driver really does something is after the read divergence it writes to register (signaling??).
%
%
%This is the source of divergence. 
%From the code level, different values being \textbf{read} leads to different execution paths (than what's recorded);
%from the 
% 

%\subsection{Replay}






==> record-recycle3.tex <==
% !TeX root = main.tex

%\section{\sys{}}
\section{Record}
\label{sec:record}
%\Note{may be useful}
%\Note{thoughts -- device states and state changing events}
%Clearly define some generic device states such as "prepare req", "wait for CMD", and "wait for job compl.", "check job status".
%Based on these clearly defined states, we can systematically map state changing events to these  device states \& state transitions.

%The trustlet IO can be served by replaying a collection of interaction sequences. 
%These sequences can be collected by exercising the full driver with a small set of concrete inputs. 
%and serve the trustlets with the resultant trace library. 

%In this section, we describe the recorder design, which extracts the ``golden'' state transition path by recording the driver/device interactions with a small set of concrete inputs from both user program and kernel.

%\paragraph{Workflow}

\input{


We describe how developers use a recorder, formulate the recording problem,
and present key techniques.
% Next, we formulate the recording problem, discuss key challenges, and present solutions.

\paragraph{How to use}
To generate a \teedriver{}, e.g. for MMC, developers launch a record \textit{campaign}, 
exercising the driver in multiple record runs. 
In each run, the developers supply a different sample input, e.g. $BlkCount=1, RW=0$; 
they pick the inputs to be what their trustlets would actually invoke the  driver with; 
from the run, a recorder program produces an interaction template. 
%a recorder logs raw interaction events, processes them, and produces an \textit{interaction template}. 
As the record campaign produces multiple templates, the recorder reports a cumulative
coverage of the input space, e.g. $0<BlkCount<32, RW=\{0|1\}$. \xzlNote{multi funcs?}
If the developers see a desirable input $X$ uncovered, they do a new record run with input $X$ to extend the input coverage. 
They conclude the campaign upon satisfaction of the coverage. 



%\input{thoughts}

%\input{fig-workflow}


\input{fig-rec-path}

\subsection{Problem formulation}
%\Note{can be greatly compressed}
%It is sufficient to exercise the full driver with a set of concrete inputs, 
%record the induced interaction trace, and replay the traces to satisfy the needs of trustlets. 
%It is sufficient to exercise the full driver with a set of concrete inputs, and serve the trustlets with the resultant trace library. 

%It is sufficient to serve the trustlets with a library of traces, which are recorded by exercising the full driver with a small set of concrete inputs. 

%it is sufficient to record only the driver/device interactions induced by a set of concrete inputs. 

%The basic unit for record/replay is a request.
%An MVP driver supports a set of requests from trustlets. 
%For instance, a request of MMC storage driver reads 1 block. 
%While commodity drivers expose complex request interfaces, e.g. XXXX, 
%Because of the simple semantics, the device state transitions in executing each request are simple. 
%Given a full driver, 
%To derive the MVP driver from a full driver, 
%the trustlet developers define a set of requests;
%to do so, they provide a variety of sample inputs. 
%The principle is their trustlets would invoke the full driver with. 

\begin{comment}
\paragraph{The inputs to a full driver} can be described as a vector of variables, 
e.g. $\langle RW, BlkCount,DMABuf,... \rangle$.
The variables are either from user programs explicitly (e.g. $RW$ as the access type and $BlkCount$ as the requested block count) or the kernel (e.g. $DMABuf$ as the address of a kernel-supplied DMA buffer). % clock sources
%\Note{two dimensions on DMA buffers:} their types and how many instances each type has.
%Of the input vector, 
%some variables are supplied by user programs explicitly, e.g. access type (read/write) and block count (BlkCount). 
%which are supplied by the developers to the test harness. 
%Examples include the access type (RW) and the block count (BlkCount). 
%Others are from the kernel environment, which is often implicit to the programs/developers, e.g. DMA buffer address and clock sources.
%\Note{use DMA memory onward}
%the recorder instruments kernel APIs in order to trace them and override their values when needed. 
%Since the kernel input is often implicit to the trustlets/developers, 
%the recorder instruments kernel APIs in order to trace the kernel input and override its values when needed. 
%Examples include DMA buffer addresses (DMABuf) and clock sources. 

%\textbf{A record campaign} derives a MVP driver\Note{not defined} from a full driver:
%\paragraph{A record campaign} describes the collective recording intentions of the developer, consisting of multiple outstanding record runs. 
%A single record run $F$ explores the single state transition path of a full driver by exercising the full drivers with one concrete input vector $S$. %denoted by $F(S)$.
%$N$ recording campaigns with concrete inputs $\{s_1,...,s_N\}$ form a collection of recordings.
%;in $N$ runs with $N$ concrete inputs $\{s_1,...,s_N\}$, 
%each being an assignment to the input vector $s$. 
% In each run, the recorder exercises the full driver with a concrete input, which is value of the input vector $s$. 
%To exercise the full driver, the record harness feeds it with a set of concrete inputs, a variety of concrete inputs $\{s_1,...,s_n\}$. 
%For each concrete input $s_i$, 
%For a record run, the developers supply values for
%the program input variables in the input vector, e.g. $RW=R,BlkCount=4$.
\paragraph{A record run} exercises a state transition path for the device. 
For the run, the developers set the user program's input variables, e.g. $RW=R,BlkCount=4$;
%The developers pick the values to be what their trustlets would actually invoke the full driver with.
%The system provides coverage summary for the record campaign, e.g. how many blocks are covered by the record campaign? 
%The recorder automatically sets values for the kernel input variables, e.g. $DMABuf=0x42000000$.
%the recorder fills the remaining variables with values from kernel, e.g. $DMABuf=0x42000000$.
the kernel provides the remaining input variables which are traced by the recorder, e.g. $DMABuf=0x42000000$.
%The goal is to control and trace these values for replay. 
%The goal is to explicitly control these variables for replay.
%\Note{Note that during replay run all inputs might be parameterized, based on constraint which we will discuss later.} 
\end{comment}
%the recorder instruments kernel APIs in order to trace them and override their values when needed. 

%The recorder feeds the full driver with concrete input. 
%each is consisting of values for the input variables in $S$. 

\paragraph{Record runs}
A record campaign consists of multiple runs. 
In each record run, a harness program invokes an kernel entry function for completing a trustlet IO request chosen by the developer, e.g. write of multiple blocks or retrieval of an image.  
To complete the request, the kernel function invokes one or multiple functions of the target driver. 
%A record run R(F,S) invokes $F$, an kernel entry function for completing a trustlet IO request, e.g. write of multiple blocks or retrieval of an image.  To complete the request, $F$ invokes one or multiple functions of the target driver. 
For examples, the program may invoke
(1) an existing ``kern\_write'' kernel entry, which invokes ``bcm2835\_request\_submit'' of MMC driver.
or (2) a customized ``image\_capture'' kernel entry, which invokes a series of IOCTLs of VCHIQ ($\sim$20 SLoC).

\paragraph{Interfaces to record}
% Three pairs of input/output pertain to recording. 
The recorder interposes on three interfaces of driver execution. %to log their input/output. % and logs the input/output. 
%\Note{be careful and consistent in using input/output}

%Program/driver: the input to the driver 
%The input S to the entry function $F$ can be represented as a vector of variables, e.g. $\langle RW, BlkCount,DMABuf,... \rangle$. $F$ will return with output to the program. 
%The variables are either from user programs, e.g. the access type ($RW$) and  the requested block count ($BlkCount$); or from the kernel, e.g. the address of a kernel-supplied DMA buffer ($DMABuf$). % clock sources
\begin{myitemize}
\item 
\textit{Program $\leftrightarrow$ driver}: the inputs from a harness program are a list of variables, e.g. $\langle RW, BlkCount,DMABuf,... \rangle$; 
the driver output to the program is an execution result, e.g. completion status. 

%\item 
%\textit{Program $\leftrightarrow$ driver}: the inputs from the harness program can be represented as a vector of variables, e.g. $\langle RW, BlkCount,DMABuf,... \rangle$; 
%the output to the program is the execution result, e.g. completion status. 

\item 
\textit{Driver $\leftrightarrow$ environment}: the driver invokes kernel APIs for allocating shared memory (DMA), generating random numbers and timekeeping. 
Notably for DMA allocation: the driver inputs -- allocation sizes, may be derived from program inputs; 
the kernel outputs are allocated DMA addresses. 
Kernel memory APIs (e.g. kmalloc) are not included because by design devices shall not use memories allocated by them, which may be cache-incoherent.
%Other kernel inputs include random numbers and clock ticks. 
% can be fixed/emulated for record and replay. 
%A notable API is DMA memory allocation: the driver provides allocation sizes and the kernel returns allocated buffers. 
%Other kernel inputs include random numbers and clock ticks. 

\item 
\textit{Driver $\leftrightarrow$ device}: 
the driver reads and writes from/to the device via registers and shared memory. 
It also receives interrupts from the device. 
%the output to the device includes writes to registers and descriptors in shared memory; the inputs from the device include values read from registers and descriptors and interrupt events. 
%the stimuli to the device includes writes to registers and in-memory descriptors; the responses from the device include values read from registers and descriptors and interrupt events. 
\end{myitemize}




% program input/output, driver/device interactions, kernel API calls/outcome. 

%\paragraph{Raw traces from record runs}
%%-- register IOs, DMA memory consumption\Note{discuss}, and interrupts;
%%During a record run, the recorder traces the data flow of concrete input $S$ as well as a sequence of driver/device interaction events $E$. %-- register IOs, DMA memory consumption\Note{discuss}, and interrupts;
%%\Note{XXX -- 1) highlight this is not full driver execution path, 2) fold ``dump shared mem'' into this?}
%%Each event $E$ is a tuple $<t,ev,args>$: $t$ is the timestamp; 
%%$ev$ is the event type, e.g. register read or DMA memory consumption\Note{must define early}; 
%%$args$ are the event arguments, e.g. the value from a register read or DMA memory contents. 
%%A sequence of events $\{E_1, ..., E_n\}$ hence instantiates one concrete state transition path.
%Each event is a tuple $<t,ev,args>$: $t$ is the timestamp; 
%$ev$ is the event type;
%$args$ are the event arguments. 
%Table XXX lists all the raw events. 
%%The recorder will trace: 
%%All register access (including values), device memory updates (including contents), and interrupts (including types). 
%%The recorder also traces device responses $S_{ker}$, which may be state changing events. 
%% The record has no control of the response values. 
%%Examples: register read. 
\Note{motivate template: why not ask developer provide all inputs and replay concrete values? device may give different inputs...Why only a single state transition path -- push to extreme is symdrive. This is our design decision and ``reuse unit'' simple IO function..}
\Note{evaluate developer efforts -- motivate automatic approach and sym execution}
\paragraph{Recording outcome: \template{}s}
%Towards maximizing raw traces' usefulness to replay, 
%We want to generalize reuse the same state transitions as much as possible by parameterizing the input variables of a recording. %produced by concrete ones.
%E.g. we do not want to record "read/write 1 block" for every single block of a disk. 
%Additionally, considering a raw recording run comprises of thousands of events, we must automate raw recording processing.
%We have the following challenges: 
%Towards maximizing raw traces' usefulness to replay, 
%\sys{}'s key constructs are \template{}s. 
%The recorder derives an interaction template from a single record run's raw trace. 
%An interaction template is the generalization of the raw (input/output) log from a single record run. 
%It strikes a balance between simplicity and portability (?) usefulness in replay (?). 
%One one hand, 
%the template consists a straight line of replay actions. 
%If the replayer finishes the replay actions in sequence without errors, the replay run must exercise the same path of device state transition as in the record run, or the ``faithful path''. 
%% it encodes a fixed path of device state transitions -- the same path exercised in the record run, or the ``faithful path''. 
%On the other hand, 
%the template allows dynamic inputs (from program/environment/device) as long as no deviation from the faithful path. 
%A template generalizes the sequence of raw (input/output) events from a single record run. 
%The template specifies an \textit{envelope} for the input/output events in replay\Note{as replay action? seems repetitive to below paragraph}. 
%%The event sequence is almost the same as the logged (with exception, see below), 
%%The event sequence in the template has is almost the same semantics as the logged events (with exception, see below); 
%%The template prescribes a sequence of input/output events with almost the same semantics as the logged raw events (with exception, see below); 
%The template prescribes a sequence of input/output events with the same semantics as the logged raw events; 
%yet, the template's events specify parameterized output and allow dynamic input 
%% yet, their output values are parameterized and they allow dynamic inputs (from program/environment/device) 
%-- to the extent that the device state still remain on the faithful path. 
%%-- as long as the device state does not deviate from the faithful path. 
%\xzlNote{may move to intro}
From a single record run, the recorder distills an interaction template from the raw logs recorded from the three interfaces. 
A template exports a callable interface to the replayer.  
The interface has the same signature as the recording entry function. 
% it accepts a range of viable input values as defined by a predicate C, which is not limited to $S$. 
Underneath its interface, a template consists of a sequence of replay actions. 
To execute a replay action, the replayer initiates one or multiple input/output events resembling those logged during recording, e.g. to write a register or shared memory. % or to poll a register in a loop. 
Table ~\ref{tab:replay_actions} lists all the replay actions. 

An input event V=<I,C> expects an input value V from interface I, e.g. accept a variable from program, get an DMA buffer from the environment, or read a register value from device. 
The value V is optional, e.g. an interrupt event has no value. 
When V is expected, it must satisfy the constraint C, e.g. a register read must match the one recorded.
A constraint violation will be rejected by the replayer as a failure. 
%\Note{order must follow as well}

An output event <I,V> writes a value V to an interface I. 
For instance, write to a descriptor field or set a DMA allocation length to the environment. 
V can be a concrete value or a function of an earlier input value V, i.e. parameterized. 
 
%\xzlNote{maybe discuss how to match the whole seq in replay}
The replayer proceeds with replay actions sequentially.
It verifies if all input events satisfy their constraints;
otherwise it deems the replay incorrect and attempts to re-execute the template.
%It verifying inputs, sending to devices, getting outputs and matching them... Reject if a single mismatch.
\Note{moved from S5}The recorder ships a package of \template{}s, encrypted and signed by the developers.
It is a compressed image...

\input{tab-replay-actions}


%To execute a replay action $<op,args>$, the replayer initiates one or multiple interaction events, e.g. to write a register or to poll a register in a loop. 
%Table XXX lists all the replay actions. 
%A replay action can be parameterized, in which case its arguments $args$ are not concrete but a function of the input $S$. 
%For example ... 

%An \template{} encodes a fixed path of device state transitions -- the same path exercised in the record run, or the ``faithful path''. 
%If a replay run of the template receives input value satisfying the predicate C and reproduces the template's event-change events, the replay run must exercise the path of device state transition and is thus correct. 


\begin{comment} ---- old writing --- -
%each \template{} finishes a fixed path of device state transitions. 
%A trace template for serving a request $R$ captures a bare minimum slice in the device FSM needed to finish the request $R$. 
%an \template{} $T$ is specialized to a request interface $R$: 
An \template{} only captures one path, i.e. a minimum slice of the device state machine needed to finish $R$. 
%finishes a fixed path of device state transitions. 
The path contains no conditional branches. 
Accordingly, the recorder only exercises only one code path in the full driver; 
it eschews from high path coverage and stays away from much cold code where bugs are more likely \xzlNote{cite}. 



%An action may output a value $args$ to the device, e.g. a register write, for which the value can either be concrete or parameterized, i.e. as functions of the request's input $s$. 
%Notably, an action may consume an input value from the device, e.g. an interrupt or read of in-memory descriptors, 
%for which $args$ specify the value transforms and constraints, e.g. acceptable values from a register or descriptor read.




The end result is a \template{}. 
%Under a request interface $R$ is an \textit{\template{}} $T$, 
Generated by the recorder, it is replayed in response to a trustlet's invocation of driver function. 
$T$ is a sequence of parameterized replay actions, which is the actual code the replayer runs.
Table XXX lists all the replay actions. 
Each replay action $<t,op,args>$ incarnates as one or multiple interaction events $E$.   
An action may output a value $args$ to the device, e.g. a register write, for which the value can either be concrete or parameterized, i.e. as functions of the request's input $s$. 
Notably, an action may consume an input value from the device, e.g. an interrupt or read of in-memory descriptors, 
for which $args$ specify the value transforms and constraints, e.g. acceptable values from a register or descriptor read.




\Template{}s strike a balance between simplicity and usefulness. 
A template exports the same callable interface as the driver entry function $F$. 
%a trace template imposes minimum constraints on its parameter values and interaction events, 
%an \template{} accepts wide ranges of parameter values and allows a family of alternative interaction sequences, 
an \template{} accepts as many input values as possible and allows as many alternative interaction sequences as possible -- 
as long as the device state transitions stay on the golden path. 
%a trace template minimizes the constraints on its parameter values and interaction events. 

An \template{} $T_i$ therefore generalizes beyond the concrete input $s_i$ and the exact interaction sequence in the record run. 





On one hand, 
%each \template{} finishes a fixed path of device state transitions. 
%A trace template for serving a request $R$ captures a bare minimum slice in the device FSM needed to finish the request $R$. 
an \template{} $T$ is specialized to a request interface $R$: 
it only captures the golden path, i.e. a minimum slice of the device state machine needed to finish $R$. 
%finishes a fixed path of device state transitions. 
The path contains no conditional branches. 
Accordingly, the recorder only exercises only one code path in the full driver; 
it eschews from high path coverage and stays away from much cold code where bugs are more likely \xzlNote{cite}. 
%The path is known ``golden'', i.e. to finish the request by the full driver correctly. 
%The simplicity results in ease of record/replay and validation. 
%To produce a \template{}, 
%the recorder only exercises only one code path in the full driver; 
%it eschews from high patch coverage and stays away from cold code where bugs are more likely \xzlNote{cite}. 
%The template and the replayer are easy to validate and recover via re-execution.  
%\paragraph{Parameterized input values}
%\paragraph{Generalizing (Parameterizing?) inputs and interactions}
%On the golden path of state transitions, 
%A trace template to the maximum extent permitted by the 
%Without deviating from the golden path of state transitions, 
%a trace template minimizes the constraints on its parameter values and interaction events. 



For a concrete input $s_i$, the recorder exercises the full driver and produces a request interface $R_i$ callable to the trustlets. %which the trustlets can invoke at run time; 
%the input values viable to $R_i$ not only include $s_i$ but also a range of other values. 
the input values to $R_i$ are not limited to $s_i$ but a range of viable values. 
%$R_i$ not only accepts $s_i$ as its input value but also a range of other viable values. 
%the concrete inputs that acceptable to 
%the set of input 
%the acceptable input values to $R_i$ is a superset of $s_i$. 





%we want to be able to replay it with a wider range of input values, not limited to the concrete value used in recording. 
%E.g. we do not want to record "read/write 1 block" for every single block of a disk. 
%Additionally, considering a raw recording run comprises of thousands of events, we must automate raw recording processing.
%We have the following challenges: 


%\paragraph{Raw recording outcome}
%As the outcome of a record run $F(s')$, 
%the recorder produces a request interface $R = (S, C)$ callable to the trustlets, where $S$ is the input vector and $C$ is a constraint on $S$\Note{need to motivate C}.
%%Similar to the full driver, the request interface accepts a vector of input variables; 
%%The request interface $R_i$ accepts the same input variables as the full driver. 
%%$R_i$ accepts the same input variables as the full driver. 
%%The input values acceptable to $R_i$ include, but not limited to, the concrete input $s_i$ used in recording; 
%$S$ include, but are not limited to, the concrete input $s'$ used in recording. 
%Additionally, variables of $S$ are parameterizable under the constraint $C$.
%\Note{what about kernel inputs}
%which is conjunction $\wedge$ of transfer functions on the data flow of $S$;
%$R$ applies to $S$ during replay. %the set of acceptable input values.
%\Note{1) catalog of interaction events, 2) what about input vectors have implicit transfer functions but have constraints. e.g. DMA address allocated by kernel is by default always page aligned} 

%The input values to $R_i$ are not limited to $s_i$ but a range of viable values. 
\end{comment} 

\begin{comment} % - not here? 
\paragraph{Execution model}
%Each register access site: source line information; callstack trace. 
% All requests are initiated from the CPU side, either by trustlets or a periodic timer. 
% The device cannot initiate requests to the driver. 
%A handler is atomic.
%To execute it, the TEE driver always starts from the clean-slate state and returns to the state. 
%A TEE driver only handles one request from trustlets at a time. % and hence does not execute handlers concurrently. 
%An MVP driver comprises a collection of request handlers. 
%A collection of trace templates constitute an MVP driver. 
%The recorder extracts a small subset of a full driver's behaviors to be an MVP driver. 
%An MVP driver implements a small subset of a full driver's behaviors. 
Compared to the full driver, 
an MVP driver constrains the device state space and therefore 
prevents many potential state divergences. 

%An MVP driver limits concurrency and eliminates the entailed nondeterminism. 
%the driver only executes one handler at a time and 
%a handler submits one hardware job to the device at a time. 
The MVP driver limits hardware concurrency: 
it serializes concurrent request invocations; 
each request execution serializes its hardware jobs. 
%To avoid state divergence resulted from hardware concurrency,  
% at one given moment, the driver submits at most one outstanding request to the device. 
%\textit{Reset to the clean slate.}
%To further constrain state transitions,
The MVP driver frequently resets the device. 
%to partition the device state space and to recover from replay failures. 
Prior to servicing each request, the driver does a soft reset (via trace replaying), bringing the device back to a clean-slate state -- as if the device just finishes initialization in the boot up process. 
%Upon boot up, the driver executes an initialization handler and reaches a clean slate state where the device is idle and ready for the next request. 

%The MVP driver uses device as for fault tolerance 
The MVP driver relies on device reset to recover from replay failures. 
Once the driver detects a divergence at any moment in trace replay (i.e. mismatched state-changing events), 
it resets the device to the clean-slate state and re-executes the request. 
By construction, each request execution is idempotent. 
Failed execution attempts have no side effect on the eventual execution success. 

Section XXX will evaluate the efficacy of device reset and its performance overhead.
%The resets incur performance overhead, which we will evaluate in Section XXX. 
%As we will show in Section XXX, re-execution is adequate to work around most of the state divergences which are transient. 


% the replayer simply soft-resets the device to the clean-slate state and re-executes the handler. 
% While the driver/device may still interact in a non-deterministic fashion, our system learns the \textit{envelop} of the interactions and emits simple logic (code) to accommodate the non determinism. 
% The replayer the driver simply soft-resets the device, bring it back to the clean-slate state, and re-executes the handler. 


% Ex: MMC: loss of medium/card (removal), device bus errors (so that message CRC is wrong); bus timeout (takes too long to response? device power errors? )
% Section XXX also studies fatal divergences (albeit rare) that cannot be handled in this way. 


%\paragraph{Request-driven executions}
%\paragraph{Request-response executions}
% \textit{Atomic handlers}
%\textit{Transactional handlers}
%\textit{Request handlers.}
%\textit{Trace template}
\end{comment}

%\paragraph{\Template{}s}
%Under the hood of each request $R_i$ is an \textit{\template{}} generated by the recorder.  

%To back each request $R_i$, the recorder generates an \textit{\template{}}, 
%which is to be replayed in response to a trustlet's invocation of the request $R_i$. 

%\paragraph{\Template{}s}
%Under a request interface $R$ is an \textit{\template{}} $T$, 
%which is generated by the recorder and to be replayed in response to a trustlet's invocation of $R$. 
%$T$ is a sequence of parameterized replay actions, which is the actual code the replayer runs. 
%Table XXX lists all the replay actions. 
%Each replay action $<t,op,args>$ incarnates as one or multiple interaction events $E$.   
%%An action may output a value $args$ to the device, e.g. a register write, for which the value can either be concrete or parameterized, i.e. as functions of the request's input $s$. 
%Notably, an action may consume an input value from the device, e.g. an interrupt or read of in-memory descriptors, 
%for which $args$ specify the value constraints, e.g. acceptable values from a register or descriptor read. 

%The \template{} accepts an input vector and runs a sequence of replay actions: 
%% \Note{segmented by CPU \& IRQ contexts at recording time...} 
%register accesses; loads of memory snapshots; delays; 
%depositing/extracting output or input at specified memory locations. 
%The replay actions are parameterized, 
%i.e. their arguments, such as the value written to a register, are expressed as functions of the input vector. 

\begin{comment}
The recorder produces an \template{}: 
(1) A vector variable as the input; 
%as a subset of all the inputs ($s \in s'$) on which interaction events have value dependencies.
(2) A constraint C on the input vector, defining a family of acceptable input values
%The constraints extends the input from the point value $s$ used in recording.  
(3) A sequence of parameterized replay actions. \xzlNote{merge}
The \template{} accepts an input vector and runs a sequence of replay actions: 
% \Note{segmented by CPU \& IRQ contexts at recording time...} 
register accesses; loads of memory snapshots; delays; 
depositing/extracting output or input at specified memory locations. 
The replay actions are parameterized, 
i.e. their arguments, such as the value written to a register, are expressed as functions of the input vector. 
Table XXX lists the replay actions. 
\end{comment}

%a balance between input-specific optimization and usefulness (? generality). 
%specializing device state transitions (the source of driver complexity) while allowing generality in input values. 
%Trace templates strike a balance between specializing device state transitions (the source of driver complexity) and parameterized inputs. % generality. 
%\Template{}s strike a balance between code specialization and input generalization. 
%An \template{} follows a key principle: 
%it captures the golden path of device state transitions while generalizing to any inputs that share the path. 

%\Note{compress}
%\Template{}s strike a balance between simplicity and usefulness. 
%%\paragraph{Specialized device state transitions}
%On one hand, 
%%each \template{} finishes a fixed path of device state transitions. 
%%A trace template for serving a request $R$ captures a bare minimum slice in the device FSM needed to finish the request $R$. 
%an \template{} $T$ is specialized to a request interface $R$: 
%it only captures the golden path, i.e. a minimum slice of the device state machine needed to finish $R$. 
%%finishes a fixed path of device state transitions. 
%The path contains no conditional branches. 
%Accordingly, the recorder only exercises only one code path in the full driver; 
%it eschews from high path coverage and stays away from much cold code where bugs are more likely \xzlNote{cite}. 
%%The path is known ``golden'', i.e. to finish the request by the full driver correctly. 
%%The simplicity results in ease of record/replay and validation. 
%%To produce a \template{}, 
%%the recorder only exercises only one code path in the full driver; 
%%it eschews from high patch coverage and stays away from cold code where bugs are more likely \xzlNote{cite}. 
%%The template and the replayer are easy to validate and recover via re-execution.  
%
%%\paragraph{Parameterized input values}
%%\paragraph{Generalizing (Parameterizing?) inputs and interactions}
%%On the golden path of state transitions, 
%%A trace template to the maximum extent permitted by the 
%%Without deviating from the golden path of state transitions, 
%%a trace template minimizes the constraints on its parameter values and interaction events. 
%On the other hand, 
%%a trace template imposes minimum constraints on its parameter values and interaction events, 
%%an \template{} accepts wide ranges of parameter values and allows a family of alternative interaction sequences, 
%an \template{} accepts as many input values as possible and allows as many alternative interaction sequences as possible -- 
%as long as the device state transitions stay on the golden path. 
%%a trace template minimizes the constraints on its parameter values and interaction events. 
%%Replay of the template accepts \textit{a wide range} of input parameters and allows a family of alternative interaction sequences. 
%An \template{} $T_i$ therefore generalizes beyond the concrete input $s_i$ and the exact interaction sequence in the record run. 
%
%\paragraph{Example} A request can be write MMC blocks, where $s_{app}$ includes the buffer address and the block count (with constraint $<10$); 
%$s_{ker}$ is a series of DMA buffer addresses needed by the request execution. 
%Examples include reading one block from an MMC storage and capturing an image at some resolution. 


%Each request is to finish a simple IO task needed by trustlets, for which the CPU submits one or several hardware jobs to the device for execution. 


\begin{comment} --- %useful?-----
% \paragraph{Debugging information}
% \paragraph{Mapping execution to the full driver}
%\paragraph{Holding the full driver accountable}
%\textit{Interpretable replay}
%\textit{Mapping interaction events to the full driver}
\textit{Accountable interactions}
%The TEE driver ensures accountability for its replay. 
%The recorder emits debugging information to accompany driver/device interactions. 
The recorder maps each replay action to a context in the full driver execution where the action was recorded. 
The information includes 
the source code location and a callstack trace. 
%  the source line and the callstack trace in the full driver. 
%The replayer hence associates every interaction it replays with a source location and a callstack trace in the full driver. 
This associates a sequence of interaction events to an execution path of the full driver. 
To debug any replay bugs, developers just reason about the corresponding full driver execution. 
\end{comment}

%For instance, 
%in case any action triggers device state divergence, the developers can always  pinpoint a location and a context in the full driver, allowing them to reason about any replay issues just reason about the full driver execution. 

%Limit driver dynamism. Use or configure driver for deterministic interactions.


\subsection{Key challenges \& solutions}
\Note{symbols vs concrete values -- cleanly emit them in templates}
%\paragraph{Problem definition}
%The recorder generates an \template{} $T(R)$ for a given request $R$: 
%We address three challenges:

\begin{comment}
The recorder feeds the full driver with concrete input $s=\langle s_{app}, s_{ker} \rangle$.  
%The full driver and the underlying device accepts inputs from two sources.
%The input comes from two sources. 
$S_{app}$ is the program input, for which developers supply concrete values intended to be used by trustlets.
Examples include data (address) and buffer length. 
$S_{ker}$ is the kernel input. 
It is often implicit to the trustlets/developers. 
The recorder instruments kernel APIs in order to records $S_{ker}$ and override its values when needed. 
Examples: clock sources, prngs, DMA buffer addresses. 

\paragraph{Our goal} 
We want to reuse the same state transitions as much as possible by parameterizing the input variables of a recording. %produced by concrete ones.
E.g. we do not want to record "read/write 1 block" for every single block of a disk. 
Additionally, considering a raw recording run comprises of thousands of events, we must automate raw recording processing.
We have the following challenges: 
\end{comment}

%We next discuss key techniques for automatically generating \template{}s. 
%\sys{} retrofits a few known software analysis techniques to automatically generate \template{}s. 
We next discuss automatic generation of \template{}s, for which \sys{} retrofits a suite of known software analysis techniques. 

%\paragraph{Challenge I: How to parameterize inputs\st{replay actions}?}
The key design of templates{} is to handle input variation:
a replay run receiving input values different from the record run. On the three interfaces: 
(1) from programs: 
a template allows trustlets to supply dynamic input values; 
%trustlets may supply dynamic input values, which a template allows by design; 
(2) from the environment: results from kernel APIs invocation may vary. For example, DMA memory allocator may return different addresses at its discretion; 
(3) from the device: values read from registers or descriptor fields may be  time-dependent or data-dependent which can be nondeterministic.
For example, a register shows a device's internal FIFO watermark; 
a descriptor field shows the length of an upcoming data frame. 

%The replayer handles the input value variation as dictated by templates. 


\input{fig-exec-path}
\paragraph{How to identify constraints of input events?}
%The recorder includes in a template constraints which reject input values that will deviate the device state from the faithful path of transitions.
%\Note{check use of predicates}
%\Note{clarify the relationships between constraints and device state divergence to motivate constraints}: predicates of state changing events which driver assess.
Constraints to a template are what lanes to a vehicle, which keep device state transitions in check: input values failing to satisfy their constraints lead to device state divergences, hence will be rejected by the replayer.
%A template includes such constraints, so it rejects any input values that lead to device state divergences. 

%For example, when the input $BlkCount$ exceeds 65536, the device will fail the transmission because its internal FIFO will overflow. 
An obvious constraint is of an input event from \textit{driver $\leftrightarrow$ device} interface, e.g. read from a command status register;
the template specifies a constraint that only accepts an input value exactly as logged. 
%An obvious constraint are state-changing events from device, e.g. read from a command status register. 
%\Note{state changing events as input from device}
%The template specifies a constraint that only accepts an input value exactly as logged. 
Other constraints are more subtle. 
While variation in an input value itself does not indicate device state changes, the value may impact the driver execution and hence state-changing output to the device. 
For instance, the driver reads a FIFO statistics register (time-dependent input value, not corresponding to device state); 
finding the watermark too high, the driver writes to a configuration register to tune the device bus bandwidth (changing the device state). 

%For instance, the driver submits a different \xzlNote{what} command to device when it finds the device's FIFO watermark too high. 

To identify such constraints, 
our solution is to explore the driver's multiple executing paths and assess if they lead to different device state transitions, as shown in Figure~\ref{fig:exec-path}.
To do so, the recorder uses concolic execution \xzlNote{cite}
%As the driver executes with a concrete input $S$ and encounters a conditional branch pertaining $S$, the recorder makes the driver continue on both executing paths (one is \textit{actual} and one is alternative) 
%and compare their subsequent device state transitions. 
As the driver executes with a concrete input $S$ and encounters a conditional branch pertaining $S$, the recorder forks the driver execution, explores both (one is associated with $S$ and the other is alternative), 
and compares their subsequent device state transitions. 
%to see if their device state transitions may diverge in the future. 
%Throughout the execution, the recorder collects all conditional predicates that the input must satisfy to avoid device state divergence from the concrete path. 
Throughout the execution, the recorder collects the conjunction of path conditions that lead to the same sequence of state-changing events, which serve as the constraints the input events must satisfy to stay on the same device state transition path. 
%prevent the device state from deviating from the actual transitions. 
\sect{design:replay} will present implementation details. 


\paragraph{How to parameterize output events?}
% We avoid such device state divergence in replay by only accepting device response values satisfying certain constraints. 
% The replayer accommodates value variation that do not alternate the device state. 
%Input values satisfying the constraints will not alternate the device state. 
%For them, 
Along the faithful path of device state transitions, 
the recorder discovers the \textit{data dependency} between inputs and outputs across the three interfaces.
% and accordingly parameterizes output values in templates. 
%The data dependencies exist across the three interfaces. 
Notable examples include the following. 
(1) Output to device depends on input from program. % device?
For example, a MMC driver aligns the block address input variable by shifting it right then left by 3 bits, and writes the result to a SDARG register; 
%For example, depending on RW, a MMC driver shifts the XXX input by XXX and writes the remaining XXX bits to a register XXX; 
(2) Output to device depends on input from kernel, e.g. a driver writes the DMA address returned by kernel API to a device register. 
(3) Output to kernel depends on input from program, e.g. memory allocation size depends on the number of requested blocks by program. 
(4) Output to kernel depends on input from device, e.g. the driver allocates a DMA buffer of the same size as the incoming data frame. 

%\xzlNote{Liwei: check the lingo used in prior taint tracking / sym exec work; update the writing below}
The recorder discovers data dependencies with dynamic taint tracking: tainting all input variables, propagating the taints in driver execution and accumulating operations on the taint value until the taints reach sink (i.e. output to an interface).
The recorder emits the output value as the input symbol with the accumulated operations. 
%All existing DTA techniques propagate taint labels from the taint source to the sinks during the target program’s execution based on a set of rules for every executed statement. The final taint results are computed by propagating and composing the individual per-statement taint rules together


% The recorder encodes such value dependency in replay actions. 

%The key is to track how input variables flow into the $args$ of the driver/device interaction events $E$. 
%%replay action. % 
%To do so, the recorder retrofits the well-known taint tracking technique. 
%It taints the input variables;
%it not only tracks its whereabouts but also propagates any transformation of the variables (e.g. the value is right shifted XX bits) to the $args$ of interaction event.
%The transformation includes the alignment of addresses which an device often expects.


%After the full driver, input variables are encoded inside a register value or a field of in-memory descriptor captured by $E$.
%The value may not always be of a word size (i.e. 32bit);
%it could be encoded in bit fields. 
%%How to map $S$ to $args$ in $E$?
%For example, in Figure~\ref{fig:code} a full driver takes the block address from user program as an input variable and passes it to the device via RegBufAddr register, while the command is only XXX-bit of the value passed to RegCmd register. 
%%and writes to an in-memory descriptor. 
%
%\textbf{Solution: taint tracking.}
%The key is to track how input variables flow into the $args$ of the driver/device interaction events $E$. 
%%replay action. % and encode the dependency in the replay actions. 
%To do so, the recorder retrofits the well-known taint tracking technique. 
%It taints the input variables;
%it not only tracks its whereabouts but also propagates any transformation of the variables (e.g. the value is right shifted XX bits) to the $args$ of interaction event.
%The transformation includes the alignment of addresses which an device often expects.



% --- Liwei's -----
%Even if the recorder knows which fields of an $arg$ in an interaction event $E$ to parameterize, it is not free to parameterize however it wants.
%This is because the replay must also stay on the same state transition path, after supplying the new concrete values to input variables.
%An example is a device often sets a largest data transmission length due to the hardware limits on its internal FIFO size.
%Failing to do so might cause the device to reject data transmission, leading to divergent path.
%Solutions: constrain and elimination.  
%Driver input: constrain the input to only the recorded concrete state transitions; kernel env: reproduce with high fidelity; 
%Device input: detect and bail out (only deal with polling loops) 

%\textbf{Solution: concolic execution.}
%The key is to discover each conditional predicate an input vector depends on, since they induce device state transitions.  
%%The collective conditional predicates (of code) are guaranteed to belong to one state transition path (of device). 
%As long as the conditional predicates are respected by new concrete values during replay, the execution path is the same, hence the state transition path.
%Note the execution path belongs to the set of execution paths of a state transition path.\Note{reword}
%
%To do so, \sys{} runs concolic execution, a well-known software testing technique.
%With each execution path explored by a concrete input vector, \sys{} collects the encountered conditional predicates pertaining to an input variable.
%Collectively the predicates form a constraint on an input vector.
%During replay, \sys{} evaluates the input vector against the constraint;
%only when the predicates for each input variable is satisfied will the input vector be accepted. 
%The evaluation is streamlined and fast since \sys{} does not generate general inputs by solving the satisfiability problem.
%it finds out the constraints on the symbol values that will keep the state transitions under the concrete input $s$ unchanged. 
%it finds out the constraints on the symbols that will keep the state transitions the same as the state transitions induced by the concrete input value. 
%\Note{The key} of using sym exec is to finds out the def-use of events and inputs.
%E.g. ``does read(RegA)=128 affect the state transitions?''  

%\sys{} constrains the input values to allow only the golden path of state transitions. 
%For uncontrollable inputs $S_{dev}$ we detect tolerable range ...
%the input values may alter the sequence of interactions and then device state transitions. 

%Examples: 
%when the block number exceeds a page, the driver will schedules more than one DMA transactions \Note{improve }.
%
%\Note{a subtle assumption we have is:} as long as replay follows the same constraint, the device shall go through the same state transitions.

%\Note{A constraint also specifies what can be parameterized -- } only if no state changing events depend on it.  

\paragraph{How to record in-memory descriptors?}
%The driver/device interfaces not only include fixed registers but a set of descriptors, which the driver dynamically allocates in the shared memory. 
%Examples include ... 
%% To record interactions, the recorder must dump these descriptors. 
%These descriptors must be dumped in record and reconstructed in replay.
As described in Section~\ref{sec:bkgnd:model}, 
the driver $\leftrightarrow$ device interfaces include descriptors which the driver dynamically allocates in the shared memory. 
These descriptors must be dumped in record and reconstructed in replay.
While the driver often determines the number of descriptors based on the driver input, 
% it is difficult for a template to support a varying number of descriptors. 
% to parameterize a collection of descriptors. 
% it is difficult to parameterize a collection of descriptors, 
% i.e. making one template capable of creating a varying number of descriptors. 
%it is difficult to make one template capable of creating a varying number of descriptors. 
%it is difficult to make one template capable of creating a varying number of descriptors. 
%it is difficult to parameterize a collection of descriptors, i.e. encoding in one template how to create a varying number of descriptors. 
it is difficult to parameterize the number of descriptors.
%\Note{to compress}
This is because the driver, per the device protocol, often links descriptors as pointer-based structures such as lists or arrays of lists; 
it may further optimize the structures based on the number of descriptors. 
For instance, for every eight sectors of a request an MMC driver allocates a page and associates a descriptor with the page;
it links them via a physical pointer field in the descriptor and writes the address of the head to DMA register. %... runs a sophisticated function $BlkCount$ ... to coalesce and optimize ... the structure layout. 
%Even if the recorder exploits some drive-specific heuristics to extract such logic, e.g. to create a list of $N$ descriptors, 
%the resultant template is likely brittle. 
While it may be possible to extract the logic with some drive-specific heuristics, such heuristics is likely brittle; 
both the recorder and the replayer will be more complex in order to encode and interpret the logic. 

%It is difficult for the recorder to discover and then encode such rich driver logic in a template, e.g. to create a list of $N$ descriptors. 

%To this end, we mandate that one template only allows a fixed number of in-memory descriptors, which ensures 
%To this end, one template must allocate the same number of in-memory descriptors as , which ensures 
%To this end, we mandate that a replay run must allocate the same number of in-memory descriptors as the record run, safely reusing the topology of descriptors as recorded.
%To this end, 
For simplicity,
we mandate that a template must allocate the same number of in-memory descriptors as the record run, allowing safe reuse of the descriptor topology as recorded.
% ensuring an identical topology of descriptors. 
% To give the replayer freedom in allocating memory for the descriptors,
To ensure that the replayer can allocate descriptors at memory addresses of its choice, 
the recorder taints the allocation addresses of individual descriptors and tracks its sink to discover the pointer fields embedded in descriptors. 
%In a replay run, the replayer can reconstruct the data structure of descriptors by reproducing the descriptor allocations, loading memory dumps of descriptors, and rewriting the address fields. 
As such, the replayer can reconstruct the topology of descriptors by loading the dumps of shared memory and rewriting the pointer fields. 

%\paragraph{How to tolerate nondeterministic polling loops? }
\paragraph{How to record polling loops? }
The other major source of nondeterminism is polling loops. 
For example, a driver waits for a previous command to finish by polling a command status register; 
the number of register reads is often nondeterministic, as it depends on the timing of command execution.
While conceptually simple, 
a polling loop is known difficult to dynamic code analysis, 
as it many generate many, sometimes infinite, alternative executing paths. \xzlNote{cite} 
To explore all paths looking for device state divergence is simply expensive. 

Fortunately for us, the polling loops in driver/device interfaces are often succinct, local, and have clear a code structure.
For example, the Rpi3 MMC driver implements polling loops by either using standard kernel register polling function (e.g. readl\_poll\_timeout) or a short while loop (<10 SLoC).
Our solution is to lift loops as a replay action, which conducts the same, simple operation of original loops -- waiting for a bit to flip or a value to be reached.
% the alternative interaction sequences. 
With static code analysis,
we find the loops and lift each loop as a standalone replay action, which allows for a varying number of register reads in replay.
\xzlNote{cite Dr Loop}. 

% ---- old ---- 
%\paragraph{How to tolerate nondeterministic device response? }
%Not all device responses correspond to device state changes. 
%Some device responses can be nondeterministic; 
%even in a faithful replay they commonly differ from what were recorded. 
%
%One major source of nondeterminism is values from registers or descriptor fields that are time-dependent or data-dependent.
%%Examples include a device's performance counter and the length of an incoming data frame. 
%%Examples include a device's performance counter or internal FIFO length, of which the values depend on the read timing. 
%For example, a register shows a device's internal FIFO watermark; 
%a descriptor field shows the length of an upcoming data frame. 
%
%While the variation in value itself does not indicate changes in device state, it may impact the driver execution and hence subsequent device/driver interactions in two ways. 
%%(1) Causal dependency. 
%(1) Device state divergence. 
%% For instance, the driver submits a different command to device based on a predicate of the register value. 
%For instance, the driver submits a different \xzlNote{what} command to device when it finds the device's FIFO watermark too high. 
%We avoid such device state divergence in replay by only accepting device response values satisfying certain constraints. 
%(2) Value dependency. 
%For instance, the driver allocates a DMA buffer of the same size as the incoming data frame, and writes the buffer address to a device register. 
%Therefore, we parameterize subsequent replay actions against the device response. 
%
%
%% To tolerate the value variation in replay, 
%% Our solution is to prevent device state divergence by only allowing register values under certain constraints and to encode value dependency by parameterizing subsequent replay actions. 
%
%We use the same technique as the one for driver inputs.  
%%the recorder uses concolic execution to find out constraints that the response value must satisfy in order to avoid device state divergence; 
%The recorder uses concolic execution to extract from the kernel execution any predicate that the read value must satisfy to avoid device state divergence in subsequent interactions. 
%It taints and propagates the response value to subsequent interaction events. 
%
%
%The other major source of nondeterminism is polling loops. 
%For example, a driver waits for a previous command to finish by polling a command status register, where the number of register reads depends on the timing of command execution.
%Our solution is to derive \textit{behavior envelopes} for loops. 
%% the alternative interaction sequences. 
%With static code analysis,
%we lift each loop as a standalone replay action, 
%which may take a varying number of iterations in replay.
%\xzlNote{cite Dr Loop}. 



%------------- old writing ------------------

%\paragraph{How to tolerate alternative interaction sequences? }
%Since not all interaction events correspond to device state changes, 
%a replay run's interaction events may differ from what were recorded -- even when if replay is faithful. 
%The difference can even be nondeterministic across runs. 
%For example, a driver waits for a previous command to finish by polling a command status register, where the number of register reads depends on the timing of command execution.
%
%Our solution is to derive \textit{behavior envelopes} for the alternative interaction sequences. 
%We identify two major sources: 
%(1) Polling loops, which are the dominant causes of alternative interactions (accounts for XXX\%). 
%We lift each loop as a standalone replay action with static code analysis \xzlNote{cite Dr Loop}. 
%(2) Read from statistical registers. 
%Examples include a device's performance counter or internal FIFO length, of which the values depend on the read timing. 
%% Read from Input from the device for statistic purpose. 
%%Values read from from statistics registers. 
%%For example, the driver reads the timestamp for timekeeping purposes. 
%The recorder uses concolic execution to extract from the kernel execution any predicate that the read value must satisfy to avoid device state divergence in subsequent interactions. 

%Even in a successful replay run,
%the interaction sequences often deviate from that in the record run. 
%For example, a driver waits for previous command to finish by polling a command status register, which may differ across different replay runs. 
%Most such discrepancies do not imply replay failures because they are not caused by device state divergences. 

%\textbf{Solution: static code analysis.}
%Our key insight is to generate replay actions that can tolerate alternative interaction sequences, as they are caused by two major sources: 
%(1) polling loops, the dominant causes of benign interaction discrepancies (accounts for XXX\%). 
%%For example, a driver polls a status register until the current hardware job finishes. 
%The number of polling depends on the timing of job execution. 
%%A loop terminates depending on a device input and executes 
%%While the number of iterations varies across runs, the loop does not deviate device state transitions. 
%Our experience is the polling is simplistic -- often just under a while. 
%The driver instruments all such loops and lift each loop to a replay action. 
%%(e.g. indicating the device becomes idle), 
%%where the number of register reads varies across runs; 
%(2) Statistics input from the device. 
%%Values read from from statistics registers. 
%For example, the driver reads the timestamp for timekeeping purposes. 
%%where the read value depends on the exactly when the read is attempted. 
%%It addresses two major causes. 
%%(1) a driver polls a ``device idle'' register bit until it flips,
%
%%Examples include a register showing the hardware FIFO length. 
%%The replayer should tolerate such benign discrepancies. 
%%To do so, the recorder extracts the envelope of all interaction sequences that correspond to the golden path of device state transitions. 
%%It instruments the code of polling loops and lift them.
%The driver runs def-use analysis to identify such interaction events that neither change device states nor the subsequent interactions. 
%Their values will hence be ignored in the replay action.


%\paragraph{Example} A request can be write MMC blocks, where $s_{app}$ includes the buffer address and the block count (with constraint $<10$); 
%$s_{ker}$ is a series of DMA buffer addresses needed by the request execution. 
%Examples include reading one block from an MMC storage and capturing an image at some resolution. 




%The family extends the concrete input 
%A (allowable? acceptable) family of input S as the extension of the concrete input ($s \in S$). 
% Replay can feed in any input $s'$ in the input family ($\forall s' \in S $) without introducing device state divergence. 
%(u npreventable divergence may still happen and be detected)

%Extending $s$ (a point value) to $S$ make recording more useful, e.g. not only write one block but write block count $<64$. 


%\paragraph{Recording inputs}

%from the device $S_{dev}$: reads of register/shared memory, interrupt occurrences. 
%The recorder (and replayer) can supply and record $S_{app}$ and $S_{ker}$.
% it can only observe (record) $S_{dev}$. 
%Changes to driver inputs have the following impacts. 
%The recorder supplies concrete input values 
%The input values have the following impacts. 
%The following dependencies exists between 

%\begin{itemize}
%%\item 
%%\Note{How to know if the inputs can be parameterized at all?}
%
%\item 
%%How to replay with a new input  $s' (s' \in S$)?
%%How to identify the parameter set $s$ and parameterize the interaction events? 
%%How to identify the parameter set $S$ and parameterize the replay actions?
%How to parameterize the replay actions?
%For example, a full driver takes the data address as an input variable, aligns the address to the page boundary, and writes to an in-memory descriptor. 
%The key is to identify value dependency between the input and the 
%replay action. % and encode the dependency in the replay actions. 
%To do so, the recorder taints the input variables and propagates any transformation of the variables to the $args$ of replay actions.
%%symbols and record the interaction events as encodings of input symbols. 
%
%%\sys{} records the {value dependency} between the driver inputs and the interaction events. 
%%We parameterize these interaction events as function of the input values. 
%%Deviation from the golden transitions means replay errors. 
%%how to constrain input s that deviates states from the golden transitions. 
%%The input can come from programs or the device. 
%
%%Not alternating device state transitions, new inputs may affect values of interaction events. 
%%This is the most common case. 
%
%\item 
%%How to deal with input values that cause device state divergence. 
%%How to identify the input family S that does not introduce device state divergence. 
%%How to identify the input family $S$ (the constraint that defines the input family)? 
%%How to identify the parameter set $s$ and the value constraints? 
%How to identify the input constraint $C$?
%The key is to discover the dependency between the input value and the induced device state transitions.  
%%Solutions: constrain and elimination.  
%%Driver input: constrain the input to only the recorded concrete state transitions; kernel env: reproduce with high fidelity; 
%%Device input: detect and bail out (only deal with polling loops) 
%To do so, \sys{} replaces input variables with symbols and runs symbolic execution; 
%%it finds out the constraints on the symbol values that will keep the state transitions under the concrete input $s$ unchanged. 
%it finds out the constraints on the symbols that will keep the state transitions the same as the state transitions induced by the concrete input value. 
%%\sys{} constrains the input values to allow only the golden path of state transitions. 
%%For uncontrollable inputs $S_{dev}$ we detect tolerable range ...
%%the input values may alter the sequence of interactions and then device state transitions. 
%
%Examples: 
%when the block number exceeds a page, the driver will schedules more than one DMA transactions \Note{improve}. 
%
%
%\item 
%%%How to handle the discrepancy that may emerge between the recorded interaction sequence and the replay interactions? 
%%How to treat the record/replay discrepancy? 
%%Discrepancy may arise between the interaction sequences of the record run and a replay run. 
%%%Even with an acceptable input, the recorded sequence of interactions may differ
%%%do not affect replay correctness. 
%%%Avoid unnecessary constraints at the replay time. 
%%Most such discrepancies are benign: they are not caused by device state divergence and hence do not imply replay failures. 
%%%The most common cause is execution timing. 
%How to tolerate alternative interaction sequences? 
%%Even if a replay run reproduces the device state transitions of the record run, their interaction sequences may not match.  
%%Even if a replay run succeeds per our definition in XXX, its interaction sequence may not match that 
%Even in a successful replay run,
%the interaction sequence often deviate from that in the record run. 
%Most such discrepancies do not imply replay failures because they are not caused by device state divergences. 
%To this end, the recorder extracts the envelope of all interaction sequences that correspond to the golden path of device state transitions. 
%It addresses two major causes. 
%%(1) a driver polls a ``device idle'' register bit until it flips,
%(1) Polling loops, the dominant causes of benign interaction discrepancies (accounts for XXX\%). 
%For example, a driver polls a status register until the current hardware job finishes. 
%The number of polling depends on the timing of job execution. 
%%A loop terminates depending on a device input and executes 
%%While the number of iterations varies across runs, the loop does not deviate device state transitions. 
%The driver instruments all polling loops and lift each loop to a replay action. 
%%(e.g. indicating the device becomes idle), 
%%where the number of register reads varies across runs; 
%(2) Statistics input from the device. 
%%Values read from from statistics registers. 
%For example, the driver reads a FIFO length register, 
%where the read value depends on the exactly when the read is attempted. 
%%Examples include a register showing the hardware FIFO length. 
%%The replayer should tolerate such benign discrepancies. 
%%To do so, the recorder extracts the envelope of all interaction sequences that correspond to the golden path of device state transitions. 
%%It instruments the code of polling loops and lift them.
%The driver uses symbolic execution to identify such interaction events that neither change device states nor the subsequent interactions. 

%\end{itemize}

%\sys{} should discover such benign discrepancies \textit{in recording} and tolerate them in replay. 
%It thus avoids imposing unnecessary constraints on the interactions at the replay time. 
%\st{It leaves unpreventable state divergence for the replayer to detect.}


\begin{comment}
How to tolerate nondeterministic interactions that do not change device state transitions? 
%do not affect replay correctness. 
%Avoid unnecessary constraints at the replay time. 
Even to repeat the same device state transitions, 
the driver/device interactions may vary across repeated runs. 
Examples include (1) a driver polls a ``device idle'' register bit until it flips,
%(e.g. indicating the device becomes idle), 
where the number of register reads varies across runs; 
(2) read value of a statistics register showing the hardware FIFO length. 
Since the replay is correct, 
we discover them in recording and tolerate them in replay. 
The replayer avoids imposing unnecessary constraints on the interactions at the replay time. 
The replayer will differentiate such nondeterminism from nondeterministic interaction events of state divergence (thus replay failures). 
\end{comment}




% ----------- useful example? --------------- %
\begin{comment}
Writes of dynamic, input-independent values are more subtle as they might alter device states. 
E.g. device FSM expects an ever increasing command serial number otherwise it faults. 
\sys{} first applies a simple heuristics -- it fuzzes the values by randomly generating them\Note{how many bytes?? this needs a type??}.
If \sys{} observes no divergence in subsequent interactions, it fills the fields with random number at replay time. 
Otherwise, it prompts the developer about the source location that fills the field and asks the developer to provide corresponding synthesis function. 
Luckily, the synthesis function is already encoded in many a field. 
E.g. in the `tag' field of USB command, it is filled by simply incrementing the prior value by 1.
\end{comment}

%\item Device inputs. 
%\textbf{Value dependency} (driver output to user apps): taint tracking and capture the dependencies. 
%%as long as control flow \textbf{or subsequent interaction sequence} is not conditioned on them, \sys{} either ignores their values.
%This is because reads reflect FSM state...as long as the native driver tolerates them, as do we.

%\subsection{The recording mechanism}
\subsection{Recorder implementation}
\label{sec:record:impl}

The recorder instantiates as a harness program, % to exercise the driver, 
a suite of kernel instrumentation, % to trace interactions, 
a symbolic execution engine, \xzlNote{S2E}
and a trace processor. 
We focus on last three components in this section.
We will describe device-specific harness programs in Section~\ref{sec:case}.
%This is shown in Figure XXX. 

\begin{comment}
\Note{moved from S2}
\paragraph{Discovering driver/device interfaces} % which must be recorded. 
At the record time, 
\sys{} needs to take a series of snapshots of the interfaces. 
(1) CPU and devices share a wide interface: registers, DMA buffers, and in-memory descriptors. 
To accommodate complex driver/device interactions, 
in-memory descriptors may further embed pointers to each other, e.g. to form a scatter-gather list. \Note{cite}
%The data structures must be captured as part of the device/driver interactions. For instance, DMA is controlled by an 8-word in-memory data structure... The VCHIQ ...  firmware ... FSM ... containing pointers to each other to form a list...
(2) 
\sys{} should identify \textit{parameterizable} interface fields, i.e. to be overridden with new values at the replay time. 
Examples include registers pointing to the base of in-memory descriptors and 
fields in in-memory descriptors pointing to input/output buffers. 
Their values depend on physical memory layout which can vary across runs. 
%The replayer must override these fields at run time, because their values depend on physical memory layout which can varies across runs. 
(3) 
The interface may span additional hardware components such as a standalone DMA engine in a separate address range and power controllers (??).
\end{comment}


\paragraph{Static code instrumentation}
%We uses userspace test harness to exercise the full driver of interest in a Linux kernel. 
%We control the test inputs, such as physical address of the input/out data buffers, and their lengths.
%We instrument the kernel code for the following purposes. 
The recorder interposes the following kernel source locations on the three interfaces. % automatically. 
Table~\ref{tab:instrumentation} provides detailed functions.
\input{tab_instrumentation}

\begin{myenumerate}
	\item 
	$Program\leftrightarrow driver$: the set of syscalls back the record entry, which may span multiple syscalls (e.g. multiple ioctl for retrieving images from camera). 
	The recorder taints their arguments. % syscall number (?).
	E.g. for pread, the recorder taints its file descriptor pointing to the device file, the output buffer, the offset (i.e. block id), and read size (i.e. block count).
	
	\item 
	$Driver\leftrightarrow environment$: they are a set of standard kernel services provided to drivers. 
	The recorder logs their inputs and outputs.
	Notably for DMA APIs (e.g \code{dma\_alloc\_coherent}), the recorder customizes the DMA pool and mandates each allocation for descriptor lands in a separate page.
	The recorder logs allocation sizes and addresses;
	it symbolizes and taints the addresses for reconstructing the pointer structure of them.
	
	\item 
	$Driver\leftrightarrow device$: the recorder manipulates page permission bits to capture and log register accesses, descriptors writes, and to dump descriptor memory.
%	To do so, it disables RW bits for register address pages and W bits for descriptor pages.
%	In the page fault handler which traps accesses to these pages, the recorder enables the permission bits temporarily to log access type (i.e. read/write), addresses and values.
%	If the value being written is a descriptor address, the recorder dumps its content; 
%	additionally, the recorder places stubs in interrupt handlers to dump all descriptors immediately after an IRQ.
	To do so, it flips RW bits for register pages and W bits for descriptor pages.
	Upon trapped accesses, the recorder logs the access type (RW), physical address, and values.
%	In the page fault handler which traps accesses to these pages, the recorder enables the permission bits temporarily to log access type (i.e. read/write), addresses and values.
	If the write value points to a descriptor page, the recorder dumps the page and keeps updating a most recent one.
%	in case the recorder keeps updating the dump for the same descriptor (i.e. identified by its page), 
%	additionally, the recorder places stubs in interrupt handlers to dump all descriptors immediately after an IRQ.
%	The recorder places stub in two places to dump the descriptor content:
%	the recorder logs kernel's standard register accessors to dump their types (readl/writel), register addresses and values. 
%	Last, it injects code to dump their content (e.g. via hex\_dump) in two places: 
%	1) whenever their address are used being written an output event and 2) immediately after an interrupt.
%	This is to ensure the dumped content is consistent with the one used by device;
	This ensures recording completeness and consistency of descriptor seen by device: 
	the rational is by the time a descriptor address is sent to the device, it is ready to be used (and to be dumped);
%		the rational is by the time its address is sent to the device or from the device, it is ready to be used;
	even if the driver modifies the descriptor after the dump, the recorder traps and logs the modifications, which will be replayed.
	%the recorder bookkeeps all allocated descriptors and tracks their addresses and sizes. 
	%	To ensure the dumped content is consistent with the one used by device, the recorder bookkeeps all allocated descriptors and tracks their addresses and sizes. 
	%	The rationale is by the time its address is notified to the device, it is ready to be used.
%	In case their content change even after they are dumped, the recorder sets read-only permission of their pages to trap any writes and re-dump them.
%	However, in practice we have not found any such writes. 	
\end{myenumerate}

The recorder runs static code analysis to extract polling loop.
It logs entry/exits of the polling loop as well as the loop conditions.
Note that loop body, which is the polling of a register is captured via instrumentation in $driver\leftrightarrow device$ interface. 
%Note that loop body, which is the polling of a register is captured via instrumentation in driver/device interface. 
In practice we have found simple code analysis tool (e.g. XXX) suffices to recover almost all loops.

Most of the instrumentation is automatic. The only manual effort is to identify and annotate a handful of kernel APIs. 
Because these APIs are independent of specific drivers, the annotation is done once for each kernel version. 

\begin{comment}
\Note{old writing-- }

(1) Driver input from the kernel.
The propose is to interposes a set of standard kernel APIs and trace the input values: % and inject new values as needed. 
allocating DMA memory (e.g. dma\_alloc\_coherent), timekeeping (), and \xzlNote{add}.  % random number generator 
The recorder bookkeeps allocated memory regions in order to dump them. 
%Notably, the recorder overrides the kernel's DMA memory allocator with a custom allocator, allowing customization of the driver's memory layouts. \xzlNote{needed?}
%The custom allocator serves pages from a pool reserved at boot time at control of \sys{} (Linux CMA). 
%Note that memory efficiency is not a concern, because the replayer does not inherit memory layout at recording time. 

(2) Driver/device interactions. 
The purpose is to log the raw interaction events. 
 %and functions that map register banks declared in device trees (e.g. ioremap);
%We also trap access to iomem by toggling the read/write bit of their PTEs to ensure no register is left out.
The recorder instruments register accessors (readl/writel). 
It injects code to dump device memory regions prior to submission of a hardware job and right after a job's completion \xzlNote{how is this done}. 
%The recorder identifies device memory regions via interposing the kernel's DMA allocations. 
% right before trigger register writes, i.e. a register write that kicks off an upcoming hardware job and immediately precede an interrupt notifying the job status. 
%The snapshots contain in-memory descriptors as part of the driver/device interfaces. 
%We identify trigger registers in a dry run prior to recording. 
	
(3) 
Polling loops. The purpose is to tolerate the nondeterministic number of iterations as discussed above. 
%The number of iterations is nondeterministic depending on timing. 
%Examples include wait for register to be ready, wait hardware FIFO to become available. 
%Symbolic execution of loop creates a large number of execution paths. 
As done in prior systems~\cite{symdrive}, the recorder runs static code analysis to recognize polling loops and parse them. 
For each polling loop, the instrumented code emits one replay action, 
which preserves the loop structure: the terminating conditions and the interaction events within the loop body. 
%As a result, recording does not generate alternative execution paths. 
%Optionally, the loop's body repeats a segment of interactions. 

%(4) Bulk data copy. 
(4) DMA data copy. 
The purpose is to track tainted input data as the data is moved with an DMA engine, e.g. across user/kernel buffers. \Note{discuss}
The recorder instruments the DMA APIs. 
\end{comment}

%Note that the above instrumentation is done only to a number of generic kernel APIs that are independent of specific drivers. 
%It is a one-time effort for a given kernel release. 

%\paragraph{Dumping shared memory}
%\xzlNote{Liwei fill in}
%``when to dump DMA memory?''
%``what if the driver changes the memory after the DMA addr is assigned to a reg?''
%
%%After static code instrumentation, prior to the very initial recording, the first question \sys{} faces is -- when to dump shared memory during recording?
%While \sys{} instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
%It does not know \textit{when} drivers fill them with commands, messages, etc.
%Taking their snapshots at arbitrary times results in inconsistent values.
%%E.g. they may be modified by driver at different layers and times.
%
%Our solution is to take snapshots of all of them before writes to \textit{trigger} registers, i.e. a register write that kicks off the upcoming hardware job. 
%Our rationale is simple: the write to trigger register is a handoff point; 
%at the point, the driver must provide the device final information about the hardware job. 
%Finding the trigger register is straightforward: \sys{} runs a test once and identifies register writes that immediately precede interrupts, which are often used to notify job status.
%This heuristics narrows down from tens of registers to 1--2 registers per device.
\begin{comment}
\paragraph{Logging DMA interactions}
Besides register accesses, shared DMA memory serves as the alternative driver/device interaction. 
To capture such interactions, the overarching guideline is to log DMA allocations and dump their content as well. 
The recorder addresses following three specific problems:

\textbf{When to dump in-memory descriptors?}
While the recorder instruments DMA APIs, it only knows the information (e.g. address, size) as they are allocated.
It does not know \textit{when} drivers fill them with commands, messages, etc.
Dumping their contents at arbitrary times results in inconsistent values.
To address this, the recorder dumps their memory as long as their addresses are consumed, i.e. when being written into a register or another descriptor, and keeps the most recent one.
This is because by the time the device is notified about descriptor addresses, it expects them to be ready. 
\xzlNote{what if data contents changed afterwards}

\textbf{How to reconstruct linked descriptor structure?}
A device may use multiple descriptors for one userdata transfer with a large length, e.g. each descriptor contains only one 4KB page. 
Instead of being used individually, the descriptors may embed pointers to each other, forming a linkedlist.
The recorder must capture the data structure for a faithful replay.
To this end, it taints the allocated addresses of the descriptors, propagates them to registers and other descriptors, and enforces a constraint on them, e.g. the field must be filled by address of some dumped descriptor. 
%later when the descriptor is loaded during replay, the replayer address 
By doing this, the recorder preserves the same pointer structure. 
Section~\ref{sec:case:mmc} will show a detailed example.
%For example 
\end{comment}

\begin{comment}
% obsolete
1. propagates the driver input to DMA allocation size
2. logs every DMA allocation (addr, size) as part of the raw trace;
3. taints the allocated addr and propagates to registers/descs (for reconstruct descriptor pointers);

Differentiate allocations for data vs. for metadata. 
\end{comment}

\paragraph{Exercising the full driver}
\Note{check impl details}
The recorder executes the driver on S2E with dynamic taint analysis:
%\Note{repeat}
it kicks off the driver with concrete inputs supplied by a harness program; 
along the concrete execution path, it explores the effect of inputs by collecting path conditions, propagating taint operations, and comparing state-changing events.  
%The recorder executes the driver with concrete inputs supplied by developers. 
%On the same code path, it also performs symbolic execution with the input replaced as symbols.  
The purposes are (1) to discover the input constraints $C$ needed to detect and avoid device state divergence; 
(2) to discover data dependencies between input and output events to parameterize replay actions. 
\Note{check the conflicts of path conditions. In theory these shall not happen.}
\Note{check constraints -- can it refer to symbol? how to resolve? or simply define constraints are set of relations between input value and concrete values}
%\Note{overlap with taint tracking? The goals seems to only identify predicates}
% (2) to discover the input constraints $C$ needed to stay on the current path of device transitions. 

%Developers provide concrete inputs, which are used to select execution paths (prune execution paths). 
%It propagates the transformation applied to input symbols. 

Example: 
in a record run, one of the driver's input variable $BlkCount$ is assigned with a concrete value 6. 
Later, the driver's executing path reaches a conditional predicate $BlkCount>8$.
The recorder's symbolic executor forks the execution into two copies: one with constraint $BlkCount<=8$ and one with $BlkCount>8$. 
The recorder runs both copies and compare their subsequent device state transitions (by matching their state-changing events as described in Section XXXX). 
If the state transitions diverge later, 
e.g. because the driver invokes only one DMA transfer when $BlkCount<=8$ and invokes more when $BlkCount > 8$, 
the recorder only continues the executing path exercised by the concrete input ($BlkCount=6$) and prunes the other; 
it adds $BlkCount<=8$ to the input constraint.
%A possible cause, for example, is that the driver configures the device to use DMA data transfer only when $C>=16$. 
If the two copies show no divergence in device transitions, 
no input constraint will be added. 
This is because the path conditions only affect the driver's control flow without alternating the device states, 
e.g. the driver uses different memory allocation strategies per the $BlkCount$ value.
%e.g. the driver does different bookkeeping depending on the $BlkCount$ value.

 %not visible to the device. 

% ---- useful example --- 
\begin{comment}
The same applies to the inputs from kernel environment $S_{ker}$.
Kernel environments: reproduce with high fidelity
Example: block count, the driver checks for its value. 
If it is less than a page size (i.e. eight 512-byte blocks), driver combines them as one page access through DMA.
The analysis captures such an "if" check, conditioned on block count and hence deem the input non-parameterizable. 

Otherwise, the execution constrains the input X to select the same path as the concrete input x; 
it prunes alternative paths. 
The rationale is only to record the beaten path exercised by the concrete input (our hypothesis). 
This avoids state (path) explosion and makes recording inexpensive. 
\end{comment}

% The recorder also uses symbolic execution to explore the effect of 
%The recorder also explores the effect of device response. 
%The recorder applies the same techniques to explore the of device response, 
The recorder applies the same techniques to treat input values from \textit{driver $\leftrightarrow$ device} interface, 
%i.e. values flowing from the device to the driver in interaction events. 
i.e. values read from device registers or in-memory descriptors. 
%For a response $r$, e.g. a register read, 
%(1) The recorder replaces a device-response value $r$ with a symbol $R$ and propagates $R$ in the subsequent driver execution. 
(1) The recorder uses a concrete input value $V$ from device in the subsequent driver execution. 
% to program-visible outputs or subsequent interaction events. 
For example, the driver reads a register showing the buffer size needed by the device for storing incoming data; %the next image frame; 
%the recorder then propagates the symbol to the size argument of a subsequent call to DMA buffer allocation. 
the recorder symbolizes the value then propagates it to the size argument of a subsequent call to DMA buffer allocation. 
%the device specifies its demanded buffer size via a register value; the recorder propagates the size to a future kernel buffer allocation. 
(2) The recorder derives a constraint on the input event which $V$ belongs to. 
If $V$ is already known as a state-changing event, e.g. read from a command status register returning a new value $v$, 
the recorder mandates that the concrete value $v$ must be exactly matched in replay. 
Otherwise, the recorder executes with the symbol to discover the constraint on $V$ that will prevent the subsequent device state transitions from deviating the transitions induced by the concrete input $V=v$.
\Note{USB device ID, USB data toggle} 
%Otherwise, the recorder uses symbolic execution to discover the constraint on $R$ that will prevent the subsequent device state transitions from deviating the transitions induced by the concrete input $R=r$. 
%The recorder then mandates the value of the must satisfy the constraint. 
% will raises an error if it observes the value of $r$ violates the constraint. 
%The replayer will raises an error if it observes the value of $r$ violates the constraint. 
% The resultant trace template raises an replay-time errors when $r$'s 

%The device inputs are concrete and also assigned with symbols. 
%The symbols are propagated in subsequent execution. 
%If divergence in state transitions are found dependent on any device input symbols, \sys{} stops with errors -- it does not support that. 


%\paragraph{Emitting \template{}s}
\paragraph{Trace processor}
%\Note{needs work}
%Based on the trace of interaction events, the discovered dependencies, and the value constraints, 
%Based on traced driver inputs and interaction events, 
%Based on the sequence of traced interaction events, 
%the recorder emits the sequence of replay actions. % all register accesses,  device memory dumps, and interrupts. 
%In the replay actions, 
emits replay actions from the raw logs of instrumented code and concolic driver execution in a single record run, producing an interface template.
The implementation is straightforward: 
\begin{myitemize}
	\item
	For \code{read},
	it emits input events by replacing concrete program/environment/device input values of a raw log entry with parameters and adds their constraints, which are an expected value or a range.

	\item 
	For \code{write},
	it replaces the concrete values being written to device in the raw log with accumulative taint operations from its taint source, if any;
		
	\item 
	For \code{poll}, 
	it fills the loop condition with the conditions logged by static code analysis results;


	\item 
	For other replay actions: 
	it emits a \code{load\_mem} whenever a descriptor is snapshotted;
	it emits a \code{wait\_for\_irq} whenever an IRQ occurred in a record run;
	it emits a \code{delay} as logged from kernel delay functions.
\end{myitemize}
%The recorder derives a sequence of replay actions from raw interaction events.
%to emit input events, it replaces concrete program/environment/device input values of a raw log entry with parameters and adds their constraints, which are an expected value or a range;
%%for replay actions that output values to the device, e.g. a register write,
%to emit output events, it replaces the concrete values being written to device in the raw log with accumulative taint operations from its taint source, if any;
%to emit 
%%For replay actions that consume values from the device, e.g. a register read,
%%the recorder annotate with the viable ranges of expected values. 
%%if value dependency is present, e.g. a checksum of output data, or concrete values if the dependency is absent, e.g. control commands. 
%%(from the device or the driver) as well as any transformation applied. 
%%Examples: the data buffer address shifts right then left 3 bits in an field of the descriptor; checksum. 
%%\sys{} records concrete values of interaction events if no value dependency is discovered, e.g. the registers encoding control commands and device status. 
%%Other interface fields are recorded as concrete value only; they do not encode input symbols, e.g. they may encode request or protocol semantics. 
%The recorder also emits time intervals between interaction events. 

\begin{comment}
\textbf{Resolving input-dependent fields.}
The following is an example list of them:
\begin{myitemize}
	\item 
	\textit{Block ID} specifies starting sector to access in a storage device. 
	
	\item 
	\textit{Block count} specifies how many sectors to access. 
	
	\item 
	\textit{Input/output buffer address} specifies data page source or destination.
	
	\item 
	\textit{Input/output Buffer length} specifies size of the input/out buffer.
	
	\item
	\textit{Descriptor address} specifies locations of in-memory descriptors. 
	
	\item 
	\textit{Descriptor size} specifies size of the descriptors. 
	Note the information about descriptor address \& size is not tracked from user inputs but from kernel DMA APIs. 
\end{myitemize}
\end{comment}

\input{replay}


%\xzlNote{--- Obsolete ---}
%
%\paragraph{Limitations}
%For simplicity, \sys{} gives up on devices where state transitions depend on IO data \textit{content}, a behavior commonly seen on network interface cards (NICs).
%% Notable examples include network interface cards. 
%%Notable examples include network interface cards. 
%An example is BCM4329, a WiFi NIC that implements 802.11 MAC in its firmware. 
%Its Linux driver sends different commands to the NIC based on the header content of received WiFi packets. 
%%Related to above, \sys{} cannot replay interrupt handlers with control flows dependent This is because our recording method cannot capture all possible branches (thus interrupt events) in the interrupt handler. For each handler, the type of expected interrupt event is pre-determined. 
%%  --- NOTE: the above is fine, we can detect it; the only problem is there can be lots of divergences at replay time. 
%Fortunately, protecting NICs with secure IO is not as crucial as other devices, because security-sensitive network traffic through NIC is often protected with end-to-end encryption. 

%Fortunately, we deem NICs are \textit{not} our priority, as the TEE can protect network packets with end-to-end encryption. 
%Record and replay must be on same model of hardware platform. same device?? same SoC??? The hardware configuration should agree. 

%\Note{fix the following}
%Recording start after kernel power/clock init.. which is assumed to be integral..
%We donot record their init (as reg access) due to the complexity beyond MMC....

%Cannot dynamically switch between configurations (?). \Note{maybe we can?}










==> related-recycle.tex <==
% !TeX root = main.tex
\section{Related Work}
\label{sec:related}

We discuss prior works we have not covered so far.
\paragraph{Driver reuse}
How to reuse kernel drivers has been a fascinating research question. 
By ``lift and shift'', ~\cite{rumpkernel, sgx-lkl} transplant the whole drivers as-is by wrapping them with a shim layer for foreign environment (e.g. SGX) in the spirit of a library OS~\ref{drawbridge}; 
~\cite{uboot,optee} trims down individual drivers (e.g. UART) to fit into the foreign environment;
~\cite{termite,termite-2,revnic} synthesizes the drivers from formal their specifications or through reverse engineering.
Like prior works, \sys{} shares the driver reuse goal;
unlike them, \sys{} adds negligible codebase, does not require developer knowledge nor a formal specification. 

\paragraph{Program analysis}



\begin{myenumerate}
	\item Reverse engineering~\cite{revnic}:
	no kernel source code needed because it reverse engineers binary code (e.g. a Windows driver);
	need to understand device FSM because developer needs at least write some boilerplate template code (handling some branches in device FSM).
	This is required for each other driver (paper only shows NIC).
	
	\item From specification~\cite{termite}:
	no kernel source code needed but developer has to write up a device specification for the tool to synthesize from.
	Generated code must comply to host OS APIs.
	This is required for each other driver.
	
\end{myenumerate}
	
The approach requires most intimate knowledge of the device, as it is essentially building anew/re-inventing the wheel. 








Linux and its derivation: BSD, Rumpkernel, UBoot. 

Defeaturing is already done (implicitly) via manual code tailoring or porting: Rumpkernel, UBoot, etc. 
Manually tailor/refactor/derive Linux driver code. 
See limited success on some simple drivers (UART); 
Problems: 
high code complexity, high kernel dependencies -- mismatch the constrained TEE environment; 
high engineering efforts (per driver, SoC). 


\Note{must be rewritten}
\paragraph{Record and replay} is known useful for diagnosis, debugging, and security analysis~\cite{sanity, replayConfusion, rtag}. 
It has been applied to mobile UI apps~\cite{reran,mobiplay}, 
web apps~\cite{mahimahi}, virtual machines~\cite{reVirt}, networks~\cite{ofrewind}, and whole systems~\cite{R2}. 
\sys{} is inspired by the prior work, e.g. constraining dynamism for deterministic replay. 
None of the prior works has applied the idea to GPU registers and memory. 

Quite related to \sys{}, recording syscalls has been popular in reverse engineering GPU runtimes~\cite{rosenzweig-m1, grate, panfrost, patrace}.
By changing LD\_PRELOAD of a GPU app, the developers intercept IOCTL commands between the runtime and the kernel, manipulate the commands, and observe the results. 
Compared to it, \sys{} targets a different goal (minimizing GPU software), records a lower level (registers and memory), and entails different techniques (e.g. interval compression, input/output localization, etc.)


\begin{comment}
Targeting application instrumentation, system diagnosis, or reproducing bugs for debugging, record and replay approach is broadly studied: i) on mobile environment to reproduce GUI gestures~\cite{reran} including network activities and various sensor inputs~\cite{valera}, or improve real-time interaction between mobile app and the user~\cite{mobiplay}; ii) on desktop/server environment to reproduce behavior of web applications~\cite{mahimahi}, entire system~\cite{R2, RR} or virtual machine~\cite{reVirt}. Besides, some works adopts record and replay technique for the security analysis to detect vulnerabilities~\cite{sanity, replayConfusion, rtag} or network troubleshooting~\cite{ofrewind}.
\end{comment}


\textbf{Prior works using program analysis}
\begin{myitemize}
	\item 
	Symdrive -- aim to reconstruct complete device FSM via symbolic execution and source-to-source transformation. Test devices without the device existing. 
	
	\item 
	Dr.Checker -- bug finding using well-known program analysis techniques. Statically check source code for violation, e.g. use after free, overflow
	
	\item 
	Charm -- system support for dynamic analysis on mobile devices 
	
	\item 
	Termite1,2 -- driver synthesis from specification with user guide
	
	\item 
	RevNIC -- reverse engineering of device driver binary. Works for close-sourced NIC drivers. 
	
	\item 
	Howard. Dynamic analysis in recovering binary data back to their \code{struct}.
	
	\item 
	BinRec. Selective binary lifting. Use concrete inputs to discover a code path, and lift it in IR and recompile. Fallback to native code if the execution is off the beaten path (ensuring conservative program behavior). 
	
\end{myitemize}


\paragraph{Prior efforts on re-engineering stacks} 

\textbf{VS Discorver:}~\cite{discoverer}.

Difference: 
\begin{myitemize}
	\item goal: ours is for driver reuse, their is for the sake of rev engineering. 
	\item scope: (as goals differ). 
	For messages, we only care about "a few" fields that describe the data (size, length, off). They seek to reveal "each" field of a message format.
	We deal with extra register access.
\end{myitemize}
Similarities:
\begin{myitemize}
	\item subject: both deal with message passing and message formats. 
	\item approach: the taxonomy of "constant vs variable" is similar. 
	seq alignment vs diff, whereas the latter is a subset (?).
\end{myitemize}




\paragraph{Trusted execution environment}
\Note{must be rewritten}
%Thanks to its strong security guarantees but modest overhead,
Thanks to its strong security guarantees, 
prior works utilize TEE to isolate entire application~\cite{trustshadow} or security-sensitive software components~\cite{rubinov16icse}, to support secure compute primitives~\cite{streambox-tz}, to protect machine learning inference~\cite{occlumency} and training~\cite{darkneTZ}.
While the current TEE is limited on CPU computation, prior works proposed solutions that leverage TEE to protect GPU computation by isolating potentially vulnerable GPU software stack~\cite{slalom} and/or hardware modification~\cite{graviton, HIX, hetee}.

\paragraph{Secure storage for TrustZone}

SBD~\cite{sbd} still uses normal world OS,


\paragraph{Device checkpoint}

Prior works~\cite{fgft} shows it possible to save a device's (most) state by its register values. 

\paragraph{Driver reuse/synthesis}

\Note{from transkernel. to adapt}
Extensive work transplants device drivers to a separate core~\cite{picodriver}, user space~\cite{microdrivers}, or a separate VM~\cite{Levasseur2004}.
%They can be transplanted together with its enclosing kernel to a dedicated core~\cite{picodriver} or VM~\cite{Levasseur2004}.
However, the transplant code cannot operate independent of the kernel, whereas ours must execute autonomously.

Encapsulating the NetBSD kernel subsystems (e.g., drivers) behind stable interfaces respected by developers, 
rump kernel~\cite{rumpkernel} seeks to enable their reuse in foreign environments, e.g., hypervisors. 

\Note{to adapt and revisit}

Driver synthesis: Termite~\cite{termite,termite-2}

In theory, automatic device driver synthesis tools like Termite~\cite{termite} can synthesize PM code given formal device specifications, either derived from the documentation or RTL (register transfer level) description of a device. 
Model device states and kernel framework/interfaces and synthesize code to drive state transitions. 
However, it is unclear whether deriving such formal specifications is any easier, if not harder, than writing driver PM code. 

Formal specifications rarely exist. They do not include hardware quirks which are crucial for drivers to function. 

Comparing to it, \sys{}'s goal is different: to derive a simpler (and hence less error prone) driver from an existing mature driver. 
To do so, records a subset of state transitions in an empirical fashion. 

RevNIC~\cite{revnic} tries to synthesize a (full-fledged) open-source driver from a binary one. 
It reconstructs a state machine describing the driver with symbolic executions. 
It pays high complexity for being thorough: 
setting up a virtual machine, setting up symbolic execution, writing template driver code, etc. 

\Note{There is a large family of symbolic execution work on software testing...}

To reduce security risks imposed by such rapidly-evolving and unstable interfaces, \cite{lock-in-pop} proposes  by constraining kernel path to a small set of most often executed paths, which are less likely to be buggy.

%\paragraph{Secure client ML}
%%Yubara, occulumency, darkne TZ cannot support GPU computation
%%Slalom only support GPU computation
%%partitioning - yubara, occulumency, darkne TZ, slalom
%Prior works have transformed the ML themselves rather than the GPU stack.
%By outsourcing security-sensitive parts to TEE~\cite{occlumency}, they accomplished secure client ML while preserving model-privacy~\cite{ternary, darkneTZ}.
%However, they are limited on CPU-only computation; its model-privacy is orthogonal to and easily combined with the \sys{}.
%Meanwhile, Slalom~\cite{slalom} proposed secure heterogeneous computation by homomorphic encryption. 
%However, it burdens client devices with huge computational complexity; its limited linear operations preclude a full GPU-accelerated computation.

%However, its additional complexity burdens client devices; the limited linear opeartions preclude a full GPU-accelerated computation.
%Meanwhile, Slalom~\cite{slalom} proposed secure heterogeneous computation by homomorphic encryption. However, its additional compute complexity 
%is cannot fit well for client devices; the limited linear operations make it difficult to support a full GPU-accelerated computation.

%Prior work has transformed the ML themselves rather than the GPU stack. 
%Slalom~\cite{slalom} proposed secure heterogeneous computation by homomorphic encryption. It outsources computation intensive parts of DNN to GPU while data is encrypted. The computation is verified later from CPU-TEE. While it provides data confidentiality, it does not fit well for the end-devices as homomorphic encryption brings about significant performance degradation due to additional computations. Moreover, it is limited on linear operations which makes it difficult to support diverse computation~\cite{darkneTZ}.


==> replay-correctness-recycle.tex <==
% !TeX root = main.tex
%\subsection{Why replay works -- replay correctness analysis}
\subsection{Why driverlets work}
%\subsection{Device state and replay correctness}
\label{sec:design:theory}


\paragraph{Expressiveness}
% A \teedriver{} \textit{approximates} the functionalities (features) of the full driver. 
% To trustlets, it offers a tradeoff between practicality and simplicity. 
% To trustlets, it is sufficiently expressive at low complexity. 
A \teedriver{} is a practical \textit{subset} to the functionalities (features) of the full driver. 
To trustlets, it provides core IO functions at lowest complexity. 
The \teedriver{} retains the capabilities to access arbitrary data at the granularities (with options/flags) specified in record runs, 
e.g. accessing any flash chunk in 1, 4, 16 blocks. 
It gives up the driver's functionalities: 
(1) accessing data at arbitrary granularities, e.g. to read a chunk of 32 blocks, trustlets need to call the \teedriver{} to read two 16-block chunks;
(2) driver's optimization for large, asynchronous data transfers; 
(3) dynamic device management, e.g. hot plug. 

\xzlNote{Merge the above writing to below}

%The replayer provides the same level of correctness guarantee as a full driver does. 
%does in \textit{assessing} the correctness of a request execution. 
%if a request is completed successfully. 
%This means that when the replayer deems a request is completed successfully, the assessment is as sound as one made by the full driver. 
%This means that when the replayer assesses that the GPU has completed a request successfully, the assessment is as sound as one made by the full driver. 
%Our approach -- replaying driver/device interactions -- raises a top question: 
%Our approach raises a top question: 
We next discuss a key question: 
%how do we assure that a replay run is correct?
how does a replayer assure a replay run is correct?
We want the replayer to provide the same level of correctness guarantee as the driver does: 
when the replayer asserts that it completes a given request with success, the assertion is as sound as one made by the driver. 

%when the replayer asserts a replay run completes with success, the assertion is as sound as one made by the full driver. 
%This means that an assessment of successful request completion made by the replayer is as sound as one made by the full driver. 

%Our rationale is based on the following observations. 
% on devices and mature drivers: 
%We have the following observations on driver designs: 
%Our rationales are as follows. 
%on equivalence of device state transitions. 

%\textit{cc and replay correctness}: 
We first define a \textit{faithful replay}, a notion common in record/replay systems~\cite{r2}. 
%As we ensure that the via path of device state transitions is unique, 
%As only one path of device state transitions is via for a success run, we have: 
As described above, the driver allows only one path of device state transitions for completing given hardware jobs. We have: 
% and base it on device state transitions: 
%in Section~\ref{sec:bkgnd:model}.

%\begin{theorem}
\begin{definition}[Faithful replay]
%\begin{definition}[Faithful replay]
	If in a replay run, the sequence of stimuli to the device FSM and the device state transitions exactly match those in a successful record run, then both runs complete the same hardware jobs and the replay is faithful. 
%	If in a replay run, the same sequence of state-changing events (i.e. path of device state transitions) exactly matches that in a successful recording run, then both runs complete the same sequence of jobs and the replay succeeds. 
	%\end{theorem}
\end{definition}
%%Built on the above definition, 
%%the replayer assesses replay success by comparing device state transitions in the replay run with those in the recording run. 
%%Our rationale is as follows. 
%Our rationale is that 
%%To repeat the same hardware jobs, a device's paths of state transitions only diverge for two reasons. 
%%(1) Some divergences reflect alternative paths to finish the same hardware jobs. 
%%First, there exist alternative paths to finish the same hardware jobs correctly. 
%by constraining a device's state space, we can ensure there is only one path to finish a given set of hardware jobs correctly.
%%Although such one is path guaranteed by hardware, alternative transition path might happen due to other conditions... 
%To do so, we eliminate all the root causes of alternative transition paths outside user/kernel inputs, including device hardware concurrency and platform runtime power management.  
% %and serialize hardware job submission in recording as well as replay runs.
%%A notable source of alternative transition paths is a device's hardware concurrency. 
%%\xzlNote{more?}
%%When multiple jobs are queued with the device, the number of completion interrupts and their order can be nondeterministic. 
%%For instance, if CPU submits multiple USB transfers at a time, a USB controller may  opportunistically coalesce the completion interrupts of these transfers. 
%%In response, we eliminate all but one alternative path of transitions. 
%%For example, we serialize hardware job submissions both in the recording run and in the replay run. 

Given the definition,
%we further establish \textit{replay correctness} on state-changing events, the external representation of state transitions. 
we further establish \textit{replay correctness} on the external observation of state transitions. 
%As the above definition associate replay correctness to device states, 
%it raises two questions. 
%The above definition raises two design questions. 

%A device's state changes as interactions and execution continue. 

%\begin{theorem}[Replay correctness by observational equivalence]
\begin{thm}[Replay correctness]
	If the replayer observes the same sequence of state-changing events as the driver observes at record time, 
	%If the replayer observes the same sequence of state-changing events as recorded, 
	then as far as the driver is concerned, 
%	the device state transitions are the same as recorded, i.e. a faithful replay. 
	the replay is faithful. 
	% and the device completes the same request. 
	% (despite of difference in IO data contents).
	%The replay therefore succeeds. 
	Given the gold driver assumption (\S\ref{sec:bkgnd:model}), 
	the replay is therefore correct. 
\end{thm}

In other words, the replayer is as capable as the gold driver on inferring device state and hence detecting any state divergence, i.e. replay failures. 
Suppose there is a state divergence undetected to the replayer, 
e.g. an MMC controller corrupts data silently despite of all matched state-changing events, 
the divergence could have been missed by the driver as well, a situation should not have occurred to a gold implementation. 

%it could have been missed by the full driver as well. 
%This means there is a bug in the driver. 
%
%\textbf{What if the replayer fails to detect state divergence?} 
%E.g. a MMC controller corrupts data silently despite of all matched state-changing events. 
%Thus the divergence could have been missed by the mature driver as well, a situation should not occurring in a golden implementation. 

\begin{comment}
Achieving \textit{replay correctness} is not difficult.
Later we will show -- as long as we constrain the state space in aforementioned way, i.e. serialize hardware jobs, disable device runtime power management, the observed state changing events always stay the same. 
\end{comment}

Figure~\ref{fig:code} (b) shows an example. 
The replayer deems the replay run correct, because all the state-changing events match those in the record run (a), except for the generalized values in output events. 

\paragraph{Handling state divergence}
%We deem any mismatched state changing events which deviate from the faithful path as failure in job execution. 
%We deem all other device state transitions which deviate from the faithful path as failure in job execution. 
%other than the successful path, all other device state transitions imply failure in job executions. 
%Resource availability at the SoC level, 
%Should the replayer observe any state changing event mismatching the recording, 
%it deems that the device state has deviated from the faithful path and a failure in job execution. 
Should the replayer observe any state changing event mismatching the recording, 
it deems a failure in job execution. 
Figure~\ref{fig:code} (c) shows the scenario, where the IRQ status (\code{0x2}) mismatches the recording (\code{0x1}).
%In Figure~\ref{fig:code}, replay run 2 fails, because its state-changing events diverge from those in the recording run -- will be re-executed.
%The replayer treats any state changing event that mismatches the recording as  indication of deviation from the faithful path as failure in job execution. 
Fundamentally,
such divergences happen because the device FSM has received unexpected stimuli from sources beyond the control of the recorder and the replayer. 
We identify three major sources. 
(1) Residue states left by prior jobs.
%For example, device power states are kept high for a while after executing a job\Note{cite};
For example, device FIFOs are yet to be flushed\Note{cite};
at different times the replayer may read different number of available slots.
(2) Fluctuation in chip-level hardware resources, 
including power supply, clock rates, and memory bandwidth. 
For example, an under-current condition of an SD card during a replay run can trigger an interrupt previously unlogged. 
(3) Unexpected hardware failures. 
%For example, an MMC controller losing the flash media because of SD card removal. 
For example, a media accelerator losing the connection to the image sensor because the latter has been heated by direct sunlight for long. \xzlNote{cite}
% https://www.flir.com/support-center/iis/machine-vision/knowledge-base/common-causes-of-imaging-sensor-failures-or-malfunctions/

%it may finds incorrect message CRC because of bus error; 
%a bus transaction may time out because the flash peripheral has a power failure. 
%heavy contention on the main memory will cause commands to media accelerator to timeout.
%These divergences cannot be fully prevented. 

Because these failures are unpreventable by software, the replayer detects the resultant divergences from state-changing events and attempts recovery by restarting the execution. 
We will discuss the efficacy of re-execution in \sect{eval}. 


\Note{merge below}
\xzlNote{move below to motivations}
The mechanism serves three important purposes:
\begin{myenumerate}
	\item 
	Prevent state divergences. 
	In conjunction with single-threaded, sequential replayer design, it constraints the device state space by mandating a uniform initial states.
	This is also done in a recording run, e.g. to prevent non-determinism from residue states (\S~\ref{sec:design:theory}).
	
	\item 
	Better resilience.
	As described earlier, the replayer resets device state as an attempt to recover from failed replay due to state divergence. 
	%	detects device state divergence by matching each observed stage-changing event with the \template{}. 
	%	In case this is a mismatch, e.g. a device interrupt which was not recorded in the \template{}, the replayer reports a failure. 
	%	The MVP driver relies on device reset to recover from replay failures. 
	%	Once the driver detects a divergence at any moment in trace replay (i.e. mismatched state-changing events), 
	%	it resets the device to the clean-slate state and re-executes the request. 
	By construction, each request execution is idempotent. 
	Failed replay attempts have no side effect on the eventual execution success. 
	In case of persistent divergence, the replayer fails by reporting meaningful errors: the source line information and callstack; dump register value and decode. 
	
	\item 
	Mitigate side channels.
	This is in case the device is shared by trustlets.
	Although we trust them, by design they shall not observe residue device states left by each other.
	
\end{myenumerate}



%If we assume that the full driver is a golden implementation: 
%it performs interactions sufficient to detect any device state divergence, then the above theorem establishes replay \textit{correctness} based on comparison of interaction traces.  



%
%\Note{lwg: to merge}
%The key idea is to extract a ``stable/beaten'' path. 
%To this end, we assume a \textit{demi}-deterministic device model for drivers we target... 
%That is, for a given set of fixed/controlled inputs, the device will only go through one fixed FSM transition path -- the path we set to extract;
%yet they may exhibit different hw/sw interactions (e.g. reg access values) by appearance. \Note{these will be reflected in recording...}
%
%These inputs are 
%1) user inputs, i.e. block IDs requested by users; 
%2) kernel contexts\Note{a little vague -- kernel states used to bookkeep device states??}, 
%3) spontaneous events: e.g. device hotplug.\Note{is this a user input?}
%
%During recording we exploit the \st{demi-deterministic} nature.
%We control/fix the inputs by eliminating sharing and hardware concurrency.
%At one time, the path takes only one job submitted us; 
%there's no background activities such as runtime suspend/resume, merging of user jobs.

\begin{comment}
\paragraph{Request execution equivalence}
From the driver's POV, 
its \textit{full} knowledge about device state transitions is 
the sequence of state-changing events (including their semantics, parameters, and values read/written). 
If in separate runs the driver sees \textit{equivalent} sequences of state-changing events, 
then as far as the driver (the golden implementation) is concerned, the device goes through the same state transitions and has finished the same request (albeit on different input/output). 
Example: a USB controller accesses 500 registers...

The same rationale applies to a replayer, whose goal is to reproduce a request as recorded.
If the replayer sees the same series of state-changing events as recorded, 
%then as far as the driver is concerned (to the best knowledge of the driver), 
then the device in the replay has finished the same request as recorded. 

For this reason, the replayer is as capable as the full driver on assessing device states (i.e. detecting correctness violation). 
If there is a state divergence undetected to the replayer (e.g. silent data corruption despite equivalent state-changing histories), it could have been missed by the full driver as well. 
This means there is a bug in the driver. 

Its assessment of request correctness is sound. 

%This means that when the replayer deems a request is completed successfully, the assessment is sound. 

\end{comment}


==> sys-model-recycle.tex <==
% !TeX root = main.tex
\subsection{System model}
% \paragraph{Hardware model for secure IO}
\label{sec:bkgnd:model}


%\Note{The flow: 
%	First, we assume a gold driver impl and the  demi-deterministic device FSMs -- so that such a ``replay path'' can be extracted...
%	We then define device states -- reflected by driver control flow and are agnostic to us. 
%	Then describe device state transitions -- marked by state-changing events (control read/write, irqs). 
%	Then we set to reproduce such a state transition path which is recorded... 
%	We define replay success and correctness as follows...}

\paragraph{SoC hardware}
We assume an SoC with Arm TrustZone. % and the following hardware support. 
%(1) A device instance is exclusively assigned to TEE. 
An IO device instance is exclusively assigned to the TrustZone TEE. 
This is feasible as a modern SoC often has multiple independent instances of the same device, e.g. 4--6 MMC controllers~\cite{imx6sx,imx7,tegra2rtm}. % each of which function independently. 
% For instance, 
% each of which can connect to separate storage peripherals. 
% At the boot time, a secure monitor at EL3 the IO devices to TEE and routes their interrupts to either accordingly. 
%(2) The TEE has a dedicated address spaces. 
Through an address space controller (TZASC), the Arm SoC maps selected physical memory regions and device registers to the TEE, isolating them from the normal-world OS. 
% The TZASC hardware also ensures that any system bus masters respect the TrustZone. For instance, a DMA engine can only access secure memory regions when it is invoked by the TEE. 
%Because IO devices assigned to normal/secure worlds may nevertheless share common clock sources and power domains, the TEE should protect clock and power registers as done in prior work~\cite{secloak}. We will will present more details in Implementation (Section XXX). 


\paragraph{Targeted IO devices}  % (scope; device model)  
We focus on IO devices that have strong use cases in TEE. 
%These devices manipulate sensitive IO data while lacking capability to protect the data, e.g. with end-to-end encryption. 
These devices manipulate sensitive IO data while lacking end-to-end encryption for protecting the data.
Examples include USB storage, 
video/audio devices, 
%USB storage and input/output devices, 
%SPI or I2C sensors, 
%cameras, 
and display controllers. 
% Our design is based on the foll
We make the following assumptions. % on IO devices. 

\begin{myitemize}
	\item 
	\textit{Driver/device interactions.}
	%	\textit{Input/output events.}
	The driver interacts with a device via registers, shared memory, and interrupts. 
	In particular, the driver may dynamically allocate descriptors in the shared memory, e.g. MMC allocates one descriptor per data page.
	% To record interactions, the recorder must dump these descriptors. 
	The driver uses register and/or DMA to move data to/from the device.  
	%We do not assume that the devices use IOMMU. 
	The device does not use IOMMU. 
	To our knowledge, these are true for today's mobile and embedded SoCs.
	
	
	\item 
	\textit{Request and response.}
	%CPU requests a device to execute hardware jobs in a request/response fashion.  interactions support a request/response pattern (although multiple/many outstanding requests are allowed). 
	%	Devices support a request/response model in executing a hardware job initiated by CPU, although other executions such as job streaming are possible. 
	%	Devices support a request/response model in executing a hardware job initiated by CPU, although other executions such as job streaming are possible. 
	To execute hardware jobs, 
	the driver and the device communicate in a request/response pattern. 
	The driver initiates a job request by configuring a device's registers and/or descriptors in the shared memory; it kicks start the job via a register write; the device executes the job and responds with an outcome. % by interrupting CPU. 	
	Example hardware jobs include a USB transfer of 16 flash blocks and capturing an image frame at a given resolution. 	
	%\Note{Aside from user input} a request also comes from kernel contexts, e.g. DMA phys pointer...	
	%	This precludes devices that work only autonomously, which in other way around initiate a request, 
	%	Most devices for secure IO fit in the request/response pattern. 
	We do not support devices that only initiate requests autonomously, %proactively. 
	e.g. isochronous USB devices initiating periodic transactions for CPU to handle. %start-of-frame 
	
	\item 
	%	\textbf{Device states}	
	%	A device by design behaviors in job execution. 	
	%	on an internal finite state machine (FSM) \Note{cite}, 
	\textit{Device FSM.}	
	A device operates its internal finite state machine (FSM) and decides its behaviors~\cite{rpi3-sdhost,usb-driver,software-fsm}. 
	The FSM encodes the driver/device protocol and the device's internal logic.
	%	As the driver interacts with the device, 
	As a driver runs, 
	%	it supplies stimuli to the device FSM, e.g. new jobs and changes to the device configuration; 
	%	the device state makes transitions accordingly. 
	it sends outputs to the device, 
	%	e.g. a register write for changing the device configuration; 
	e.g. a register write for starting a data transfer job; 
	%	e.g. new jobs and changes to the device configuration; 
	the output stimulates the device to change its internal state. 
	%which drive the device state to change. % transition from one to the next. 	
	%	which drive the device state transitions. 
	The state transitions, however, are independent of IO data content.
	%		\Note{check sum?}
	%	For instance, a display controller's state is independent of the pixel colors it renders;
	For instance, the state of a MMC controller is unaffected by the content of the block being read. 
	%	Although we assume that a device has an internal FSM, we do not assume the knowledge of the FSM's specifications. 
	%	This is because commodity devices often have unpublished FSMs and their states are often not exposed to software explicitly.  
	%	\xzlNote{grey box?}
	%	Our approach is therefore agnostic to FSM internals.
	
	\item 		
	\textit{State-changing events.}
	%	A device's state is not directly exposed to software. 
	%	To infer the state changes, the full driver, by design, continuously monitor \textit{state-changing events}: 
	%	To operate on a device, a driver needs to know the device's state.
	%	By design, a driver needs to know a device's state at run time, e.g.
	%	so it can send commands to the device when the device is ready. 
	%	Unable to read out the device state directly,
	% \Note{need to highlight status register read is different from actual device state}, 
	%	the driver often infers the state from its observation of \textit{state-changing events}, i.e.
	%	Often, a device's FSM and state are both internal. % with unpublished details. 
	%	Although we assume an internal FSM of the device, 
	%	we do not assume the knowledge of the FSM's specifications. 
	%	We assume an internal FSM of the device but not the knowledge of the FSM's specification. 
	%%	we do not assume the knowledge of the FSM's specifications. 
	%	This is because commodity devices often have unpublished FSMs, whose states are not exposed to software fully and explicitly.  
	As commodity devices often have unpublished FSMs, whose states are not exposed to software fully and explicitly.  
	Rather, a driver operates on a device by implicitly inferring the device's state from its \textit{state-changing events}. %which are
	%	the driver's inputs to the device that \textit{may} change the device state and 
	%	the outputs from the device that \textit{may} indicate state changes. 	
	%a subset of inputs/outputs from/to device that may change the device state or indicate state changes.
	They are a subset of interaction events.
	%	The driver does so from its observation of \textit{state-changing events}, which are
	%	%	the driver's inputs to the device that \textit{may} change the device state and 
	%	%	the outputs from the device that \textit{may} indicate state changes. 	
	%	a subset of inputs/outputs from/to device that may change the device state or indicate state changes.
	%	Our solution is for the replayer to reproduce the full driver's events of changing the device state. 
	%	As the full driver interacts with the device, it induces the device's state transitions, which 
	%As the full driver interacts with the device\Note{, driving it to go through different phases of job execution...}, it induces the device's state transitions, which the driver continuously assesses through \textit{state-changing events}.
	%The driver does the assessment solely based on its observation of \textit{state-changing} events, 
	%i.e. interaction events that \textit{may} change the device state or indicate changes to the state. 
	%	stimuli it sends to the device that \textit{may} change the device state and 
	%	responses it receives from the device that \textit{may} indicate state changes. 
	
	%	all interaction events that \textit{may} change the device state or indicate the state \textit{may} have changed. 
	%We define state-changing events broadly, so that we err on the side of falsely assessing a successful replay as failure, rather than a failed replay as a success. The former can be overcome with re-execution while the latter will cause silent errors. Therefore, the assessment of replay success is sound. 
	State-changing events happen at access to register and shared memory as well as interrupts. 
	Specifically, they include the following: 
	\begin{myenumerate}
		\item 
		Control path actions: 
		writes to registers or shared memory, which kick off hardware jobs or update device control/configuration; 
		reads from registers or shared memory, whose values reflect the changes of device/job runtime status or have side effects.
		%	\Note{to discuss: what's the diff with above?}
		
		\item 
		Data path actions:
		data move between device and shared memory. 
		They do not include the actual data content or buffer addresses\Note{check, rephrase}.	
		
		\item 
		Interrupts from the device. 
	\end{myenumerate}
	
	%	\begin{enumerate}
	%	\item 
	%	writes to registers or shared memory, which kick off hardware jobs or update device control/configuration; 
	%	%	\Note{to discuss: what's the diff with above?}
	%	
	%	\item 
	%	reads from registers or shared memory, whose values reflect the changes of device/job runtime status or have side effects;
	%	
	%	
	%	\item 
	%	the \textit{internal} execution of hardware jobs; %not including the actual data content or buffer addresses; 	
	%	
	%	\item 
	%	interrupts from the device. 
	%	\end{enumerate}
	
	%	Note that the state-changing events are perceived from driver's POV and are not a direct mapping of internal device FSM.
	%	For instance, to execute hardware jobs the device may endure many internal state transitions.
	%	\Note{unified the term of states}
	Identifying them is not difficult; 
	%	the descriptions of device registers/shared memory are often prescribed as comments of kernel driver source\Note{cite}.
	their descriptions are often prescribed as comments of kernel driver source\Note{cite}, which we assume 
	
	
	%	\begin{itemize}
	%	\item 
	%	the events of data write/read via either registers or shared memory\Note{how to capture shared memory read?}, not including the actual data content or buffer addresses; 
	%	\item 
	%	the events of register or shared memory write, that update device control/configuration; 
	%	\Note{to discuss: what's the diff with above?}
	%	\item 
	%	the events of register or shared memory read, except the read returns a stale value and is known free of side-effect;
	%	\item 
	%	interrupts from the device. 
	%	\end{itemize}
	
	%	(1) the events of data write/read via either registers or shared memory, not including the actual data content or buffer addresses; 
	%	(2) the events of register or shared memory write, that update device control/configuration; 
	%	(3) the events of register or shared memory read, except the read returns a stale value and is known free of side-effect;
	%%	read of device control or configuration, unless the read is side-effect free and returns a stale value as an earlier read; % the same value of the most recent read; 
	%	(4) any interrupts from the device. 
	
	Figure~\ref{fig:code} shows an example, which underscores all state-changing events in the recording run (a) on a fictional device FSM. 
	
	%	any register write operations, except the content of written IO data or addresses; 
	%	any register read operations, except 
	%	control writes to device, e.g. write to a command register; 
	%	control reads from device returning fresh values, e.g. a bit flipped in an in-memory descriptor; 
	%	any interrupts. 
	
	%	The events do not include: 
	%	read/write of data contents; 
	%	control reads without side effect or returning stale values, e.g. return from a performance counter. 
	
	
	
	%\item Shared memory:  memory barrier??), which signals ... the shared memory synchronization point?
	%
	%\item 
	%\Note{merge this}
	%
	%%In executing jobs, devices 
	%a device's behaviors, or its state transitions, 
	%For instance, a display controller's state is independent of the pixels it  renders. 
\end{myitemize}

%\paragraph{Device states}
%%\Note{To make replaying possible...the states are demi-deterministic...given an input, the interactions are deterministic in the sense of same set of register accesses..values..XXX}
%%Our rationale is based on our 
%Our guarantee is based on the following observation. 
%%We have the following observation on device states. 
%%A device's state is the device's whole knowledge for determining how it willexecute the current request. 
%A device, by hardware design, 
%%determines how it executes hardware jobs based on an internal \textit{state}. 
%decides its execution behaviors based on an internal \textit{state}. 
%The state encodes the device's current protocol step, its configuration, and pending hardware jobs. 
%%The state encodes (1) the current protocol step the device is participating in, e.g. wait for a command; (2) the device's current configuration, e.g. command types and bus width; 
%%(3) any hardware jobs the device has admitted and yet to complete. 
%%(3) any intermediate results the device may have (??). 
%The state, however, is independent of input/output data content per our model in \sect{bkgnd:model}.
%%As the full driver interacts with the device and submits a series of hardware jobs, the device's state follows a path of transitions. 
%As the full driver interacts with the device, it induces the device's state transitions. 
%the device's state changes accordingly.  
%We define a device state as a tuple <P,C>, where P is the device's protocol step, e.g. WAIT\_FOR\_COMMAND or COMPLETED; C is the the device's current configuration, e.g. data rate and bus width. 
% including in-memory descriptors visible to the device. 

%\paragraph{Causes of state divergence}
%Even to repeat the same interaction sequence, the device state in replay may diverge from recording. 
% Why the device state in replay may diverge from recording, 
%even with the same interaction sequence?
%Why would device state divergence occur, 
%even if CPU repeats the same sequence of hardware jobs? 
%Why might a device's state diverge, 
%even if it repeats the same sequence of hardware jobs? 
%even if CPU replays the same  interaction sequence?
%The major sources are two. 
%Even to execute the same hardware jobs, a device may show different state transitions across runs. 
%What if the device state transitions at the replay time diverge from those at the record time? 
%How to handle divergences in device state transitions?
%Even to execute the same hardware jobs, a device may follow different paths of state transitions across runs. 
%If left unconstrained, a device may take different paths of state transitions to 
%Even to execute the same hardware jobs, 
%a device's path of state transitions in replay may diverge from what was recorded. 

%Since a successful run always follow the same device state transitions. 
%We therefore associate replay correctness to device state transitions: 
%The above analysis shows that a successful replay is implied by device state transitions: 
%The above analysis shows that a successful replay always reproduces the recorded device state transitions: 
%With the above analysis, we consider a successful replay as:

%\paragraph{Observation of device state}
%\paragraph{Assessing device state transitions}
%
%Built on the above definition, 
%the replayer assesses replay success by comparing device state transitions in the replay run with those in the recording run. 
%%\Note{recording run itself is non-deterministic...define such a ``gold'' path which is exemplified by recordings...}
%%How does the full driver detect device state divergence? 
%%How does the replayer detect device state divergence? 
%%How does the replayer keep track of device state transitions? 
%However, a device's state is often internal and is not directly visible to software. 
%
%Our solution is for the replayer to reproduce the full driver's events of changing the device state. 
%%The rationale is as follows.
%We have the following observations. 
%%By its design, 
%%the full driver interacts with the device continuously and As the driver interacts with the device in many rounds, assesses if the device state have deviated from known correct transitions. 
%In the recording run, 
%%the full driver has been assessing if the device state have deviated from known correct transitions. 
%the full driver's confidence in execution correctness is based on its continuous assessment of device states.
%%have deviated from known correct transitions. 
%The driver does the assessment solely based on its observation of \textit{state-changing} events, 
%%i.e. interaction events that \textit{may} change the device state or indicate changes to the state. 
%i.e. all interaction events that \textit{may} change the device state or indicate the state \textit{may} have changed. 
%%We define state-changing events broadly, so that we err on the side of falsely assessing a successful replay as failure, rather than a failed replay as a success. The former can be overcome with re-execution while the latter will cause silent errors. Therefore, the assessment of replay success is sound. 
%State-changing events include: 
%interrupts; 
%control writes to device, e.g. write to a command register; 
%control reads from device returning fresh values, e.g. a bit flipped in an in-memory descriptor. 
%The events do not include: 
%read/write of data contents; 
%control reads without side effect or returning stale values, e.g. return from a performance counter. 
%\Note{maybe tie this to control flow decisions -- driver relies on control reads to make control flow decisions, etc. 
%	Example is reading performance counters, power states etc. are unconditional -- no control flow dependent on them. 
%	However, reading IRQ status reg is control-flow dependent, i.e. state-changing, where the driver assesses the bit masks and make decisions. 
%}

%To implement the comparison, the recorder extracts from its interaction trace a subsequence of state-changing events and compare the subsequence to that from the recorded trace. 

\input{fig-code}



%\textbf{Define: equivalence of interaction sequences}
%A recursive definition? Why needed? Used to prune execution paths. 

\begin{comment}
\begin{myitemize}
\item 
an interrupt, including its semantics and source (?); 
\item 
write of a register of device configuration or metadata;
\item 
read of a register (configuration or metadata) returning different value from previous read
\item
read of an in-memory descriptor field returning a different value 
\end{myitemize}

Non-example: ...
\begin{myitemize}
\item 
read of register returns the same value. And the read has no side effect. 
\item 
read of statistics registers (performance counters)
\end{myitemize}
\end{comment}


%A device often does not expose its internal FSM (e.g. there is no register showing it). 
%During driver/device interactions, a driver continuously assesses the device state. 
%The driver does so by learning from interaction events that suggest potential device state changes, or \textit{state-changing events}. 

%We define state-changing events: interaction events that may affect device behavior in request execution. (waypoints of the device state transitions)

%For instance, an MMC controller... determined by the ...
%rendering to a specific screen region, reading one block from eMMC, 

%As a driver interacts with the device, the driver continuously assesses (learns) device states from the interaction events that indicate possible updates to the device state. 

% assess if the device state diverges from the correct transitions. 

% If we make the following assumption: 
%If we assume the full driver is correct: 
%\begin{assumption}[A golden driver]
%	The full driver performs interactions sufficient to detect any device state divergence. 
%\end{assumption}

\paragraph{The gold driver.}
We assume that the driver implements sufficient state-changing events, so that it can assess if the device has finished the state transitions needed by given hardware jobs. 
% The full driver may have other semantic bugs, 
We do not rule out other bugs in the driver, 
of which consequence will be discussed in \sect{eval}. 

%It achieves desired device functions by implementing state-changing events faithfully and overseeing their correctness.

%We call such driver a \textit{golden} driver.
%Note that a golden driver does not have to be bug-free. 


%The above assumptions lead to a simple, practical design. 
%We will discuss its limitations in Section XXX. 


==> tab-case-study.tex <==
% !TeX root = main.tex
\begin{table}
\centering
%	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/tab_case_summary}
	%\vspace{-5mm}
%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
	\caption{list only the dynamic fields which need annotation and developer knowledge; kernel version: v4.19, commit \#: XXXXXX}
	\label{tab:tab_case_study}
	%\vspace{-10mm}		% use as needed
\end{table}


==> tab-dev-knowledge.tex <==
% !TEX root = main.tex
\begin{table}[h]
	\centering
	\includegraphics[page=1,width=0.48\textwidth{}]{./figs/tab_dev_knowledge}
	\caption{Developer knowledge required by diff approaches.}
	\label{tab:dev-know}
\end{table}


==> tab-s2e.tex <==
% !TeX root = main.tex
\begin{table}
	\centering
	%	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/tab_s2e}
	\vspace{-5mm}
	%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
	\caption{Retrofitted S2E plugins and our modifications.}
	\label{tab:s2e}
%	\vspace{-2.5em}		% use as needed
\end{table}

\begin{table}
	\centering
	%	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/tab_instrumentation}
	\vspace{-5mm}
	%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
	\caption{The list of kernel functions we emulate using FunctionModels plugin.}
	\label{tab:emu}
	\vspace{-10mm}		% use as needed
\end{table}

==> tab-trace.tex <==
% !TeX root = main.tex
\begin{table}[h]
\centering
%	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/tab_trace}
	%\vspace{-5mm}
%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
	\caption{recorded campaign for targeted devices.}
	\label{tab:trace}
	%\vspace{-10mm}		% use as needed
\end{table}


==> tab-usb-record.tex <==
% !TeX root = main.tex
%\begin{table}[h]
%	\centering
%	%	\vspace{1pt}
%	\includegraphics[width=0.48\textwidth{}]{./figs/tab_usb_replay_actions}
%	%\vspace{-5mm}
%	%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
%	\caption{USB replay action breakdown of the interaction templates given input vector}
%	\label{tab:usb:replay_action}
%	%\vspace{-10mm}		% use as needed
%\end{table}


\begin{table}[h]
\centering
%	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/tab_usb_record}
	%\vspace{-5mm}
%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
	\caption{Recording outcome of USB input variables, among which SCSI/CSW/Userdata are from kernel.}
	\label{tab:usb:record}
	%\vspace{-10mm}		% use as needed
\end{table}




==> tab-usb-templates.tex <==
% !TeX root = main.tex
\begin{table}[h]
	\centering
	%	\vspace{1pt}
	\includegraphics[width=0.48\textwidth{}]{./figs/tab_usb_replay_actions}
	%\vspace{-5mm}
	%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
	\caption{USB replay action breakdown of the interaction templates given input vector}
	\label{tab:usb:replay_action}
	%\vspace{-10mm}		% use as needed
\end{table}




==> tab_instrumentation.tex <==
% !TeX root = main.tex
%\begin{table}
%\centering
%%	\vspace{1pt}
%	\includegraphics[width=0.48\textwidth{}]{./figs/tab_instrumentation}
%	\vspace{-5mm}
%%	\caption{A breakdown of \sys{} source, whose 4K LoC are in on-device TCB.}
%	\caption{The list of kernel functions we emulate using FunctionModels plugin.}
%	\label{tab:instrumentation}
%%	\vspace{-10mm}		% use as needed
%\end{table}


==> thoughts.tex <==
% !TeX root = main.tex
\subsection{Thoughts}

\Note{Clarify: what are the problems? why do we care about loops?}

\Note{The driver model should be stated earlier}
\paragraph{What device drivers work with Razor (driver model)?}
The key requirement seems whether user inputs can ``dictate'' a stable driver/device interactions.
This can be elaborated as:
\begin{myitemize}
	\item 
	Data out of the code path.
	Per input, the code path is ``stable'' (limited/bounded non-deterministic, e.g. a few). 
	\Note{this implicitly specifies data is out of device FSM transitions}.

	\item 
	Have parameterizable fields.
	Code paths react to different inputs. 
	
\end{myitemize}

\subsubsection{A case for \sys{}}
We make a case for \sys{}'s novel use of Record-and-Replay.
\Note{a case for Minimal Viable Prototype Driver??}

\textbf{RnR for driver reuse}
Prior use of RnR is mainly for bug finding, which is one type of differential analysis (i.e. same inputs, observe divergence).
The intuition behind the use case is -- it assumes a symbolic execution tree/FSM for the code being tested (e.g. userspace program, driver); 
by replaying, it deterministically controls the inputs to drive FSM transitions/instantiating symbols of the execution tree, so as to expose bugs due to non-determinism (i.e. state divergence). 

Our key insight is RnR captures a \Note{beaten} state transition path of the FSM;
by carefully parameterizing input-dependent fields, the path can be expressed as a code path and reused for a generic class of input (suitable for TEE).  

The code path (i.e. the recording) is a \textit{streamlined} execution path (i.e. no if-else branches), as a resemblance to one concrete path of the symbolic execution tree of the original driver.
It contains serialized driver/device interactions -- register accesses, snapshot of allocated shard memory taken at trigger registers\Note{justify the driver/device interactions earlier on \& trigger register, etc.}. 

However, across different runs \Note{just mention we can run multiple times but do not need to mention diff analysis} a raw streamlined execution path exhibits non-determinism: 1) it contains different number interactions (i.e. path length varies), 2) the accessed registers/interfaces have different values.


How to resolve the non-determinism on the path and find parameterizable fields to reuse at replay time?
Our observation is the execution path has only two sources of non-determinism: 1) loops, which cause the non-deterministic number of recorded interactions, 2) dynamic values, which are dictated by inputs or dynamic by nature (e.g. performance counter).

%Unrolled loop means on the code path, there are non-deterministic numbers of repetitive driver/device interactions. 
%Dynamic values means, given different user/kernel inputs the snapshots of the interactions (i.e. register access values, memory dumps of descriptors) may vary. 
%Why loop only? Because if-else conditions (control flow) are already captured.

Focusing on the two sources of non-determinism, \sys{} incorporates well-known program analysis techniques to address them as follows.

\paragraph{Resolving loops}
Simply observing nearby source code is not gonna work, as a loop body may be constructed at a higher order, e.g. in caller.

To this end, \sys{} runs loop analysis to identify any loop structure. 
The analysis generates the same loop structure on the path; 
it also preserves the loop conditions, which is often a condition variable to wait on and also max number of trials. 
Examples include wait for register to be ready, wait hardware FIFO to become available. 



\paragraph{Resolving dynamic values}
Dynamic values can be further categorized as input-dependent and input-independent values.

\textbf{Resolving input-dependent ones.}
\sys{} first resolves input-dependent values by taint tracking all inputs (e.g. block id, count). 
The goal is to find \textbf{potential} parameterizable ones at replay time. 

The following is an example list of them:
\begin{myitemize}
	\item 
	\textit{Block ID} specifies starting sector to access in a storage device. 
	
	\item 
	\textit{Block count} specifies how many sectors to access. 
	
	\item 
	\textit{Input/output buffer address} specifies data page source or destination.
	
	\item 
	\textit{Input/output Buffer length} specifies size of the input/out buffer.
	
	\item
	\textit{Descriptor address} specifies locations of in-memory descriptors. 
	
	\item 
	\textit{Descriptor size} specifies size of the descriptors. 
	Note the information about descriptor address \& size is not tracked from user inputs but from kernel DMA APIs. 
\end{myitemize}

The taint analysis tool tracks the above inputs and also their \textit{transforms} along the way, e.g. the data buffer address shifts right then left 3 bits in an field of the descriptor. 
The transforms will be applied when parameterizing them.

In deciding what input values can be parameterized, the analysis follows one principle -- as long as the control flow \Note{more relaxed condition -- as long as it is not related to device states?} of the recorded code path is strictly not contingent on the input value, it can be parameterized. 

For example, data addresses, once allocated, are aligned and assigned to corresponding fields in descriptors, without being checked by device FSM;
they are identified as parameterizable (with the alignment transform). 
For block count, the driver checks for its value. 
If it is less than a page size (i.e. eight 512-byte blocks), driver combines them as one page access through DMA.
The analysis captures such an "if" check, conditioned on block count and hence deem the input non-parameterizable. 

\sys{} then reports the parameterizability of each input. 
We found XXX inputs are parameterizable and XXX are non-parameterizable.

\textbf{Resolving input-independent ones.}
They are not tainted by inputs but show changes across runs. 
Examples include command serial numbers, timestamps. 
 
\sys{} first treats reads of them.
The treatment is similar to finding parameterizable inputs.
\sys{} taints them; 
as long as control flow is not conditioned on them, \sys{} either ignores their values.
This is because reads reflect FSM state...as long as the native driver tolerates them, as do we.

Writes of dynamic, input-independent values are more subtle as they might alter device states. 
E.g. device FSM expects an ever increasing command serial number otherwise it faults. 
\sys{} first applies a simple heuristics -- it fuzzes the values by randomly generating them\Note{how many bytes?? this needs a type??}.
If \sys{} observes no divergence in subsequent interactions, it fills the fields with random number at replay time. 
Otherwise, it prompts the developer about the source location that fills the field and asks the developer to provide corresponding synthesis function. 
Luckily, the synthesis function is already encoded in many a field. 
E.g. in the `tag' field of USB command, it is filled by simply incrementing the prior value by 1. 

 
\paragraph{Preserving concrete values}
These values are static and stay the same.
\sys{} captures them as-is. 




\Note{Below obsolete..}
\paragraph{To resolve the dynamic values. }
Razor combines differential program analysis with taint analysis   -- view device driver as a gray box -- inputs are user inputs and kernel states, output is device function (?). 

The insight is that dynamic values only have two types: input-dependent \& input-independent. Input -- user input + kernel context (memory).
Each dynamic values to be paramaterized has a \textit{constraint}.
A constraint specifies two aspects on the value: 1) \st{a range}, 2) a transform.
Transform defines how the input is finally encoded. E.g. due to alignment or must be encode in bit fields. 
\Note{why is range needed}

To find all dynamic values, Razor uses \st{differential} program analysis (i.e. using same inputs):

Step 1: taint all inputs to find input-dependent fields.

\begin{myitemize}
	\item 
	Taint track user inputs, e.g. block address, length, data buffer address. 
	
	\item 
	Taint track DMA allocation for any physical pointers.
	They include both in-memory descriptor and kernel data buffer address.
\end{myitemize}

For block address, lengths -- they can be tracked down to the driver/device boundary... as they are also the direct inputs to protocol/FSM...

For addresses, the challenge is how to separate output buffer (for user data) from kernel buffer (for in-mem descriptors).
This is because regardless of the supplied user data buffers, kernel always allocates its own buffers from DMA pool first then copy data to user-supplied data buffers.

%\begin{myitemize}
%	\item 
%	Step1. Same user inputs + taint driver DMA memory pool -- this finds all phys pointer from the DMA pool and are regarded as in-memory descriptors.
%	Taint analysis tells the developer the data structure of the descriptor. 
%	This discovers all interfaces...
%	
%	
%	\item 
%	Step2. Taint user inputs + same memory layout -- finds “parameterizable” fields of user fields and also input-independent values...
%\end{myitemize}


For input-independent (hitchhike with process later)
\begin{myitemize}
	\item 
	Same user inputs + same memory layout -- finds input-independent values. E.g. counter. 
\end{myitemize}



\textbf{To resolve constraints}
Taint analysis on inputs (user \& kernel memory) keeps track of each transform done on the input and reports. 
E.g. an \textit{addr} has been shifted right then left 3 bits for alignment. 
\Note{Taint analysis by default will figure out the ``transform''; it can also deal with complex transforms like checksum}

\paragraph{Implementation details}

\textbf{To record driver}
View a driver as three parts, which Razor records -- init, function, reset.

How to find each?
init -- driver probing stage, by convention;

function -- driven by test harness to test out driver functions, by intuition.

How to find reset which resets the device to a clean slate state?
Two approaches:

Let developers annotate the function and Razor exercises. The challenge is twofold: 1) the developer may have poor knowledge (e.g. USB data toggling reset is hard to find) and cannot find the function; 2) the reset function may be up to current device \& kernel states to perform action. It is hard to say the recording is valid.
\Note{if we embed in some heuristics in finding reset functions, this approach seems fine}

Also record, as if it is due to unexpected device states at runtime. The challenge is it is not triggered by user inputs and the fault context must be emulated.
May be addressed by fuzzing (?).

What does our approach look like? 
A combination of differential program analysis and tain analysis 


Some other challenges:
\begin{myitemize}
	\item 
	“Scanning interfaces” is vague -- memory dump, byte by byte? Word by word?  For register -- bit by bit? There needs to a unified framework which needs a type to scan. 
	How to define \Note{types} for interface fields? 
	\Note{not needed}
	
	\item 
	Alignment issue? Potentially solvable by gathering all recorded values and scanning 0s from LSM. -- alignment is an attribute of a field. 
	This points out constraints on \textit{how} fields can be parameterized, i.e. they cannot be freely parameterized. 
	\Note{constraint}
	
	\item 
	What are the constraints of the parameterizable fields?
	
	\item 
	How to taint track fields in shared memory? I.e. they may be modified by the device (e.g. GPU).
	
	A generic solution for in-memory descriptor?
	Register access is fine -- pinpoint the location. 
	
	\item 
	Userspace test harnesses will cause significant changes to driver behavior.
	Although they achieve same functional equivalence, how does a developer choose one that suits best?
	
	\item 
	Replay speed/timing -- can we replay as fast as possible? 
	The answer must be yes, as long as no artificial delay is recorded. 

\end{myitemize}




\paragraph{unorganized thoughts}
\begin{myitemize}
	\item we seek to understand -- what is the least dynamism required for a device to perform its basic functions (e.g. rw data, capture datapoint)?
	
	\item defeaturing is not only getting rid of (unnecessary) kernel contexts but also a large part of code that deals with "dynamism", which leads to many conditional branches (i.e. FSM transitions) -- \Note{this also our key mechanism to get rid of vulnerabilities}
	
	
	\item experimentally, the only dynamism required (or divergence allowed) is about data but not control, e.g. data dst/src, size. 
	This is true in storage and vchiq cam.
	
	\item consequently, the \textit{only} knowledge developer needs to understand is data structure that describes the data (i.e. DMA desc.). 
	E.g. which offsets specify data src during replay, proper DMA descriptor.
	
	\item 
	the impl. of test harness directly affects the recording. 
	Can provide "enough" options (e.g. img res, format) of test harness and thus supplying "diverse enough" recordings to replay.
	\Note{how to select the "right" test harness if there's a performance difference?}
	
	\item robustness of replay on non-recoverable divergence. 
	Simple dev like SDhost might be settled by resetting. 
	VideoCore is much more complex -- firmware is an OS. 
	What if the states are messed up (e.g. firmware is overflowed and re-written) lead to non-recoverable divergence? 
	
	\item heuristics and assumptions: 1) device has no iommu; 2) DMA address must imply data move between kernel \& device and needs attention. 
	
	\item Partial-porting is infeasible -- one cannot easily and cleanly decouple a single path out of the whole complex FSMs.
	
	\item how to decide if one field is parameterizeable? Size is not. What about starting address? \Note{have a table}
	
	\item What about the constraints on parameterized field? Alignment, size, etc. 
	
	\item what if the parameterized user input is not straightforward? E.g. being encoded inside a few bits in a cmd.
	
	\item set relations: dynamic values = parameterizable fields V ignorable values
	
\end{myitemize}

==> todo.tex <==
% !TeX root = main.tex

%\jin{Should we stress on mobile GPU?} - yes. or embedded GPU. 

% \jin{How to describe ML training result? Federated and transfer learning}
%\Note{explain GPU memory}


\Note{top issues: divergence (correctness guarantee); developer efforts}

\Note{"how does different tests/host environment affect recordings?" "will they differ each time for each developer?"}


\Note{TCP/IP test gen (diff analysis)}


\Note{add this to impl}

Because IO devices assigned to normal/secure worlds may nevertheless share common clock sources and power domains, the TEE should protect clock and power registers as done in prior work~\cite{secloak}. We will will present more details in Implementation (Section XXX). 


\xzlNote{high-level: why template? program input space; input from the device. why only one state path? It's our reuse unit. a tradeoff between simplicity and practicality}

\xzlNote{high-level: why sym exec easier than dev from scratch? our sym exec is a humble, common task. already implemented as plugins somewhere else (eg the woot 17 paper)}

Survey device drivers in common TEEs: Trusty, OPTEE, Knox, QSEE

\xzlNote{What if developers find templates not enough?}

\xzlNote{checksum may be brought up}

\xzlNote{Cite GPURip}

\xzlNote{Debugging information in template}

\xzlNote{Device reset??}

\xzlNote{Highlight device descriptors}

Discuss Table~\ref{tab:eval:build-from-scratch}
